Robust Linear Regression: Gradient-descent, Early-stopping, and Beyond

In this work we study the robustness to adversarial attacks, of early-stopping strategies on gradient-descent (GD) methods for linear regression. More precisely, we show that early-stopped GD is optimally robust (up to an absolute constant) against Euclidean-norm adversarial attacks. However, we show that this strategy can be arbitrarily sub-optimal in the case of general Mahalanobis attacks. This observation is compatible with recent findings in the case of classification~\cite{Vardi2022GradientMP} that show that GD provably converges to non-robust models. To alleviate this issue, we propose to apply instead a GD scheme on a transformation of the data adapted to the attack. This data transformation amounts to apply feature-depending learning rates and we show that this modified GD is able to handle any Mahalanobis attack, as well as more general attacks under some conditions. Unfortunately, choosing such adapted transformations can be hard for general attacks. To the rescue, we design a simple and tractable estimator whose adversarial risk is optimal up to within a multiplicative constant of 1.1124 in the population regime, and works for any norm.

==> early-stopped adversarial training/abstract.tex <==
\begin{abstract}
In this work we study the robustness to adversarial attacks, of early-stopping strategies on gradient-descent (GD) methods for linear regression. More precisely, we show that early-stopped GD is optimally robust (up to an absolute constant) against Euclidean-norm adversarial attacks. However, we show that this strategy can be arbitrarily sub-optimal in the case of general Mahalanobis attacks. This observation is compatible with recent findings in the case of classification~\cite{Vardi2022GradientMP} that show that GD provably converges to non-robust models. To alleviate this issue, we propose to apply instead a GD scheme on a transformation of the data adapted to the attack. This data transformation amounts to apply feature-depending learning rates and we show that this modified GD is able to handle any Mahalanobis attack, as well as more general attacks under some conditions. Unfortunately, choosing such adapted transformations can be hard for general attacks. To the rescue, we design a simple and tractable estimator whose adversarial risk is optimal up to within a multiplicative constant of 1.1124 in the population regime, and works for any norm.
% This transformation is in fact an optimal transport map in the Wasserstein-2 sense from the initial distribution to the . 
% Finally, we propose a simple and tractable method early-stopped gradient descent scheme and show that our method allows to significantly improve the robustness of classical learning method and can be applied either at inference or during the training stage. 
% Adversarially robust learning aims to design algorithms that are robust to small adversarial perturbations on input variables. Beyond the existing studies on the predictive performance to adversarial
% samples, our goal is to understand statistical properties of adversarially robust estimates and analyze
% adversarial risk in the setup of linear regression models. By discovering the statistical minimax rate
% of convergence of adversarially robust estimators, we emphasize the importance of incorporating model
% information, e.g., sparsity, in adversarially robust learning. Further, we reveal an explicit connection of
% adversarial and standard estimates, and propose a straightforward two-stage adversarial learning framework, which facilitates to utilize model structure information to improve adversarial robustness. In
% theory, the consistency of the adversarially robust estimator is proven and its Bahadur representation is
% also developed for the statistical inference purpose. The proposed estimator converges in a sharp rate
% under either low-dimensional or sparse scenario. Moreover, our theory confirms two phenomena in adversarially robust learning: adversarial robustness hurts generalization, and unlabeled data help improve
% the generalization. In the end, we conduct numerical simulations to verify our theory.
\end{abstract}


==> early-stopped adversarial training/other_files/beyond.tex <==
\subsection{Going beyond linear models}
\textcolor{red}{Don't activate. This is broken!}

Let $P$ be the marginal distribution of the features and let the ground-truth $f_0$ be any function in $L^2(P)$, linear or not. We will now show that shrinkage always improves the robustness of $f_0$. Given any $\alpha \in [0,1]$, consider the shrunk version $f_\alpha := (1-\alpha) f_0$ of $f_0$. WLOG, suppose $E(f_0,r) > 0$ and define $\beta = \beta(P) := \|f_0\|_{L^1(P)} / \|f_0\|_{L^2(P)}$ and $\theta(r) = \theta(P,r) := \sqrt{E(f_0,r)}/\|f_0\|_{L^2(P)}$, where
\begin{eqnarray}
\|f_0\|_{L^m(P)} := (\mathbb E_P |f(x)|^m)^{1/m},\,\text{ for all }m \in [1,\infty).
\end{eqnarray}
By definition, it is clear that $\beta \le 1$ and $\theta(r) \le r \|f_0\|_{Lip}/\|f_0\|_{L^2(P)}$, where
\begin{eqnarray}
\|f_0\|_{Lip} := \sup_{x,x' \in \mathbb R^d,\,x' \ne x}\frac{|f_0(x')-f_0(x)|}{\|x'-x\|}
\end{eqnarray}
is the Lipschitz constant of $f_0$ w.r.t the attacker's norm $\|\cdot\|$.
% We will prove the following result which shows that shrinkage always improves the robust accuracy of the ground-truth model by at least $67\%$ at the price of a small decrease in normal accuracy.

\begin{restatable}[Robustness boosting by shrinkage]{thm}{}
It holds that
\begin{eqnarray}
\inf_{\alpha \in [0,1]} E(f_\alpha,r) \le E(f_{\alpha_{opt}(r)},r),
\end{eqnarray}
where
\begin{itemize}
\item[(A)] If $\theta(r) \le \beta$, then $\alpha_{opt}(r) = 0$, i.e no shrinking is necessary. If $\theta(r) \ge 1/\beta$, then $\alpha_{opt}(r) = 1$, i.e $f_0$ is shrunk to zero.
    \item[(B)] If $\beta \le \theta(r) \le 1/\beta$, then
$\alpha_{opt}(r) \in [0,1]$ is as given by
\begin{eqnarray}
\label{eq:alphaboost}
\alpha_{opt}(r) := \frac{E(f_0,r)-\|f_0\|_{L^1(P)}\sqrt{E(f_0,r)}}{E(f_0,r) + \|f_0\|_{L^2(P)}^2 - 2\|f_0\|_{L^1(P)}\sqrt{E(f_0,r)}} = \frac{\theta(r)^2 - \beta\theta(r)}{h_\beta(\theta(r))}.
\end{eqnarray}
Moreover, it holds that
\begin{align}
\inf_{\alpha \in [0, 1]}\frac{E(f_\alpha,r)}{E(f_0,r)} &\le \frac{E(f_{\alpha_{opt}(r)},r)}{E(f_0,r)} = \frac{1-\beta^2}{h_\beta(\theta(r))},\\
\frac{E(f_{\alpha_{opt}(r)})}{\|f_0\|_{L^2(P)}^2} &\le \left(\frac{1-\beta}{h_\beta(\theta(r))}\right)^2,
\end{align}
\end{itemize}
\end{restatable}
Note that as expected $\alpha_{opt}(r) = 0$ for $r$ sufficiently small (more precisely, for $\theta(r) \le \beta$), meaning that, in this regime no shrinkage is required. On the other hand, $\alpha_{opt}(r) = 1$ for $r$ sufficiently large (more precisely, for $\theta(r) \ge 1/\beta$), meaning in this regime, that it is to optimal to shrink all the way to the zero model!

\paragraph{Example; linear models.}
For example, if $f_0(w) \equiv x^\top w_0$ (i.e, $f_0$ is linear) and $P=N(0,\Sigma)$, then $\beta = c_0 := \sqrt{2/\pi}$ and $\theta(r) = r\|w_0\|_\star/\|w_0\|_\Sigma = r/r_0$, where $r_0 = \|w_0\|_\Sigma/\|w_0\|_\star$ is the scalar which was encountered before.
% Consequently, $ (1-\beta^2)(1+\beta)/2\le 0.33$ and $(1+\beta)^2/4 \le .81$. This corresponds to a gain in robustness of at least $(100-33/(1+r_0/r)^2)\% \ge 67\%$ at the price of an at most $81/(1+r_0/r)^{2}$ percent decrease in normal accuracy. Note that in the limit $r/r_0 \to 0^+$, this loss in normal accuracy tends to zero, while the $67\%$ gain in robust accuracy remains!

\begin{proof}[Proof of theorem]
The robust risk of $f_\alpha$ writes $E(f_\alpha, r):=\mathbb E_P\sup_{\|\delta\| \le 1}(f_\alpha(x+\delta)-f_0(x))^2=\mathbb E_P \sup_{\|\delta\| \le r}((1-\alpha) f_0(x+\delta) - f_0(x))^2$.
One computes
\begin{eqnarray*}
\begin{split}
&\sup_{\|\delta\| \le r}((1-\alpha)f_0(x+\delta) - f_0(x))^2\\
&\quad = \sup_{\|\delta\| \le r}((1-\alpha)f_0(x+\delta) - (1-\alpha)f_0(x) - \alpha f_0(x))^2\\ &\quad = \sup_{\|\delta\| \le r}(1-\alpha)^2 (f_0(x+\delta) - f_0(x))^2 \\
&\quad\quad\quad- 2\alpha(1-\alpha)f_0(x)(f_0(x+\delta) - f_0(x)) + \alpha^2 f_0(x)^2\\
&\quad \le (1-\alpha)^2\sup_{\|\delta\| \le r}(f_0(x+\delta) - f_0(x))^2  \\
&\quad\quad\quad + 2\alpha(1-\alpha)|f_0(x)|\sup_{\|\delta\| \le r}|f_0(x+\delta) - f_0(x)| + \alpha^2 f_0(x)^2.
\end{split}
\end{eqnarray*}
Taking expectations over $x \sim P$ and invoking the Cauchy-Schwarz inequality, we deduce that
\begin{eqnarray}
\begin{split}
E(f_\alpha,r)
% &:= \mathbb E_P\sup_{\|\delta\| \le r}(f_\alpha(x) - f_0(x))^2\\
&\le (1-\alpha)^2 E(f_0,r) + \alpha^2\|f_0\|_{L^2(P)}^2\\
&\quad\quad + 2\alpha(1-\alpha)\mathbb E_P |f_0(x)|\sup_{\|\delta\| \le r}|f_0(x+\delta) - f_0(x)|\\
&\le (1-\alpha)^2 E(f_0,r) + \alpha^2\|f_0\|_{L^2(P)}^2 + 2\alpha(1-\alpha)\|f_0\|_{L^2(P)}\sqrt{E(f_0,r)}\\
% &= (\alpha\|f_0\|_{L^2(P)} + (1-\alpha) \sqrt{E(f_0,r)})^2.
&= a \alpha^2 - 2b\alpha + c,
\end{split}
\end{eqnarray}
where $a=a(r):=E(f_0,r) + \|f_0\|_{L^2(P)}^2 - 2\|f_0\|_{L^2(P)}\sqrt{E(f_0,r)} = (\sqrt{E(f_0,r)}-\|f_0\|_{L^2(P)})^2 \ge 0$, $b=b(r) := E(f_0,r)- \|f_0\|_{L^2(P)}\sqrt{E(f_0,r)}$, and $c = c(r):= E(f_0,r)$. Now, the quadratic function $\alpha \mapsto a\alpha^2 - 2b\alpha + c$ is minimized when $\alpha = b/a = \alpha_{opt}(r) = \sqrt{E(f_0,r)}/|\sqrt{E(f_0,r)}-\|f_0\|_{L^2(P)}|$, where $\alpha_{opt} \in [0,1]$ is as given in \eqref{eq:alphaboost}. Moreover, the minimal value on this interval is $c-b^2/a = (\|f\|_{L^2(P)}^2-\|f\|_{L^1(P)}^2)E(f_0,r) / a$. Therefore, if $E(f_0,r) > 0$, then
\begin{eqnarray*}
\begin{split}
\inf_{\alpha \in [0, 1]}\frac{E(f_\alpha,r)}{E(f_0,r)} \le \frac{E(f_{\alpha_{opt}(r)},r)}{E(f_0,r)} &\le \frac{\|f\|_{L^2(P)}^2-\|f\|_{L^1(P)}^2}{E(f_0,r) + \|f_0\|_{L^2(P)}^2 - 2\|f_0\|_{L^1(P)}\sqrt{E(f_0,r)}}\\
&= \frac{1-\beta^2}{h_\beta(\theta(r))},
\end{split}
\end{eqnarray*}
and
\begin{eqnarray}
\begin{split}
\frac{E(f_{\alpha_{opt}(r)})}{\|f_0\|_{L^2(P)}^2} = \alpha_{opt}(r)^2 &= \left(\frac{E(f_0,r)-\|f_0\|_{L^1(P)}\sqrt{E(f_0,r)}}{E(f_0,r) + \|f_0\|_{L^2(P)}^2 - 2\|f_0\|_{L^1(P)}\sqrt{E(f_0,r)}}\right)^2\\
&\le \frac{(\theta(r)^2-\beta  \theta(r))^2}{h_\beta(\theta(r))^2}.
\end{split}
\end{eqnarray}
Diving numerators and denominators by $\|f_0\|_{L^2(P)}$ and recalling the definition of $\beta$ and $\theta(r)$ completes the proof.
\end{proof}

==> early-stopped adversarial training/other_files/ewdd_rob.tex <==
\subsection{Dynamics of robustness}
At time $t$, one computes
\begin{eqnarray}
\begin{split}
\|w(t)\|^2 &= \|\widetilde w(t) + c(t)\|^2 = \|(I_d-sG)^tw(0)+K_t(G)X^\top(Xw_\star+\eta)/n\|^2\\
&= \|(I_d-sG)^t w(0)+K_t(G)Gw_\star+K_t(G)X^\top \eta/n\|^2.
\end{split}
\end{eqnarray}
Noting once again that $w(0)$, $w_\star$, and $\eta$ are independent, one computes
\begin{eqnarray}
\begin{split}
 \overline{\mathfrak{S}}(f_t)^2 &:= \mathbb E_{\{w_\star,X,z,w(0)\}}\mathfrak{S}(f_t)^2 = \mathbb E_{\{w_\star,X,z,w(0)\}} \|w(t)\|^2
    \\
    &=  \mathbb E_{\{X,w(0)\}}\|(I_d-sG)^tw(0)\|^2 +  \mathbb E_{\{w_\star,X\}}\|K_t(G)Gw_\star\|^2 \\
    &\quad\quad\quad +  \mathbb E_{\{X,z\}}\|K_t(G)X^\top \eta/n\|^2\\
    &= \sigma_0^2 \cdot \mathbb E_X \frac{1}{d}\trace((I_d-sG)^{2t}) + \sigma_\star^2\cdot\mathbb E_X \frac{1}{d}\trace((K_t(G)G)^2)\\
    &\quad\quad\quad + \mathbb E_X\trace(K_t(G)^2\cov(X^\top \eta/n \mid X))\\
    &= \sigma_0^2\cdot \mathbb E_X\frac{1}{d}\sum_{j=1}^r (1-s\lambda_j)^{2t} + \sigma_\star^2\cdot\mathbb E_X\frac{1}{d}\sum_{j=1}^r (1-(1-s\lambda_j)^t)^2\\
    &\quad\quad\quad + \sigma_\eta^2\cdot \mathbb E_X\frac{1}{d}\sum_{j=1}^{r_\eta}\frac{(1-(1-s\lambda_j)^t)^2}{\lambda_j}.
\end{split}
\end{eqnarray}
Taking limits, we get
\begin{restatable}{thm}{}
In the limit \eqref{eq:proportionate}, it holds that
\begin{eqnarray}
\begin{split}
\frac{\overline{\mathfrak S}(f_t)^2}{\sigma_\star^2} &\overset{p}{\to} \int_0^\infty (1-(1-s\lambda)^t)^2\mu_{\mathrm{MP}(\gamma)}(\lambda)\,\dv\lambda\\
&\quad\quad\quad+ \mathrm{INR}\int_0^\infty (1-s\lambda)^{2t}\mu_{\mathrm{MP}(\gamma)}(\lambda)\,\dv\lambda\\
&\quad\quad\quad+ \frac{1}{\mathrm{SNR}}\int_1^\infty \frac{(1-(1-s\lambda)^t)^2}{\lambda}\mu_{\mathrm{MP}(\gamma)}(\lambda)\,\dv\lambda
\end{split}
\end{eqnarray}
\end{restatable}

==> early-stopped adversarial training/other_files/old.tex <==
\begin{abstract}
We consider two-layer neural networks in high dimensions trained via gradient-descent and derive a precise formula for their generalization error and robustness along the entire optimization trajectory. Our analytic expressions reveal the fine structural dependence on all problem specific parameters: scaling of sample size vs input dimension vs network width; level of label-noise; magnitude of network parameters at initialization; etc. Our work is based on techniques from random matrix theory (RMT).
\end{abstract}

\tableofcontents

\section{Introduction}
\subsection{Setup}
Let $P_x$ be a probability distribition on $\mathbb R^d$, and let $(x_1,y_1),\ldots,(x_n,y_n)$ be an iid sample of size $n$ from a distribution $P$ on $\mathbb R^d \times \{\pm 1\}$, such that
\begin{equation}
\label{eq:data}
x_i \sim P_x,\, y_i = f_\star(x_i) + \eta_i,    
\end{equation}
where $\eta_i$ is $\sigma_{\eta}^2$-subGaussian noise which is independent of $x_i$ and $f_\star:\Rd \to \mathbb R$ is possibly random function which independent of the $x_i$'s and $\eta_i$'s. For example, if $w \in \mathbb R^d$ (possibly random), then $f_\star(x) := w^\top x$ corresponds to a linear model.
Let $X$ be the random $n \times d$ matrix with $i$th row $x_i$, $y$ (resp. $\eta$) be the $n$-dimensional vector with $i$th component $y_i$ (resp. $\eta_i$). 

We will work in the so-called \emph{proportionate} high-dimensional regime
\begin{eqnarray}
\label{eq:proportionate}
n,d \to \infty,\, d/n \to \gamma_1 \in (0,\infty).
\end{eqnarray}

Given a smoothly parametrized class of functions $\mathcal F = \{f_\theta \mid \theta \in \Theta\}$ from $\Rd$ to $\mathbb R$ (e.g linear models, neural networks, etc.), the ML objective is to find $\theta \in \Theta$ which minimizes the test error, namely
\begin{eqnarray}
\etest(f_\theta) :=\|f_\theta-f_\star\|_{L^2(P_x)}^2 = \mathbb E_{P_x}|f_\theta(x)-f_\star(x)|^2.
\end{eqnarray}
Here, the parameter space $\Theta$ is a nonempty open subset of some $\mathbb R^m$. In the empirical risk minimization paradigm, one instead minimizes the training error
\begin{eqnarray}
\etrain(f_\theta) := \frac{1}{n}\sum_{i=1}^n(f_\theta(x_i)-y_i)^2.
\end{eqnarray}
and then uses "uniform convergence arguments" to relate this to $\etest(f; P)$.

\subsection{Objective}
In this manuscript, we will consider gradient-flow
\begin{eqnarray}
\theta(t) = -\nabla_{\theta(t)} \etrain(f_{\theta(t)})
\end{eqnarray}
and are interested in dynamics of the test error $\etest(f_{\theta(t)})$ and the "robustness" of $\varepsilon_{\mathrm{rob}}(f_{\theta(t)}) := \mathbb E_{P_x}\|\nabla f_{\theta(t)}(x)\|^2$. For the justification for the use of Dirichelet energy (aka square $H^1$-norm), see our older papers...


\section{Linear models}
We begin with a multivariate Gaussian linear where the features have distribution $P_x$ on $\Rd$ which admits density w.r.t to the Lebesgue measure. Suppose the labels in \eqref{eq:data} are generated from a linear function $f_\star(x) \equiv x^\top \trueweights$, where the weights $\trueweights$ have distribution $N(0,\sigma_\star^2 I_d)$, for some $\sigma_\star>0$. The funciton $f_\star$ is called the \emph{teacher} model.

% Given a "radius" parameter $R>0$, consider a linear function class $\Flin := \{x \mapsto x^\top w \mid w \in \Rd,\,\|w\| \le R\}$. By duality, minimizing $\etest(f)$ over $f \in \Flin$ amounts to solving a Ridge regression problem
% \begin{eqnarray}
% \min_{w \in \mathbb R^d}\frac{1}{n}\sum_{i=1}^n(x_i^\top w - y_i)^2 + \lambda \|w\|^2,
% \label{eq:ridge}
% \end{eqnarray}
% for an appropriate value of $\lambda=\lambda(R)>0$.
% % Defining $G_\lambda := XX^\top / d + \lambda I_n$,
% A simple calculation reveals that \eqref{eq:ridge} has unique solution given by
% \begin{eqnarray}
% \widehat{w} =  (\gram + \lambda I_d)^{-1}X^\top y/n,
% % = (1/n)X^\top \widehat c,\text{ with }\widehat{c} = G_\lambda^{-1} y.
% \end{eqnarray}
% where $\gram := X^\top X/n$.
% Consider a multivariate Gaussian linear where the features have distribution $P_x = N(0,\Sigma)$, and the weights $\trueweights$ have distribution $N(0,\sigma_\star^2 I_d)$, for some $\sigma_\star>0$.
% % , where $\Sigma$ is the covariance matrix and has SVD $\Sigma = \sum_{j=1}^d s_j u_ju_j^\top$.
% % Given a appropriate funciton $\phi:\mathbb R_+ \to \mathbb R_+$,
% % consider a source condition $\trueweights = N(\mu, \sigma_\star^2 \phi(\Sigma))$, where
% % \begin{eqnarray}
% % \phi(\Sigma) := \sum_{j=1}^d \phi(s_i)u_ju_j^\top.
% % \end{eqnarray}
% A simple computation reveals that
% \begin{eqnarray}
% \begin{split}
% \etest(\widehat w) &= B_n + V_n,
% \end{split}
% \end{eqnarray}
% where the bias and variance terms are respectively given by
% \begin{eqnarray}
% \begin{split}
% B_n &:= \sigma_\star^2 \cdot \frac{1}{n}\trace(R_n(\lambda)\Sigma R_n(\lambda)),\\
% V_n &:= \sigma_{\eta}^2\cdot \frac{1}{n}\trace(R_n(\lambda)\Sigma R_n(\lambda)\widehat{\Sigma}_n),
% \end{split}
% \label{eq:biasvariance}
% \end{eqnarray}
% where $R_n(z) := (\gram+zI_d)^{-1}$ defines the \emph{resolvent} of $\gram$.

\subsection{Dynamics of model weights}
We now present a computation which is essentially due to Andrew Saxe and co-workers \url{https://arxiv.org/pdf/1710.03667.pdf}.
Let
\begin{eqnarray}
\gram = V\Lambda V^\top
\end{eqnarray}
be the singular-value decomposition (SVD) of $\gram$, where $\Lambda=\diag(\lambda_1,\ldots,\lambda_d)$ with $\lambda_1\ge \lambda_2 \ge \ldots \ge \lambda_d \ge 0$ being the eigenvalues. 
Now, the gradient-flow evolution of the parameters of the linear model $f_t(x) := x^\top a(t)$ is,
\begin{eqnarray}
\dot a(t) = -\nabla \etrain(f_t) = -X^\top(Xa(t)-y)/n = -Ga(t) + c,
\end{eqnarray}
where $c := X^\top y/n$. This ODE can be alternatively written as $(e^{t\gram}a(t))' = e^{t\gram}c$, and direct integration gives the unique solution
\begin{eqnarray}
a(t) = \overline a(t) + c(t),
% = Ve^{-t\Lambda} V^\top a(0) + VE(t)V^\top c,
\label{eq:dynamics}
\end{eqnarray}
with $\overline a(t):=e^{-t\gram}a(0)$ and $c(t):=K_t(\gram)c$, where $(t,A) \mapsto K_t(A)$ is the mapping \emph{exponential integrator} given for any $t \ge 0$ and psd matrix $A$ by
\begin{eqnarray}
\label{eq:Kt}
K_t(A):=e^{-tA}\int_0^t e^{sA}\,\dv s = (1-e^{-tA})A^\dagger-t\Pi_{\ker A},
% =e^{-t\gram}\left(\frac{e^{t\gram}-I_d}{\gram}\right) := e^{-t\gram}t\sum_{N=0}^\infty \frac{(t\gram)^N}{(N+1)!}.
\end{eqnarray}
Here, $A^\dagger$ being the Moore-Penrose pseudo-inverse of $A$ and $\Pi_{\ker A}:=I_d-A^\dagger A$ is the orthogonal projector onto the kernel of $A$.
The following elementary lemma will be useful in the sequel.
\begin{restatable}{lm}{}{}
\label{lm:Kt}
The exponential integrator \eqref{eq:Kt} has the following properties:
\begin{itemize}
\item[(1)] $K_t(A)$ and $A$ commute for any $t \ge 0$ and psd matrix $A$. Moreover, $K_t(A)A=AK_t(A)=(I_d-e^{-tA})\Pi_{\mathrm{Im}\, A}$, where $\Pi_{\mathrm{Im}\, A} := A^\dagger A$ is the orthogonal projector onto the image of $A$.
\item[(2)] Each eigenvalue $\lambda_j(K_t(A))$ of $K_t(A)$ can be written in terms of time $t$ and the corresponding eigenvalue $\lambda_j(A)$ of $A$ like so
\begin{eqnarray}
\lambda_j(K_t(A)) =
% e^{-t\lambda_j(A)}\int_0^t e^{s\lambda_j(A)}\,\dv s =
% e^{-t\lambda_j}t\sum_{N=0}^\infty \frac{(t\lambda_j)^N}{(N+1)!} =
\begin{cases}
\dfrac{1-e^{-t\lambda_j(A)}}{\lambda_j(A)},&\mbox{ if }\lambda_j(A)>0,\\
t,&\mbox{ if }\lambda_j(A)=0.
\end{cases}
\label{eq:specK}
\end{eqnarray}
% \\
% because $a(0)$, $\trueweights$, and $\eta$ are mutually independent.
\end{itemize}
\end{restatable}
\begin{proof}
Part (1) follows from the fact that $A$ and $e^{\tau A}$ commute for any $\tau \in \mathbb R$. Part (2) follows from the fact that the funciton $g_t:z \mapsto e^{-tz}\int_0^t e^{sz}\,\dv s$ is analytic on $\mathbb C$ and so the eigenvalues of $K_t(A)$ are given by
$$
\lambda_j(K_t(A)) = \lambda_j(g_t(A)) = g_t(\lambda_j(A)) = e^{-\lambda_j(A)}\int_0^t e^{s\lambda_j(A)}\,\dv s,
$$
which evalues to the RHS of \eqref{eq:specK}.
\end{proof}
% Let $\Pi_V := VV^\top$ be the orthogonal projector for the onto the row-space of $V$, and given any $u \in \Rd$, let $u_\parallel := \Pi_V u$ (resp. $u_\perp := u-u_\parallel$) be the component parallel (resp. perpendicular) to this subspace.  We can then rewrite the dynamics \eqref{eq:dynamics} in the eigenbasis $V$ like so
% \begin{eqnarray}
% \begin{split}
% a_\parallel(t) &= e ^{-t\Lambda} a_\parallel(0) + VE(t)V^\top c\\
% a_\perp(t) &= e^{-t\Lambda}a_\perp(0).
% \end{split}
% \end{eqnarray}

\subsection{Dynamics of generalization error (isotropic features)}
For a random test input $x \sim P_x$, one computes the prediction at time $t$ is $f_t(x) = x^\top a(t) = x^\top \overline{a}(t) +x^\top c(t)$.
Thus, letting $\widetilde a(t):= \overline{a}(t)-\trueweights+c(t)$, we deduce that the generalization error at time $t$ is given by
\begin{eqnarray}
\etest(t) :=\mathbb E_x (f_t(x) - x^\top \trueweights)^2 = \mathbb E_x x^\top \widetilde a(t)\widetilde a(t)^\top x = \|\widetilde a(t)\|^2_\Sigma,
\label{eq:errordecomp}
\end{eqnarray}
where $\Sigma := \mathbb E_x \trace(xx^\top)$. Suppose that independently of the training data, the initial weights $a(0) \in \Rd$ of the student are sampled from a Gaussian distribution $N(0,\sigma_0^2 I_d)$ with variance parameter $\sigma_0 \ge 0$.

For simplicity of analysis, we will assume the following
\begin{restatable}{assume}{}{}
$P_x = N(0,I_d)$.
In particularly, this assumption implies that the covariance matrix of the features is $\Sigma=I_d$.
\end{restatable}
Thanks to a simple density argument, it is clear that, almost-surely, the Gram matrix $\gram$ has full rank $r=\min(n,d)$. One then computes
\begin{eqnarray*}
\begin{split}
&\mathbb E_{X,\eta,\trueweights,a(0)}\etest(t) = \mathbb E_{X,\eta,\trueweights,a(0)}\|K_t(\gram)c+e^{-t\Lambda} a(0)- \trueweights\|_{\Sigma}^2\\
&\quad = \mathbb E_{X,\eta}\|K_t(\gram)X^\top (X\trueweights+z)/n + e^{-t\Lambda}a(0)-\trueweights\|^2\\
&\quad = \mathbb E_{X,\eta,\trueweights,a(0)}\|K_t(\gram)X^\top z/n+e^{-t\Lambda}a(0) - (I_d-K_t(\gram)X^\top X/n)\trueweights\|^2\\
&\quad = \mathbb E_{X,\eta,\trueweights,a(0)}\|K_t(\gram)X^\top z/n - e^{-t\Lambda}a(0)-(I_d - K_t(\gram)\gram)\trueweights\|^2\\
&\quad = \sigma_{\eta}^2\cdot\mathbb E_X\frac{1}{n}\trace(K_t(\gram)^2\gram) +  \sigma_0^2\cdot\mathbb E_X\frac{1}{d}\trace(e^{-2t\gram}) + \sigma_\star^2\cdot\mathbb E_{X}\frac{1}{d}\trace((I_d-K_t(\gram)\gram)^2)\\
&\quad = \sigma_{\eta}^2\cdot\mathbb E_X\frac{1}{n}\trace(K_t(\gram)^2\gram) + \sigma_0^2\cdot\mathbb E_X\frac{1}{d}\trace(e^{-2t\gram}) + \sigma_\star^2\cdot \mathbb E_{X}\frac{1}{d}\trace((I_d-K_t(\gram)\gram)^2)\\
&\quad = \underbrace{\sigma_{\eta}^2\cdot \mathbb E_{X}\frac{1}{n}\sum_{j=1}^{r}\frac{(1-e^{-t\lambda_j})^2}{\lambda_j}}_{\text{Variance}} + \underbrace{(\sigma_0^2+\sigma_\star^2)\mathbb E_{X}\frac{1}{d}\left(d-r+\sum_{j=1}^d e^{-2t\lambda_j}\right)}_{\text{Bias}}
\end{split}
\end{eqnarray*}
Let $\mathrm{INR} := 1/\mathrm{SNR}= \sigma_\eta^2/\sigma_\star^2$, the "label-noise ratio", which captures the relative amount of label-noise, and also define $\mathrm{INR} := \sigma_0^2/\sigma_\star^2$, the "initialization-noise ratio" which captures the relative amount of noise in the initialization. We can write things more informatively like so
\begin{eqnarray}
\begin{split}
\mathbb E_{X,\eta,\trueweights,a(0)}\frac{\etest(t)}{\sigma_\star^2} &= \mathrm{INR}\cdot \mathbb E_\Lambda\frac{1}{n}\sum_{j=1}^{r}\frac{(1-e^{-t\lambda_j})^2}{\lambda_j}\\
&\quad\quad + (1+\mathrm{INR})\cdot\left(1-\frac{r}{d}+\mathbb E_\Lambda \frac{1}{d}\sum_{j=1}^r e^{-2t\lambda_j}\right).
\end{split}
\end{eqnarray}
In the limit $t \to \infty$, $n,d \to \infty$, $d/n \to \gamma_1$,
\begin{itemize}
\item The ($\sigma_\star^2$-normalized) variance term converges to $ \dfrac{\mathrm{INR}}{1-\max(1,1/\gamma_1)}$, with a singularity / pole at the interpolation threshold $\gamma_1=1$.
\item The ($\sigma_\star^2$-normalized) bias term converges to zero
$$
(1+\mathrm{INR})\cdot(1-1/\gamma_1)_+ = \begin{cases}
(1+\mathrm{INR})\cdot (1-1/\gamma_1),&\mbox{ if }\gamma_1 \ge 1,\\
0,&\mbox{ if }\gamma_1 \le 1,\\
\end{cases}
$$
\end{itemize}

\section{Dynamics of robustness}
Since the intialization $a(0)$ is centered independent of the training data, the terms $\overline a(t)$ and $c(t)$ in \eqref{eq:dynamics} have zero cross-correlation, i.e
\begin{eqnarray}
\begin{split}
\mathbb E\, \overline a(t)^\top c(t) &= \mathbb E\, a(0)^\top e^{-t\gram}K_t(\gram)X^\top y/n = 0.
\end{split}
\end{eqnarray}
One then computes the average squared $L_2$-norm of the model weights $a(t)$ at time $t$ like so,
\begin{eqnarray*}
\begin{split}
&\mathbb E_{X,\eta,\trueweights,a(0)}\|a(t)\|^2 = \mathbb E_{X,\eta,\trueweights,a(0)} \|\overline a(t)+c(t)\|^2\\
&\quad = \mathbb E_{X,\eta,\trueweights,a(0)} \|\overline a(t)\|^2+\mathbb E_{X,\eta,\trueweights}\|c(t)\|^2\\
&\quad = \mathbb E_{X,a(0)}a(0)^\top e^{-2t\gram} a(0)+ \mathbb E_{X,\eta}\| c(t)\|^2 \\
&\quad = \sigma_0^2\cdot\mathbb E_X \frac{1}{d}\trace(e^{-2t\gram}) + \mathbb E_{X,\eta,\trueweights}\|K_t(\gram)X^\top (X\trueweights+\eta)/n\|^2\\
&\quad = \sigma_0^2\cdot\mathbb E_\Lambda \frac{1}{d}\trace(e^{-2t\Lambda}) + \mathbb E_{X,\trueweights}\,\trueweights^\top \frac{X^\top X}{n} K_t(\gram)^2\frac{X^\top X}{n}\trueweights + \mathbb E_{X,\eta}\,\eta^\top \frac{X K_t(\gram)^2 X^\top}{n^2}\eta\\
&\quad = \sigma_0^2\cdot\mathbb E_\Lambda \frac{1}{d}\trace(e^{-2t\Lambda}) + \sigma_\star^2\cdot \mathbb E_X \frac{1}{d}\trace(\gram K_t(\gram)^2\gram) + \sigma_\eta^2\cdot \mathbb E_X \frac{1}{n}\trace(\gram K_t(\gram)^2)\\
&\quad = \sigma_0^2\cdot\mathbb E_\Lambda \frac{1}{d}\sum_{j=1}^de^{-2t\lambda_j} + \sigma_\star^2\cdot\mathbb E_\Lambda\frac{1}{d}\sum_{j=1}^r(1-e^{-t\lambda_j})^2 + \underbrace{\sigma_\eta^2\cdot \mathbb E_\Lambda \frac{1}{n}\sum_{j=1}^{r} \frac{(1-e^{-t\lambda_j})^2}{\lambda_j}}_{\text{Variance}}.
\end{split}
\end{eqnarray*}
This can be rewritten as 
\begin{eqnarray}
\begin{split}
\mathbb E_{X,\eta,\trueweights,a(0)}\frac{\|a(t)\|^2}{\sigma_\star^2} &= \mathrm{INR}\cdot\mathbb E_\Lambda \frac{1}{d}\sum_{j=1}^de^{-2t\lambda_j} + \mathbb E_\Lambda\frac{1}{d}\sum_{j=1}^d(1-e^{-t\lambda_j})^2\\
&\quad\quad + \mathrm{INR}\cdot \mathbb E_\Lambda \frac{1}{n}\sum_{j=1}^{r} \frac{(1-e^{-t\lambda_j})^2}{\lambda_j}.
\label{eq:linearwnorm}
\end{split}
\end{eqnarray}

\subsection{Linear models with isotropic data}
In particular, suppose an isotropic distribution of data $P_x = N(0,I_d)$. In the limit $t \to \infty$, $n,d \to \infty$, $d/n \to \gamma_1$,
\begin{itemize}
    \item The sum of the first and second terms converges to
    $$
    \mathrm{INR}\cdot (1-1/\gamma_1)_+ + \min(1,1/\gamma_1) =  \begin{cases}
        1,&\mbox{ if }\gamma_1 < 1,\\
    \mathrm{INR}\cdot(1-1/\gamma_1) + 1/\gamma_1,&\mbox{ if }\gamma_1 \ge 1,\\
    \end{cases}
    $$
\end{itemize}

\section{Random features neural network model}
Suppose the distribution of the covariates is $P_z = \phi_{\#} P_x \in \mathcal P(\mathbb R^m)$, the pushforward of $P_x$ under the random feature mapping $\phi$ from $\mathbb R^d$ to $\mathbb R^m$ given by
 \begin{eqnarray}
 \phi(x):=\sigma(Wx) = (\sigma(x^\top w_1),\ldots,\sigma(x^\top w_m))\text{ with }W=(w_1,\ldots,w_m) \in \mathbb R^{m \times d},
 \end{eqnarray}
 where $w_1,\ldots,w_d \overset{iid}{\sim} N(0,(1/m)I_m)$ are the hidden weights of two-layer neural network with activation function $\sigma:\mathbb R \to \mathbb R$. 
 
 \paragraph{Hermite coefficients.}
 We will assume the activation function $\sigma$ is square-integrable w.r.t to $N(0,1)$. For any integer $k \ge 0$, let $c_k(\sigma) := \mathbb E_{g \sim N(0,1)}[\mathrm{He}_k(g)\sigma(g)]$ be the order $k$ Hermite coefficient of $\sigma$ and let $\theta(\sigma):=c_0(\sigma^2)-c_1(\sigma)^2$. By \emph{Stein's Lemma}, it is clear that $\theta(\sigma) \ge 0$.
 
 At time $t$, the prediction of the model on a random test point $x \sim P_x$ is $f_t(x) = a(t)^\top \phi(x)$, where $a(t)$ is the $m$-dimensional vector of output weighs at time $t$, where the output weights $a(t) \in \mathbb R^m$ are given by the gradient-flow
 \begin{eqnarray}
\dot a(t) = -\nabla \etrain(f_t) = -Z^\top(Za(t)-y)/n = -Ga(t) + c,
\end{eqnarray}
where $c:=Z^\top y/n \in \mathbb R^m$ and
% \paragraph{Nonlinear Gram matrix and linear equivalent.}
% Consider the $m\times m$ random matrix $\gram$ defined by
\begin{eqnarray}
\nonlingram:=Z^\top Z/n \in \mathbb R^{m \times m},\text{ with }
Z = \phi(X) = \sigma(XW^\top) \in \mathbb R^{n \times m}.
\label{eq:Z}
\end{eqnarray}

% \begin{restatable}[Centered activation function]{cond}{}{}
% $c_0(\sigma)=0$.
% \label{cond:centered}
% \end{restatable}
It was established in \url{https://arxiv.org/abs/1904.03090} that
\begin{restatable}[Gaussian Equivalence Theorem]{prop}{}{}
The random matrix $\nonlingram$ defined in \eqref{eq:Z} has the same limiting spectral density (LSD) as the random matrix
\begin{eqnarray}
\frac{1}{n}Z_{\mathrm{lin}}^\top Z_{\mathrm{lin}},
\end{eqnarray}
where $Z_{\mathrm{lin}} := \sqrt{\theta(\sigma)}Z_0+c_1(\sigma)XW^\top \in \mathbb R^{n \times m}$, with $Z_0 \in \mathbb R^{n \times m}$ random matrix having iid entries from $N(0,1)$, and independent of $Z$ and $W$.
\end{restatable}

 \subsection{The norm of the output weights $a(t)$}
 Proceeding as in Section xyz, we obtain a representation \eqref{eq:linearwnorm}, but with $d$ replaced with $m$, i.e.,
\begin{eqnarray}
\begin{split}
\mathbb E_{X,\eta,\trueweights,a(0)}\frac{\|a(t)\|^2}{\sigma_\star^2} &= \mathrm{INR}\cdot\mathbb E_\Lambda \frac{1}{m}\sum_{j=1}^me^{-2t\lambda_j} + \mathbb E_\Lambda\frac{1}{m}\sum_{j=1}^m(1-e^{-t\lambda_j})^2\\
&\quad\quad + \mathrm{INR}\cdot \mathbb E_\Lambda \frac{1}{n}\sum_{j=1}^m \frac{(1-e^{-t\lambda_j})^2}{\lambda_j}1_{\lambda_j > 0},%\\
% &\ge \mathrm{INR}\cdot \min(1,\rho)e^{-2t\lambda_1}+(1-\rho)_+\\
% &\quad\quad + \min(1,\rho)\cdot(1-e^{-t\lambda_1})^2 \\
% &\quad\quad +\frac{1}{\mathrm{SNR}}\cdot \min(1,1/\rho)\frac{(1-e^{-t\lambda_1})^2}{\lambda_1}.
\end{split}
\end{eqnarray}
where the $\lambda_j$'s are now the eigenvalues of $\nonlingram$.

\subsection{Dynamics of robustness}
 For a test data point $x \sim \Rd$, let $f_t(x) = a(t)^\top \phi(x)$ be the prediction of the neural network at time $t$. One computes the robustness / stability of $f_t$ as
 \begin{eqnarray}
  \mathfrak{S}(f_t)^2 = \mathbb E_{P_x}\,\|\nabla f_t(x)\|^2 = a(t)^\top Ca(t),
 \end{eqnarray}
 where $C=C(W)$ is the $m \times m$ random psd matrix with entries given by
 \begin{eqnarray}
 C_{jk} = (w_j^\top w_k)\mathbb E_{P_x}[ \sigma'(x^\top w_j)\sigma'(x^\top w_k)].
 \end{eqnarray}
 Note that $\mathfrak{S}(f_t)^2$ is a random variable due to randomness in $X$, $W$, $\eta$, $a(0)$, and $a_\star$.
 Define the $m \times m$ random psd matrix $S(X)$ by
 \begin{eqnarray}
 S(X) := \frac{1}{n}\mathbb E_{f_\star}[f_\star(X)^\top f_\star(X)].
 \end{eqnarray}
 Thanks to \eqref{eq:dynamics} with $\overline{a}(t) = e^{-t\nonlingram}a(0) \in \mathbb R^m$, $c(t) = K_t(\nonlingram)c \in \mathbb R^m$, and $c=Z^\top y/n=Z^\top (f_\star(X)+\eta)/n=Z^\top f_\star(X)/n+Z^\top \eta / n \in \mathbb R^m$, one deduces
 \begin{eqnarray}
 \begin{split}
 \overline{\mathfrak{S}}(f_t)^2 &:=\mathbb E_{\{X,W\}}\, \mathfrak{S}(f_t)^2 = \mathbb E_{\{X,W,\eta,a(0)\}}\,a(0)^\top e^{-t\nonlingram}Ce^{-t\nonlingram} a(0)\\
 &\quad\quad+ \mathbb E_{\{X,W,\eta,f_\star\}}\,\frac{1}{n^2}f_\star(X)Z K_t(\nonlingram)CK_t(\nonlingram) Z^\top f_\star(X)^\top \\
 &\quad\quad + \mathbb E_{\{X,W\}}\,\frac{1}{n^2}\eta^\top ZK_t(\nonlingram)CK_t(\nonlingram)Z^\top \eta \\
 &= \sigma_0^2\cdot \mathbb E_{\{X,W\}}\,\frac{1}{m}\trace(e^{-2t\nonlingram}C)\\
 &\quad\quad + \mathbb E_{\{X,W\}}\,S(X)\frac{1}{n}Z K_t(\nonlingram)CK_t(\nonlingram) Z^\top\\
 &\quad\quad + \sigma_\eta^2\cdot \mathbb E_{\{X,W\}}\,\frac{1}{n}\trace(\nonlingram K_t(\nonlingram)^2C)\\
 &\ge \mathbb E_W \lambda_{\min}(C)\cdot\left(E_1(t)+E_2(t) + E_3(t)\right)-o_m(1),
 \end{split}
 \end{eqnarray}
 where $E_{1,2,3}(t)$ are defined by
 \begin{align}
 E_1(t) &:= \sigma_0^2\cdot \mathbb E_{X,W}\frac{1}{m}\trace(e^{-2t\nonlingram}) = \sigma_0^2\cdot\left(1-\frac{r}{m}+\mathbb E_{W,X}\frac{1}{d}\sum_{j=1}^r e^{-2t\lambda_j}\right)\\
    E_2(t) &:= \mathbb E_{X,W} \trace(S(X)\frac{1}{n}ZK_t(\nonlingram)^2Z^\top),% = \mathbb E_{X,W}\frac{1}{m}\sum_{j=1}^r(1-e^{-t\lambda_j})^2,
    \\
     E_3(t) &:= \sigma_\eta^2\cdot\mathbb E_{X,W}\frac{1}{n}\trace(\nonlingram K_t(\nonlingram)^2) = \sigma_\eta^2\cdot\mathbb E_{X,W}\frac{1}{n}\sum_{j=1}^r\dfrac{(1-e^{-t\lambda_j})^2}{\lambda_j}.
 \end{align}
 
%  In particular, if $\gamma_2 < 1$ and $\sigma_\star>0$, then there exists a sufficiently large (but finite) time $t_0=t_0(\sigma_0,\sigma_\star,\ldots)>0$ such that the first term $E_1(t)$ in the above display is negligible compared to the second and third, and so
%  \begin{eqnarray}
%  \overline{\mathfrak{S}}(f_t)^2 \le \overline{\mathfrak{S}}(f_\star)^2,\,\forall t \ge t_0.
%  \end{eqnarray}
%  That is, the student is eventually more robust / stable than the teacher, on average. For example, in the case where the output weights are initialized at zero, i.e., $\sigma_0=0$, the above inequality holds with $t_0=0$.

\subsection{Special cases}
\paragraph{Linear ground-truth} Suppose the ground-truth function is $f_\star(x) := a_\star(x)^\top \phi(x)$. The we have $S(X) = G$, and so $E_2(t) = \mathbb R$

\subsection{Emergence of double-descent in robustness curve}
Note that if $\sigma_\eta>0$ and
\begin{eqnarray}
\lim_{\substack{n,d,m \to \infty\\d/n \to \gamma_1,\,d/m \to \gamma_2}} \mathbb E_{X,W}\frac{1}{n}\trace(\nonlingram^\dagger) = \infty,
\end{eqnarray}
then $\lim\overline{\mathfrak{S}}(f_t) \ge \lim E_3(t) = \infty$ for any fixed $t \in (0,\infty]$. In particular, this would explain the results empirically observed in Dohmatob (2021).
\lorem
\lorem

\lorem 

\section{EWMD in the "correlated noise" data model}
\label{sec:known}
As in (Stephenson et al.) \url{https://arxiv.org/pdf/2108.12006.pdf}, fix $\sigma_\star^2$ and $\sigma_\epsilon^2$ and consider the following model
\begin{mdframed}
\textbf{Data model with correlated noise.}
\begin{align}
    w_\star &\sim N(0,(\sigma_\star^2/d) I_d),\\
    x_1,\ldots,x_n &\overset{iid}{\sim} P_X = N(0,I_d),\text{ independent of }w_\star,\\
    X &=  (x_1,\ldots,x_n) \in \mathbb R^{n \times d},\\
    \mathrm{SVD}\, X/\sqrt{n} &= U\Lambda^{1/2} V^\top,\text{ with }\Lambda = \diag(\lambda_1,\ldots,\lambda_r),\\
    \epsilon &= U\eta,\text{ with }\eta \sim N(0,\alpha(\Lambda))\text{ independent of }(X,w_\star),\\
    y_i &= x_i^\top w_\star + \epsilon_i,\text{ for all }i \in [n],
\end{align}
where $\alpha(\Lambda)$ is the $r \times r$ diagonal matrix defined by
$$
\alpha(\Lambda)_{j,j} := \begin{cases}0,&\mbox{ if }\lambda_j \le 1,\\
(n/d)\sigma_\epsilon^2,&\mbox{else.}
\end{cases}
$$
\end{mdframed}
Here $r=\min(n,d)$ is the rank of $X$\footnote{Note that indeed, $X$ has full rank, i.e $r=\min(n,d)$ w.p $1$.}.
Thus,
\begin{itemize}
\item The noise is correlated across different samples.
\item Noise enters eigen-directions of design matrix $X$ at different rates; the most informative directions are the most noisy.
\end{itemize}
The signal-to-noise ratio of the problem is given by $\mathrm{SNR} = \sigma_\star^2/\sigma_\epsilon^2$.

We shall work in the following high-dimensional limit
\begin{eqnarray}
\label{eq:proportionate}
n \to \infty,\, d/n \to \gamma \in (0,\infty).
\end{eqnarray}
The edge case $\gamma \to 0^+$ subsumes the setting where the input-dimension $d$ is fixed, while the sample size $n$ is cranked up.

\subsection{Gradient-descent}
Define $Q:=X^\top X/n = \sum_i x_ix_i^\top/n \in \mathbb R^{d \times d}$, $c:=X^\top y/n = X^\top (Xw_\star+\epsilon)/n \in \mathbb R^d$, where $y := (y_1,\ldots,y_n)$ is the response vector and $\epsilon := (\epsilon_1,\ldots,\epsilon_n)$ is the noise vector, so that $y=Xw_\star + \epsilon$.
% Note that, modulo rescaling, $Q$ has the same nonzero eigenvalues as the Gram matrix $G:=XX^\top/d$.
Gradient-descent on mean-squared error $\etrain(w) := \|Xw-y\|^2/n$ with stepsize $s$ gives
\begin{eqnarray}
\begin{split}
w(t) = w(t-1)-\alpha X^\top (Xw-y)/n &= (I_d-\alpha Q)w(t-1)+\alpha c\\
&= \ldots = \widetilde{w}(t)+c(t),
\end{split}
\end{eqnarray}
where $\widetilde{w}(t) := (I_d-\alpha Q)^t w(0) \in \mathbb R^d$, $c(t) := K_t(Q) c \in \mathbb R^d$, with
\begin{eqnarray}
K_t(Q) := \alpha\sum_{s=0}^{t-1}(I_d-\alpha Q)^s.
\end{eqnarray}
It is clear that $Q$ has eigenvalues $(\lambda_j)_{j \in [n]}$, whilst $K_t(Q)$ has eigenvalues given by
\begin{eqnarray}
\lambda_j(K_t(Q)) = K_t(\lambda_j)= \alpha\sum_{s=0}^{t-1}(1-\alpha\lambda_j)^s=\begin{cases}\dfrac{1-(1-\alpha\lambda_j)^t}{\lambda_j},&\mbox{ if }\lambda_j > 0,\\ t,&\mbox{ if }\lambda_j=0,
\end{cases}
\label{eq:specK}
\end{eqnarray}

The initial point $w(0)$ is assumed to be drawn from $N(0,(\sigma_0^2/d)I_d)$, independently of the data the training data. Define the initialization-noise ratio $\mathrm{INR} := \sigma_0^2/\sigma_\star^2$.

\subsection{Dynamics of test error}
At time $t$, the prediction of a random test datapoint $x \sim P_x=N(0,I_d)$ is $x^\top w(t)$, and so one computes the test error as
\begin{eqnarray}
\begin{split}
\etest(w(t)) &= \mathbb E_x(x^\top w(t)-x^\top w_\star)^2 = \|w(t)-w_\star\|^2\\
&= \|(I_d-\alpha Q)^t w(0)+K_t(Q)(X^\top w_\star+\epsilon)/n-w_\star\|^2.
\end{split}
\end{eqnarray}
Assuming that $w(0)$ is independent of $w_\star$ and $\epsilon$, we compute the test error average over all sources of randomness, denoted $\overline\varepsilon(t)$, as follows
\begin{eqnarray}
\label{eq:calc}
\begin{split}
    \overline{\mathrm{err}}_{\mathrm{test}}(t) &:= \mathbb E_{\{w_\star,X,z,w(0)\}} \etest(w(t))\\
    & =  \mathbb E_{\{w_\star,X,\epsilon,w(0)\}}\|(I_d-\alpha Q)^t w(0)+K_t(Q)X^\top(X w_\star+\epsilon)/n-w_\star\|^2\\
    &= \mathbb E_{\{X,w(0)\}}\|(I_d-\alpha Q)^tw(0)\|^2+\mathbb E_{\{X,\epsilon\}}\|K_t(Q)X^\top \epsilon/n\|^2\\
    &\quad\quad\quad+ \mathbb E_{\{w_\star,X\}}\|(I_d-K_t(Q)Q)w_\star\|^2\\
    &= \sigma_0^2\cdot \mathbb E_X \frac{1}{d}\trace((I_d-\alpha Q)^{2t})) + \mathbb E_X\frac{1}{n}\trace(K_t(Q)^2\cov((X/\sqrt{n})^\top \epsilon \mid X))\\
    &\quad\quad\quad + \sigma_\star^2\cdot \mathbb E_X \frac{1}{d}\trace((I_d-K_t(Q)Q)^2)\\
    &= \sigma_0^2\cdot \mathbb E_X \frac{1}{d}\sum_{j}(1-\alpha\lambda_j)^{2t} + \sigma_\epsilon^2\cdot \mathbb E_X\frac{1}{d}\sum_{j \mid \lambda j > 1}\frac{(1-(1-\alpha\lambda_j)^t)^2}{\lambda_j}\\
    &\quad\quad\quad + \sigma_\star^2\cdot \mathbb E_X \frac{1}{d}\sum_{j}(1-\alpha\lambda_j)^{2t}.
\end{split}
\end{eqnarray}
Note that we have used the facts that 
\begin{eqnarray*}
\begin{split}
\cov((X/\sqrt{n})^\top \epsilon \mid X) &= \cov(V\Lambda^{1/2}U^\top \epsilon \mid X)\\
&= \cov(V\Lambda^{1/2} z \mid X) = (n/d)\sigma_\epsilon^2 V\alpha(\Lambda)\Lambda V^\top,
\end{split}
\end{eqnarray*}
and $K_t(Q)^2 = VK_t(\Lambda)^2 V^\top$, which combine with \eqref{eq:specK} to give
\begin{eqnarray}
\begin{split}
\frac{1}{n}\trace(VK_t(Q)^2\cov((X/\sqrt{n})^\top\epsilon \mid X)) &= \frac{(n/d)\sigma_\epsilon^2}{n}\trace(VK_t(\Lambda)^2\alpha(\Lambda)\Lambda V^\top)\\
&= \frac{\sigma_\epsilon^2}{d}\trace(K_t(\Lambda)^2\alpha(\Lambda)\Lambda)\\
&=\frac{\sigma_\epsilon^2}{d}\sum_{j \mid \lambda j > 1}K_t(\lambda_j)^2\lambda_j\\
&= \frac{\sigma_\epsilon^2}{d}\sum_{j \mid \lambda j > 1}\frac{(1-(1-\alpha\lambda_j)^t)^2}{\lambda_j}.
\end{split}
\end{eqnarray}
Taking limits in \eqref{eq:calc}, we recover the following result
\begin{restatable}[Stephenson et al. (2021)]{prop}{}{}
It holds in the limit \eqref{eq:proportionate} that
\begin{eqnarray}
\label{eq:ewdd}
\begin{split}
\frac{\overline{\mathrm{err}}_{\mathrm{test}}(t)}{\sigma_\star^2} &\to
(1+\mathrm{INR})\left(\int_{a(\lambda)}^{b(\lambda)} (1-\alpha\lambda)^{2t}\mu_{\mathrm{MP}(\gamma)}(\lambda)\,\dv\lambda + \left(1-\frac{1}{\gamma}\right)_+\right)\\
&\quad\quad\quad+ \frac{1}{\mathrm{SNR}}\int_1^{b(\lambda)} \frac{(1-(1-\alpha\lambda)^t)^2}{\lambda}\mu_{\mathrm{MP}(\gamma)}(\lambda)\,\dv\lambda
    \end{split}
\end{eqnarray}
where $a(\gamma) := (1-\sqrt{\gamma})^2$ and $b(\gamma):=(1+\sqrt{\gamma})^2$ are the endpoints of bulk of the Marchenko-Pastur density $\mu_{\mathrm{MP}(\gamma)}$ with shape parameter $\gamma$, defined by
\begin{eqnarray}
\mu_{\mathrm{MP}(\gamma)}(\lambda) = \dfrac{\sqrt{(\lambda-a(\gamma))(b(\gamma)-\lambda)}}{2\pi\gamma \lambda}
1_{a(\gamma) \le \lambda \le b(\gamma)} + \left(1-\frac{1}{\gamma}\right)_+\delta_0(\lambda).
\end{eqnarray}
\end{restatable}


\section{Open directions}
\textcolor{red}{\textit{Out dated section contents!}}

\subsection{Other models of data}
We could consider different data models. For example
\begin{itemize}
\item[(2)] Data model with "source condition", i.e the ground-truth weights are given by $w_\star \sim N(0,\phi(\Sigma))$ where $\Sigma$ is the population covariance matrix of the covariates, and $\phi(\Sigma)$ has the same eigenvectors as $\Sigma$ by eigenvalues transformed by $\lambda \mapsto \phi(\lambda)$. For example $\phi(\lambda) \propto 1/\lambda$. Such models have been recently studied by Rozasco and co-workers.
\item[(3)] The signal + noise model suggested by Nourredine.
\item[(4)] ...
\end{itemize}


\subsection{Neural networks and kernel methods} We could consider the case of learning with wide neural networks , in the following regimes:
\begin{itemize}
\item infinite-width RF
\item infintie-width NTK
\item width but finite-width RF
\item width but finite-width NTK
\end{itemize}
The first two regimes as instances of regression in RKHS, and thanks to representer theorems + RMT, should be reducible to the case of ordinary regression (i.e the case studied in Stephenson et al.).

Presumably, the last 2 regimes will be the most difficult (because the Gram matrix $(G)_{ik} = m^{-1}\sum_{j=1}^m \sigma(x_i^\top w_j)\sigma(x_k^\top w_j)$ has nasty structure which is difficult to analyze, unlike the kernel regimes). However, all we need is the limiting spectral distribution of the Gram matrix (even in implicit form, via fixed-point equations, etc.). Maybe we can use Noureddine's "uniform CLT" to reduce the situation to the kernel regime ? 


==> early-stopped adversarial training/other_files/source_condition.tex <==
\section{Source condition}
Let $\Sigma = V\Lambda V^\top = \sum_{j=1}^d \lambda_j v_j v_j^\top$ and $\phi(\Sigma) := \sum_j \phi(\lambda_j)v_jv_j^\top$. Consider the data model
\begin{eqnarray}
\begin{split}
x_1,\ldots,x_n &\sim N(0,\Sigma),\\
w_\star &\sim N(0, (r_\star^2/d)\phi(\Sigma)),\\
\epsilon &\sim N(0,\sigma_\eta^2 I_n),\\
y_i &= x_i^\top w_\star + \epsilon_i,\text{ for all }i \in [n]
\end{split}
\end{eqnarray}

\begin{eqnarray}
\begin{split}
e(t) &= \mathbb E_{\{X,w_\star,\epsilon,w(0)\}}\|w(t)-w_\star\|^2_\Sigma\\
&= \mathbb E_{\{X,w_\star,\epsilon,w(0)\}}\|(I_d-sQ)^t w(0) + K_t(Q)X^\top (Xw_\star+\epsilon)/n-w_\star\|_\Sigma^2\\
&= \mathbb E_{\{X,w(0)\}}\|(I_d-sQ)^tw(0)\|^2_\Sigma + \mathbb E_{\{X,w_\star\}}\|(I_d-K_t(Q)Q)w_\star\|_\Sigma^2\\
&\quad\quad\quad+ \mathbb E_{\{X,\epsilon\}}\frac{1}{n}\|K_t(Q)(X/\sqrt{n})^\top \epsilon\|_\Sigma^2\\
&= \sigma_0^2 \mathbb E_X\frac{1}{d}\trace((I_d-sQ)^t \Sigma (I_d-sQ)^t)\\
&\quad\quad\quad+ \sigma_\star^2\mathbb E_X\frac{1}{d}\trace(Q(I_d-K_t(Q))\Sigma(I_d-K_t(Q))Q\phi(\Sigma))\\
&\quad\quad\quad+ \sigma_\epsilon^2\mathbb E_X\frac{1}{n}\trace(X K_t(Q)\Sigma K_t(Q) X^\top / n)\\
&= \sigma_0^2 \mathbb E_X\frac{1}{d}\trace((I_d-sQ)^{2t} \Sigma)+ \sigma_\star^2\mathbb E_X\frac{1}{d}\trace((I_d-sQ)^t\Sigma(I_d-sQ)^t\phi(\Sigma))\\
&\quad\quad\quad + \sigma_\epsilon^2\mathbb E_X\frac{1}{n}\trace(K_t(Q)^2 Q\Sigma)\\
\end{split}
\end{eqnarray}

==> early-stopped adversarial training/sections/Eformulaproof.tex <==
\subsection{Proof of Lemma~\ref{lm:fench}: Analytic Formula for Adversarial Risk}
Recall the adversarial risk functional $E$ defined in \eqref{eq:Ewr}.

\fench*
For the proof, we will need the following auxiliary lemma.

\begin{restatable}{lm}{}
For any $x,w \in \mathbb R^d$, $r \ge 0$ and $y \in \mathbb R$, the following identity holds
\begin{eqnarray}
    \sup_{\|\delta\| \le r}((x+\delta)^\top w - y)^2 = (|x^\top w - y| + r\|w\|_\star)^2.
\end{eqnarray}
\label{lm:wellknown}
\end{restatable}
\begin{proof}
Note that $h(x,\delta)/2 = \eta(x)^2/2 + g(x,\delta)/2$, where $g(x,\delta) := w(\delta)^2-2\eta(x)w(\delta)$, and $\eta(x) := w(x) - y$, and $w(x) := x^\top w$. Now, because the function $z \to z^2/2$ is its own Fenchel-Legendre conjugate, we can "dualize" our problem as follows
\begin{eqnarray*}
\begin{split}
\sup_{\|\delta\| \le r}g(x,\delta)/2 &= \sup_{\|\delta\|_\star \le r}-\eta(x)w(\delta) + \sup_{z \in \mathbb R} zw(\delta) - z^2/2\\
&=\sup_{z \in \mathbb R}-z^2/2 + \sup_{\|\delta\| \le r}(z-\eta(x))w(\delta)\\
&= \sup_{z \in \mathbb R}r\|w\|_\star|z-\eta(x)| - z^2/2\\
&= \sup_{s \in \{\pm 1\}}\sup_{z \in \mathbb R}rs(z-\eta(x))-z^2/2\\
&= \sup_{s \in \{\pm 1\}}-r\|w\|_\star s\eta(x)+\sup_{z \in \mathbb R}r\|w\|_\star sz-z^2/2\\
&= \sup_{s \in \{\pm 1\}}-r\|w\|_\star s\eta(x) + r^2\|w\|_\star^2 /2\\
&= r\|w\|_\star |\eta(x)|+r^2\|w\|^2_\star /2.
\end{split}
\end{eqnarray*}
We deduce that
\begin{align*}
\sup_{\|\delta\| \le r}h(x,\delta)/2 &= \eta(x)^2/2+r\|w\|_\star |\eta(x)|+r^2\|w\|_\star^2 /2 = (|\eta(x)|+r\|w\|_\star)^2/2,
\end{align*}
as claimed.
\end{proof}
\begin{proof}[Proof of Lemma \ref{lm:fench}]
Indeed, thanks to Lemma \ref{lm:wellknown} with $y=x^\top w_0$, one has
$$
E^{\|\cdot\|}(w,w_0,r) := \mathbb E_{x \sim N(0,\Sigma)}\sup_{\|\delta\|\le r} h(x,\delta) = \mathbb E_{x \sim N(0,\Sigma)}[(\eta(x)+r\|w\|_\star)^2],
$$
where the functions $h$ and $\eta$ are as in the proof of Lemma \ref{lm:wellknown}. The result then follows upon noting that
\begin{eqnarray*}
\begin{split}
\mathbb E_{x \sim N(0,\Sigma)}[\eta(x)^2] &= \mathbb E_{x \sim N(0,\Sigma)}[(x^\top w - x^\top w_0)^2] = \|w-w_0\|_\Sigma^2,\\
\mathbb E_{x \sim N(0,\Sigma)}|\eta(x)| &= \mathbb E_{x \sim N(0,\Sigma)}|x^\top w - x^\top w_0| = c_0\|w-w_0\|_\Sigma, 
\end{split}
\end{eqnarray*}
where $c_0 := \sqrt{2/\pi}$.
\end{proof}


==> early-stopped adversarial training/sections/GDfailure_l1.tex <==
In high-dimensions (i.e large $d$), consider the ground-truth model $w_0 = (1,1/d^\alpha,\ldots,1/d^\alpha)$, for some positive constant $\alpha \in (0,1)$ to be prescribed later. Note that
\begin{align}
\|w_0\|_2 &= \sqrt{1 + (d-1)/d^{2\alpha}} \asymp 1,\text{ if }\alpha > 1/2,\\
\|w_0\|_1 &= 1 + (d-1)/d^\alpha = 1+d^{1-\alpha} \gg 1.
\end{align}
Thus, the optimal rescaling $a w_0$ achieves an adversarial risk of
\begin{eqnarray}
\|w_0\|_2^2 \land r^2\|w_0\|_1^2 = 1+o_d(1)\text{ for fixed }r\text{ and large }d.
\end{eqnarray}
Now, let $w=(c,0,\ldots,0)$ for some positive scalar $c$ to be prescribed later. It is clear that
\textcolor{red}{Meyer: $\|w-w_0\|_2^2 &= (c-1)^2+\frac{d-1}{d^{2\alpha}}$ ca pose pb du coup...} Ah, oui. Bon, tant pis! Oui... c'est chiant ce truc 
\begin{align}
    \|w-w_0\|_2^2 &= c^2+\frac{d-1}{d^{2\alpha}} \asymp c^2,\text{ if }c \gtrsim d^{1/2-\alpha}\\
    \|w\|_1 &= c.
\end{align}
\begin{mdframed}
The important thing here is that $w$ is a sparse vector (arbitrarily small $L_1$-norm) which approximates $w_0$ in $L_2$-norm, arbitrarily well.
\end{mdframed}

Thus, the adversarial risk of this choice for $w$ is $E(w,r) \asymp (\|w-w_0\|_2 + r\|w\|_1)^2 = (1+r)^2c^2$, and gives an upper bound for the optimal adversarial risk $E_{opt}(r)$. Therefore,
\begin{restatable}{thm}{}
For large $d$ and fixed $r,c>0$, and $\alpha \in (1/2,1)$, one has
\begin{eqnarray}
\frac{\inf_{\widehat w} E(\widehat w,r)}{E_{opt}(r)} \gtrsim \frac{1}{(1+r)^2 c^2},
\label{eq:bang}
\end{eqnarray}
where the infimum is over all rescalings, i.e models of the form $a w_0$ for some $a \in [0,1]$.
\end{restatable}
It is clear that the RHS of \eqref{eq:bang} can be made arbitrarily large by choosing $c$ sufficiently smaller than $1/(1+r)$. For example, taking $c=d^{1/2-\alpha}$, we obtain:
\begin{restatable}{cor}{}
For any $r>0$ and $\alpha \in (1/2,1)$,
\begin{eqnarray}
\frac{\inf_{\widehat w} E(\widehat w,r)}{E_{opt}(r)} \gtrsim \frac{d^{2\alpha-1}}{(1+r)^2} \overset{d \to \infty}{\longrightarrow} \infty,
\label{eq:bangbang}
\end{eqnarray}
\end{restatable}

==> early-stopped adversarial training/sections/L1business.tex <==
\subsection{Algorithm 2: Simple Thresholding-Based Algorithm in the Case of $\ell_\infty$-Norm Attacks}
Now, suppose the covariance matrix of the features $\Sigma$ is diagonal, i.e $\Sigma = \diag(\lambda_1,\ldots,\lambda_d)$. In the case of $\ell_\infty$-attacks, we provide a much simpler and faster algorithm for computing the second stage of our proposed estimator. Indeed, for $\ell_{\infty}$-attack we obtain an explicit form of the optimal solution minimizing Eq.~(\ref{eq:Etilde}) as shown in the next Proposition.
% Indeed, applying the previous Lemma \ref{lm:subdifferential} with $a=w_0$ and $g:=r\|\cdot\|_1$, we obtain that the minimizer of $w \mapsto \|w-w_0\|_\Sigma + r\|w\|_1$ is of the form $w(t)$, for some $t \in [0,\infty]$, where
% \begin{eqnarray}
% w(t) := (I+rt\Sigma^{-1} \partial \|\cdot\|_1)^{-1}(w_0),
% \end{eqnarray}
% i.e
% $(w_\star)_j:=\mbox{ST}((w_0)_j; rt/\lambda_j)$ for all $j \in [d]$,
% and $\mbox{ST}(\cdot;s)$ is the \emph{soft-thresholding} operator at level $s$, defined component-wise by
% \begin{eqnarray}
% \mbox{ST}(u; s) = (|u|-s)_+\mbox{sign}(u).
% \end{eqnarray}
% The interesting thing here is that $\mbox{ST}(u; s)=0$ as soon as $s \ge |u|$. Define the scalar $c=c(w_0,\Sigma)$ by
% \begin{eqnarray}
% c := \max_{1 \le j \le d}|(w_0)_j| \lambda_j.
% \end{eqnarray}
We deduce the following result.
\begin{restatable}{prop}{}
Let $c := \max_{1 \le j \le d}|(w_0)_j| \lambda_j$. There exists $t \in [0,c]$ such that $w(t) \in \mathbb R^d$ is  a minimizer of the convex function $w \mapsto \|w-w_0\|_\Sigma + r\|w\|_1$, where
\begin{eqnarray}
w(t)_j = \mbox{ST}((w_0)_j;rt/\lambda_j),\text{ for all }j \in [d].
\label{eq:STsol}
\end{eqnarray}
and $\mbox{ST}(\cdot;s)$ is the soft-thresholding operator at level $s$.
\end{restatable}
An inspection of \eqref{eq:STsol} reveals a kind of feature-selection. Indeed, if the $j$th component of the ground-truth model $w_0$ is small in the sense that $|(w_0)_j| \le rt/\lambda_j$, then $w(t)_j = 0$, i.e the $j$th component of $w_0$ should be suppressed. On the other hand, if $|(w_0)_j| \ge rt/\lambda_j$, then $(w_0)_j$ should be replaced by the translated version $(w_0)_j - \mathrm{sign}((w_0)_j)rt/\lambda_j$. That is weak components of $w_0$ are suppressed, while strong components are boosted.

 The result is Algorithm~\ref{alg:st}, a simple method for computing \textbf{Stage 2} of our proposed two-stage estimator (Algorithm \ref{alg:twostage}). Refer to Figure \ref{fig:algos} for an empirical illustration.

\begin{algorithm}
\caption{Non-uniform soft-thresholding which implements \textbf{Stage 2} of Algorithm \ref{alg:twostage} for diagonal covariance matrix under $\ell_\infty$-attacks.}
\textbf{Inputs: } $\widehat w_0, \widehat \Sigma$
\label{alg:st}
\begin{algorithmic}[1]
    \State \textbf{Compute} $\widehat c=\max_{1 \le j \le d}|(\widehat w_0)_j|\widehat\lambda_j$.
    \State \textbf{For each} $t$ in a finite grid of values between $0$ and $\widehat c$, use held-out to retain the value of $t$ for which the adversarial risk of $\widehat w(t)$ is minimal, where each component of $\widehat w(t)$ is given by
    $\widehat w(t)_j = \mbox{ST}((\widehat w_0)_j;rt/\widehat \lambda_j)$.
    \State \textbf{Return} $\widehat w(t)$.
    \end{algorithmic}
    \end{algorithm}
% Using the well-known \emph{Moreau Decomposition Formula} together with the facts that (1) The convex conjugate of a norm is the (convex-analytic) indicator function of the unit-ball of the dual norm; (2) the proximal operator of the indicator function of a closed convex set is the orthogonal projection operator thereupon,
% we know that, $\mbox{prox}_{\tau \|\cdot\|_\star}(w_0)$ is zero for $\|w_0\| \le \tau$, the above tractable procedure can be extended to any norm!


==> early-stopped adversarial training/sections/conclusion.tex <==
\section{Concluding Remarks}
In our work, we have undertaken a study of the robustness of gradient-descent (GD), under test-time attacks in the context of linear regression. Our work provides a clear characterization of when GD and a modified version (GD+) --with feature-dependent learning rates-- can succeed to achieve the optimal adversarial risk (up to an absolute constant). This characterization highlights the effect over the covariance structure of the features, and also, of the norm used to measure the strength of the attack.

Finally, our paper proposes a statistically consistent and simple two-stage estimator which achieves optimal adversarial risk in the population regime, up to within a constant factor. Our proposed estimator adapts to attacks w.r.t general norms, and to the covariance structure of the features.




==> early-stopped adversarial training/sections/experiments.tex <==



==> early-stopped adversarial training/sections/general_attacks.tex <==
% \section{Some Lower and Upper-Bounds for General Norms}
% \subsection{A sufficient condition for optimality}
% \label{subsec:sufficientGD}
% Consider an arbitrary attack norm $\|\cdot\|$ with dual $\|\cdot\|_\star$. We will produce a sufficient condition under which early-stopping on a specific modified GD attains optimal adversarial risk (up to within a multiplicative absolute constant). 

% Let us consider $g(w_0) \in \mathbb R^d$ be a subgradient of $\Vert\cdot\Vert_\star$ at $w_0$. Then $\|g(w_0)\| \le 1$ and $g(w_0)^\top w_0 =\|w_0\|_\star$. For example, in the case of $\ell_\infty$-norm attacks, one may take $g(w_0) = (\mbox{\sign}(w_{0,1}),\ldots,\mbox{sign}(w_{0,d}))$, with $\mbox{sign}(0) := 0$.
% In the case of of a Mahalanobis-norm attack where $\|\cdot\| = \|\cdot\|_B$ for some positive-definite matrix $B$, one can take $g(w_0) =Bw_0/\|w_0\|_B$ with $g(0) = 0$. Let us denote
% \begin{eqnarray}
% \lambda:=\frac{\|g(w_0)\|}{\|g(w_0)\|_{\Sigma^{-1}}}
% \end{eqnarray}
% For example, in the case of $\ell_\infty$-norm attacks, we have $\lambda \geq 1/ \sqrt{\text{Trace}(\Sigma^{-1})}$; In the case of euclidean attacks, we have $\lambda\geq\sqrt{\lambda_{min}^{\Vert\cdot\Vert_2}(\Sigma)}$ and more gerenarlly, for Mahalanobis attacks where $\|\cdot\| = \|\cdot\|_B$ with $B$ a positive-definite matrix, we have that $\lambda\geq \sqrt{\lambda_{min}^{\Vert\cdot\Vert_2}(B^{1/2}\Sigma^{1/2}B^{1/2})}$ can be taken. Let us now introduce the following useful lemma.
% \begin{lemma}
% \label{lem-lower-bound-adv-gene}
% Let $w_0\in\mathbb{R}^d$ and $r>0$. Then we have that
% \begin{align*}
%     \sqrt{\alpha E^{\Vert\cdot\vert}_{opt}(w_0,r)}\geq \sup_{z\in B_2^d \cap rB_{\|\Sigma^{1/2}\cdot\|}}\langle z,\Sigma^{1/2}w_0\rangle
% \end{align*}
% \end{lemma}
% Define $z(w_0) := (r \land \lambda)\Sigma^{-1/2}g(w_0) \in \mathbb R^d$, and observe that
% \begin{align}
% \|\Sigma^{1/2}z(w_0)\| &\le r\|g(w_0)\| \le r,\\ \|z(w_0)\|_2 &\le \lambda\|g(w_0)\|_{\Sigma^{-1}} \le  \|g(w_0)\|\le 1.
% \end{align}
% Thus, $z(w_0) \in B_2^d \cap rB_{\|\Sigma^{1/2}\cdot\|}$. Then using Lemma~\ref{lem-lower-bound-adv-gene}, it follows that
% \begin{eqnarray}
% \begin{split}
% \sqrt{\alpha E_{opt}^{\Vert\cdot\Vert}(r,w_0)} &\ge \max_{z \in B_2^d \cap rB_{\|\cdot\|^{\Sigma}}}z^\top \Sigma^{1/2}w_0\\
% &\ge z(w_0)^\top\Sigma^{1/2} w_0= (r \land \lambda)g(w_0)^\top w_0\\
% &= (r\land \lambda)\|w_0\|_\star,
% \end{split}
% \end{eqnarray}
% where $\alpha :=1/(1+\sqrt{2/\pi}) \approx 1.1124$.
% % Therefore, if the ground-truth model $w_0$ is "dense" in the sense that the following \emph{local condition} holds: (see examples later)
% % \begin{restatable}[Sufficient condition]{cond}{}
% % \label{cond:dense}
% % There exists a subgradient $g(w_0)$ of $\Vert\cdot\Vert_{*}$ at $w_0$ such that $\frac{\|g(w_0)\|}{\|g(w_0)\|_{\Sigma^{-1}}} \gtrsim c\frac{\|w_0\|_{\Sigma}}{ \|w_0\|_\star }$, for some absolute positive constant $c$.
% % \end{restatable}
% Let us now define
% \begin{align*}
%     c:=\frac{\lambda \Vert w_0\Vert_*}{ \Vert w_0\Vert_{\Sigma}}
% \end{align*}
% then $\alpha E_{opt}^{\Vert\cdot\Vert}(w_0,r) \ge c^2\|w_0\|_{\Sigma}^2 \land r^2\|w_0\|_\star^2 \ge (1 \land c^2) (\|w_0\|_{\Sigma}^2 \land r^2\|w_0\|_\star^2)$ which matches the value of $E^{\Vert\cdot\Vert}(w,w_0,r)$ attained by the optimal recaling of $w_0$. Thus, we arrive at the following result.
% \begin{restatable}{thm}{}
% % Suppose Condition \ref{cond:dense} is in order. 
% Denote $c:=\dfrac{\|g(w_0)\| \|w_0\|_*}{\|g(w_0)\|_{\Sigma^{-1}} \|w_0\|_{\Sigma}}$.
% Then, for any positive $r$, it holds that
% \begin{eqnarray*} \frac{\inf_{t \ge 0}E^{\Vert\cdot\Vert}(\Sigma^{-1/2}w_c^{\Sigma^{-1/2}}(t,w_0),w_0,r)}{E_{opt}^{\Vert\cdot\Vert}(w_0,r)} \le (1 \lor 1/c^2)\alpha.
% \end{eqnarray*}
% \label{thm:GDrocksdeterministic}
% \end{restatable}

% In particular, for the case of $\ell_\infty$-norm attacks, we have the following corollary.
% \begin{restatable}{cor}{}
% Consider the case where $\ell_\infty$-norm attacks. If there exists an absolute constant $\gamma>0$ such that $\|w_0\|_1 \ge \gamma \sqrt{d}\|w_0\|_2$, then
% \begin{eqnarray*} \frac{\inf_{t \ge 0}E^{\Vert\cdot\Vert}(\Sigma^{-1/2}w_c^{\Sigma^{-1/2}}(t,w_0),w_0,r)}{E_{opt}^{\Vert\cdot\Vert}(w_0,r)} \le \alpha \lor \frac{\alpha\kappa^{\Vert\cdot\Vert_2}(\Sigma)}{\gamma^2}.
% \end{eqnarray*}
% \end{restatable}
% For example, when with $w_0=(1,\ldots,1)$ --or equivalently, random $w_0 \asymp N(0,I_d)$, one can take $\gamma=1$, and observe that $\|w_0\|_1 \gtrsim d$, $\|w_0\|_2 \asymp \sqrt{d}$.


% \subsection{The Case of Failure for GD}
% We now exhibit a case where GD and general rescaling schemes fail miserably to find robust models even when they exist. Indeed, consider the case where feature covariance matrix is $\Sigma_x = I_d$ and the attacker's norm is $\ell_\infty$.
% \begin{restatable}{thm}{}
% For any value of the input-dimension $d$, it is possible to construct $w_0 \in \mathbb R^d$ and $r > 0$ such that in the limit $d \to \infty$, it holds that
% \begin{align}
% r \to 0,\,r\sqrt d &\to \infty,\\
% \frac{E_{rescale}(w_0,r)}{E_{opt}(w_0,r)} &\to \infty,
% \end{align}
% where $E_{rescale}(w_0,r)$ is the optimal adversarial risk achieved by models of the form $w=\beta w_0$ for some $\beta \in \mathbb R$. In particular, the adversarial risk of (early-stopped) GD tends to $\infty$ in the limit $d \to \infty$.
% \label{thm:bangbang}
% \end{restatable}
% \begin{proof}
% \textcolor{red}{Elvis: If we run out of space, move the proof to Appendix.}
% Let $a,\lambda>0$, $w_0:=(a+\lambda,\dots,a+\lambda,\lambda,\dots,\lambda)$ and let $\alpha\geq 1$ be the number of coordinate such that $w_{0,i}=a+\lambda$. Concrete values for $a$, $\lambda$, and $\alpha$ will be prescribed later. For such model we obtain that
% \begin{align*}
%     \Vert w_0\Vert_1 &= d\lambda + \alpha a~~\text{and}\\
%      \Vert w_0\Vert_2 &=\sqrt{\alpha(a+\lambda)^2 + (d-\alpha) \lambda^2}\\
%      &= \sqrt{\alpha a^2 + d \lambda^2 + 2\alpha a \lambda}.
% \end{align*}
% Therefore the shrinkage model obtains an error equals to:
% \begin{align*}
%     E_{rescale}(w_0,r)=\min(\alpha a^2 + d \lambda^2 + 2\alpha a \lambda, r^2( d\lambda + \alpha a)^2).
% \end{align*}
% Now let $w:=(\underbrace{a,\dots,a}_{\alpha\text{ times}},0,\dots,0)$, we obtain that
% \begin{align*}
%     \sqrt{E_{opt}(w_0,r)}\leq \Vert w - w_0\Vert_2 + r\Vert w\Vert_1=\sqrt{d}\lambda + r\alpha a
% \end{align*}
% Let us now consider the case where \begin{eqnarray}
% r=\lambda=\frac{1}{d^{1/4}\log d},\, 
% \alpha = d^{1/2},\, a=1.
% \end{eqnarray}
% Then, for large $d$ we obtain that
% \begin{align}
% &\Vert w - w_0\Vert_2 + r\Vert w\Vert_1\asymp \frac{d^{1/4}}{\log d}\\
%   &r\Vert w_0\Vert_1 \asymp  \frac{d^{1/2}}{(\log d)^2},\,\Vert w_0\Vert_2 \asymp d^{1/4}
% \end{align}
% from which follows that
% \begin{align*}
%     \frac{E_{rescale}(w_0,r)}{E_{opt}(w_0,r)}\geq \frac{\min(d^{1/2},\frac{d}{(\log d)^4})}{\frac{d^{1/2}}{(\log d)^2}}\asymp (\log d)^2\rightarrow +\infty,
% \end{align*}
% as claimed.
% \end{proof}
% \begin{mdframed}
% Here are the real assumptions of my proof: indeed if we have that
% \begin{align*}
%   \alpha\rightarrow+\infty,~~r\sqrt{d}\rightarrow+\infty,~~r\sqrt{\alpha}&\rightarrow 0, ~~\frac{ a}{\lambda}\asymp\frac{\sqrt{d}}{r\alpha}
% \end{align*}
% Then the result holds. 

% \textcolor{red}{Elvis: In fact one can show that the condition $r \to 0$ is not removable. Indeed, for any $w_0$ and \emph{fixed} $r$, one has
% $E_{rescale}(w_0,r)/E_{opt}(w_0,r) \le \max(1,r)/\min(1,r)$ which cannot turn to $\infty$ in the limit $d \to \infty$.
% }
% \end{mdframed}
% % \input{sections/GDfailure_l1}


% % \input{sections/GDfailure_l1}


==> early-stopped adversarial training/sections/junk.tex <==

\section{Without the second condition}
\subsection{Gaussian widths}
Let $g$ be an $N$-dimensional standard Gaussian random vector. Given a subset $T$ of $\mathbb R^N$,  its \emph{Gaussian width} $\omega(T)$, is defined by
\begin{eqnarray}
\mathbb E\,\sup_{x \in T}x^\top g.
\end{eqnarray}
For example, it is well-known that $\omega(B_2^N) \asymp \sqrt{N}$ while $\omega(B_1^N) \asymp \sqrt{\log N}$

\subsection{Gordon's generalization of Slepian's Lemma}
\begin{restatable}{prop}{}
Let $(X_{u,v})$ and $(Y_{u,v})$ be Gaussian processes such that $\|X_{u,v}-X_{u',v'}\| := \sqrt{\mathbb E\,(X_{u,v}-X_{u',v'})^2} \le \|Y_{u,v}-Y_{u',v'}\|$ for all $u,v,u',v'$, with equality if $u=u'$. Then,
\begin{eqnarray}
\mathbb E\,\inf_u \sup_v X_{u,v} \ge  \mathbb E\,\inf_u\sup_v Y_{u,v}.
\end{eqnarray}
\end{restatable}

\subsection{Results}
\begin{restatable}{thm}{}
Let $G$ be a an $m \times d$ random matrix with iid entries from $N(0,1)$. Then,
\begin{eqnarray}
\mathbb E\,\inf_{x \ne 0}\frac{\|(G^\top G)^{1/2}x\|_2}{\|x\|_\star} \ge (\sqrt{m}-\omega(B_{\|\cdot\|_\star}))_+^2,
\end{eqnarray}
\end{restatable}

\begin{restatable}{cor}{}
Let $G$ be as in previous theorem. Then,
\begin{align}
\mathbb E\,\inf_{x \ne 0}\frac{\|(G^\top G)^{1/2}x\|_2}{\|x\|_1} &\ge (\sqrt{m}-\sqrt{d})_+^2,\\
\mathbb E\,\inf_{x \ne 0}\frac{\|(G^\top G)^{1/2}x\|_2}{\|x\|_1} &\ge (\sqrt{m}-c\sqrt{\log d})_+^2,
\end{align}
for some absolute constant $c$.
\end{restatable}

==> early-stopped adversarial training/sections/minimax.tex <==
\section{Minimax Optimality for $\ell_p$-norm Attacks}
In this section, we will establish a minimax lower-bound for the proxy adversarial risk functional $\widetilde E$ defined in \eqref{eq:Etilde}, in the case of general feature covariance matrix $\Sigma$ and attacker norm is $\|\cdot\|_p$ with $p \in [2,\infty]$. Then, we will show that this lower-bound is attained by our proposed two-stage estimator proposed in the previous section. Thanks to Lemma \ref{lm:sandwich}, these considerations will also give a minimax theory upto a multiplicative constant, for the true adversarial risk functional $E$ defined in \eqref{eq:Ewrdef}.

\subsection{The Statistical Setup}
Consider the case where the ground-truth model $w_0$ is $s$-sparse, i.e $w_0 \in B_0^d(s)$, for some $s \in [d]$.
Consider an $\ell_p$-norm attack of magnitude $r \ge 0$. We are interested in the following minimax problem
\begin{eqnarray}
\label{eq:minimax}
\inf_{\widehat w_n}\sup_{w_0 \in B_0^d(s)}\widetilde E(\widehat w_n,w_0,r),
\end{eqnarray}
where $\widetilde E(w,w_0,r)$ is the (proxy) adversarial risk of the model $w$, as defined in \eqref{eq:Etilde}, and the infimum is taken over all estimators $\widehat w_n$ of $w_0$, based on the iid dataset $\mathcal D_n=\{(x_1,y_1),\ldots,(x_n,y_n)\}$ given in \eqref{eq:generative}. Let $X=(x_1,\ldots,x_n) \in \mathbb R^{n \times d}$ be the design matrix, and
define the following scalars
\begin{align}
\underline\theta(X,s) &:= \inf_{\delta \in B_0^d(s),\,\delta\ne 0} \dfrac{\|X\delta\|_2}{\sqrt{n}\|\delta\|_2}\label{eq:thetalow},\\
\overline\theta(X,s) &:= \sup_{\delta \in B_0^d(s),\,\delta\ne 0} \dfrac{\|X\delta\|_2}{\sqrt{n}\|\delta\|_2}\label{eq:thetahigh}.
\end{align}
In particular, $\overline\theta(X,1) = \max_{j \in [d]}\|Xe_j\|_2/\sqrt{n}$, where $e_j$ is the $j$th standard basis unit-vector in $\mathbb R^d$ so that $Xe_j \in \mathbb R^n$ is the $j$th column of $X$. Also, it should be clear that one always has the following estimates\footnote{As, a side note, these estimates can be arbitrarily loose.}
\begin{eqnarray}
\lambda_{min}(\widehat \Sigma) \le \underline\theta(X,s)^2 \le \overline\theta(X,s)^2 \le \lambda_{max}(\widehat \Sigma),
\end{eqnarray}
 where $\widehat \Sigma := X^\top X/n$ is the empirical covariance matrix as usual.
% \begin{restatable}{rmk}{}
Note that a condition of the form
\begin{eqnarray}
1-\delta_s \le \underline\theta(X,s) \le \overline\theta(X,s) \le  1+\delta_s
\end{eqnarray}
for some $\delta_s \in (0,1)$ is equivalent to a Restricted Isometry Property (RIP) for the rescaled design matrix $X/\sqrt{n}$. 
% \end{restatable}

Let $\lambda_{min} = \lambda_{min}(\Sigma)$ (resp. $\lambda_{max}=\lambda_{\max}(\Sigma)$) be the smallest (resp. largest) eigenvalue of the covariance matrix $\Sigma$. In what follows, we assume the attacker's norm is an $\ell_p$-norm for some $p \in [1,\infty]$. Let $q=q(p) \in [1,\infty]$ be the harmonic conjugate of $p$, i.e., $1/p + 1/q = 1$.

\subsection{Minimax Lower-Bounds}
\begin{restatable}{thm}{minimaxlb}
For any $p \in [2,\infty]$ and $s \in [1,d/2]$, the following minimax lower-bound on robustness error for $\ell_p$-norm attacks holds w.h.p over the noise vector $\epsilon \in \mathbb R^n$
\begin{eqnarray*}
\begin{split}
% &
\inf_{\widehat w_n}\sup_{w_0 \in B_0^d(s)}\frac{\widetilde E(\widehat w_n,w_0,r)}{\sigma_\epsilon^2}
% \\ &\quad\quad\quad
\gtrsim \frac{\log(ed/s)}{n \overline\theta(X,1)^2} (s\lambda_{min} \lor r^2 s^{2/q}).
% \begin{cases}
% r^2s^{2/q},&\mbox{ if }r\gtrsim \sqrt{\lambda_{min}/s^{2/q-1}},\\
% \lambda_{min}s,&\mbox{ else.}
% \end{cases}
\end{split}
\end{eqnarray*}
In particular, consistent $\ell_p$-norm adversarial regression in $B_0^d(s)$ can only happen if
$rs^{1/q}\sqrt{\log(ed/s)} = o(\sqrt n)$.
\label{thm:minimaxlb}
\end{restatable}

The result in proved in Appendix xyz. In the special case of $\ell_\infty$-norm attacks, we have the following corollary.
\begin{restatable}{cor}{}
If $1 \le s \le d/2$, then the following minimax lower-bound on robustness error for $\ell_\infty$-norm attacks holds w.h.p over the noise vector $\epsilon \in \mathbb R^n$
\begin{eqnarray}
\begin{split}
% &
\inf_{\widehat w_n}\sup_{w_0 \in B_0^d(s)} \frac{\widetilde E(\widehat w_n,w_0,r)}{\sigma_\epsilon^2}
% \\
% &\quad\quad\quad
\gtrsim  \frac{s\log(ed/s)}{n \overline\theta(X,1)^2} (\lambda_{min} \lor r^2 s) .
% \begin{cases}
% r^2s^2,&\mbox{ if }r \gtrsim \sqrt{\lambda_{min}/s},\\
% \lambda_{min}s,&\mbox{ else.}
% \end{cases}
\end{split}
\label{eq:minimaxlowerbound}
\end{eqnarray}
In particular, consistent $\ell_\infty$-norm adversarial regression in $B_0^d(s)$ can only happen if
$r s\sqrt{\log(ed/s)} = o(\sqrt n)$.
\end{restatable}

\subsection{Minimax Optimality of Proposed Estimator}
We will now show that our proposed two-stage estimator attains the minimax lower-bound in \eqref{eq:minimaxlowerbound}.

For any $c \ge 0$, define the nonnegative scalar
\begin{eqnarray}
\label{eq:theta}
\theta(X,s,c) := \inf_{\delta \in B^d_1(s,c)}\frac{\|X\delta\|_2}{\sqrt{n}\|\delta\|_2},
\end{eqnarray}
where $B^d_1(s,c) := \{\delta \in \mathbb R^d \mid 0 < \|\delta\|_1 \le (1+c)\sqrt{s}\|\delta\|_2\}$. Note that $B_0^d(s) \subseteq B_0^d(s,c)$ for all $c \ge 0$. The following technical condition was introduced in \cite{BickelSimultaneous2009} (see also \cite{BellecSlopeMeets2018}).
\begin{restatable}[Sparse Restricted Eigenvalue (SRE) condition]{cond}{sre}
\label{cond:sre}
$\overline\theta(X,1) = O(1)$ and $\theta(X,s,c) > 0$.
\end{restatable}
The following result is one of our main contributions.
\begin{restatable}[Minimax optimality of the square-root Lasso for robust learning]{thm}{minimax}
\label{thm:minimax}
Suppose Condition SRE$(s,7)$ is in order with $1 \le s \le d/2$.
Suppose the first stage of our two-stage estimator is the square-root Lasso (SQL) estimator $\widehat w_n^L(\lambda)$ with tuning parameter \begin{eqnarray}
\label{eq:lambdaoptlasso}
\lambda \asymp \sqrt{\dfrac{\log(2d/s)}{n}}.
\end{eqnarray}
Then our final estimator is minimax optimal in \eqref{eq:minimax}, uniformly for all $\ell_p$-norm attacks with $p \in [2,\infty]$.

In particular, in the noiseless case where $\sigma_\epsilon=0$, the OLS estimator (if it exists!), is minimax optimal uniformly on $p$.
\end{restatable}
% \textcolor{red}{Elvis: We probably need an estimator which doesn't require knowledge of the sparsity level $s$. This can be done via a so-called \emph{Lepski-type procedure} \url{https://arxiv.org/pdf/1703.02907.pdf}.}


==> early-stopped adversarial training/sections/minimax_proofs.tex <==
\section{Minimax Theory}
\subsection{Proof of Theorem \ref{thm:minimaxlb}: Minimax Lower-Bound}
\minimaxlb*
\begin{proof}[Proof of Theorem \ref{thm:minimaxlb}]
It was shown in [Theorem 7.1, Bellec et al. 2018] \url{https://arxiv.org/pdf/1605.08651.pdf} that if $1 \le s \le d/2$, then 
\begin{eqnarray}
\Delta(s,q) := \inf_{\widehat w_n}\sup_{w_0 \in B_0^d(s)}\|\widehat w_n - w_0\|_q \gtrsim \frac{\sigma_\epsilon}{\overline\theta(X,1)}\cdot \psi(q),
\end{eqnarray}
holds w.h.p over the noise vector $\epsilon \in \mathbb R^n$, where
$\psi(s,q) :=  s^{1/q}\sqrt{\dfrac{\log(ed/s)}{n}}$.
Since $\|\widehat w_n - w_0\|_{\Sigma}^2 \ge \lambda_{\min}\|\widehat w_n - w_0\|_2^2$, we deduce from \eqref{eq:reconciled} that w.h.p and in expectation over the noise vector $\epsilon \in \mathbb R^n$,
\begin{eqnarray*}
\begin{split}
\inf_{\widehat w_n}\sup_{w_0 \in B_0^d(s)} \widetilde E_p(\widehat w_n,r)  &\gtrsim \sigma_\epsilon^2\cdot \max(\lambda_{\min}(\Sigma)\Delta(s,2)^2, r^2 \Delta(q,s)^2)\\
&\gtrsim \frac{\sigma_\epsilon^2\cdot}{\overline\theta(X,1)^2} \cdot \max(\lambda_{\min}(\Sigma)\psi(s,2)^2,r^2\psi(s,q)^2)\\
&= \frac{\sigma_\epsilon^2}{\overline\theta(X,1)^2}\cdot \frac{\log(ed/s)}{n}\cdot \max(\lambda_{\min}(\Sigma)s, r^2 s^{2/q}),
\end{split}
\end{eqnarray*}
which completes the proof.
% The first part of the result then follows upon noting that $r^2s^{2/q} \ge \lambda_{\min}\cdot s$ iff $r \ge \sqrt{\lambda_{\min}/s^{2/q-1}}$.
\end{proof}

\subsection{Minimax Optimality of Our Proposed Two-Stage Estimator}
Note the definition of $\theta(X,s,c)$ from \eqref{eq:theta} and recall the following condition
\sre*

We restate the theorem to be proved for convenience.
\minimax*
The following oracle bound which established in \cite{BellecSlopeMeets2018}, will be crucial to the proof.
\begin{restatable}[Corollary 4.3 of \cite{BellecSlopeMeets2018}]{prop}{}
Suppose Condition SRE$(X,s,7)$ is in order and the ground-truth model $w_0$ is $s$-sparse. Consider a Lasso estimator $\widehat w_n^L(\lambda)$ tuned with $\lambda \ge \lambda_{n,d,r,1/2}^\star$ where
\begin{eqnarray}
\lambda_{n,d,s,\gamma}^\star := \sigma_\epsilon\cdot \frac{4+\sqrt{2}}{\gamma}\sqrt{\frac{\log(2e d/s)}{n}},\text{ for all }\gamma \in (0,1).
\end{eqnarray}
Then, for any $1 \le q \le 2$, it holds w.h.p over  the noise vector $\epsilon \in \mathbb R^n$, the following holds for the Lasso estimator 
\begin{align}
    \|\widehat w_n^L(\lambda)-w_0\|_q &\lesssim \frac{ \lambda s^{1/q}}{\theta(X,s,7)^2}.
\end{align}
\label{prop:belleclasso}
\end{restatable}

The following result which is a corollary to Proposition \ref{prop:belleclasso} above, will be one of our main workhorses. 
\begin{restatable}{prop}{}
Suppose Condition SRE$(X,s,7)$ is in order and the ground-truth model $w_0$ is $s$-sparse. Let $p \in [2,\infty]$ and let $q=q(p) \in [1,2]$ be the harmonic conjugate of $p$. Consider an $\ell_p$-norm attack of magnitude $r \ge 0$.
Then, for any $\lambda \ge \lambda_{n,d,s,1/2}^\star$ (defined in Prop. \ref{prop:belleclasso}), it holds w.h.p over the noise vector $\epsilon \in \mathbb R^n$ that
\begin{eqnarray}
\widetilde E(\widehat w_n^L(\lambda),w_0,r) \lesssim  \frac{(s\lambda_{max} \lor r^2s^{2/q})\lambda^2}{\theta(X,s,7)^4}.
\label{eq:lassoEtilde}
\end{eqnarray}
\end{restatable}
\begin{proof}
Thanks to Proposition \ref{prop:belleclasso} above, the following hold w.h.p over the noise vector $\epsilon$
\begin{eqnarray*}
\begin{split}
&\widetilde E(\widehat w_n^L(\lambda),w_0,r) \asymp (\|\widehat w_n^L(\lambda)-w_0\|_{\Sigma} + r\|\widehat w_n^L(\lambda)-w_0\|_q)^2\\
&\quad\quad\le (\sqrt{\lambda_{max}}\|\widehat w_n^L(\lambda)-w_0\|_2+r\|\widehat w_n^L(\lambda)-w_0\|_q)^2\\
&\quad\quad\lesssim \left(\frac{\sqrt{\lambda_{max}}\cdot\lambda s^{1/2}}{\theta(X,s,7)^2} +  \frac{r\lambda s^{1/q}}{\theta(X,s,7)^2}\right)^2\\
&\quad\quad= \frac{\lambda^2(s\lambda_{max} \lor r^2 s^{2/q})}{\theta(X,s,7)^4},
\end{split}
\end{eqnarray*}
as claimed.
\end{proof}
We are now read to proof Theorem \ref{thm:minimax}.

\begin{proof}[Proof of Theorem \ref{thm:minimax}]
Indeed, with the choice of $\lambda$ given in \eqref{eq:lambdaoptlasso}, the upper-bound \eqref{eq:lassoEtilde} matches the minimax lower-bound \eqref{eq:minimaxlowerbound}, upto multiplicative absolute constants which only depend on the design matrix $X$, the covariance matrix $\Sigma$, and the noise level $\sigma_\epsilon$.
\end{proof}


==> early-stopped adversarial training/sections/not_include/everything_else.tex <==
\section{Isotropic Case}
In that case, we propose to generalize the above strategy to any positive-definite matrix $M\in\mathcal{S}_d^{++}(\mathbb{R})$. More precisely, we consider the GD descent scheme applied to the following objective function:
\begin{align*}
    E_{M,\Sigma_x}(w):=\mathbb{E}_{(x,y)\sim P_{xy}}(w^T(M^{1/2}\Sigma_x^{-1/2}x)-y)^2
\end{align*}
which leads to the following GD path:
\begin{align*}
    w^{M,\Sigma_x}(t):= (I_d - (I_d - \alpha M)^t)M^{-1/2}\Sigma_x^{1/2}w_0\; , 
\end{align*}
and its continuous version:
\begin{align*}
    w^{M,\Sigma_x}_c(t):= (I_d - e^{-t M}) M^{-1/2}\Sigma_x^{1/2}w_0\;.
\end{align*}
Let us also also introduce the general condition number associated to $M\in\mathcal{S}_{d}^{++}(\mathbb{R})$ defined as
\begin{align*}
    \kappa^{\Vert\cdot\Vert}(M)&:=\lambda_{max}^{\Vert\cdot\Vert}(M)/\lambda_{min}^{\Vert\cdot\Vert}(M),\,\text{where }\\
    \lambda_{max}^{\Vert\cdot\Vert}(M)&:=\sup_{w\neq 0}\frac{\Vert M^{1/2}w\Vert_2^2}{\Vert \Sigma_x^{-1/2} w\Vert_*^2},\text{ and}\\
    \lambda_{min}^{\Vert\cdot\Vert}(M)&:=\inf_{w\neq 0}\frac{\Vert M^{1/2}w\Vert_2^2}{\Vert \Sigma_x^{-1/2} w\Vert_*^2}\; ,
\end{align*}


then we show the following Proposition.
\begin{prop}
For any $r\geq 0$ and $M\in\mathcal{S}_{d}^{++}(\mathbb{R})$, we have 
\begin{align*}
     \inf_{t \geq 0}E^{\Vert\cdot\Vert}(\Sigma_x^{-1/2}M^{1/2}w^{M,\Sigma_x}_c(t),r)\leq 1.68 \kappa^{\Vert\cdot\Vert}(M^{-1}) E^{\Vert\cdot\Vert}_{opt}(r)
\end{align*}
\end{prop}
Therefore along the GD schemes on the transformed data, one can find a $1.6862 \kappa^{\Vert\cdot\Vert}(M^{-1})$-optimally robust predictor. 

\begin{restatable}{assume}{}
There exists an absolute constants $\beta,\beta'$ such that $\beta' \le \|w\|_2 / \|\Sigma_x^{-1/2}w\|_\star \le \beta$  for all nonzero $w \in \mathbb R^d$.
\label{assume:coveringnumber}
\end{restatable}
% For example, in the isotropic case, i.e. $\Sigma_x=I_d$, the above assumption is satisfied with $\beta=1$, whenever the attacker's norm $\|\cdot\|$ is an $\ell_p$-norm with $p \in [2,\infty]$. On the other hand, if the attacker's norm $\|\cdot\|$ is induced by a positive-definite matrix $A$, then the condition is satisfied with $\beta=\|A\|_{op}$, the operator norm of $A$.
% This is because in this case, $\|\cdot\|_\star = \|\cdot\|_q$, where $q=q(p) \in [1,2]$ is the harmonic conjugate of $q$, and $\ell_q$ unit-ball is smaller than euclidean unit-ball (since $q \in [1,2]$), combined with the fact that the euclidean unit-ball has covering number of order $O(3/\epsilon)^d$.

Now, let $m$ be a positive integer and $G$ be an $m \times d$ random matrix with with iid entries from $N(0,1)$. Consider the Wishart random matrix $W_{rand}:=G^\top G$.
The following important lemma is proved in Appendix xyz.
\begin{restatable}{lm}{rmt}
Suppose  Assumption \ref{assume:coveringnumber} is in order. There exist absolute constant $C,\gamma \ge 1$ only depending on $\beta$ such that if $m/d \ge \gamma$, then $\kappa^{\|\cdot\|}(W_{rand}) \le C$ w.h.p.

In particular, it holds w.h.p that $W_{rand}$ is non-singular, and therefore positive-definite.
\label{lm:rmt}
\end{restatable}
Thus, normalizing with the inverse-Wishart random matrix $M_{rand} := W_{rand}^{-1}$ makes early-stopping optimal up to within an \emph{absolute} multiplicative constant!

\begin{thm}
Suppose  Assumption \ref{assume:coveringnumber} is in order. There exist absolute constant $C,\gamma \ge 1$ only depending on $\beta$ such that if $m/d \ge \gamma$, then w.h.p.
\begin{align*}
  \inf_{t \geq 0}E^{\Vert\cdot\Vert}(\Sigma_x^{-1/2}M_{rand}^{1/2}w^{M_{rand},\Sigma_x}_c(t),r)\leq 1.68 C E^{\Vert\cdot\Vert}_{opt}(r)
  \end{align*}
\end{thm}


\subsection{General / non-euclidean attacks}
Consider now the case where $\Sigma_x = \sigma^2 I_d$ but the attacker's norm $\|\cdot\|$ is not necessary euclidean. Note that $\mathcal C(\Sigma_x)$ is now the set of all positive-definite matrices of order $d$.
\begin{restatable}{assume}{}
There exists an absolute constant $\beta$ such that $\|w\|_2 \le \beta\|w\|_\star$ for all $w \in \mathbb R^d$.
\label{assume:coveringnumber}
\end{restatable}
For example, the above assumption is satisfied with $\beta=1$, whenever the attacker's norm $\|\cdot\|$ is an $\ell_p$-norm with $p \in [2,\infty]$. On the other hand, if the attacker's norm $\|\cdot\|$ is induced by a positive-definite matrix $A$, then the condition is satisfied with $\beta=\|A\|_{op}$, the operator norm of $A$.
% This is because in this case, $\|\cdot\|_\star = \|\cdot\|_q$, where $q=q(p) \in [1,2]$ is the harmonic conjugate of $q$, and $\ell_q$ unit-ball is smaller than euclidean unit-ball (since $q \in [1,2]$), combined with the fact that the euclidean unit-ball has covering number of order $O(3/\epsilon)^d$.

Now, let $m$ be a positive integer and $G$ be an $m \times d$ random matrix with with iid entries from $N(0,1)$. Consider the Wishart random matrix $W_{rand}:=G^\top G$.
The following important lemma is proved in Appendix xyz.
\begin{restatable}{lm}{rmt}
Suppose  Assumption \ref{assume:coveringnumber} is in order. There exist absolute constant $C,\gamma \ge 1$ only depending on $\beta$ such that if $m/d \ge \gamma$, then $\kappa^{\|\cdot\|}(W_{rand}) \le C$ w.h.p.

In particular, it holds w.h.p that $W_{rand}$ is non-singular, and therefore positive-definite.
\label{lm:rmt}
\end{restatable}
Thus, normalizing with the inverse-Wishart random matrix $M_{rand} := W_{rand}^{-1}$ makes early-stopping optimal up to within an \emph{absolute} multiplicative constant!
\section{A Simple Procedure: Normalization of the Data}


\subsection{Euclidean Attacks on Normalized Data}

\subsection{General Attacks on Normalized Data}


\section{Statistical Study}

\subsubsection{The case where $d=1$}
In the one dimensional setting we obtain the following result.
\begin{prop}
By denoting $\sigma^2$ the covariance of $x$, we obtain that
\begin{itemize}
    \item if $r\leq \sigma \sqrt{2/\pi}$, then $E(t,r)$ is a decreasing function with respect to $t$, in particular we have:
    \begin{align*}
         E(\infty,r)\leq  E(t,r)~~\forall t\geq 0~~\text{and}~~t_{\text{opt}}:=+\infty
    \end{align*}
    \item if $ \sigma \sqrt{2/\pi} < r < \sigma \sqrt{\pi/2}$, then $t\in\mathbb{R}_{+}\xrightarrow{} E(t,r)$ admits a unique mizimizer attained for 
    \begin{align*}
        t_{\text{opt}} := \frac{\log\left(\frac{r(r-\sigma\sqrt{2/\pi})}{\sigma^2 + r^2 - 2\sigma r\sqrt{2/\pi}}\right)}{\log(1-\alpha \sigma^2)}>0
    \end{align*}
    \item if $r\geq \sigma \sqrt{\pi/2}$, then $E(t,r)$ is an increasing function with respect to $t$, in particular we have:
    \begin{align*}
         E(0,r)\leq  E(t,r)~~\forall t\geq 0~~\text{and}~~t_{\text{opt}}:=0\;.
    \end{align*}
\end{itemize}
\label{prop:lowr}
\end{prop}
\begin{proof}\mytodo{Move proof to appendix and only sketch main idea here, mostly in words ?}
In that case we have that 
\begin{align*}
    E(t,r)&= (1 - \alpha \sigma^2)^{2t} \sigma^2  \Vert w_0\Vert^2 + r^2 [1 - (1-\alpha\sigma^2)^{t}]^2 \Vert w_0\Vert^2 \\
    &+ 2 r \sqrt{2/\pi} (1 - \alpha \sigma^2)^{t} \sigma [1 - (1-\alpha\sigma^2)^{t}]\Vert w_0\Vert^2
\end{align*}
which can be written as
\begin{align*}
     E(t,r)&= \Vert w_0\Vert^2[\beta_1 (1 - \alpha \sigma^2)^{2t} +\beta_2 (1 - \alpha \sigma^2)^{t} +\beta_3]
\end{align*}
where
$\beta_1:= [\sigma^2 + r^2 -  2 r \sqrt{2/\pi} \sigma]$, $\beta_2:=-2r^2 +2 r \sqrt{2/\pi}\sigma$ and $\beta_3:=r^2$. Therefore we obtain that
\begin{align*}
    \frac{\partial E}{\partial t}(t,r) = \Vert w_0\Vert^2 \log(1-\alpha \sigma^2)(1 - \alpha \sigma^2)^{t}[2\beta_1 (1 - \alpha \sigma^2)^{t} + \beta_2]
\end{align*}
which gives us that 
\begin{align*}
     \frac{\partial E}{\partial t}(t,r)\leq 0,~~\forall t\geq 0 &\iff \beta_2\geq 0\\
     &\iff r\leq \sqrt{2/\pi}\sigma\; ,
\end{align*}
\begin{align*}
     \frac{\partial E}{\partial t}(t,r)\geq 0,~~\forall t\geq 0 &\iff -\beta_2\geq 2\beta_1\\
     &\iff r\geq \sqrt{\pi/2}\sigma
\end{align*}
otherwise (meaning that $0 < -\beta_2 < 2\beta_1)$ $E$ admits a unique minimizer in $t_{\text{opt}} =\frac{\log(-\beta_2/2\beta_1)}{\log(1-\alpha\sigma^2)}$ from which follows the result.
\end{proof}
In the following proposition, we show that in fact the early-stopping strategy is robust optimal. In the following we denote  $$E^*_r:=\inf_{w \in \mathbb R^d}E(w,r) = \inf_{w\in\mathbb{R}^d}\mathbb{E}\sup_{\Vert \delta\Vert \leq r}(w^\top (x+\delta) - w_0^\top x)^2)$$
\begin{cor}
For all $r\geq 0$, we obtain that the early-stopping strategy is optimal
$E(t_{\text{opt}},r) = E^*_r$.

In particular, we obtain that
\begin{itemize}
    \item If $r\leq \sigma \sqrt{2/\pi}$, then $E(t_{\text{opt}},r) = r^2\Vert w_0\Vert^2$.
    \item If $ \sigma \sqrt{2/\pi} < r < \sigma \sqrt{\pi/2}$, then
    \begin{align*}
    E(t_{\text{opt}},r) =  r^2\Vert w_0\Vert^2  \frac{(1-2/\pi)\sigma^2}{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}.
\end{align*}
\item If $ r \geq \sigma \sqrt{\pi/2}$, then
%\begin{align*}
 $   E(t_{\text{opt}},r) = \Vert w_0\Vert_{\Sigma_x}^2$.
%\end{align*}
\end{itemize}
\end{cor}

\begin{remark}
Observe that the asymptotic regime (true solution of the OLS problem) is not optimal as soon as $r>\sigma \sqrt{2/\pi}$ and therefore early stopping becomes beneficial in this setting. More specifically, we have that if $ \sigma \sqrt{2/\pi} < r < \sigma \sqrt{\pi/2}$
\begin{align*}
   E(t_{\text{opt}},r)/ E(t_{\infty},r)= \frac{(1-2/\pi)\sigma^2}{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}\in]2/\pi,1[
\end{align*}
and if  $ r \geq \sigma \sqrt{\pi/2}$, we obtain that 
\begin{align*}
  E(t_{\text{opt}},r)/ E(t_{\infty},r)= \sigma^2/r^2\leq \frac{2}{\pi}
\end{align*}
Therefore the robust error of the true OLS solution can be arbitrarily large when the radius of the attack $r$ goes to infinity while early stopping is always optimal.   
\end{remark}

Let us now focus on the empirical regime where we have only access to $n\geq 1$ samples from the data distribution. Let us denote $(x_i,y_i)_{i=1}^n$ $n$ i.i.d samples where $x_1\sim\mathcal{N}(0,\Sigma_x)$, $y_1 = w_0^{T}x_1 +\epsilon_1$, $\epsilon_1\sim\mathcal{N}(0,\Sigma_\epsilon)$ and  $\epsilon_1\indep x_1$. In the following we denote $\widehat{\text{Cov}}(x,\epsilon) := \frac{1}{n}\sum_{i=1}^n \epsilon_i x_i$, $\widehat{\Sigma}_x: =\frac{1}{n}\sum_{i=1}^n x_ix_i^\top $, $\widehat{w}(t)=K_t(\widehat{\Sigma}_x)(\widehat{\Sigma}_x w_0+\widehat{\text{Cov}}(x,\epsilon))$ and $\gamma_n:= \widehat{\Sigma}_x^{-1}\widehat{\text{Cov}}(x,\epsilon)$. Let us now present our main result. As we deal with the one dimensional case, we will also denote $\widehat{\sigma}^2:=\widehat{\Sigma}_x$. We have exhibited three regimes which covers all the possible behaviors in the next three following Proposition.


We have an upper-bound control of the tails of $\gamma_n$ as follows.
\begin{prop}
Let $\delta>0$, then as soon as $n>4\log(1/\delta)$ there exists a universal constant $K>0$ such that for all
\begin{align*}
   t\leq \frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})}
\end{align*}

we have that
\begin{align*}
    \mathbb{P}(\gamma_n\geq t)\leq \exp\left(-Knt^2\frac{(1-2\sqrt{log(1/\delta)})^2}{\sigma_\epsilon^4}\right) + \delta
\end{align*}
In particular, as soon as $n>\log(1/\delta)\max(4,1/K)$, then with a probability $\geq 1-2\delta$, we have
\begin{align*}
\gamma_n \leq \sqrt{\frac{\log(1/\delta)}{Kn}}\frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})}
\end{align*}
\end{prop}
\begin{proof}

\end{proof}

% \begin{restatable}{lm}{}
% $|\gamma_n| = o_n(1)$ w.p $1-o_n(1)$.
% \end{restatable}
% \begin{proof}
% Indeed, it is well-known result in classical statistics that, because the dimension is fixed, $\widehat\sigma^2 = \sigma^2+o_{n,\mathbb P}(1)$\footnote{Alternative, a self-contained proof of this fact can be given by direct concentration arguments}. Now, let $z_n:= \frac{1}{n}\sum_{i=1}^n \epsilon_i x_i$. Note that the variance of $z_n$ is $\sigma^2\cdot\sigma_\epsilon^2/n$. A direct application of Chebychev's inequality gives
% $$
% \left|z_n\right| \le t \text{ w.p }1-\frac{\sigma^2\sigma_\epsilon^2}{nt^2}.
% $$
% Taking $t=\sigma\sigma_\epsilon\sqrt{(\log n)/n}$, we deduce that $|z_n| \le \sqrt{(\log n)/n}=o_n(1)$ w.p $1-1/\log n=o_n(1)$.
% \end{proof}
% Note that the confidence in the above lemma can be increased to $1-1/n^c$ (with $c=\Omega(1)$), but $1-1/\log n = o_n(1)$ will suffice for our purposes.

\begin{prop}
Assume that  $\gamma_n\geq 0$, then we obtain that
\begin{itemize}
    \item if $r\in[0,\sigma\sqrt{2/\pi}]$, then $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in
    \begin{align*}
        \hat{t}_{opt} := \frac{\log(\gamma_n/(\gamma_n+\Vert w_0\Vert_2))}{\log(1-\alpha \widehat{\sigma}^2)}>0~~\text{and}~~
        E(\widehat{w}(\hat{t}_{opt}),r) = r^2\Vert w_0\Vert^2
    \end{align*}
    \textcolor{red}{Elvis: Note that $\hat t_{opt} = \omega_{n,\mathbb P}(1)$ since $\gamma_n = o_{n,\mathbb P}(1)$.}
    \item if $r\in]\sigma\sqrt{2/\pi},\sigma\sqrt{\pi/2}[$, then $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in
      \begin{align*}
       & \hat{t}_{opt} := \frac{\log\left(\frac{r^2(\Vert w_0\Vert+\gamma_n)+\sigma^2\gamma_n - r\sqrt{2/\pi}\sigma (\Vert w_0\Vert +2\gamma_n)}{(c+\gamma_n)(\sigma^2 + r^2 - 2r\sqrt{2/\pi}\sigma)}\right)}{\log(1-\alpha \widehat{\sigma}^2)}>0~~\text{and}\\
        &E(\widehat{w}(\hat{t}_{opt}),r) = r^2\Vert w_0\Vert^2  \frac{(1-2/\pi)\sigma^2}{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}
    \end{align*}
    \item if $r\geq\sigma\sqrt{\pi/2} $, then $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in 
     \begin{align*}
        \hat{t}_{opt} := 0~~\text{and}~~
        E(\widehat{w}(\hat{t}_{opt}),r) = \Vert w_0\Vert_{\Sigma_x}^2\;.
    \end{align*}
\end{itemize}
\end{prop}

\begin{prop}
Assume that $\gamma_n\in[-\Vert w_0\Vert,0[$, and let us denote $$\sigma \sqrt{\pi/2}\geq \tilde{r}(\gamma_n):=\frac{2\sqrt{2/\pi}\sigma\left[(\Vert w_0\Vert+2\gamma_n)+\sqrt{\Vert w_0\Vert^2 - (2\pi-4)\gamma_n(\Vert w_0\Vert +\gamma_n)}\right]}{4(\Vert w_0\Vert +\gamma_n)}\geq \sigma\sqrt{2/\pi}.$$ \textcolor{red}{Elvis: Note that $\tilde{r}(\gamma_n) = \sigma\sqrt{2/\pi}+o_{n,\mathbb P}(1)$.} Then we obtain that
\begin{itemize}
    \item  if  $r\in[0,\tilde{r}(\gamma_n)]$ then $t\xrightarrow{} E(\widehat{w}(t),r)$ is a decreasing function, in particular we have that $\hat{t}_{opt} := +\infty$ and 
   \begin{align*}
        E(\widehat{w}(\hat{t}_{opt}),r) = \sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n \textcolor{red}{= r^2\Vert w_0\Vert^2 + o_{n,\mathbb P}(1)}.
    \end{align*}
\item if $r\in]\tilde{r}(\gamma_n), \sigma \sqrt{\pi/2}[$ then $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in 
 \begin{align*}
       & \hat{t}_{opt} := \frac{\log\left(\frac{r^2(\Vert w_0\Vert+\gamma_n)+\sigma^2\gamma_n - r\sqrt{2/\pi}\sigma (\Vert w_0\Vert +2\gamma_n)}{(c+\gamma_n)(\sigma^2 + r^2 - 2r\sqrt{2/\pi}\sigma)}\right)}{\log(1-\alpha \widehat{\sigma}^2)}>0~~\text{and}\\
        &E(\widehat{w}(\hat{t}_{opt}),r) = r^2\Vert w_0\Vert^2  \frac{(1-2/\pi)\sigma^2}{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}
    \end{align*}
\item if $r\geq  \sigma \sqrt{\pi/2}$, then $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in 
     \begin{align*}
        \hat{t}_{opt} := 0~~\text{and}~~
        E(\widehat{w}(\hat{t}_{opt}),r) = \Vert w_0\Vert_{\Sigma_x}^2\;.
    \end{align*}
\end{itemize}
\end{prop}

\begin{prop}
Assume that $\gamma_n<-\Vert w_0\Vert$, then for all $r\geq 0$, $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in 
     \begin{align*}
        \hat{t}_{opt} := 0~~\text{and}~~
        E(\widehat{w}(\hat{t}_{opt}),r) = \Vert w_0\Vert_{\Sigma_x}^2\;.
    \end{align*}
\end{prop}

Let us now study the optimality of this estimator.
\begin{prop}
We have the following results:
\begin{itemize}
\item If $\gamma_n\geq 0$, then for all $r\geq 0$, we have that 
$$E(\widehat{w}(\hat{t}_{opt}),r) = E^{*}_r\; , $$
\item If $\gamma_n\in[-\Vert w_0\Vert,0[$ and $r>\tilde{r}(\gamma_n)$ we have that 
$$E(\widehat{w}(\hat{t}_{opt}),r) = E^{*}_r\; , $$
\item If $\gamma_n< -\Vert w_0\Vert$ and $r\geq \sigma\sqrt{\pi/2}$ we have that  $$E(\widehat{w}(\hat{t}_{opt}),r) = E^{*}_r\; .$$
\end{itemize}
meaning that under these conditions the empirical estimator obtained using an early-stopping strategy on the test robust error is optimally robust.
\end{prop}
\begin{remark}
It is worth noting that
\begin{align*}
    \tilde{r}(\gamma_n)\xrightarrow[\gamma_n\xrightarrow{}_{-} 0]{} \sigma\sqrt{2/\pi}~~\text{and}~~\tilde{r}(\gamma_n)\xrightarrow[\gamma_n\xrightarrow{}_{+} -\Vert w_0\Vert]{} \sigma \sqrt{\pi/2}
\end{align*}
\end{remark}

We can also quantify in the left regimes, how far is the error of the empirical estimator using early-stopping from the optimally robust error $E^{*}_r$.  

\begin{prop}
If $\gamma_n\in[-\Vert w_0\Vert,0[$, then
     \begin{itemize}
        \item if $r\in[0,\sigma\sqrt{2/\pi}]$, then 
        \begin{align*}
            E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r &= \frac{\sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n}{r^2\Vert w_0\Vert^2} \\
            &\geq 1+(\pi/2 -1)\frac{\gamma_n^2}{\Vert w_0\Vert^2}
        \end{align*}
        \item if $r\in]\sigma\sqrt{2/\pi},\tilde{r}(\gamma_n)]$, then 
                \begin{align*}
                1 \leq E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r\leq  1+(\pi/2 -1)\frac{\gamma_n^2}{\Vert w_0\Vert^2}\textcolor{red}{=1+o_{n,\mathbb P}(1)}.
        \end{align*}
     where $$E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r = (\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}) \frac{ \sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n}{ r^2\Vert w_0\Vert^2 (1-2/\pi)\sigma^2}$$
    \end{itemize}


% \begin{itemize}
%     \item if $\sigma^2\geq 1/2$ then:
%     \begin{itemize}
%         \item if $r\in[0,\tilde{r}(\gamma_n)]$, then 
%         \begin{align*}
%             E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r = \frac{\sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n}{r^2\Vert w_0\Vert^2}\textcolor{red}{=1+o_{n,\mathbb P}(1)}. 
%         \end{align*}
%         \item if $r\in]\tilde{r}(\gamma_n),\sigma\sqrt{2/\pi}]$, then 
%             \begin{align*}
%         1 \leq E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r =\frac{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}{(1-2/\pi)\sigma^2} 
%         \end{align*}
%     \end{itemize}
%     \item if $\sigma^2<1/2$ then:
%      \begin{itemize}
%         \item if $r\in[0,\sigma\sqrt{2/\pi}]$, then 
%         \begin{align*}
%             E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r &= \frac{\sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n}{r^2\Vert w_0\Vert^2} \\
%             &\geq 1+(\pi/2 -1)\frac{\gamma_n^2}{\Vert w_0\Vert^2}
%         \end{align*}
%         \item if $r\in]\sigma\sqrt{2/\pi},\tilde{r}(\gamma_n)]$, then 
%                 \begin{align*}
%                 1 \leq E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r\leq  1+(\pi/2 -1)\frac{\gamma_n^2}{\Vert w_0\Vert^2}\textcolor{red}{=1+o_{n,\mathbb P}(1)}.
%         \end{align*}
%      where $$E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r = (\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}) \frac{ \sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n}{ r^2\Vert w_0\Vert^2 (1-2/\pi)\sigma^2}$$
%     \end{itemize}
% \end{itemize}
\end{prop}


We have also that:
\begin{prop}
If $\gamma_n < -\Vert w_0\Vert$, then
\begin{itemize}
    \item if $r\in[0,\sigma\sqrt{2/\pi}]$, then we have
    \begin{align*}
        E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r = \frac{\sigma^2}{r^2}\geq \pi/2
    \end{align*}
    \item if $r\in]\sigma\sqrt{2/\pi},\sigma\sqrt{\pi/2}[$, then 
        \begin{align*}
        1 \leq  E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r = \frac{\sigma^2}{r^2} 
        \frac{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}{(1-2/\pi)\sigma^2}\leq \frac{\pi}{2}
    \end{align*}
\end{itemize}
\end{prop}

In the next Proposition we quantify the optimality of the early-stopping estimator in probability.
\begin{prop}
Let $\delta>0$, then we obtain that
\begin{itemize}
    \item if $r \geq \sigma \sqrt{\pi/2}$, then for all $n\geq 1$, $\widehat{w}(\hat{t}_{opt})$ is optimally robust a.s. meaning that
    $$ E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r  = 1 ~~\text{a.s.}$$
   \item  if $ \sigma \sqrt{2/\pi} < r < \sigma \sqrt{\pi/2}$, then for $n\geq N_1(\delta,K,\sigma_\epsilon,\Vert w_0\Vert)$, we have that with probability $\geq 1-2\delta$
 
   \begin{align*}
        E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r \leq 1 + \sqrt{\frac{\pi-2}{2}}  \sqrt{\frac{\log(1/\delta)}{Kn}}\frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})}
   \end{align*}
%   \begin{itemize}
%       \item if $\sigma \sqrt{2/\pi} < r < \sigma \sqrt{2/\pi}+\epsilon$,
%       then with proba s.t. $\tilde{r}(\gamma_n)\leq \sigma \sqrt{2/\pi}+\epsilon$, $-\Vert w_0\Vert_2<\gamma_n<0$ and 
%   $$1+(\pi/2 -1)\frac{\gamma_n^2}{\Vert w_0\Vert^2}\leq E_1$$
%     \item (compute $\tilde{r}(\gamma_n)\leq \sigma \sqrt{2/\pi}+\epsilon$) then with proba  if $r>\sigma \sqrt{2/\pi}+\epsilon$, it is optimal.
%   \end{itemize}
    \item if $r \leq\sigma \sqrt{2/\pi} $, then for $n\geq N_2(\delta,K,\sigma_\epsilon,\Vert w_0\Vert)$  we have that with probability $\geq 1-2\delta$
   \begin{align*}
        E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r &\leq 1 +  \frac{2(\sqrt{2/\pi}\sigma-r)}{r\Vert w_0\Vert} \sqrt{\frac{\log(1/\delta)}{Kn}}\frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})}  \\ + &\left(\sqrt{\frac{\log(1/\delta)}{Kn}}\frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})}\right)^2 \frac{r^2+\sigma^2-2r\sqrt{2/\pi}\sigma}{r^2\Vert w_0\Vert^2} 
   \end{align*}
\end{itemize}
\end{prop}
\begin{proof}
Denotes $C(\delta,n,\sigma_\epsilon):=\sqrt{\frac{\log(1/\delta)}{Kn}}\frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})} $, then 
 $N_1(\delta,K,\sigma_\epsilon,\Vert w_0\Vert)$ has to be chosen as the smallest integer $n\geq 1$ such that $n\geq \log(1/\delta)\max(4,1/K)$, $C(\delta,n,\sigma_\epsilon)\leq \Vert w_0\Vert$ and such that $\frac{\sqrt{\Vert w_0\Vert^2 + 2\Vert w_0\Vert(\pi-2)(\Vert w_0\Vert -C(\delta,n,\sigma_\epsilon))C(\delta,n,\sigma_\epsilon)} - \Vert w_0\Vert}{2(\Vert w_0\Vert - C(\delta,n,\sigma_\epsilon))}\leq \frac{\pi-2}{2}$.
 In order to choose  $N_2(\delta,K,\sigma_\epsilon,\Vert w_0\Vert)$, we just require that $n\geq\log(1/\delta) \max(4,1/K)$ and $C(\delta,n,\sigma_\epsilon)\leq \Vert w_0\Vert$.
\end{proof}


\subsection{The case when $d>1$}
In this setting, a simple extension from the 1D case would be to consider $\Sigma_x=\sigma^2\text{Id}_d$ with $\sigma>0$. In that case, we recover the same results as the one obtained in the one dimensional case, meaning that the the early-stopping strategy is optimally robust in population. However in the general case, it may happens that $t\mapsto E_r(w(t),r)$ admits multiple local minima in the population regime, and therefore early-stopping would not be able to recover the global minimizer. In order to alleviate this issue, we propose to normalize the data using the covariance matrix. Assume for now that we are given the covariance matrix $\Sigma_x$ and let us denote $z:=\Sigma_x^{-1/2}x\sim\mathcal{N}(0,\text{Id})$, and $\widetilde{w}_0: = \Sigma_x^{1/2}w_0$, then observe that the model becomes $y=z^\top(\widetilde{w}_0)+\epsilon$. We will also denote in the following the normalized standard risk as
\begin{align*}
    E_{\text{norm}}(w):= \mathbb{E}[(z^\top w - y)^2]
\end{align*}
and $(w_{\text{norm}}(t))_{t\geq 0}$, the sequence produced by the GD scheme on $E_{\text{norm}}$. Let us also denote the adversarial risk on the normalized data as
\begin{align*}
    E_{\text{norm}}(w,r) = \mathbb{E}(\sup_{\Vert \delta\Vert \leq r}(w^\top (z+\delta) - \widetilde{w}_0^\top z)^2).
\end{align*}
First observe that the early stopping strategy on $(w_{\text{norm}}(t))_{t\geq 0}$ is optimally robust w.r.t to $E_{\text{norm}}(w,r)$, meaning that $E_{\text{norm}}(w_{\text{norm}}(t),r)$ admits at most one global minimizer and 
 $$\inf_{t\geq 0} E_{\text{norm}}(w_{\text{norm}}(t),r) = \inf_{w\in\mathbb{R}^d}  E_{\text{norm}}(w,r)\; .$$
Let us now study the robustness of such predictor on the adversarial risk of the true data. 
% Indeed let us first introduce the following result.
% \begin{lm}
% For all $w\in\mathbb{R}^d$, we have that
% \begin{align*}
%     E(w,r) =  E_{\text{norm},\Vert\cdot\Vert_{\Sigma_x}}(\Sigma_x^{1/2}w)
% \end{align*}
% In particular we have that
% \begin{align*}
%     E_r^{*}= \inf_{w\in\mathbb{R}^d}E_{\text{norm},\Vert\cdot\Vert_{\Sigma_x}}(w)
% \end{align*}
% \end{lm}
More precisely, we want to study the optimality of $(\Sigma_x^{-1/2}w_{\text{norm}}(t))_{t\geq 0}$ w.r.t $E(w,r)$. In fact we have the following proposition.
\begin{prop}
We have that
\begin{itemize}
    \item if $r\leq\frac{\sqrt{2/\pi}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert}$, then $t\mapsto  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)$ is a non-increasing function. In particular we have 
    \begin{align*}
        \inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r) = r^2\Vert w_0\Vert^2 ~~\text{and}~~t_{opt}=+\infty
    \end{align*}
     \item if $\frac{\sqrt{2/\pi}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert}\leq r\leq \frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert}$, then $t\mapsto  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)$ admits a unique minimizer. In particular we have 
    \begin{align*}
        \inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r) = \frac{r^2\Vert w_0\Vert^2  \Vert w_0\Vert_{\Sigma_x}^2(1-2/\pi)}{r^2\Vert w_0\Vert^2 +\Vert w_0\Vert_{\Sigma_x}^2 - 2r\sqrt{2/\pi}\Vert w_0\Vert\Vert w_0\Vert_{\Sigma_x}}
    \end{align*}
    and
        \begin{align*}
        t_{\text{opt}}= \frac{\log\left(\frac{r\Vert w_0\Vert(r\Vert w_0\Vert -\sqrt{2/\pi} \Vert w_0\Vert_{\Sigma_x})}{\Vert w_0\Vert_{\Sigma_x}^2 + r^2\Vert w_0\Vert^2 -2r\sqrt{2/\pi}\Vert w_0\Vert \Vert w_0\Vert_{\Sigma_x}}\right)}{\log(1-\alpha)}
    \end{align*}
     \item if $r\geq \frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert}$, then $t\mapsto  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)$ is a non-decreasing function. In particular we have 
    \begin{align*}
        \inf_{t\geq 0} E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r) = \Vert w_0\Vert^2_{\Sigma_x} ~~\text{and}~~t_{opt}=0
    \end{align*}
\end{itemize}
\end{prop}
In the following proposition we study the optimality of our proposed procedure.
\begin{prop}
We have that for all $r\geq 0$, 
\begin{align*}
    E_r^{*} \leq \inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r) \leq E_{r\sqrt{\Vert \Sigma_x\Vert_{\text{op}}\Vert \Sigma_x^{-1}\Vert_{\text{op}}}}^{*}
\end{align*}
In particular we obtain that
\begin{itemize}
    \item if $r\leq\frac{\sqrt{2/\pi}\Vert w_0\Vert}{\Vert w_0\Vert_{\Sigma_x^{-1}}}$, then we have that
    \begin{align*}
          E_r^{*} = \inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)
    \end{align*}
   
   \item if $\frac{\sqrt{2/\pi}\Vert w_0\Vert}{\Vert w_0\Vert_{\Sigma_x^{-1}}} \leq r\leq  \frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x^2}}{\Vert w_0\Vert_{\Sigma_x}}$, then we have that
       \begin{align*}
      1 \leq \frac{\inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)}{E_r^{*}}\leq \Vert \Sigma_x\Vert_{\text{op}}\Vert \Sigma_x^{-1}\Vert_{\text{op}}
    \end{align*}
   
    % \item if  $\frac{\sqrt{2/\pi}\Vert w_0\Vert}{\Vert w_0\Vert_{\Sigma_x^{-1}}}<r<\frac{\sqrt{2/\pi}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert_{\Sigma_x}}$, then we have that
    % \begin{align*}
    %     1 \leq \frac{\inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)}{E_r^{*}} \leq \Vert \Sigma_x\Vert_{\text{op}}\Vert \Sigma_x^{-1}\Vert_{\text{op}}
    % \end{align*}
    
    % \item if $ \frac{\sqrt{2/\pi}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert_{\Sigma_x}} \leq r \leq  \frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert_{\Sigma_x}}$, then we obtain that
    
    % \item  if $\frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert_{\Sigma_x}} \leq r < \frac{\sqrt{2/\pi}\Vert w_0\Vert_{\Sigma_x^2}}{\Vert w_0\Vert_{\Sigma_x}}$, then we obtain that
    
    
    \item if $r\geq \frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x^2}}{\Vert w_0\Vert_{\Sigma_x}}$, then we have that
       \begin{align*}
          E_r^{*} = \inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)
    \end{align*}
\end{itemize}
\end{prop}
\begin{proof}
Observe that for all $w\in\mathbb{R}^d$, we have that
\begin{align*}
    E_{\text{norm}}(w,r) &= \Vert \Sigma_x^{-1/2}w - w_0\Vert_{\Sigma_x}^2 + r^2\Vert \Sigma_x^{-1/2}w\Vert_{\Sigma_x}^2 \\
    &+2r\sqrt{2/\pi} \Vert \Sigma_x^{-1/2}w - w_0\Vert_{\Sigma_x}\Vert \Sigma_x^{-1/2}w\Vert_{\Sigma_x}
\end{align*}
and recall that we have $$\sqrt{\lambda_{\text{min}}}\Vert w\Vert \leq \Vert w \Vert_{\Sigma_x}\leq \sqrt{\lambda_{\text{max}}}\Vert w\Vert $$
where we have denoted $\lambda_{\text{min}}:=1/\Vert \Sigma_x^{-1}\Vert_{\text{op}}$ and $\lambda_{\text{max}}:=\Vert \Sigma_x\Vert_{\text{op}}$.
Therefore we obtain that for all $w\in\mathbb{R}^d$
\begin{align*}
 E(\Sigma_x^{-1/2}w,\sqrt{\lambda_{\text{min}}}r)  \leq  E_{\text{norm}}(w,r)\leq E(\Sigma_x^{-1/2}w,\sqrt{\lambda_{\text{max}}}r).
\end{align*}
In addition recall that for all $r'\geq 0$ we have 
\begin{align*}
    \inf_{w\in\mathbb{R}^d}E_{\text{norm}}(w,r') = \inf_{t\geq 0}E_{\text{norm}}(w_{\text{norm}}(t),r') 
\end{align*}
from which follows that
\begin{align*}
 E_r^{*}\leq \inf_{t\geq 0}E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r) &\leq \inf_{t\geq 0}E_{\text{norm}}(w_{\text{norm}}(t),r/\sqrt{\lambda_{\text{min}}}) \\
 &\leq  \inf_{w\in\mathbb{R}^d}E_{\text{norm}}(w,r/\sqrt{\lambda_{\text{min}}})\\
 &\leq E_{\sqrt{\lambda_{\text{max}}/\lambda_{\text{min}}}r}^*
\end{align*}
% Then we have that
% \begin{align*}
%   \frac{\inf_{w\in\mathbb{R}^d}E_{\text{norm}}(w,r)}{\max(1,\Vert \Sigma_x\Vert_{\text{op}})}  \leq E_r^{*}:=\inf_{w\in\mathbb{R}^d}E(w,r)\leq \frac{\inf_{w\in\mathbb{R}^d}E_{\text{norm}}(w,r)}{\min(1,1/\Vert \Sigma_x^{-1}\Vert_{\text{op}})}
% \end{align*}
% Therefore we obtain that
% \begin{align*}
%     \inf_{t\geq 0}E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)&\leq \frac{\inf_{t\geq 0}E_{\text{norm}}(w_{\text{norm}}(t),r)}{\min(1,1/\Vert \Sigma_x^{-1}\Vert_{\text{op}})}\\
%     &\leq \frac{\inf_{w\in\mathbb{R}^d}E_{\text{norm}}(w,r)}{\min(1,1/\Vert \Sigma_x^{-1}\Vert_{\text{op}})}\\
%     &\leq  \frac{\max(1,\Vert \Sigma_x\Vert_{\text{op}})}{\min(1,1/\Vert \Sigma_x^{-1}\Vert_{\text{op}})} E_r^{*}
% \end{align*}
\end{proof}
The above Proposition shows that for all $r\geq 0$, there exists $r'$ such that
\begin{align*}
     \sqrt{\frac{\lambda_{\text{min}}}{\lambda_{\text{max}}}} r\leq r'\leq r~~~\text{and}~~\inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r') = E_r^{*}
\end{align*}
Therefore the early-stopping strategy with normalized data is able to recover exactly the optimally robust predictor which requires to solve the above equation. In order to alleviate this issue, we propose instead a simple predictor where we choose the radius of the attack on the normalized data to be exactly the same as the one on the true data, meaning that we consider here $r'=r$. By doing so, that we show that early-stopping is both optimally robust  with respect to $\ell_2$ attacks on the normalized data (i.e.  $E_{\text{norm}}$) uniformly on $r$ and almost optimally robust on $\ell_2$ attacks on the unormalized data (i.e. $E$) uniformly on $r$ as soon as the problem is well conditioned. 


In order to obtain an estimator of such predictors we simply propose to use an empirical estimator of the covariance matrix using half of the dataset $\widehat{\Sigma}_x:= \frac{2}{n}\sum_{i=1}^{\lfloor n/2 \rfloor} x_ix_i^T$. Then, we can perform a GD descent scheme with an early stopping strategy on the left points, namely $(\widehat{\Sigma}_x^{-1/2} x_i,y_i)_{i=1}^{\lceil n/2 \rceil}$, and show that this strategy is with high probability almost optimally robust. 



\section{Robustness via shrinkage to zero}
\mytodo{Link the ideas presented hereunder to the so-called "Stein shrinkage" \url{http://proceedings.mlr.press/v32/muandet14.pdf}}

In the particular case where $M=I_d$, we obtain that $A_M=\Sigma_x^{-1/2}$ and we can write the updates of GD scheme as follows:
\begin{align*}
    w^{I_d}(t):= (1 - (1 - \alpha)^t)\Sigma^{1/2}w_0\; .
\end{align*}
This scheme corresponds to apply a GD scheme on the normalized data, i.e. on the following objective 
\begin{align*}
    E_{I_d}(w)=\mathbb{E}_{(x,y)\sim P_{xy}}(w^T(\Sigma_x^{-1/2} x)-y)^2\; .
\end{align*}
Therefore by considering the following path $(A_{I_d} w^{I_d}(t))_{t\geq 0}$, the proposed GD scheme is drawing all the predictors on the chord $[0,w_0] := \{\beta w_0 \mid \beta \in [0, 1]\}$ that joins $w_0$ to the origin. In the following, we focus on the robustness of such predictors.

\subsection{Optimizing over a chord}
We set $c_0:=\sqrt{2/\pi}$. Consider the problem of minimizing the robust risk $w \mapsto E^{\Vert\cdot\Vert }(w,r)$ over $[0,w_0]$. Now, for any $\beta \in [0, 1]$, one has
\begin{align*}
E^{\Vert\cdot\Vert}(\beta w_0,r) &= (1-\beta)^2\|w_0\|_{\Sigma_x}^2  + \beta^2r^2\|w_0\|_\star^2 \\
&+ 2c_0\beta(1-\beta)r\|w_0\|_{\Sigma_x}\|w_0\|_\star \\
&= a\beta^2 - 2b\beta + c,
\end{align*}
a quadratic polynomial in $\alpha$ with coefficients $a=a(w_0,r) := \|w_0\|_{\Sigma_x}^2 + r^2\|w_0\|_\star^2 - 2c_0r\|w_0\|_{\Sigma_x}\|w_0\|_\star$, $b=b(w_0,r) := \|w_0\|_{\Sigma_x}^2-c_0r\|w_0\|_{\Sigma_x}\|w_0\|_\star$, and $c=c(w_0,r) = \|w_0\|_{\Sigma_x}^2$. On the other hand, it is clear that the leading coefficient $a(w_0,r)$ is itself a quadratic in $r$ with discriminant $\|w_0\|_\Sigma^2\|w_0\|_\star^2(c_0^2-1)$ which is strictly negative because $c_0^2 = 2/\pi < 1$. Thus, $\beta \mapsto E^{\Vert\cdot\Vert}(\beta w_0, r)$ is a convex one-dimensional quadratic function. Therefore a simple early-stopping strategy is able to capture its minimum. 


Let us now focus on the robustness of such the minimizer of this specific path. First, we observe that this function is minimized at $\beta_{opt}(w_0,r)$ the unique point of $[0,1]$ which is closest to the real number $\widetilde\beta_{opt}(w_0,r) \in \mathbb R$ defined by
\begin{align*}
\widetilde\beta_{opt}(w_0,r) := \frac{\|w_0\|_{\Sigma_x}^2-c_0r\|w_0\|_{\Sigma_x}\|w_0\|_\star}{\|w_0\|_{\Sigma_x}^2 + r^2\|w_0\|_\star^2 - 2c_0r\|w_0\|_{\Sigma_x}\|w_0\|_\star}.
\end{align*}

% \begin{restatable}{lm}{}
% For any fixed $z \in \mathbb R^d$, it holds that
% \begin{eqnarray}
% \lim_{r \to 0^+}\widetilde\alpha_{opt}(z,r) = 1,\,\lim_{r \to \infty}\widetilde\alpha_{opt}(z,r) = 0.
% \end{eqnarray}
% Moreover, if $\|\cdot\|_\star = \|\cdot\|_\Sigma$ (i.e if the attacker's norm is $\|\cdot\|_{\Sigma{-1}}$), then
% \begin{eqnarray}
% \widetilde\alpha_{opt}(z,r) = (1-c_0 r) / (1+r^2-2c_0r).
% \end{eqnarray}
% \end{restatable}

% \begin{restatable}{rmk}{}
% In isotropic case, we know from Prop \ref{prop:normalized} that the minimizer of the normalized energy $w \mapsto E(w,r)$ is $w_{opt}(r) = (1+\lambda_{opt}(r))^{-1} w_0$,
% where $\lambda_{opt}(r)$ is given in \eqref{eq:lambdaopt}. This is consistent with the above lemma as one easily verifies that for $c_0 < r < 1/c_0$, 
% $$
% (1+\lambda_{opt}(r))^{-1} = ((r^2+1-2c_0 r)/(1-c_0r))^{-1} = (1-c_0r)/(1+r^2-2c_0 r) = \alpha_{opt}(r).
% $$
% \end{restatable}

Now, define $r_0(w_0)$, $r_1(w_0)$, and $r_2(w_0)$ by 
\begin{align*}
r_0(w_0)&:=\frac{\|w_0\|_{\Sigma_x}}{\|w_0\|_\star},\, r_1(w_0):=c_0r_0(w_0),\,\\
r_2(w_0)&:= \frac{1}{c_0^2} r_1(w_0) = \frac{1}{c_0}r_0(w_0).
\end{align*}
We will denote them respectively $r_0$, $r_1$ and $r_2$ in the following for simplicity. In the case where the attacker's norm is the $\ell_\infty$-norm so that its dual $\|\cdot\|_\star$ is the $\ell_1$-norm, $r_0$ (in fact, $1/r_0(w_0)$) can be thought of as the sparsity level of $w_0$.
A simple computation reveals that
\begin{eqnarray}
\beta_{opt}(z,r)% \min(\max(\widetilde\alpha_{opt}(z,r),0), 1)
= \begin{cases}
1, &\mbox{ if }0 \le r < r_1,\\
\widetilde\beta_{opt}(w_0,r),&\mbox{ if }r_1\le r \le r_2,\\
0,&\mbox{ if } r > r_2.
\end{cases}
\end{eqnarray}
Finally, note that
\begin{eqnarray*}
E(\beta_{opt}(z,r)z,r) = \begin{cases}
r^2\Vert w_0\Vert_{*}^2, &\mbox{ if }0 \le r < r_1,\\
\dfrac{(1-c_0^2)\|w_0\|_{\Sigma_x}^2}{h(r_0/r)},&\mbox{ if }r_1 \le r \le r_2,\\
\|w_0\|_{\Sigma_x}^2,&\mbox{ if } r > r_2.
\end{cases}
\end{eqnarray*}
where the function $h:\mathbb R \to \mathbb R$ is defined by
\begin{eqnarray}
h(t) := t^2+1-2c_0 t.
\end{eqnarray}
% FWIW, note that
% $(t-1)^2 \le h(t) \le t^2 + 1$ for any $t \in \mathbb R$.

% Putting things together, we obtain the following result.
% \begin{restatable}{prop}{}
% For any nonzero $z \in \mathbb R^d$, the minimum of $w \mapsto E(w,r)$ over the chord $[0,z]$ is attained at the point $\alpha_{opt}(z,r) z$. That is,
% \begin{eqnarray}
% \inf_{w \in [0,z]}E(w, r) = E(\alpha_{opt}(z,r)z,r)
% = \begin{cases}
% E(z,r),&\mbox{ if }0 \le r < r_1(z),\\
% \dfrac{r^2(1-c_0^2)\|z\|_\Sigma^2\|z\|_\star^2}{a(z,r)},&\mbox{ if }r_1(z) \le r \le r_2(z),\\
% E(0,r) = \|w_0\|_\Sigma^2,&\mbox{ if }r > r_2(z).
% \end{cases}
% \end{eqnarray}
% \label{prop:alpha}
% \end{restatable}

The following Proposition quantifies the improvement of the robust error of our proposed predictor compared to the generative model.
\begin{prop}
 For any nonzero model $w_0 \in \mathbb R^d$, it holds that
\begin{itemize}
\item[(A)] If $0 \le r \le r_1(w_0)$, then $E^{\Vert\cdot\Vert}(\beta_{opt}(w_0,r),r) = E^{\Vert\cdot\Vert }(w_0,r)$.
\item[(B)] If $r_1(w_0) \le r \le r_2(w_0)$, then
$\dfrac{E^{\Vert\cdot\Vert}(\beta_{opt}(w,r),r)}{E^{\Vert\cdot\Vert}(w_0,r)} = \dfrac{1-c_0^2}{h(r/r_0(w))} \le 1$.
\item[(C)] If $r \ge r_2(w)$, then $\dfrac{E^{\Vert\cdot\Vert}(\beta_{opt}(w,r),r)}{E^{\Vert\cdot\Vert}(w,r)} =  \dfrac{\|w_0\|_\Sigma^2}{r^2\Vert w_0\Vert_{*}^2} \le 1$.
\end{itemize}
\end{prop}




\subsection{A note on the euclidean case}
In the case of euclidean attacks, we can obtain finer results. 
\begin{restatable}{rmk}{}
Define $R_1 = R_1(w_0) := c_0\|w_0\|_2/\|w_0\|_{\Sigma^{-1}}$ and $R_1 = R_2(w_0):=(1/c_0)\|w_0\|_{\Sigma^2}/\|w_0\|_{\Sigma}$. 
It was shown in Proposition 1 of \url{https://arxiv.org/pdf/2012.10278.pdf} that 
\begin{itemize}
    \item If $ 0 \le r \le R_1$, then $E_{opt}(r) = E(w_0,r) = r^2\|w_0\|_2^2$.
    \item If $r \ge R_2$, then
    $E_{opt}(r) = E(0,r) = \|w_0\|_\Sigma^2$.
\end{itemize}
\label{rmk:extremes}
\end{restatable}
Little was said for $r \in [R_1,R_2]$; the analysis in that interval is untractable, except in the special case where the covariance matrix is the identity matrix. We will remedy the situation by settling for near-optimal solutions: that is points whose robust risk $E(w,r)$ is within a multiplicative factor the global minimum $E_{opt}(r)$. 

The following lemma will be useful in the special case of euclidean attacks.
\begin{restatable}{lm}{}
In the case of euclidean attacks, it holds that
$r_1 \ge R_1$ and $R_2 \ge r_2$.
\end{restatable}
\begin{proof}
Indeed,  we have
\begin{align}
r_1 &\ge R_1 \text{ iff } \|w_0\|_{\Sigma^{-1}}\|w_0\|_{\Sigma} \ge \|w_0\|_2^2 = \langle w_0, w_0\rangle,\\
R_2 &\ge r_2 \text{ iff }\|w_0\|_{\Sigma^2}\|w_0\|_2 \ge \|w_0\|_\Sigma^2 \text{ iff }\|\Sigma w_0\|_2 \|w_0\|_2 \ge \langle \Sigma w_0,w_0\rangle.
\end{align}
Thanks to Cauchy-Schwarz inequality, and the fact that the $\ell_2$-norm is self-dual while $\|\cdot\|_{\Sigma}$ and $\|\cdot\|_{\Sigma^{-1}}$ are duals of one another, the rightmost side (and therefore the leftmost side too) of the each of the above equivalencies is satisfied.
\end{proof}
In particularly, if $\Sigma = \sigma^2 I_d$ (or more generally, if $w_0$ is an eigenvector of $\Sigma$), then $r_1 = R_1$ and $r_2 = R_2$.

\subsection{Main results}
Let $\lambda_{min}$ (resp. $\lambda_{max}$) be the smallest (resp. largest) value of the ratio $r_0(w) := \|w\|_\Sigma/\|w\|_\star$ over non-zero vectors $w \in \mathbb R^d$. That is,
\begin{eqnarray}
\lambda_{max} := \sup_{w \in \mathbb R^d,\,w \ne 0}r_0(w)^2,\, \lambda_{min} := \inf_{w \in \mathbb R^d,\,w \ne 0}r_0(w)^2.
\end{eqnarray}
Also, let $\kappa(\Sigma)=\kappa^{\|\cdot\|}(\Sigma)$ be the \emph{condition number} of $\Sigma$ w.r.t the norm $\|\cdot\|$, i.e
\begin{eqnarray}
\kappa(\Sigma) := \lambda_{max}/\lambda_{min},\,\kappa^0(\Sigma):=\lambda_{max}/r_0(w_0)^2,\,\kappa^1(\Sigma) := r_0(w_0)^2/\lambda_{min}.
\end{eqnarray}
In the particular case of euclidean attacks, $\lambda_{max}$ (resp. $\lambda_{min}$) corresponds to the largest (resp. smallest) eigenvalue of $\Sigma$. In this case $\kappa(\Sigma)$ is the usual condition number of $\Sigma$.
In any case, it always holds that $\kappa(\Sigma) \ge \max(\kappa^0(\Sigma),\kappa^1(\Sigma))$ and $\min(\kappa^0(\Sigma),\kappa^1(\Sigma)) \ge 1$ with $\kappa(\Sigma) = 1$ iff the attacker's norm $\|\cdot\|$ is proportional to $\|\cdot\|_{\Sigma^{-1}}$. For example, this is the case when $\Sigma = \sigma^2 I_d$ and the attacker's norm is euclidean.
On the other hand, note that $\kappa(\Sigma)$ can be arbitrarily large. For example, if $\Sigma=I_d$ and the attacker's norm $\|\cdot\|$ is the $\ell_\infty$-norm, then it is easy to see that $\kappa(\Sigma) = d$.

The following lemma will be useful.
\begin{restatable}{lm}{}
Define $\gamma_r(w_0) := \inf_{w \in \mathbb R^d}\|w-w_0\|_\Sigma + r\|w\|_\star$. Then,
\begin{align}
     \gamma_r(w_0) &\ge \min(1,r/\sqrt \lambda_{max})\|w_0\|_\Sigma,\\
     \gamma_r(w_0) &\ge \min(\sqrt \lambda_{min},r)\|w_0\|_\star.
\end{align}
\label{lm:densesparse}
\end{restatable}
\begin{proof}
Let $w \in \mathbb R^d$.
Indeed, by definition of $\lambda_{max}$, it holds that $\|w\|_\star \ge \|w\|_\Sigma/\sqrt\lambda_{max}$, and so one may write $$
\|w-w_0\|_\Sigma + r\|w\|_\star \ge \|w-w_0\|_\Sigma + (r/\sqrt\lambda_{max})\|w\|_\Sigma \ge \min(1,r/\sqrt\lambda_{max})\|w_0\|_\Sigma,
$$
which proves the first lower-bound.
Similarly, by definition of $\lambda_{min}$, it holds that $\|w-w_0\|_\Sigma \ge \sqrt\lambda_{min}\|w-w_0\|_\star$, and so
$$
\|w-w_0\|_\Sigma + r\|w\|_\star \ge \sqrt\lambda_{min}\|w-w_0\|_\star + r\|w\|_\star \ge \min(\sqrt\lambda_{min},r)\|w_0\|_\star,
$$
which proves the second lower-bound.
\end{proof}

We are now ready to state the main result of this section wherein we show that optimizing on the chord $[0,w_0]$ gives a point which is optimal up to within a multiplicative factor of $1.747\kappa(\Sigma)$. Viz,
\begin{restatable}{thm}{}
We have the following:
\begin{itemize}
\item[(A)] In the case of an attack of magnitude $r$ w.r.t to an arbitrary norm $\|\cdot\|$, for  $r_1 \le r \le r_2$, it holds that
\begin{eqnarray}
\dfrac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)}
% \le \dfrac{2(1-c_0^2)}{1+c_0}\frac{\lambda_{min} \land r^2}{h(r_0/r)}\kappa(\Sigma)
\le \dfrac{2}{(1+c_0)c_0^2}\kappa^0(\Sigma) \approx 1.747\kappa^0(\Sigma).
\end{eqnarray}
\item[(B)] In the case of euclidean attacks, if $0 \le r \le R_1$ or $r \ge R_2$, then it holds that $E(\alpha_{opt}(w_0,r),r) = E_{opt}(r)$. In addition, if $R_1 < r <R_2 $, then $\dfrac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} \leq\kappa^1(\Sigma)$.
\end{itemize}
\end{restatable}
\mytodo{Extend part (B) to general non-euclidean norm attacks.}\\
\begin{proof}
We first prove part A of the result. One computes
\begin{eqnarray}
\begin{split}
\frac{2}{1+c_0} \cdot E_{opt}(r) &\ge \left(\inf_{w \in \mathbb R^d} \|w-w_0\|_\Sigma + r\|w\|_\star\right)^2\\
% &\ge \left(\inf_{w \in \mathbb R^d}\sqrt{\lambda_{min}}\|w-w_0\|_\star + r\|w\|_\star\right)^2\\
&\ge (\lambda_{min} \land r^2)\|w_0\|_\star^2 \lor (1 \land r^2/\lambda_{max})\|w_0\|_\Sigma^2,
\end{split}
\label{eq:toto}
\end{eqnarray}
where the first step is thanks to Lemma \ref{lm:burger} below and the second step is thanks to Lemma \ref{lm:densesparse}.
On the other hand, for $r_1 \le r \le r_2$, we deduce from Proposition \ref{prop:alpha} that
\begin{eqnarray}
\begin{split}
E(\alpha_{opt}(w_0,r),r) &= \frac{(1-c_0^2)\|w_0\|_\Sigma^2}{h(r_0/r)}
% &\le \frac{(1-c_0^2)\|w_0\|_\Sigma^2}{h(r_0/r_2)}
\le \frac{1-c_0^2}{h(r_0/r)}\lambda_{max}\|w_0\|_\star^2 \le \lambda_{max}\|w_0\|_\star^2,
\end{split}
\label{eq:tata}
\end{eqnarray}
where we have used the fact that $h(t) := t^2+1-2tc_0 \ge h(c_0) = 1-c_0^2$ for all $t \in \mathbb R$. On the same interval, \eqref{eq:toto} further gives
\begin{eqnarray}
\begin{split}
\frac{2E_{opt}(r)}{(1+c_0)\|w_0\|_\star^2} &\ge \lambda_{min} \land r^2 \ge \lambda_{min} \land r_1^2 \ge  \lambda_{min} \land c_0^2\lambda_{min}=c_0^2\lambda_{min},\\
\frac{2E_{opt}(r)}{(1+c_0)\|w_0\|_\Sigma^2} &\ge 1 \land r^2/\lambda_{max} \ge 1\land r_1^2/\lambda_{max} \ge  1 \land c_0^2 r_0^2/\lambda_{max} =\frac{c_0^2r_0^2}{\lambda_{max}} = \frac{c_0^2}{\kappa^0(\Sigma)},
\end{split}
\end{eqnarray}
and we deduce that
\begin{eqnarray}
\begin{split}
E_{opt}(r) &\ge \frac{(1+c_0)}{2}(\lambda_{min} \land r^2)\|w_0\|_\star^2 \ge \dfrac{(1+c_0)c_0^2}{2}\lambda_{min}\|w_0\|_\star^2,\\
E_{opt}(r) &\ge \frac{(1+c_0)}{2}(1 \land r^2/\lambda_{max})\|w_0\|_\Sigma^2 \ge \dfrac{(1+c_0)c_0^2}{2}\kappa^0(\Sigma)\|w_0\|_\Sigma^2.
\end{split}
\label{eq:titi}
\end{eqnarray}
Putting \eqref{eq:tata} and \eqref{eq:titi} together gives
\begin{eqnarray*}
\begin{split}
1 \le \frac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} &\le \frac{2}{(1+c_0)c_0^2}\frac{(1-c_0^2)}{h(r_0/r)}\kappa^0(\Sigma) = \frac{2}{(1+c_0)c_0^2}\frac{1-c_0^2}{h(r_0/r)}\kappa^0(\Sigma)\\
&\le \frac{2}{(1+c_0)c_0^2}\kappa^0(\Sigma),
%1 \le \frac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} &\le \frac{2}{(1+c_0)c_0^2}\frac{(1-c_0^2)}{h(r_0/r)}\frac{\lambda_{max}}{\lambda_{min}} = \frac{2}{(1+c_0)c_0^2}\frac{1-c_0^2}{h(r_0/r)}\kappa(\Sigma)\\
%&\le \frac{2}{(1+c_0)c_0^2}\kappa(\Sigma),
\end{split}
\end{eqnarray*}
as desired.

We now prove part B. If $r \le R_1$ or $r \ge R_2$, part B follows directly from Proposition \ref{prop:alpha} and Remark \ref{rmk:extremes}, since $R_1 \ge r_1$ and $R_2 \le r_2$ as already mentioned above.

If $R_1 \le r \le r_1$ (resp. $r_2 \le r \le R_2$), then thanks to Proposition \ref{prop:alpha} we have $E_{opt}(r) \ge E_{opt}(R_1) = R_1^2\|w_0\|_2^2$ and $E(\alpha_{opt}(w_0,r),r)\leq r_1^2\|w_0\|_2^2$ which gives that
\begin{align*}
    E(\alpha_{opt}(w_0,r),r)/E_{opt}(r)\leq r_1^2/R_1^2\leq \kappa^1(\Sigma).
\end{align*}
In addition if $r_2 \le r \le R_2$, we have that $E(\alpha_{opt}(w_0,r),r)=\|w_0\|_{\Sigma}^2$ and $E_{opt}(r) \ge E_{opt}(R_1) = R_1^2\|w_0\|_2^2$, which gives that
\begin{align*}
    E(\alpha_{opt}(w_0,r),r) / E_{opt}(r)\leq
    \frac{1}{c_0^2}\frac{\|w_0\|_{\Sigma^{-1}}^2\|w_0\|_{\Sigma}^2}{\|w_0\|_2^2 \|w_0\|_2^2}\leq \frac{ \kappa^1(\Sigma)}{c_0^2}
\end{align*}
\end{proof}

\begin{restatable}{lm}{}
\label{lm:burger}
If $u,v,\beta \ge 0$ with $\beta \le 1$, then
\begin{eqnarray}
\frac{(1+\beta)}{2}(u+v)^2 \le u^2 + v^2 + 2\beta u v \le (u+v)^2.
\end{eqnarray}
\end{restatable}
\begin{proof}
The second inequality follows directly from the fact that $0 \le \beta \le 1$. For the first inequality, simply observe that
$$
2(u^2 + v^2 + 2\beta u v)  - (1+\beta)(u+v)^2 = (1-\beta)(u-v)^2 \ge 0.
$$
\end{proof}


\subsection{Exact Optimality for Euclidean Attacks}
There is a setting however where we can guarantee that early-stopping captures the infimum. Indeed let us consider the case where  $\Sigma=\sigma^2 I_d$ and $\Vert\cdot\Vert=\Vert\cdot\Vert_2$, then we obtain the following sharper result.
\begin{prop}
For all $r\geq 0$, we have 
\begin{align*}
    \inf_{t\geq 0} E^{\Vert\cdot\Vert_2}(w(t),r) =  E^{\Vert\cdot\Vert_2}_{opt}(r).
\end{align*}
In addition, if $r\leq \sqrt{2/\pi}\frac{\Vert w_0\Vert_2}{\Vert w_0\Vert_{\Sigma_x^{-1}}}$ or 
$r\geq \sqrt{\pi/2}\frac{\Vert w_0\Vert_{\Sigma_x^2}}{\Vert w_0\Vert_{\Sigma_x}}$, then $t\mapsto  E^{\Vert\cdot\Vert_2}(w(t),r) $ is monotone and if $\sqrt{2/\pi}\frac{\Vert w_0\Vert_2}{\Vert w_0\Vert_{\Sigma_x^-1}}<r<\sqrt{\pi/2}\frac{\Vert w_0\Vert_{\Sigma_x^2}}{\Vert w_0\Vert_{\Sigma_x}}$, then $t\mapsto  E^{\Vert\cdot\Vert_2}(w(t),r) $ admits exactly one local minimum which is global.
\end{prop}
Therefore in the isotropic case we obtain exact optimal robustness and we show that early-stopping on the GD scheme is able to capture it. In order to generalize the above idea in the general setting we will focus in the following on the robustness of the GD descent on normalized data.


\section{Some cleanup and refinements}
\textcolor{red}{The objective is to refine / clarify some of the ideas developed in the previous section. Most importantly, we try to see how far we can go without ever uttering the work "gradient descent".}
\subsection{Redefining spectral quantities}
Define scalars $\lambda_{max}$, $\lambda_{\min}$, and $\kappa(\Sigma)$, by
\begin{align}
\lambda_{max} &:= \|\Sigma^{1/2}\|_\star^2 = \sup_{w \ne 0}\frac{\|\Sigma^{1/2} w\|_\star^2}{\|w\|_\star^2},\\
\lambda_{\min} &:= \|\Sigma^{-1/2}\|_\star^{-2} = \inf_{w \ne 0}\frac{\|\Sigma^{1/2} w\|_\star^2}{\|w\|_\star^2},\\
\kappa(\Sigma) &:= \lambda_{max}/\lambda_{min}.
\end{align}
In the particular case where the attacker's norm is euclidean, we have $\lambda_{max} = \|\Sigma\|_{op}$, $\lambda_{\min} = 1/\|\Sigma^{-1}\|_{op}$, and $\kappa(\Sigma) = \|\Sigma\|_{op} \|\Sigma^{-1}\|_{op}$ is the usual condition number of $\Sigma$. Of course, these perfectly match the considerations of the previous subsection. In the case of $\ell_\infty$-norm attacks, it might be handy to note that for any matrix $A=(a_{ij})_{i,j} \in \mathbb R^{m \times d}$, one has
\begin{eqnarray}
\|A\|_1 = \max_{1 \le j \le d} \sum_{i=1}^m|a_{ij}| = \text{ max }\ell_1\text{ norm of a column of }A.
\end{eqnarray}

\begin{restatable}{lm}{}
For any $w \in \mathbb R^d$ and $r \ge 0$, we have
\begin{align}
 E(\Sigma^{-1/2}w,r\sqrt{\lambda_{min}})  \leq  E_{norm}(w,r)\leq E(\Sigma^{-1/2}w,r\sqrt{\lambda_{max}}).
\end{align}
\end{restatable}
\begin{proof}
Indeed, by definition of $E_{norm}$, $\tilde w_0$, $\lambda_{max}$, and $\lambda_{min}$, one computes
\begin{eqnarray*}
\begin{split}
E_{norm}(w,r) &= \|w-\tilde w_0\|_2^2 + r^2\|w\|_\star^2 + 2c_0\|w-\tilde w_0\|_\star\|w\|_\star\\
&= \|\Sigma^{-1/2}w-w_0\|_{\Sigma}^2 + r^2\|w\|_\star^2 + 2c_0\|\Sigma^{-1/2}w-w_0\|_\Sigma \|w\|_\star\\
&= \|\Sigma^{-1/2}w-w_0\|_{\Sigma}^2 + r^2\|\Sigma^{1/2}\Sigma^{-1/2}w\|_\star^2\\
&\quad\quad\quad + 2c_0\|\Sigma^{-1/2}w-w_0\|_\Sigma \|\Sigma^{1/2}\Sigma^{-1/2}w\|_\star\\
&\le \|\Sigma^{-1/2}w-w_0\|_{\Sigma}^2 + r^2\lambda_{max}\|\Sigma^{-1/2}w\|_\star^2\\
&\quad\quad\quad + 2c_0r\sqrt\lambda_{max}\|\Sigma^{-1/2}w-w_0\|_\Sigma \|\Sigma^{-1/2} w\|_\star\\
&= E(\Sigma^{-1/2} w,r\sqrt\lambda_{max}).
\end{split}
\end{eqnarray*}
Analogously, one shows that $E_{\mathrm{norm}}(w,r) \ge E(\Sigma^{-1/2}w,r\sqrt\lambda_{min})$.
\end{proof}

\subsection{Reduction to "one-dimensional" case: normalization}
The following is a refinement of the first statement of Prop 4.11. The aim is to make it clear that the aforementioned proposition has nothing to do with gradient-descent, etc.
\begin{restatable}{thm}{}
For any $r \ge 0$, let $w_{norm}(r)$ be a minimizer of $E_{norm}(w,r)$ over $w \in \mathbb R^d$. Then, it holds that
\begin{align}
E(w_{norm}(r),r) &\le E_{opt}(r\sqrt{\kappa(\Sigma)})\\
&\le \kappa(\Sigma) E_{opt}(r).
\end{align}
\end{restatable}
\mytodo{Tightness: construct an example where $r > 0$, $\kappa(\Sigma) > 1$, and $E(w_{norm}(r),r) = \kappa(\Sigma)E_{opt}(r)$.}
\begin{proof}
Indeed, using the previous lemma, one computes
\begin{eqnarray*}
\begin{split}
E_{opt}(r) &:= \inf_w E(w,r) \le E(w_{norm}(r),r) \\
&\le E_{norm}(w_{norm}(r),r/\sqrt\lambda_{min}) = \inf_w E_{norm}(w,r/\sqrt\lambda_{min})\\
&\le \inf_w E(\Sigma^{-1/2} w,r\sqrt{\lambda_{max}/\lambda_{min}}) = \inf_w E(\Sigma^{-1/2} w,r\sqrt{\kappa(\Sigma)}) \\
&= \inf_w E(w,r\sqrt{\kappa(\Sigma)}) = E_{opt}(r\sqrt{\kappa(\Sigma)}).
\end{split}
\end{eqnarray*}
The second part of the claimed inequalities follows from the lemma below applied with $a = \sqrt{\kappa(\Sigma)}$.
\end{proof}
\begin{restatable}{lm}{}
For any $w \in \mathbb R^d$, $r \ge 0$, and $a \ge 1$, it holds that
\begin{eqnarray}
E(w,ar) \le a^2 E(w,r),
\end{eqnarray}
with equality if $w=w_0$.
\end{restatable}
\begin{restatable}{rmk}{}
Note that if $w$ is close to zero, then $E(w,ar)$ ought to be close to $E(w,r)$ which is $\|w_0\|_\Sigma^2$, and can be much less than upper-bound than $a^2\|w_0\|_\Sigma^2$ proposed by the lemma. thus, the upper-bound in the lemma can be arbitrarily off / bad.
\end{restatable}

\begin{proof}[Proof of lemma]
Indeed, one computes
\begin{eqnarray*}
\begin{split}
E(w,ar) &= \|w-w_0\|_\Sigma^2 + a^2r^2\|w\|_\star^2 + 2ac_0r\|w-w_0\|_\Sigma\|w\|_\star\\
&\le a^2\|w-w_0\|_\Sigma^2 + a^2r^2\|w\|_\star^2 + 2ac_0r\|w-w_0\|_\Sigma\|w\|_\star\\
&\le a^2 (\|w-w_0\|_\Sigma^2 + r^2\|w\|_\star^2 + 2(1/a) c_0r\|w-w_0\|_\Sigma\|w\|_\star)\\
&\le a^2 E(w,r),
\end{split}
\end{eqnarray*}
where we have used the fact that $1 \le a^2$ and $1/a \le 1$, on the second and last lines respectively.
\end{proof}

We can now generalize this procedure to all attacks. Indeed the main difference is that in the general we do not have acccess to $R_1$ and $R_2$, however we can still obtain an approximation of $R_1$ and $R_2$ using our approximation $\gamma_r(w_0)$. Note also that in the general case, we still have a bias which has a U form and therefore we can still apply early-stopping on the normalized data and obtain for free our best estimator. 


\subsection{Explicit solution for isotropic case}
Proposition 1  of \url{https://arxiv.org/pdf/2012.10278.pdf} can be used to salvage an explicit formula for minimizer of $w \mapsto E_{\text{norm}}(w,r)$ in the case of euclidean attacks.
Indeed,
\begin{restatable}{prop}{}
For any $r \ge 0$, a minimizer of $w \mapsto E_{norm}(w,r)$ is given by $w_{norm}(r) = (1+\lambda_{opt}(r))^{-1}w_0$, where
\begin{eqnarray}
\lambda_{opt}(r) = \begin{cases}
0,&\mbox{ if }r \le c_0,\\
(r^2 - c_0 r)/(1 - c_0 r), &\mbox{ if }c_0 < r < 1/c_0,\\
\infty,&\mbox{ if }r \ge 1/c_0.
\end{cases}
\label{eq:lambdaopt}
\end{eqnarray}
\label{prop:normalized}
\end{restatable}
Importantly, $w_{norm}(r)$ corresponds to \textit{shrinking} $w_0$ towards zero!












% \section{Robustness via shrinkage to zero}
% \mytodo{Link the ideas presented hereunder to the so-called "Stein shrinkage" \url{http://proceedings.mlr.press/v32/muandet14.pdf}}
% \subsection{Optimizing over a chord}
% For any model nonzero $z \in \mathbb R^d$, consider the chord $[0,z] := \{\alpha z \mid \alpha \in [0, 1]\}$ that joins $z$ to the origin. This chord corresponds to shrinking $z$ to zero. As before, set $c_0:=\sqrt{2/\pi}$. Consider the problem of minimizing the robust risk $w \mapsto E(w,r)$ over $[0,z]$. Now, for any $\alpha \in [0, 1]$, one has
% \begin{eqnarray}
% E(\alpha z,r) = (1-\alpha)^2\|z\|_\Sigma^2  + \alpha^2r^2\|z\|_\star^2  + 2c_0\alpha(1-\alpha)r\|z\|_\Sigma\|z\|_\star = a\alpha^2 - 2b\alpha + c,
% \end{eqnarray}
% a quadratic polynomial in $\alpha$ with coefficients $a=a(z,r) := \|z\|_\Sigma^2 + r^2\|z\|_\star^2 - 2c_0r\|z\|_\Sigma\|z\|_\star$, $b=b(z,r) := \|z\|_\Sigma^2-c_0r\|z\|_\Sigma\|z\|_\star$, and $c=c(z,r) = \|z\|_\Sigma^2$. On the other hand, it is clear that the leading coefficient $a(z,r)$ is itself a quadratic in $r$ with discriminant $\|z\|_\Sigma^2\|z\|_\star^2(c_0^2-1)$ which is strictly negative because $c_0^2 = 2/\pi < 1$. Thus, $\alpha \mapsto E(\alpha z, r)$ is a convex one-dimensional quadratic function. We conclude that this function is minimized at $\alpha_{opt}(z,r) = $ the unique point of $[0,1]$ which is closest to the real number $\widetilde\alpha_{opt}(z,r) \in \mathbb R$ defined by
% \begin{eqnarray}
% \widetilde\alpha_{opt}(z,r) := \frac{b(z,r)}{a(z,r)} = \frac{\|z\|_\Sigma^2-c_0r\|z\|_\Sigma\|z\|_\star}{\|z\|_\Sigma^2 + r^2\|z\|_\star^2 - 2c_0r\|z\|_\Sigma\|z\|_\star}.
% \end{eqnarray}

% \begin{restatable}{lm}{}
% For any fixed $z \in \mathbb R^d$, it holds that
% \begin{eqnarray}
% \lim_{r \to 0^+}\widetilde\alpha_{opt}(z,r) = 1,\,\lim_{r \to \infty}\widetilde\alpha_{opt}(z,r) = 0.
% \end{eqnarray}
% Moreover, if $\|\cdot\|_\star = \|\cdot\|_\Sigma$ (i.e if the attacker's norm is $\|\cdot\|_{\Sigma{-1}}$), then
% \begin{eqnarray}
% \widetilde\alpha_{opt}(z,r) = (1-c_0 r) / (1+r^2-2c_0r).
% \end{eqnarray}
% \end{restatable}

% \begin{restatable}{rmk}{}
% In isotropic case, we know from Prop \ref{prop:normalized} that the minimizer of the normalized energy $w \mapsto E(w,r)$ is $w_{opt}(r) = (1+\lambda_{opt}(r))^{-1} w_0$,
% where $\lambda_{opt}(r)$ is given in \eqref{eq:lambdaopt}. This is consistent with the above lemma as one easily verifies that for $c_0 < r < 1/c_0$, 
% $$
% (1+\lambda_{opt}(r))^{-1} = ((r^2+1-2c_0 r)/(1-c_0r))^{-1} = (1-c_0r)/(1+r^2-2c_0 r) = \alpha_{opt}(r).
% $$
% \end{restatable}

% Now, in the general case, define $r_0(z)$, $r_1(z)$, and $r_2(z)$ by \begin{eqnarray}
% r_0(z):= \frac{\|z\|_\Sigma}{\|z\|_\star},\, r_1(z):=c_0r_0(z),\,
% r_2(z) := \frac{1}{c_0^2} r_1(z) = \frac{1}{c_0}r_0(z).
% \end{eqnarray}
% In the case where the attacker's norm is the $\ell_\infty$-norm so that its dual $\|\cdot\|_\star$ is the $\ell_1$-norm, $r_0$ (in fact, $1/r_0(z)$) can be thought of as the sparsity level in $z$.
% A simple computation reveals that
% \begin{eqnarray}
% \alpha_{opt}(z,r) = % \min(\max(\widetilde\alpha_{opt}(z,r),0), 1)
% = \begin{cases}
% 1, &\mbox{ if }0 \le r < r_1(z),\\
% \widetilde\alpha_{opt}(z,r),&\mbox{ if }r_1(z) \le r \le r_2(z),\\
% 0,&\mbox{ if } r > r_2(z).
% \end{cases}
% \end{eqnarray}
% Finally, note that
% \begin{eqnarray}
% E(\alpha_{opt}(z,r)z,r) = \begin{cases}
% E(z,r), &\mbox{ if }0 \le r < r_1(z),\\
% c(z,r)-\dfrac{b(z,r)^2}{a(z,r)} =\dfrac{(1-c_0^2)\|z\|_\Sigma^2}{h(r_0(z)/r)},&\mbox{ if }r_1(z) \le r \le r_2(z),\\
% E(0,r) = \|z\|_\Sigma^2,&\mbox{ if } r > r_2(z).
% \end{cases}
% \end{eqnarray}
% where the function $h:\mathbb R \to \mathbb R$ is defined by
% \begin{eqnarray}
% h(t) := t^2+1-2c_0 t.
% \end{eqnarray}
% FWIW, note that
% $(t-1)^2 \le h(t) \le t^2 + 1$ for any $t \in \mathbb R$.

% Putting things together, we obtain the following result.
% \begin{restatable}{prop}{}
% For any nonzero $z \in \mathbb R^d$, the minimum of $w \mapsto E(w,r)$ over the chord $[0,z]$ is attained at the point $\alpha_{opt}(z,r) z$. That is,
% \begin{eqnarray}
% \inf_{w \in [0,z]}E(w, r) = E(\alpha_{opt}(z,r)z,r)
% = \begin{cases}
% E(z,r),&\mbox{ if }0 \le r < r_1(z),\\
% \dfrac{r^2(1-c_0^2)\|z\|_\Sigma^2\|z\|_\star^2}{a(z,r)},&\mbox{ if }r_1(z) \le r \le r_2(z),\\
% E(0,r) = \|w_0\|_\Sigma^2,&\mbox{ if }r > r_2(z).
% \end{cases}
% \end{eqnarray}
% \label{prop:alpha}
% \end{restatable}

% The following theorem quantifies the improvement of the robust error of any model.
% \begin{restatable}{thm}{}
%  For any nonzero model $w \in \mathbb R^d$, it holds that
% \begin{itemize}
% \item[(A)] If $0 \le r \le r_1(w)$, then $E(\alpha_{opt}(w,r),r) = E(w,r)$.
% \item[(B)] If $r_1(w) \le r \le r_2(w)$, then
% $\dfrac{E(\alpha_{opt}(w,r),r)}{E(w,r)} = \dfrac{1-c_0^2}{h(r/r_0(w))} \le 1$.
% \item[(C)] If $r \ge r_2(w)$, then $\dfrac{E(\alpha_{opt}(w,r),r)}{E(w,r)} =  \dfrac{\|w_0\|_\Sigma^2}{E(w,r)} \le 1$.
% \end{itemize}
% \end{restatable}

% For simplicity of notation, write $r_1  := c_0 r_0$, and $r_2 := r_0/c_0$, where $r_0:=\|w_0\|_\Sigma/\|w_0\|_\star$.

% \subsection{A note on the euclidean case}
% In the case of euclidean attacks, we can obtain finer results. 
% \begin{restatable}{rmk}{}
% Define $R_1 = R_1(w_0) := c_0\|w_0\|_2/\|w_0\|_{\Sigma^{-1}}$ and $R_1 = R_2(w_0):=(1/c_0)\|w_0\|_{\Sigma^2}/\|w_0\|_{\Sigma}$. 
% It was shown in Proposition 1 of \url{https://arxiv.org/pdf/2012.10278.pdf} that 
% \begin{itemize}
%     \item If $ 0 \le r \le R_1$, then $E_{opt}(r) = E(w_0,r) = r^2\|w_0\|_2^2$.
%     \item If $r \ge R_2$, then
%     $E_{opt}(r) = E(0,r) = \|w_0\|_\Sigma^2$.
% \end{itemize}
% \label{rmk:extremes}
% \end{restatable}
% Little was said for $r \in [R_1,R_2]$; the analysis in that interval is untractable, except in the special case where the covariance matrix is the identity matrix. We will remedy the situation by settling for near-optimal solutions: that is points whose robust risk $E(w,r)$ is within a multiplicative factor the global minimum $E_{opt}(r)$. 

% The following lemma will be useful in the special case of euclidean attacks.
% \begin{restatable}{lm}{}
% In the case of euclidean attacks, it holds that
% $r_1 \ge R_1$ and $R_2 \ge r_2$.
% \end{restatable}
% \begin{proof}
% Indeed,  we have
% \begin{align}
% r_1 &\ge R_1 \text{ iff } \|w_0\|_{\Sigma^{-1}}\|w_0\|_{\Sigma} \ge \|w_0\|_2^2 = \langle w_0, w_0\rangle,\\
% R_2 &\ge r_2 \text{ iff }\|w_0\|_{\Sigma^2}\|w_0\|_2 \ge \|w_0\|_\Sigma^2 \text{ iff }\|\Sigma w_0\|_2 \|w_0\|_2 \ge \langle \Sigma w_0,w_0\rangle.
% \end{align}
% Thanks to Cauchy-Schwarz inequality, and the fact that the $\ell_2$-norm is self-dual while $\|\cdot\|_{\Sigma}$ and $\|\cdot\|_{\Sigma^{-1}}$ are duals of one another, the rightmost side (and therefore the leftmost side too) of the each of the above equivalencies is satisfied.
% \end{proof}
% In particularly, if $\Sigma = \sigma^2 I_d$ (or more generally, if $w_0$ is an eigenvector of $\Sigma$), then $r_1 = R_1$ and $r_2 = R_2$.

% \subsection{Main results}
% Let $\lambda_{min}$ (resp. $\lambda_{max}$) be the smallest (resp. largest) value of the ratio $r_0(w) := \|w\|_\Sigma/\|w\|_\star$ over non-zero vectors $w \in \mathbb R^d$. That is,
% \begin{eqnarray}
% \lambda_{max} := \sup_{w \in \mathbb R^d,\,w \ne 0}r_0(w)^2,\, \lambda_{min} := \inf_{w \in \mathbb R^d,\,w \ne 0}r_0(w)^2.
% \end{eqnarray}
% Also, let $\kappa(\Sigma)=\kappa^{\|\cdot\|}(\Sigma)$ be the \emph{condition number} of $\Sigma$ w.r.t the norm $\|\cdot\|$, i.e
% \begin{eqnarray}
% \kappa(\Sigma) := \lambda_{max}/\lambda_{min},\,\kappa^0(\Sigma):=\lambda_{max}/r_0(w_0)^2,\,\kappa^1(\Sigma) := r_0(w_0)^2/\lambda_{min}.
% \end{eqnarray}
% In the particular case of euclidean attacks, $\lambda_{max}$ (resp. $\lambda_{min}$) corresponds to the largest (resp. smallest) eigenvalue of $\Sigma$. In this case $\kappa(\Sigma)$ is the usual condition number of $\Sigma$.
% In any case, it always holds that $\kappa(\Sigma) \ge \max(\kappa^0(\Sigma),\kappa^1(\Sigma))$ and $\min(\kappa^0(\Sigma),\kappa^1(\Sigma)) \ge 1$ with $\kappa(\Sigma) = 1$ iff the attacker's norm $\|\cdot\|$ is proportional to $\|\cdot\|_{\Sigma^{-1}}$. For example, this is the case when $\Sigma = \sigma^2 I_d$ and the attacker's norm is euclidean.
% On the other hand, note that $\kappa(\Sigma)$ can be arbitrarily large. For example, if $\Sigma=I_d$ and the attacker's norm $\|\cdot\|$ is the $\ell_\infty$-norm, then it is easy to see that $\kappa(\Sigma) = d$.

% The following lemma will be useful.
% \begin{restatable}{lm}{}
% Define $\gamma_r(w_0) := \inf_{w \in \mathbb R^d}\|w-w_0\|_\Sigma + r\|w\|_\star$. Then,
% \begin{align}
%      \gamma_r(w_0) &\ge \min(1,r/\sqrt \lambda_{max})\|w_0\|_\Sigma,\\
%      \gamma_r(w_0) &\ge \min(\sqrt \lambda_{min},r)\|w_0\|_\star.
% \end{align}
% \label{lm:densesparse}
% \end{restatable}
% \begin{proof}
% Let $w \in \mathbb R^d$.
% Indeed, by definition of $\lambda_{max}$, it holds that $\|w\|_\star \ge \|w\|_\Sigma/\sqrt\lambda_{max}$, and so one may write $$
% \|w-w_0\|_\Sigma + r\|w\|_\star \ge \|w-w_0\|_\Sigma + (r/\sqrt\lambda_{max})\|w\|_\Sigma \ge \min(1,r/\sqrt\lambda_{max})\|w_0\|_\Sigma,
% $$
% which proves the first lower-bound.
% Similarly, by definition of $\lambda_{min}$, it holds that $\|w-w_0\|_\Sigma \ge \sqrt\lambda_{min}\|w-w_0\|_\star$, and so
% $$
% \|w-w_0\|_\Sigma + r\|w\|_\star \ge \sqrt\lambda_{min}\|w-w_0\|_\star + r\|w\|_\star \ge \min(\sqrt\lambda_{min},r)\|w_0\|_\star,
% $$
% which proves the second lower-bound.
% \end{proof}

% We are now ready to state the main result of this section wherein we show that optimizing on the chord $[0,w_0]$ gives a point which is optimal up to within a multiplicative factor of $1.747\kappa(\Sigma)$. Viz,
% \begin{restatable}{thm}{}
% We have the following:
% \begin{itemize}
% \item[(A)] In the case of an attack of magnitude $r$ w.r.t to an arbitrary norm $\|\cdot\|$, for  $r_1 \le r \le r_2$, it holds that
% \begin{eqnarray}
% \dfrac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)}
% % \le \dfrac{2(1-c_0^2)}{1+c_0}\frac{\lambda_{min} \land r^2}{h(r_0/r)}\kappa(\Sigma)
% \le \dfrac{2}{(1+c_0)c_0^2}\kappa^0(\Sigma) \approx 1.747\kappa^0(\Sigma).
% \end{eqnarray}
% \item[(B)] In the case of euclidean attacks, if $0 \le r \le R_1$ or $r \ge R_2$, then it holds that $E(\alpha_{opt}(w_0,r),r) = E_{opt}(r)$. In addition, if $R_1 < r <R_2 $, then $\dfrac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} \leq\kappa^1(\Sigma)$.
% \end{itemize}
% \end{restatable}
% \mytodo{Extend part (B) to general non-euclidean norm attacks.}\\
% \begin{proof}
% We first prove part A of the result. One computes
% \begin{eqnarray}
% \begin{split}
% \frac{2}{1+c_0} \cdot E_{opt}(r) &\ge \left(\inf_{w \in \mathbb R^d} \|w-w_0\|_\Sigma + r\|w\|_\star\right)^2\\
% % &\ge \left(\inf_{w \in \mathbb R^d}\sqrt{\lambda_{min}}\|w-w_0\|_\star + r\|w\|_\star\right)^2\\
% &\ge (\lambda_{min} \land r^2)\|w_0\|_\star^2 \lor (1 \land r^2/\lambda_{max})\|w_0\|_\Sigma^2,
% \end{split}
% \label{eq:toto}
% \end{eqnarray}
% where the first step is thanks to Lemma \ref{lm:burger} below and the second step is thanks to Lemma \ref{lm:densesparse}.
% On the other hand, for $r_1 \le r \le r_2$, we deduce from Proposition \ref{prop:alpha} that
% \begin{eqnarray}
% \begin{split}
% E(\alpha_{opt}(w_0,r),r) &= \frac{(1-c_0^2)\|w_0\|_\Sigma^2}{h(r_0/r)}
% % &\le \frac{(1-c_0^2)\|w_0\|_\Sigma^2}{h(r_0/r_2)}
% \le \frac{1-c_0^2}{h(r_0/r)}\lambda_{max}\|w_0\|_\star^2 \le \lambda_{max}\|w_0\|_\star^2,
% \end{split}
% \label{eq:tata}
% \end{eqnarray}
% where we have used the fact that $h(t) := t^2+1-2tc_0 \ge h(c_0) = 1-c_0^2$ for all $t \in \mathbb R$. On the same interval, \eqref{eq:toto} further gives
% \begin{eqnarray}
% \begin{split}
% \frac{2E_{opt}(r)}{(1+c_0)\|w_0\|_\star^2} &\ge \lambda_{min} \land r^2 \ge \lambda_{min} \land r_1^2 \ge  \lambda_{min} \land c_0^2\lambda_{min}=c_0^2\lambda_{min},\\
% \frac{2E_{opt}(r)}{(1+c_0)\|w_0\|_\Sigma^2} &\ge 1 \land r^2/\lambda_{max} \ge 1\land r_1^2/\lambda_{max} \ge  1 \land c_0^2 r_0^2/\lambda_{max} =\frac{c_0^2r_0^2}{\lambda_{max}} = \frac{c_0^2}{\kappa^0(\Sigma)},
% \end{split}
% \end{eqnarray}
% and we deduce that
% \begin{eqnarray}
% \begin{split}
% E_{opt}(r) &\ge \frac{(1+c_0)}{2}(\lambda_{min} \land r^2)\|w_0\|_\star^2 \ge \dfrac{(1+c_0)c_0^2}{2}\lambda_{min}\|w_0\|_\star^2,\\
% E_{opt}(r) &\ge \frac{(1+c_0)}{2}(1 \land r^2/\lambda_{max})\|w_0\|_\Sigma^2 \ge \dfrac{(1+c_0)c_0^2}{2}\kappa^0(\Sigma)\|w_0\|_\Sigma^2.
% \end{split}
% \label{eq:titi}
% \end{eqnarray}
% Putting \eqref{eq:tata} and \eqref{eq:titi} together gives
% \begin{eqnarray*}
% \begin{split}
% 1 \le \frac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} &\le \frac{2}{(1+c_0)c_0^2}\frac{(1-c_0^2)}{h(r_0/r)}\kappa^0(\Sigma) = \frac{2}{(1+c_0)c_0^2}\frac{1-c_0^2}{h(r_0/r)}\kappa^0(\Sigma)\\
% &\le \frac{2}{(1+c_0)c_0^2}\kappa^0(\Sigma),
% %1 \le \frac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} &\le \frac{2}{(1+c_0)c_0^2}\frac{(1-c_0^2)}{h(r_0/r)}\frac{\lambda_{max}}{\lambda_{min}} = \frac{2}{(1+c_0)c_0^2}\frac{1-c_0^2}{h(r_0/r)}\kappa(\Sigma)\\
% %&\le \frac{2}{(1+c_0)c_0^2}\kappa(\Sigma),
% \end{split}
% \end{eqnarray*}
% as desired.

% We now prove part B. If $r \le R_1$ or $r \ge R_2$, part B follows directly from Proposition \ref{prop:alpha} and Remark \ref{rmk:extremes}, since $R_1 \ge r_1$ and $R_2 \le r_2$ as already mentioned above.

% If $R_1 \le r \le r_1$ (resp. $r_2 \le r \le R_2$), then thanks to Proposition \ref{prop:alpha} we have $E_{opt}(r) \ge E_{opt}(R_1) = R_1^2\|w_0\|_2^2$ and $E(\alpha_{opt}(w_0,r),r)\leq r_1^2\|w_0\|_2^2$ which gives that
% \begin{align*}
%     E(\alpha_{opt}(w_0,r),r)/E_{opt}(r)\leq r_1^2/R_1^2\leq \kappa^1(\Sigma).
% \end{align*}
% In addition if $r_2 \le r \le R_2$, we have that $E(\alpha_{opt}(w_0,r),r)=\|w_0\|_{\Sigma}^2$ and $E_{opt}(r) \ge E_{opt}(R_1) = R_1^2\|w_0\|_2^2$, which gives that
% \begin{align*}
%     E(\alpha_{opt}(w_0,r),r) / E_{opt}(r)\leq
%     \frac{1}{c_0^2}\frac{\|w_0\|_{\Sigma^{-1}}^2\|w_0\|_{\Sigma}^2}{\|w_0\|_2^2 \|w_0\|_2^2}\leq \frac{ \kappa^1(\Sigma)}{c_0^2}
% \end{align*}
% \end{proof}

% \begin{restatable}{lm}{}
% \label{lm:burger}
% If $u,v,\beta \ge 0$ with $\beta \le 1$, then
% \begin{eqnarray}
% \frac{(1+\beta)}{2}(u+v)^2 \le u^2 + v^2 + 2\beta u v \le (u+v)^2.
% \end{eqnarray}
% \end{restatable}
% \begin{proof}
% The second inequality follows directly from the fact that $0 \le \beta \le 1$. For the first inequality, simply observe that
% $$
% 2(u^2 + v^2 + 2\beta u v)  - (1+\beta)(u+v)^2 = (1-\beta)(u-v)^2 \ge 0.
% $$
% \end{proof}

% \section{Estimation}
% In order to estimate our new predictor we propose the following estimator
% \begin{align*}
%     \widehat{w}_{0,\text{rob}}:= \max(\min(1,b(\widehat{w_0},r)/a(\widehat{w_0},r)),0)\widehat{w_0}
% \end{align*}
% where $\widehat{w}_0$ is an estimator of the generative model $w_0$ given samples. We just need to control the error in the different norm of our estimator $\widehat{w}_0$ compared to the true $w_0$ in order to control the robust error of our estimator.

% \input{beyond.tex}

% \section{Spectral decomposition in case of euclidean attack}
% Assume the attacker's norm is euclidean.
% Also, suppose the "ridge-ing matrix" $\Sigma$ diagonalizes in the same orthonormal basis $\{v_1,v_2,\ldots\}$ as population covariance matrix of the features, namely $L_K=\Sigma_x$.
% As we already saw, in the case of gradient-descent with / without robustness training, we should have the dynamics $w_M(t) = K_t(L_K)L_K w_0 = \sum_j \sum_{ 0\leq s\leq t-1} (1-\alpha \lambda_j)^{s} \lambda_j c_j v_j$, where $c_j := \langle v_j, w_0\rangle$. Thus, at time $t$, the hard robust risk writes
% \begin{eqnarray}
% \begin{split}
%     E_M(t;r) := E(w_M(t);r) = B(t) + r^2 V(t) + r\sqrt{8/\pi} \sqrt{A(t)}\sqrt{V(t)},
% \end{split}
% \end{eqnarray}
% where $B(t):=\sum_j (1-\beta_j(t)\lambda_j)^2\lambda_j c_j^2$ and
% $V(t) := \sum_j (1-\alpha\widetilde\lambda_j)^{2t}\lambda_jc_j^2$,
% and $c_j := \langle v_j,w_0\rangle$.
% Note that for any $t$, $V(t)$ is an non-increasing function of $\Sigma$, whilst $B(t)$ is a non-decreasing function of $\Sigma$.

% \section{Interlude: some interesting computations}
% Noting that $1/2 \le \sqrt{2/\pi} \le 1$, it is clear from \eqref{eq:E} that for any $w \in \mathbb R^d$, we have
% \begin{eqnarray}
% \label{eq:sandwich}
% \sqrt{2/\pi}\overline E(w; r) \le E(w; r) \le \overline E(w; r),
% \end{eqnarray}
% where $\overline E(w; r) := (\|w-w_0\|_\Sigma + r\|w\|_\star)^2$, where, $\|\cdot\|_\star$ is the dual of the attacker's norm $\|\cdot\|$. Thus, the functions $E$ and $\overline E$ are within a constant factor of one another, i.e they are comparable. The gain here is that, compared to $E(w; r)$, it is easier to analyze $\overline E(w; r)$ w.r.t $w$.
% Though the $1/2$ factor is clearly not optimal, it will suffice for our purposes\footnote{In fact positive constant factor $\alpha = \Omega(1)$ will do.}

\subsection{Optimizing over sub-level curves of ordinary test error}
Note that the robustness test error of the ground-truth model $w_0$ (which minimizes the ordinary test error) is $E(w_0;r) = r^2\|w_0\|_\star^2$.
We shall now compute lower-bounds for the robustness test error $E(w; r)$, on sub-level sets of the ordinary test error $E(w)= E(w,0) = \|w-w_0\|_{\Sigma_x}^2$, i.e over all $w$'s which have a given value of ordinary test error $E(w)\le E_0$, where $E_0 \ge 0$ is a fixed threshold / level.
We will do analogous computations over sub-level sets of ordinary training error later.

\begin{restatable}{thm}{}
For any threshold $E_0 \ge 0$, it holds that
\begin{eqnarray}
    \inf_{E(w) \le E_0} E(w; r) \ge \frac{r^2}{2}\left(\inf_{\|v\|_2 \le E_0}\|w_0-\Sigma_x^{-1/2}v\|_\star^2\right).
\end{eqnarray}
In particular, if the attacker's norm is an $\ell_p$-norm for some $p \in [1,\infty]$, then
\begin{eqnarray}
\inf_{E(w) \le E_0} \frac{E(w; r)}{E(w_0;r)} \ge \frac{C_p}{2}\cdot  \left(1-\sqrt{\frac{E_0}{\|\Sigma_x\|_{\mathrm{op}}\|w_0\|_{p^\star}^2}}\right)_+^2,
\end{eqnarray}
where $p^\star \in [1,\infty]$ is the harmonic conjugate of $p$, i.e $1/p+1/p^\star = 1$, and
\begin{eqnarray}
C_p := \begin{cases}
d^{1-2/p},&\mbox{ if }1 \le p < 2,\\
1,&\mbox{ else.}
\end{cases}.
\end{eqnarray}
\end{restatable}
Thus, for $\ell_p$-norm attacks with $p \in [2,\infty]$, if $E_0 \lesssim \|\Sigma_x\|_{\mathrm{op}}\|w_0\|_{p^\star}^2$, any linear model $w$ with ordinary test error at least $E_0$ must suffer robustness test error $E(w; r) \gtrsim E(w_0; r)=r^2\|w_0\|_\star^2$.
\begin{proof}
To simplify notations, let $\Sigma_x=\Sigma$. One computes
\begin{eqnarray}
\begin{split}
\inf_{\|w-w_0\|_{\Sigma}^2 \le E_0} \sqrt{\overline E(w; r)}&= \inf_{\|w-w_0\|_{\Sigma}^2 \le E_0} \|w-w_0\|_\Sigma + r\|w\|_\star\\
&= \inf_{\|w\|_{\Sigma} \le E_0} \|w\|_\Sigma+r\|w+w_0\|_\star\\
&= \inf_{\|w\|_2 \le E_0} \|w\|_2+r\|\Sigma^{-1/2}w+w_0\|_\star\\
&= \inf_{\|w\|_2 \le E_0} \|w\|_2+\sup_{\|z\| \le r}z^\top(\Sigma^{-1/2}w+w_0)\\
&=\sup_{\|z\| \le r}z^\top w_0 + \inf_{\|w\|_2\le E_0}\|w\|_2+\overline z^\top w,\text{ with }\overline z := \Sigma^{-1/2}z\\
&= \sup_{\|z\| \le r}z^\top w_0 + \inf_{\|w\|_2 \le E_0} \sup_{\|u\|_2 \le 1}u^\top w + \overline z^\top w\\
&=\sup_{\|z\| \le r}z^\top w_0 + \sup_{\|u\|_2 \le 1}\inf_{\|w\|_2 \le E_0} u^\top w + \overline z^\top w\\
&= \sup_{\|z\| \le r}z^\top w_0 + \sup_{\|u\|_2 \le 1}-E_0\cdot\|u+\overline z\|_2\\
&= \sup_{\|z\| \le r}z^\top w_0 - E_0\cdot \inf_{\|u\|_2 \le 1}\|u+\overline z\|_2\\
&= \sup_{\|z\| \le r}z^\top w_0 -  E_0\cdot(\|\overline z\|_2-1)_+ \\
 &\ge \sup_{\|z\| \le r}z^\top w_0 -  E_0\cdot \|\overline z\|_2\\
 &=\inf_{\|v\|_2 \le E_0}\sup_{\|z\| \le r}z^\top w_0 -  z^\top\Sigma^{-1/2}v\\
 &= r\inf_{\|v\|_2 \le E_0}\|w_0-\Sigma^{-1/2}v\|_\star,
\end{split}
\end{eqnarray}
which proves the first part upon combining with \eqref{eq:E}.

Finally, if the attacker's norm is an $\ell_p$-norm, then thanks to Lemma \ref{lm:noneuclideanlstsq} below applied with $q=p^\star=p/(p-1)$, the last expression can be further lower-bounded by $$
r\cdot\min(1,d^{1/2-1/p})\cdot \left(\|w_0\|_\star-\sqrt{\dfrac{E_0}{\|\Sigma_x\|_{\mathrm{op}}}}\right)_+.
$$
\end{proof}
\begin{restatable}{lm}{}
\label{lm:noneuclideanlstsq}
Let $A$ be an $m \times d$ matrix and $b \in \mathbb R^m$. Then, for any $q \in [1,\infty]$, it holds that
\begin{eqnarray}
\inf_{\|v\|_2 \le r} \|Av-b\|_q \ge \min(1,d^{1/q-1/2})(\|b\|-r\|A\|_{\mathrm{op}})_+.
\end{eqnarray}
\end{restatable}
\begin{proof}
Define $\alpha_q :=\inf_{\|v\|_2 \le r}\|Av-b\|_q$. Since $\|v\|_q \ge \min(1,d^{1/q-1/2})\|v\|_2$ for any $v \in \mathbb R^d$, we know that
$\alpha_q \ge \min(1,d^{1/q-1/2})\alpha_2$.
We now lower-bound $\alpha_2$ to complete the proof. By "dualizing", one has
\begin{eqnarray}
\begin{split}
\alpha_2 &= \inf_{\|z\|_2 \le r}\|Az-b\|_2 = \inf_{\|z\|_2 \le r}\sup_{\|v\|_2 \le 1}v^\top(b-Az)\\
&= \sup_{\|v\|_2 \le 1}v^\top b+\inf_{\|z\|_2 \le r}-v^\top Az
= \sup_{\|v\|_2 \le 1} v^\top b - r\|Av\|_2\\
&\ge \sup_{\|v\|_2 \le 1} v^\top b - r\|A\|_{\mathrm{op}}\|v\|_2 = (\|b\|-r\|A\|_{\mathrm{op}})_+.
\end{split}
\end{eqnarray}
Putting things together gives the claimed lower-bound.
\end{proof}

==> early-stopped adversarial training/sections/outline.tex <==
\subsection{Outline of Manuscript}
In Section \ref{sec:preliminaries}, we present the problem setup, main definitions, and some preliminary computations. The adversarial risk of (early-stopped) GD in the infinite-sample regime is analyzed in Section \ref{sec:gd}; cases of optimality and sub-optimality of this scheme are characterized. In Section \ref{sec:gdplus}, GD+ (an improved version of GD) is proposed, and its adversarial risk in the population regime is studied. In Section \ref{sec:algorithmic}, we consider the finite samples regime and we propose a simple two-stage estimator, which works for all attacker norms. Its adversarial risk is shown to be optimal up to within a multiplicative factor, and additive statistical estimation error due to finite samples.

==> early-stopped adversarial training/sections/powerlaw.tex <==
\section{Power-Law Phenomena in the Finite-Sample Regime}
Let  $\Sigma = \sum_{j=1}^d \lambda_j v_jv_j^\top$ be the SVD of the feature covariance matrix $\Sigma$. As usual, let $w_0 \in \mathbb R^d$ be the ground-truth linear model, and set $c_j := w_0^\top v_j$ for all $j \in [d]$.
We make the following structural assumption motivated by \url{https://arxiv.org/pdf/2203.06176.pdf}.
\begin{mdframed}
\begin{restatable}[Power law regime]{assume}{}
    Suppose there exist constants $\gamma \in (0,\infty)$ and $\delta \in [0,\infty)$ such that 
    \begin{eqnarray}
    \lambda_j \asymp j^{-1-\gamma}\text{ and }c_j^2 \asymp j^{-\delta}\text{ for all }j \in [d].
    \label{eq:powerlaws}
    \end{eqnarray}
    \label{ass:powerlaws}
\end{restatable}
\end{mdframed}
Such a spectral decay has been observed in real world datasets like MNIST, FashionMNIST, etc. See \url{https://arxiv.org/pdf/2203.06176.pdf} and references therein.

In the regime covered by Assumption \ref{ass:powerlaws}, we shall provide a complete analysis of GD, and prescribe a closed-form expression for the optimal stopping time w.r.t adversarial risk.

\subsection{Local Random Matrix Theory}
Recently, the scope of applicability of RMT-based arguments has significantly been extended by \cite{Knowles2014AnisotropicLL}. For our own purposes, we shall only need a very rudimentary version of these developments, which we now present below. 

\begin{restatable}{df}{}
Let $S$ be a $d \times d$ positive-definite matrix with eigenvalues $\lambda_1(S),\ldots,\lambda_d(S)$.
For any positive $\lambda$, let $\kappa_S(\lambda,n)$ be the unique positive solution to the algebraic equation
\begin{equation}
    1 = \frac{\lambda}{\kappa} + \frac{1}{n}\sum_{j=1}^d \frac{\lambda_j(S)}{\lambda_j(S) + \kappa}.
\end{equation}
In particular, when $S$ is the covariance matrix $\Sigma$ of the features, we will simply write $\kappa = \kappa(\lambda,n) = \kappa_\Sigma(\lambda,n)$.
\label{df:kappa}
\end{restatable}
 The parameter $\lambda$ should be thought of as \emph{explicit} ridge regularization, while $\kappa$ should be thought of as \emph{implicit} ridge regularization.  Note that in the fixed-$d$ large-$n$ regime, one has $\kappa(\lambda,n) \approx \lambda$ with equality if $n=\infty$.

Let $\widehat\lambda_1,\widehat \lambda_2,\ldots,\widehat\lambda_d \ge 0$ be the eigenvalues of the empirical covariance matrix $\widehat\Sigma := X^\top X/n$. The following hypothesis allows us to swap in the population covariance matrix $\Sigma$ for empirical covariance matrix $\widehat\Sigma$ in setting computations, even though we do not have the convergence $\widehat\Sigma \to \Sigma$.
\begin{restatable}[A Local Marchenko-Pastur Hypothesis]{assume}{}
Let $I \subseteq (0,\infty)$. Assume that: for all $u,v \in \mathbb R^d$ such that $\|u\|_\Sigma^2,\|v\|_\Sigma^2 \le 1$, the following holds
\begin{align}
\frac{1}{n}\sum_{i=1}^n \frac{1}{\widehat\lambda_i + \lambda} &= \frac{1}{\kappa} + o_{\mathbb P}(1)\label{eq:hype1},\\
u^\top \lambda(\widehat\Sigma + \lambda I_d)^{-1} v &= u^\top \kappa(\Sigma+\kappa I_d)^{-1} v + o_{\mathbb P}(1)\label{eq:hype2},
\end{align}
uniformly over $\lambda \in I$.
\end{restatable}
Under setting mild regularity conditions on covariance matrix $\Sigma$, the above assumption is in order, thanks to \cite[Theorem 3.6]{Knowles2014AnisotropicLL}.

 \subsection{Main Results}
For any positive $\lambda$, let $\widehat w(\lambda,n)$ correspond to the ridge estimator obtained from the dataset $\mathcal D_n$, i.e
\begin{equation}
\label{eq:ridge}
    \widehat w(\lambda,n) = (\widehat\Sigma + \lambda I_d)^{-1} X^\top y/n \in \mathbb R^{d}.
\end{equation}
One can show that $\widehat w(\lambda,n)$ has the same Euclidean adversarial risk as vanilla GD stopped at $t \propto 1/\lambda$. Thus, analyzing the latter is equivalent to analyzing the former.

 Define scale parameters $\alpha$ and $\beta$ by
 \begin{eqnarray}
 \alpha := (\delta + \gamma) / (1+\gamma),\,\beta := (1 + \delta)/(1+\gamma).
 \end{eqnarray}
 The following computes the adversarial risk attained by the ridge estimator, as a function of $\alpha$, $\beta$, $\kappa$, and the attack strength $r$.
\begin{restatable}{thm}{Epower}
\label{thm:Epower}
Grant Assumption \ref{ass:powerlaws}. For any $r \ge 0$, the Euclidean adversarial risk of the ridge estimator $\widehat w(\lambda,n)$ is given by
\begin{equation}
\label{eq:Escaling}
\begin{split}
    &E^{\|\cdot\|_2}(\widehat w(\lambda,n),w_0,r) \\
   % &\quad\quad\asymp \left(\sqrt{\kappa(\lambda,n)^\alpha + \sigma^2} + \frac{r} {\kappa(\lambda,n)^{\beta/2}}\right)^2 + o_{\mathbb P}(1)\\
    &\quad\quad \asymp \left(\kappa(\lambda,n)^{\alpha/2}  + \frac{r} {\kappa(\lambda,n)^{\beta/2}} + \sigma\right)^2 + o_{\mathbb P}(1).
    \end{split}
\end{equation}
\end{restatable}

The following corollary gives a  closed-form expression for the (inverse) time when GD should be stopped to achieve optimal (up to within a multiplicative absolute constant) adversarial risk under Assumption \ref{ass:powerlaws}.
\begin{restatable}{cor}{Epowercor}
\label{cor:Epowercor}
Grant Assumption \ref{ass:powerlaws}. If $\lambda^\star(r,n)$ is the unique $\lambda \in [0,\infty)$ which solves $\kappa(\lambda,n) = (r\beta/\alpha)^{(\alpha+\beta)/2}$, then 
\begin{equation}
    1 \le \sup_{r \ge 0}\frac{E^{\|\cdot\|_2}(\widehat w(\lambda^\star(r,n)),w_0,r)}{ E^{\|\cdot\|_2}_{opt}(w_0,r)} = O_{\mathbb P}(1).
\end{equation}
\end{restatable}
\begin{restatable}{rmk}{}
Even in the infinite-sample case (i.e $n=\infty$) where $\kappa(\lambda,n) = \lambda$, the above corollary already tells us something highly nontrivial: the optimal ridge (i.e inverse-time) parameter is given by $\lambda^\star(r) = (r\beta/\alpha)^{(\alpha+\beta)/2}$,  a nontrivial polynomial in the attack strength $r$.
\end{restatable}
\begin{proof}[Proof of Corollary \ref{cor:Epowercor}]
Differentiating $\kappa^{\alpha/2} + r\kappa^{-\beta/2}$ w.r.t $\kappa$ and setting to zero, gives $\kappa = (r\beta/\alpha)^{(\alpha+\beta)/2}$. Combining with the preceding theorem shows the optimality of the prescribed value of ridge regularization $\lambda$. The proof is completed by recalling the following result established in \cite{Xing2021}: the linear model which achieves optimal adversarial risk is a ridge.
\end{proof}

==> early-stopped adversarial training/sections/powerlaws_proofs.tex <==
\section{Power-Law Phenomena in Finite-Sample Regimes: Proof Theorem \ref{thm:Epower}}
\Epower*

For the proof of the theorem, we will need some auxiliary results.

 \subsection{Some Preliminary computations}
\paragraph{Change of variables.}
As observed in \url{https://arxiv.org/pdf/2203.06176.pdf}, the dataset $\mathcal D_n$ can be equivalently realized as follows. Fix a smoothing parameter $\theta > 0$  and let $\widetilde x_i(\theta) := (x_i, \theta^{1/2}\epsilon_i) \in \mathbb R^{d + 1}$ and $w_0(\theta) := (w_0, \theta^{-1/2}) \in \mathbb R^{d + 1}$ for all $i \in [n]$, and note that $y_i = \widetilde x_i^\top \widetilde w_0$. That is, we have effectively absorbed the label noises $\epsilon_i$ into the features $x_i$.

Observe that $\theta \mapsto x_i(\theta)$ is a continuous function from $(0,\infty)$ to $\mathbb R^{d+1}$ with
$ \lim_{\theta \to 0^+} x_i(\theta) = (x_i,0)$. Moreover, it is clear that the covariance matrix $\Sigma(\theta) \in \mathcal S_{++}^{d+1}$ of of each $\widetilde x_i$ is given by
\begin{eqnarray}
\Sigma(\theta) = \begin{bmatrix}
\Sigma & 0\\
0 & \theta\sigma^2
 \end{bmatrix}.
 \end{eqnarray}
 Clearly, $\theta \mapsto \Sigma(\theta)$ defines a continuous function from $(0,\infty)$ to $\mathcal S_{++}^{d+1}$, with 
 \begin{eqnarray}
\lim_{\theta \to 0^+}\Sigma(\theta) = \begin{bmatrix}
\Sigma & 0\\
0 & 0
 \end{bmatrix}.
 \end{eqnarray}
  Note that the eigenvectors of $\Sigma(\theta)$ are of the form $v_j(\theta) = (v_j,0) \in \mathbb R^{d + 1}$ for all $j \in [d]$, and $v_{d+1}(\theta) = (0_d,1) \in \mathbb R^{d+1}$, with corresponding eigenvalues $\lambda_j(\theta)$ being $\lambda_j$ and $\theta\sigma^2$ respectively. One computes the alignment between $w_0(\theta)$ and each of these eigenvectors as
 $$
 c_j(\theta) := w_0(\theta)^\top v_j(\theta) =
 \begin{cases}
 w_0^\top v_j =: c_j,&\mbox{ if }1 \le j \le d,\\
 \theta^{-1/2},&\mbox{ if }j=d+1.
 \end{cases}
 $$
 
 Finally, let $X(\theta) := (x_1(\theta),\ldots,x_n(\theta)) \in \mathbb R^{n \times (d+1)}$ be the smoothed design matrix and let $\widehat\Sigma(\theta) := X(\theta)^\top X(\theta)/n \in \mathcal S_+^{d+1}$ be the associated empirical covariance matrix.

 
 \paragraph{Power-law computations.}
 Consider the power laws \eqref{eq:powerlaws}. Let $j^\star := \inf\{j \in [d] \mid \kappa \ge \lambda_j\}$ with the convention that $\inf\emptyset = \infty$. Then, it is easy to see that if $j^\star \ne \infty$, then
 \begin{eqnarray}
j^\star \asymp \kappa^{-\frac{1}{1+\gamma}}.
\end{eqnarray}
Now, $\sum_{j=1}^d \dfrac{\lambda_j}{\lambda_j + \kappa} \asymp j^\star + \dfrac{1}{\kappa}\sum_{j=j^\star}^d \lambda_j \asymp j^\star + \dfrac{1}{\kappa}\int_{j^\star}^d t^{-1-\gamma}\dv t \asymp j^\star + \dfrac{(j^\star)^{-\gamma}}{\kappa} \asymp j^\star \asymp \kappa^{-\frac{1}{1+\gamma}}$. We conclude that $\kappa=\kappa(\lambda,n)$ must satisfy
$1 \asymp \lambda\kappa^{-1} + \dfrac{1}{n}\kappa^{-\frac{1}{1+\gamma}}$.
In particular, we have
\begin{align}
    \kappa &\asymp \lambda+1/n\text{ in the limit }\gamma\to 0^+\\
    \kappa &\asymp \lambda + 1/n^2 + \sqrt \lambda/n \asymp (\sqrt\lambda + 1/n)^2 \text{ in the limit }\gamma \to 1.
\end{align}
Also, for $\lambda$ sufficiently small, we have
\begin{equation}
\label{eq:ridgelesskappa}
    \kappa \asymp 1/n^{1+\gamma}.
\end{equation}
 
\subsection{Dynamics of Ordinary Risk}
Let $\widehat w(\lambda,n,\theta)$ be the ridge estimator obtained from $X(\theta)$ and $y$, i.e
\begin{eqnarray}
\widehat w(\lambda,n,\theta) = (X(\theta)^\top X(\theta)/n+\lambda I_{d+1})^{-1}X(\theta)^\top y/n = (\widehat\Sigma(\theta) + \lambda I_{d+1})^{-1}\widehat\Sigma(\theta) w_0(\theta)  \in \mathbb R^{d+1}.
\end{eqnarray}
Note that the first $d$ coordinates of $\lim_{\theta \to 0^+}\widehat w(\lambda,n,\theta)$ correspond tot eh ridge estimator obtained from $X$ and $y$, i.e
\begin{equation}
    \widehat w(\lambda,n) = (\widehat\Sigma + \lambda I_d)^{-1} X^\top y/n \in \mathbb R^{d}.
\end{equation}
Let $\kappa(\theta) := \kappa_{\Sigma(\theta)}(\lambda,n)$. One computes the risk of $\widehat w(\lambda,n,\theta)$ as follows
\begin{equation}
\begin{split}
    E(\widehat w(\lambda,n,\theta)) &= \|(\widehat\Sigma(\theta) + \lambda I_d)^{-1}\widehat\Sigma(\theta) w_0(\theta)-w_0(\theta)\|_\Sigma^2 = \|\lambda(\widehat \Sigma(\theta) + \lambda I_{d+1})^{-1}w_0(\theta)\|_{\Sigma(\theta)}^2 \\
    &= w_0^\top \lambda(\widehat\Sigma(\theta) + \lambda I_{d+1})^{-1}\Sigma(\theta)\lambda (\widehat\Sigma(\theta) + \lambda I_{d+1})^{-1}w_0(\theta)
    \\
    &= w_0(\theta)^\top \kappa(\theta) (\Sigma(\theta) + \kappa(\theta) I_{d+1})^{-1}\Sigma(\theta)\kappa(\theta) (\Sigma(\theta) + \kappa(\theta) I_{d+1})^{-1}w_0(\theta) + o_{\mathbb P}(1),\text{ thanks to \eqref{eq:hype2}}\\
    &= \kappa(\theta)^2w_0(\theta)^\top \Sigma(\theta)(\Sigma(\theta)+\kappa(\theta) I_{d+1})^{-2}w_0(\theta) + o_{\mathbb P}(1) = \kappa(\theta)^2\sum_{j=1}^{d+1}\dfrac{\lambda_j(\theta)c_j^2}{(\lambda_j(\theta)+\kappa(\theta))^2} + o_{\mathbb P}(1)\\
    &= \kappa(\theta)^2\sum_{j=1}^d \dfrac{\lambda_j c_j^2}{(\lambda_j+\kappa(\theta))^2} + \kappa^2\frac{\theta\sigma^2(\theta^{-1/2})^2}{(\theta\sigma^2 + \kappa(\theta))^2} + o_{\mathbb P}(1)\\
    &= \kappa(\theta)^2\sum_{j=1}^d \dfrac{\lambda_j c_j^2}{(\lambda_j+\kappa(\theta))^2} + \frac{\sigma^2}{(\theta\sigma^2/\kappa(\theta) + 1)^2} + o_{\mathbb P}(1),
    \end{split}
    \label{eq:wizard}
\end{equation}
In the limit $\theta\to 0^+$, the second term in the rightmost side of \eqref{eq:wizard} tends to $\sigma^2$. As, for the second term, let $\kappa(0^+) := \lim_{\theta\to 0^+}\kappa(\theta)$. By definition, one has
$$
1 = \frac{\lambda}{\kappa(\theta)} + \frac{1}{n}\sum_{j=1}^d\frac{\lambda_j}{\lambda_j + \kappa(\theta)} + \frac{1}{n}\frac{\theta\sigma^2}{\theta\sigma^2 + \kappa(\theta)} \overset{\theta\to 0^+}{\longrightarrow} \frac{\lambda}{\kappa(0^+)} + \frac{1}{n}\sum_{j=1}^d\frac{\lambda_j}{\lambda_j + \kappa(0^+)},
$$
and we deduce that $\kappa(0^+) = \kappa$, by Definition \ref{df:kappa}. Thus, in the limit $\theta \to 0^+$, the second term in \eqref{eq:wizard} simplifies to
\begin{equation}
    \begin{split}
    \kappa^2\sum_{j=1}^d \dfrac{\lambda_j c_j^2}{(\lambda_j+\kappa)^2} &\asymp \kappa^2\sum_{j=1}^{j^\star}\frac{c_j^2}{\lambda_j} + \sum_{j=j^\star}^d \lambda_jc_j^2 = \kappa^2\sum_{j=1}^{j^\star}j^{1+\gamma-\delta} + \sum_{j=j^\star}^d j^{-1-\gamma-\delta}\\
    &\asymp \kappa^2\int_1^{j^\star} t^{1+\gamma-\delta}\dv t + \int_{j^\star}^d t^{-1-\gamma-\delta}\dv t \asymp \kappa^2 (j^\star)^{2+\gamma-\delta} + (j^\star)^{-\gamma-\delta}\\
    &\asymp \kappa^{2-1-(1-\delta)/(1+\gamma)} + \kappa^{(\gamma+\delta)/(1+\gamma)} \asymp  \kappa^\alpha,
    \end{split}
\end{equation}
where $\alpha := (\delta + \gamma)/(1+\gamma) \in (0,1)$.
We have thus proved the following result.
\begin{restatable}{prop}{}
For any $\lambda \ge 0$, it holds under Assumption \ref{ass:powerlaws} that \begin{eqnarray} 
E(\widehat w(\lambda,n)) \asymp \kappa(\lambda,n)^\alpha + \sigma^2 + o_{\mathbb P}(1).
\end{eqnarray}
where $\alpha := (\delta+\gamma)/(1+\gamma) \in (0,1)$. In particular, $\lim_{\lambda \to 0^+}E(\widehat w(\lambda,n)) = 1/n^{(\delta+\gamma)} + \sigma^2 + o_{\mathbb P}(1)$.
\end{restatable}


% \paragraph{Variance term: ridgeless case.}
% The variance of the generalization error of the ridge estimator $\widehat w(\lambda,n)$ is given for $\lambda \to 0^+$ and $n \ge d + 2$ by
% \begin{equation*}
%     \begin{split}
%     \lim_{\lambda\to 0^+}Var (\widehat w(\lambda,n)) &= \epsilon^\top X\widehat\Sigma^{-1}\Sigma\widehat\Sigma^{-1}X^\top \epsilon/n^2 = \frac{\sigma^2}{n}\trace (\Sigma \widehat \Sigma^{-1})  + o_{\mathbb P}(1) \\
%      &=  \sigma^2 \frac{d}{n-d-1}\trace(\Sigma\Sigma^{-1}) + o_{\mathbb P}(1) \asymp  \sigma^2d \cdot \frac{d/n }{1-d/n} + o_{\mathbb P}(1). 
%     \end{split}
% \end{equation*}
 
% \paragraph{Variance term: ridgeful case.}
% Let $X/n = USW^\top$ be the SVD of $X/n$.
% \begin{restatable}[Correlated noise]{assume}{}
% Suppose the noise vector $\epsilon \in \mathbb R^n$ is such that $X^\top \epsilon/$, with $z \sim N(0,D)$.
% \end{restatable}
% Under the above assumption, one computes
% \begin{equation}
%     \begin{split}
%     Var(\widehat w(\lambda,n)) = \epsilon^\top X(\widehat\Sigma + \lambda I_d)^{-1}\Sigma(\widehat\Sigma + \lambda I_d)^{-1} X^\top \epsilon/n^2 
%     \end{split}
% \end{equation}
\subsection{Dynamics of Adversarial Risk}
The squared Euclidean norm of the ridge estimator $\widehat w(\lambda,n)$ is given by
\begin{equation}
    \begin{split}
    \|\widehat w(\lambda,n)\|^2_2 &= w_0^\top\widehat\Sigma^2(\widehat\Sigma + \lambda I_d)^{-2}w_0 = w_0^\top \Sigma^2(\Sigma + \kappa I_d)^{-2}w_0 + o_{\mathbb P}(1),\text{ thanks to \eqref{eq:hype2}}\\
    &= \sum_{j=1}^d \frac{\lambda_j^2 c_j^2}{(\lambda_j+\kappa)^2} + o_{\mathbb P}(1) \asymp \sum_{j=1}^{j^\star} c_j^2 + \frac{1}{\kappa^2}\sum_{j=j^\star}^d \lambda_j^2 c_j^2 + o_{\mathbb P}(1)\\
    &\asymp \int_1^{j^\star}t^{-\delta}\dv t + \frac{1}{\kappa^2}\int_{j^\star}^d t^{-2-2\gamma-\delta}\dv t + o_{\mathbb P}(1)\\
    &\asymp (j^\star)^{1-\delta} + \frac{1}{\kappa^2}(j^\star)^{-1-2\gamma-\delta} + o_{\mathbb P}(1) \asymp (j^\star)^{1-\delta} + o_{\mathbb P}(1)\\
    &\asymp \kappa^{-(1-\delta)/(1+\gamma)} + \kappa^{-2+(1+2\gamma+\delta)/(1+\gamma)} + o_{\mathbb P}(1)\\
    &\asymp \kappa^{-(1+\delta)/(1+\gamma)} + o_{\mathbb P}(1).
    \end{split}
\end{equation}
We have thus proved the following result.
\begin{restatable}{prop}{}
For any $\lambda \ge 0$, it holds under Assumption \ref{ass:powerlaws} that
\begin{equation}
    \|\widehat w(\lambda,n)\|^2_2 \asymp \kappa(\lambda,n)^{-\beta} + o_{\mathbb P}(1),
\end{equation}
where $\beta := (1+\delta) / (1+\gamma) \in (1,2)$.
\end{restatable}
\begin{restatable}{rmk}{}
Interestingly, note that if $\kappa(\lambda,n) \to 0$ (which is what happens in the ridgeless case, because we can show via \eqref{eq:hype1} that the derivative of $\kappa(\lambda,n)$ w.r.t $\lambda$ is at least $1$ for any $\lambda > 0$), one has
\begin{eqnarray}
E(\widehat w(\lambda,n) ) \to \sigma^2,\text{ while } \|\widehat w(\lambda,n)\|_2^2 \to \infty,\text{ even  though }\|w_0\|_2^2 = \sum_{1 \le j \le d}j^{-1-\gamma} \le \zeta(1+\gamma)  < \infty.
\end{eqnarray}
\end{restatable}

\subsection{The Proof}
We are no in shape to proof Theorem \ref{thm:Epower}.
\begin{proof}[Proof of Theorem \ref{thm:Epower}]
Indeed, thanks to the preceding two propositions, and the fact that
$$
E^{\|\cdot\|_2}(\widehat w(\lambda,n),w_0,r) \asymp (\sqrt{E(\widehat w(\lambda,n))}+r\|\widehat w(\lambda,n)\|_2)^2,
$$
the claimed identity \eqref{eq:Escaling} holds.
\end{proof}

==> early-stopped adversarial training/sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
\paragraph{Notations.}
Let us introduce some basic notations. Additional technical notations are provided in the appendix.

$[d]$ denotes the set of integers from $1$ to $d$ inclusive. The maximum (resp. minimum) of two real numbers $a$ and $b$ will be denoted $a \lor b$ (resp. $a \land b$). The operator norm of a matrix $A$ is denoted $\|A\|_{op}$ and corresponds to the positive square-root of the largest eigenvalue of $AA^\top$. Given a positive-definite (p.d.) matrix $S \in \mathbb R^{d \times d}$ and a vector $w \in \mathbb R^d$, the Mahalanobis norm of $w$ induced by $S$ is defined by $\|w\|_S := \sqrt{w^\top S w}$.  We denote respectively $M_d(\mathbb R)$ and $\mathcal S_d^{++}(\mathbb R)$ the set of $d\times d$ matrices and positive-definite matrices. Given $p \in [1,\infty]$, its harmonic conjugate, denoted $q(p)$ is the unique $q \in [1,\infty]$ such that $1/p+1/q=1$. 
% For example, $1$ and $\infty$ are harmonic conjugates of one another, while $2$ is its own harmonic conjugate. 
% The orthogonal projection operator onto a closed convex subset of $\mathbb R^d$ is denoted $\mbox{proj}_C$.
% The indicator function of a subset $C$ of $\mathbb R^d$ is the function $i_C:\mathbb R^d \to (-\infty,\infty]$, defined by $\sigma_C(x) = 0$ if $x \in C$, and $\sigma_C(x) = \infty$ otherwise.
% The dual $\|\cdot\|_\star$ of a norm $\|\cdot\|$ on $\mathbb R^d$, denoted $\|\cdot\|_\star$, is the norm defined by
% \begin{eqnarray}
% \|w\|_\star := \sup_{z \in % B^d_{\|\cdot\|}}z^\top w,
% \end{eqnarray}
% Thus, $\|\cdot\|_\star$ and $\|\cdot\|$ are support functions of one another.
For a given norm $\Vert\cdot\Vert$, we denote $\|\cdot\|_\star$ its dual norm, defined by
\begin{eqnarray}
 \|w\|_\star := \sup\{x^\top w \mid x  \in \mathbb R^d,\,\|x\| \le 1\},
\end{eqnarray}
Note that if the norm $\|\cdot\|$ is an $\ell_p$-norm for some $p \in [1,\infty]$, then the dual norm is the $\ell_q$-norm, where $q$ is the harmonic conjugate of $p$. For example, the dual of the euclidean norm (corresponding to $p=2$) is the euclidean norm itself, while the dual of the usual $\ell_\infty$-norm is the $\ell_1$-norm.

The unit-ball for a norm $\|\cdot\|$ is denoted $B_{\|\cdot\|}^d$, and defined by $B_{\|\cdot\|}^d := \{x \in \mathbb R^d \mid \|x\| \le 1\}$.
% When $\|\cdot\|$ is an $\ell_p$-norm, we write $B_p^d$ for $B_{\|\cdot\|_p}^d$.
Given any $s \ge 0$, set of $s$-sparse vectors in $\mathbb R^d$ is denoted $B_0^d$ and defined by
\begin{eqnarray}
\label{eq-sparse-ball}
B_0^d(s) := \{w \in \mathbb R^d \mid \|w\|_0 \le s\}.
\end{eqnarray}
% Note that $B_0^d(0) = 0$ and $B_0^d(s)=\mathbb R^d$ for all $s \ge d$.
% The usual notation $\mathcal O_d(1)$ (resp. $\mathcal O_{d,\mathbb P}(1)$) is used to denote a quantity which remains bounded (resp. bounded in probability) in the limit $d \to \infty$. Likewise $o_{d}(1)$ (resp. $o_{d,\mathbb P}(1)$) denotes a quantity which goes to zero (resp. which goes to zero in probability) in the limit $d \to \infty$. As usual, the acronym "a.s" stands for \emph{almost-surely}, while "w.p $p$" stands for \emph{with probability at least $p$}.

Finally, define absolute constants $c_0:=\sqrt{2/\pi}$, $\alpha := 2/(1+c_0) \approx 1.1124$ and $\beta=1.6862$.


\subsection{Problem Setup}
\label{subsec:setup}
Fix a vector $w_0 \in \mathbb R^d$, a positive definite matrix $\Sigma$ of size $d$, and consider an i.i.d. dataset $\mathcal D_n = \{(x_1,y_1),\ldots,(x_n,y_n)\}$ of size $n$, given by
\begin{align}
\label{eq:generative}
y_i &= x_i^\top w_0 + \epsilon_i,\text{ for all }i \in [n]
\end{align}
where $x_1,\ldots,x_n$ i.i.d $\sim N(0, \Sigma)$ and $\epsilon_1,\ldots,\epsilon_n$ i.i.d $\sim N(0,\sigma_\epsilon^2)$ independent of  the $x_i$'s.
% \begin{eqnarray}
% \begin{split}
% x_1,\ldots,x_n &\overset{iid}{\sim} N(0, \Sigma),\\
% \epsilon_1,\ldots,\epsilon_n &\overset{iid}{\sim} N(0,\sigma_\epsilon^2),\text{ independent of  the }x_i\text{'s},\\
% y_i &= x_i^\top w_0 + \epsilon_i,\text{ for all }i \in [n].
% \end{split}
% \label{eq:generative}
% \end{eqnarray}
Thus, the distribution of the features is a centered multivariate Gaussian distribution with covariance matrix $\Sigma$, while $w_0$ is the generative model. $\sigma_\epsilon \ge 0$ measures the size of the noise. 
% A priori, we will not assume that $w_0$ or $\Sigma$ are known.
These assumptions on the model will be assumed along all the formal claims of the paper. We also refer to $n$ as the  \emph{sample size}, and to $d$ as the \emph{input-dimension}.

In most of our analysis, except otherwise explicitly stated,  we will consider the case of infinite-data regime $n = \infty$ --or more generally $n \gg d$, which allows us to focus on the effects inherent to the data distribution (controlled by feature covariance matrix $\Sigma$) and the inductive bias of the norm w.r.t which the attack is measured, while side-stepping issues due to finite samples and label noise. Also
note that in this infinite-data setting, label noise provably has no influence on the learned model.

% For notational simplicity, write $X:=(x_1,\ldots,x_n) \in \mathbb R^{n \times d}$ (the design matrix), $y:=(y_1,\ldots,y_n) \in \mathbb R^n$ (the response vector), and $\epsilon := (\epsilon_1,\ldots,\epsilon_n) \in \mathbb R^n$ (the noise vector).

\subsection{Adversarial Robustness Risk}
Given a linear model $w \in \mathbb R^d$, an attacker is allowed to swap a clean test point $x \sim N(0,\Sigma)$ with a corrupted version $x' = x + \delta$ thereof. The perturbation $\delta=\delta(x) \in \mathbb R^d$ is constrained to be small: this is enforced by demanding that $\|\delta\| \le r$, where $\|\cdot\|$ is a specified norm and $r \ge 0$ is the attack budget. One way to measure the performance of a linear model $w \in \mathbb R^d$ under such attacks of size $r$, is via it so-called adversarial risk~\citep{madry2017towards,Xing2021}.
\begin{restatable}{df}{}
For any $w \in \mathbb R^d$ and $r \ge 0$, define the adversarial risk of $w$ at level $r \ge 0$ as follows
\begin{eqnarray}
\label{eq:Ewrdef}
\begin{split}
E^{\|\cdot\|}(w,w_0,r) := % \sup_{T: \|T-I\|_\infty \le r} \mathbb E_{x'\sim T|_{\#}N(0,\Sigma)}(w^\top x' - x^\top w_0)^2\\
%&= 
\mathbb E_{x}\left[\sup_{\|\delta\| \le r}((x+\delta)^\top w - x^\top w_0)^2\right],
\end{split}
\end{eqnarray}
where $x \sim N(0,\Sigma)$ is a random test point.
\end{restatable}
It is clear that $r \mapsto E^{\|\cdot\|}(w,w_0,r)$ is a non-decreasing function and $E^{\|\cdot\|}(w,w_0,0)$ corresponds to the  ordinary risk of $w$, namely
\begin{eqnarray}
\label{eq-ordinary-risk}
E(w,w_0) := \mathbb E_x[(x^\top w - x^\top w_0)^2] = \|w-w_0\|_\Sigma^2.
\end{eqnarray}
% Let $\|w\|_\star := \sup_{\|z\| \le 1}z^\top w$ be the dual of the attacker's norm and $\|w\|_\Sigma := \sqrt{w^\top \Sigma w}$ be the Manhalanobis norm induced by the covariance matrix $\Sigma$.
In classical regression setting, the aim is to find $w$ which minimizes $E(w,w_0)$. In the adversarial setting studied here, the aim is to minimize $E^{\|\cdot\|}(w,w_0,r)$ for any $r \ge 0$.

We will henceforth denote by $E^{\|\cdot\|}_{opt}(w_0,r)$ the smallest possible adversarial risk of a linear model for $\|\cdot\|$-attacks of magnitude $r$, that is
\begin{eqnarray}
\label{eq:Eopt}
E^{\|\cdot\|}_{opt}(w_0,r) := \inf_{w \in \mathbb R^d} E^{\|\cdot\|}(w,w_0,r).
\end{eqnarray}

 We start with the following well-known elementary but useful lemma which proved in the supplemental. Also see \cite{Xing2021,javanmard2022precise} for the special case of Euclidean-norm attacks.
\begin{restatable}{lm}{fench}
Recall that $c_0=\sqrt{2/\pi}$, then for any $w \in \mathbb R^d$ and $r \ge 0$, it holds that
\begin{align}
\label{eq:Ewr}
\begin{aligned}
 E^{\|\cdot\|}(w,w_0,r) &= \|w-w_0\|_{\Sigma}^2+r^2\|w\|_\star^2\\
 &\quad\quad +2c_0 r\|w-w_0\|_\Sigma\|w\|_\star.
 \end{aligned}
\end{align}
\label{lm:fench}
\end{restatable}
The mysterious constant $c_0=\sqrt{2/\pi}$ in Lemma \ref{lm:fench} corresponds to the expected absolute value of a  standard Gaussian random variable. In order to obtain a robust predictor to adversarial attacks, one aims at minimizing the adversarial risk introduced in~\eqref{eq:Ewrdef}. However the objective function of the problem, even in the linear setting~\eqref{eq:Ewr}, is rather complicated to optimize due to its non-convexity.

\section{A Proxy for Adversarial Risk}
The following lemma will be one of the main workhorses in subsequent results, as it allows us to replace the adversarial risk functional $E$ with a more tractable proxy $\widetilde E$.
\begin{restatable}{lm}{sandwich}
\label{lm:sandwich}
For any $w \in \mathbb R^d$ and $r \ge 0$, it holds that
 \begin{eqnarray}
 \label{eq:sandwich0}
 E^{\|\cdot\|}(w,w_0,r) \le \widetilde E^{\|\cdot\|}(w,w_0,r) \le \alpha\cdot E^{\|\cdot\|}(w,w_0,r),
 \end{eqnarray}
 where $\alpha := 2/(1+\sqrt{2/\pi}) \approx 1.1124$~~ and
 \begin{align}
 \label{eq:Etilde}
     \widetilde E^{\|\cdot\|}(w,w_0,r) &:= (\|w-w_0\|_\Sigma+r\|w\|_\star)^2.
 \end{align}
 \end{restatable}

The result is proved in the appendix.
% The following corollary will be one of our main workhorses for obtaining near-optimal robust estimators.
Since $\alpha \approx 1.1124$, the above approximation would allow us to get rougly $90\%$-optimality in the adversarial risk by minimizing the (much simpler) proxy function $w \mapsto\widetilde{E}^{\|\cdot\|} (w,w_0,r)$ instead. This will precisely be the focus of the next sections.
% Also,
% unlike $E(w,r)$ defined previously, (the square root of) $\widetilde E(w,r)$ defines a proper measure of the distance of $w$ from $w_0$. Furthermore,
% because all norms on $\mathbb R^d$ (being a finite-dimensional Banach space) are equivalent, any consistent estimator $\widehat w_n$ of $w_\star$ will have $E(\widehat w_n,r) = o_{n,\mathbb P}(1)$. However, as we shall see, the robustness constraint might slow the rates of convergence, i.e compared to normal learning, more samples are required for robust learning.

We also denote $\widetilde E_{opt}^{\Vert\cdot\Vert}(w_0,r)$ the smallest possible value of the adversarial risk proxy $\widetilde{E}^{\|\cdot\|}(\cdot,w_0,r)$.
% , that is
% \begin{eqnarray}
% \label{eq:Etildeopt}
% \widetilde E_{opt}(w_0,r) := \inf_{w \in \mathbb R^d} \widetilde E(w,w_0,r).
% \end{eqnarray}


==> early-stopped adversarial training/sections/primal_dual.tex <==
\section{Efficient Algorithms for Attacks in General Norms}
\label{sec:algorithmic}
We propose a simple tractable estimator whose adversarial risk is optimal up to within a multiplicative constant of 1.1124. Here, we drop the assumption of infinite training data $n=\infty$. Thus, the estimators are functions of the finite-training dataset $D_n:=\{(x_1,y_1),\ldots,(x_n,y_n)\}$, generated according to \eqref{eq:generative}.
% Second we consider recently propose definition of adversarial risk under which the generative model has optimal adversarial risk, and derive the minimax optimal adversarial risk.
% Our algorithm works for any covariance matrix $\Sigma_x$ and attacker norm with tractable proximal operator.

\subsection{A Two-Stage Estimator and its Statistical Analysis}
Consider any vector $\widehat w$ which minimizes the adversarial risk proxy $w \mapsto \widetilde E^{\Vert\cdot\Vert}(w,w_0,r)$ defined in \eqref{eq:Etilde}. Note apart from its clear dependence on the generative model $w_0$, $\widetilde E^{\Vert\cdot\Vert}$ also depends on the feature covariance matrix $\Sigma$. However, we don't assume that $w_0$ nor $\Sigma$ are known before hand; it has to be estimated from the finite training dataset $\mathcal D_n$.  Thus, we propose a two-stage estimator  described below in Algorithm \ref{alg:twostage}.
\begin{algorithm}
\caption{Proposed Two-Stage Estimator.}
\label{alg:twostage}
\begin{algorithmic}[1]
    \State \textbf{Stage 1:} Compute consistent estimators $\widehat w_0$ and $\widehat \Sigma$ from $w_0$ and $\Sigma$ respectively, from the data $\mathcal D_n$.
    \State \textbf{Stage 2:} Compute $\widehat w$ which minimizes the adversarial risk proxy $w \mapsto \widetilde{E}^{\Vert\cdot\Vert}(w,w_0,r)$ defined in \eqref{eq:Etilde}. See Algorithms \ref{alg:pd} and \ref{alg:st} for implementations of this step.
\end{algorithmic}
\end{algorithm}

\textbf{Stage 1} of Algorithm \ref{alg:twostage} can be implemented using off-the-shelf estimators which adapt to the structural assumptions on $\Sigma$ and $w_0$ and $\Sigma$ (sparsity, etc.). Later, we will provide simple tractable algorithms for implementing \textbf{Stage 2}. Note that \textbf{Stage 2} implicitly requires the knowledge of the attacker-norm as it aims at minimizing $\widetilde{E}^{\Vert\cdot\Vert}$.

\begin{figure}
    \centering
    \includegraphics[width=.48\textwidth]{sections/d=200_s=10_p=inf_isotropic=False_use_oracle=False_nu=10000.png}
    \caption{Experiments with our two-stage estimator Algorithm \ref{alg:twostage}. Here, we focus on  $\ell_\infty$-norm-attacks. "1+2" means \textbf{Stage 2} of our Algorithm \ref{alg:twostage} is computed via the primal-dual algorithm (Algorithm \ref{alg:pd}), while "1+3" means it is computed via the Algorithm \ref{alg:st}. The experimental setting here is: input-dimension $d=200$; covariance matrix $\Sigma$ of the features = heterogeneous diagonal, with entries from $\mathrm{Exp}(1)$ distribution; the generative $w_0$ is $s$-sparse vector (with $s=10$), normalized so that $\|w_0\|_\Sigma^2 = 1$.
    Notice how the adversarial risk of the estimator improves with number of samples $n$, as expected. See supplemental for details.
    }
    \label{fig:algos}
\end{figure}

\subsection{Consistency of Proposed Two-Stage Estimator}
We now establish the consistency of our proposed two-stage estimator $\widehat w$ computed by Algorithm \ref{alg:twostage}.
Let $\widehat \Sigma$ be an operator-norm consistent data-driven minimax estimator for $\Sigma$, and %, over some prior class $\mathfrak S$ of covariance matrices.
% We will assume that we're either (1) in low-dimensional regime $n \gg d$ so that we can take $\widehat \Sigma = X^\top X/n$, or (2) $\Sigma$ is known to us, and so we can take $\widehat \Sigma = \Sigma$.
let $\widehat w_0$ be a consistent estimator of the generative model $w_0$.
% , over some prior class $\mathcal C_0$ for $w_0$ (e.g $s$-sparse vectors in $\mathbb R^d$).
Define error terms
\begin{eqnarray}
e_1 := % \sup_{w_0 \in \mathcal C_0}
\|\widehat w_0-w_0\|_2,\, e_2 := % \inf_{\Sigma \in \mathfrak S}
\|\widehat \Sigma-\Sigma\|_{op}.%\, e_3 := \sup_{w_0 \in \mathcal C_0}\|\widehat w_0-w_0\|_\star. 
\end{eqnarray} 
% Consistency of the estimators $\widehat w_0$ and $\widehat \Sigma$ means that $e_1,e_2 = o_{n,\mathbb P}(1)$. 
We are now ready to state the adversarial risk-consistency result for our proposed two-stage estimator (Algorithm \ref{alg:twostage}).
\begin{restatable}{thm}{stats}
\label{thm:stats}
For all $r \ge 0$, it holds that
\begin{align*}
\widetilde E_{opt}^{\Vert\cdot\Vert}(w_0,r) &\le \widetilde E^{\Vert\cdot\Vert}(\widehat w,w_0,r) \le \widetilde E_{opt}^{\Vert\cdot\Vert}(w_0,r) + \Delta,\\
E_{opt}^{\Vert\cdot\Vert}(w_0,r) &\le E^{\Vert\cdot\Vert}(\widehat w,w_0,r) \le \alpha E_{opt}^{\Vert\cdot\Vert}(w_0,r)+\Delta,
\end{align*}
where $\alpha := 2/(1+c_0) \approx 1.1124$, $\Delta = O(e_1^2 + e_2^2)$, where the hidden constant in the big-O is of order $\max(\|\Sigma\|_{op}^2, \|w_0\|_\Sigma^2)$.
\end{restatable}
% Note that in the above theorem, the second inequality follows from the first, thanks to Lemma \ref{lm:sandwich}.
Thus, our proposed two-stage estimator is robust-optimal up to within a multiplicative factor $2/(1+c_0)\approx 1.1124$, and an additive term $O(e_1^2+e_2^2)$ which is due to estimation error of $w_0$ and $\Sigma$ from training data.
Note that if we assume that the covariance matrix $\Sigma$ of the features is known, or equivalently that we have access to an unlimited supply of unlabelled data from $N(0,\Sigma)$, then we effectively have $e_2 = 0$. In this case, the statistical error of our proposed estimator $\widehat w$ is dominated by the error $e_1^2$ associated with estimating the generative model $w_0$. Under sparsity assumptions, this error term is further bounded by $\dfrac{\sigma_\epsilon^2s\log(ed/s)}{n}$ (thanks to the following well-known result), which tends to zero if the input dimension $d$ does not grow much faster than the sample size $n$.
.
\begin{restatable}[\citep{BickelSimultaneous2009,BellecSlopeMeets2018}]{prop}{}
If $1 \le s \le d/2$, then under some mild technical conditions, it holds w.h.p that
\begin{eqnarray}
\inf_{\widehat w_0}\sup_{w_0 \in B_0^d(s)} \underbrace{\|\widehat w_0-w_0\|_2}_{e_1} \asymp \sigma_\epsilon\sqrt{\frac{s\log(ed/s)}{n}}.
\end{eqnarray}
where $ B_0^d(s)$ is defined in Eq.~(\ref{eq-sparse-ball}). Moreover, the above minimax bound is attained by the square-root Lasso estimator with tuning parameter $\lambda$ given by
%\begin{eqnarray}
%\label{eq:lambdaoptlasso}
$\lambda \asymp \sqrt{\dfrac{\log(2d/s)}{n}}$.
% \end{eqnarray}
\label{prop:lassobellec}
\end{restatable}
% Thus, the generative model $w_0$ can be consistently estimated from training data under sparsity assumptions and if the input-dimension does grow too fast.

\begin{restatable}{rmk}{}
Note that, in the special case of Euclidean-norm attacks, our Theorem \ref{thm:stats} (which works for all attack norms) recovers the adversarial risk-consistency result established in \citep{Xing2021} as a special case.
\end{restatable}
% \textcolor{red}{Elvis: Include a table with precise upper-bounds under sparsity assumptions, etc.}

\subsection{Algorithm 1: Primal-Dual Algorithm}
We now device a simple primal-dual algorithm for computing the second stage of our proposed estimator (Algorithm \ref{alg:twostage}). The algorithm works for any covariance matrix $\Sigma$ and norm-attack with tractable proximal operator.

Let $\widehat w_0$ and $\widehat \Sigma$ be the estimates computed in the \textbf{Stage 1} of Algorithm \ref{alg:twostage}.
Define and $K := \widehat \Sigma^{1/2}$,
$a := K\widehat {w_0}$,
% $w^1 := \Sigma^{-1/2} w_0$,
$f(z) := \|z-a\|_2$, $g(w) := r\|w\|_\star$. Recall now that 
$\sqrt{\widetilde{E}^{\Vert\cdot\Vert}(w,w_0,r)} =  \|w-w_0\|_{\Sigma} + r\|w\|_\star$ and so for any model $w$. Then by "dualizing", we get that 
\begin{eqnarray}
\begin{split}
&\inf_{w \in \mathbb R^d} \|w-w_0\|_{\Sigma} + r\|w\|_\star= \inf_{w \in \mathbb R^d} f(Kw) + g(w)\\
&= \inf_{w \in \mathbb R^d} g(w) + \sup_{z \in \mathbb R^d} z^\top K w - f^\star(z)\\
&= \inf_{w \in \mathbb R^d}\sup_{z \in \mathbb R^d} \underbrace{z^\top K w - f^\star(z) + g(w)}_{H(w,z)},
\end{split}
\end{eqnarray}
where $f^\star$ is the Fenchel-Legendre transform of $f$.
Consider the following so-called Chambolle-Pock algorithm \citep{ChambollePock2010} for computing a saddle-point for the function $H$.

\begin{algorithm}
\caption{Primal-Dual algorithm which implements \textbf{Stage 2} of Algorithm \ref{alg:twostage}. Only one iteration is shown here.}
\label{alg:pd}
\textbf{Inputs: } $\widehat w_0, \widehat \Sigma,\eta_1,\eta_2,z^{(0)}=w^{(0)}=\mathbf{0}_d.$
\begin{algorithmic}[1]
\State $z^{(t+1)} \leftarrow  \mathrm{proj}_{B_{\|\cdot\|_2}^d}(z^{(t)} + \eta_2 \widehat\Sigma^{1/2} (u^{(t)}- \widehat w_0))$
\State $w^{(t+1)} \leftarrow \mathrm{prox}_{\eta_1r\|\cdot\|_\star}(w^{(t)}-\eta_1 \widehat\Sigma^{1/2} z^{(t+1)})$,
\State $u^{(t+1)} \leftarrow 2w^{(t+1)}-w^{(t)}$
\end{algorithmic}
\end{algorithm}
% Here, $\mbox{proj}_C:\mathbb R^d \to C$ is the orthogonal projector unto the subset $\mathbb R^d$, and $\mbox{prox}_h:\mathbb R^d \to \mathbb R^d$ is the proximal operator of the function $h:\mathbb R^d \to \mathbb R$ (See Appendix xyz for formal definition).
Here, the $\eta_k$'s are stepsizes chosen such that $\eta_1\eta_2 \|\widehat\Sigma\|_{op}^{1/2} < 1$.
The nice thing here is that the projection onto the $\ell_2$-ball (line 1) admits a simple analytic formula.
In the case of $\ell_\infty$-norm-attacks, the second line corresponds to the well-known soft-thresholding operator; etc. Refer to Figures \ref{fig:algos}~\&~\ref{fig:comparison} for empirical illustrations of the algorithm. The following convergence result follows directly from \citep{ChambollePock2010}.
\begin{restatable}{prop}{}
\label{prop:pd}
Algorithm \ref{alg:pd} converges to a stationary point $(w^{(\infty)},z^{(\infty)})$ of the $H$ at an ergodic rate $O(1/t)$.
\end{restatable}

\begin{figure}
\vspace{-0.1cm}
\centering
%\includegraphics[width=1\linewidth]{figures/comparison_xing.png}
\includegraphics[width=1\linewidth]{sections/d=100_s=10_p=2_isotropic=False_use_oracle=False_nu=10000.png}
\caption{We compare our proposed two-stage estimator given in Alg. \ref{alg:twostage} with the one proposed in~\cite{Xing2021}, in the specific setting of Euclidean attacks when varying sample size $n$ and attack strength $r$. Here, \textbf{Stage 2} of our two-stage estimator is computed via Alg. \ref{alg:pd}. Dashed and plain lines respectively represent the standard and adversarial risks.  We see that though more general, our algorithm is able to recover similar performances as \cite{Xing2021} in the special case of Euclidean attacks. %See appendix for further details.
}
\label{fig:comparison}
\vspace{-0.1cm}
\end{figure}



\input{sections/L1business}


==> early-stopped adversarial training/sections/rmt.tex <==

\section{Proof of Lemma \ref{lm:rmt}}
Recall that $G$ is and $m \times d$ random matrix with iid entries from $N(0,1)$ (where $m/d \ge \gamma > 1$), and $W_{rand} := G^\top G$.

% \rmt*
Recall that "w.h.p" (with high-probability) is used to characterize a statement which holds except for an event with probability exponentially small in $d$.

For proving the lemma, We will need the following well-known auxiliary lemmas.
\begin{restatable}{lm}{}
There exists an absolute constant $c$ such that if $z \sim N(0,I_m)$, then $\mathbb P(\|z\|_2 \le u\sqrt{m}) \le (cu)^m$, for all $u \ge 0$.
\end{restatable}
\begin{proof}
Let $\mathcal S_\epsilon$ a maximal $(\|\cdot\|_\star,\epsilon)$-net for the unit-sphere $\mathcal S_{\|\cdot\|_\star}(\mathbb R^d) := \{w \in \mathbb R^d \mid \|w\|_\star = 1\}$. By a simple volume-packing argument it is easy to see that $|\mathcal S_\epsilon| = O(3/\epsilon)^d$ for any $\epsilon \in (0,1]$. By a clear abuse of language, we will identity each element of $\mathcal S_\epsilon$ by it center $w$. We will use a classical "epsilon-net" argument to control $\lambda_{max}^{\|\cdot\|}(W_{rand})$ and $\lambda_{min}^{\|\cdot\|}(W_{rand})$ separately.

\paragraph{Step 1: Controlling $\lambda_{max}^{\|\cdot\|}(W_{rand})$.}
By compactness of the unit-sphere $\mathcal S_{\|\cdot\|_\star}(\mathbb R^d)$ and continuity of $w \mapsto \|Gw\|_2$, the exists $z \in S_{\|\cdot\|_\star}(\mathbb R^d)$ such that $\|Gz\|_2 = \sup_{\|w\|_\star=1}\|Gw\|_2$. Let $w \in \mathcal S_\epsilon$ such that $\|z-w\|_\star \le \epsilon$.
A simple computation reveals that, if $\epsilon \le 1/2$, then
\begin{eqnarray}
\sqrt{\lambda_{max}^{\|\cdot\|}(W_{rand})} = \sup_{\|w\|_\star=1}\|Gw\|_2 = \|Gz\|_2 \le \|Gw(z)\|_2 + \|G(z-w(z))\|_2 \le \sup_{w \in S_\epsilon}\|Gw\|_2 + \sqrt{\lambda_{max}^{\|\cdot\|}(W_{rand})}/2,
\end{eqnarray}
that is $\lambda_{max}^{\|\cdot\|}(W_{rand}) \le 4\sup_{w \in \mathcal S_\epsilon}\|Gw\|_2^2$.
Thus, for any $\epsilon \le 1/2$ and $s \ge 0$, we have
\begin{eqnarray}
\begin{split}
\mathbb P(\lambda_{max}^{\|\cdot\|}(W_{rand}) \ge s^2m)
% = \mathbb P(\sup_{\|w\|_\star=1}\|Gw\|_2 \ge s)
&\le \mathbb P(\sup_{w \in \mathcal S_\epsilon}\|Gw\|_2 \ge s\sqrt{m}/2)\\
&\le |\mathcal S_\epsilon|\cdot\sup_{w \in \mathcal S_\epsilon}\mathbb P(\|Gw\|_2 \ge s/2)\\
&= O(3/\epsilon)^d\cdot\sup_{w \in \mathcal S_\epsilon}\mathbb P(\|Gw\|_2 \ge s/2).
\end{split}
\end{eqnarray}
Taking $\epsilon=1/2$ gives
$$
\mathbb P(\lambda_{max}^{\|\cdot\|}(W_{rand}) \ge s^2 m) \lesssim 6^d \cdot\sup_{\|w\|_\star=1}\mathbb P(\|Gw\|_2^2 \ge s^2m/4) \lesssim 6^d\cdot \sup_{\|w\|_\star=1}e^{-csm/\|w\|_2} \le 6^d e^{-csm/\beta},
$$
where the last but one inequality is because $Gw$ is random vector in $\mathbb R^m$ with iid coordinates from $N(0,\|w\|_2^2)$. Taking $s = 8\beta/c$ ensures that the rightmost side is of order $e^{-\Omega(d)}$. We deduce that for $C_1 := s =8\beta/c$, it holds w.h.p that
\begin{eqnarray}
\lambda_{max}^{\|\cdot\|}(W_{rand}) \le C_1^2 m.
\label{eq:rmthigh}
\end{eqnarray}

\paragraph{Step 2: Controlling
$\lambda_{min}^{\|\cdot\|}(W_{rand})$.}
By compactness, there exists $z \in \mathbb R^d$ with $\|z\|_\star=1$ such that $\|Gz\|_2 = \inf_{\|w\|_\star=1}\|Gw\|_2$. Let $w \in \mathcal S_\epsilon$ such that $\|w-z\|_\star \le \epsilon$. We deduce that
\begin{eqnarray}
\begin{split}
\sqrt{\lambda_{min}^{\|\cdot\|}(W_{rand})} = \inf_{\|w\|_\star=1}\|Gw\|_2 = \|Gz\|_2 &\ge \inf_{w \in \mathcal S_\epsilon}\|Gw\|_2 - \|G(z-w)\|_2\\
&\ge \|Gw\|_2 - \|G(z-w)\|_2\\
&\ge \inf_{w \in \mathcal S_\epsilon}\|Gw\|_2-\epsilon \sqrt{\lambda_{max}^{\|\cdot\|}(W_{rand})}\\
&\ge \inf_{w \in \mathcal S_\epsilon}\|Gw\|_2 - \epsilon C_1 \sqrt{m},\text{ w.h.p.}
\end{split}
\label{eq:smintrick}
\end{eqnarray}
On the other hand, for any $\eta > 0$, we have
\begin{eqnarray}
\begin{split}
% \mathbb P(\lambda_{min}^{\|\cdot\|}(W_{rand}) \le s^2m) = \mathbb P(\inf_{\|w\|_\star=1}\|Gw\|_2 \le s\sqrt{m}) &\le
\mathbb P(\inf_{w \in \mathcal S_\epsilon}\|Gw\|_2 \le \eta \sqrt{m})
&\le (3/\epsilon)^d \cdot \sup_{w \in \mathcal S_\epsilon} \mathbb P(\|Gw\|_2 \le \eta \sqrt{m})\\
&= (3/\epsilon)^d \cdot \sup_{w \in \mathcal S_\epsilon} \mathbb P(\|Gw/\|w\|_2\|_2 \le \eta \sqrt{m}/\|w\|_2)\\
&\le (3/\epsilon)^d \cdot \sup_{\|w\|_2 = 1} \mathbb P(\|Gw\|_2 \le \eta \sqrt{m}/\beta'),\text{ Thanks to Assumption \ref{assume:coveringnumber}}\\
&\le (3/\epsilon)^d\cdot (\eta \nu / \beta')^m,
\end{split}
\label{eq:smintrick2}
\end{eqnarray}
for an absolute constant $\nu > 0$. Thus, if $\epsilon \le \eta/(2C_1)$ with $\eta < 2C_1$, we deduce from \eqref{eq:smintrick} and \eqref{eq:smintrick2} that
\begin{eqnarray}
\mathbb P(\lambda_{min}^{\|\cdot\|}(W_{rand}) \le \eta^2 m/4) \le (3/\epsilon)^d\cdot(\eta\nu/\beta')^m + e^{-cm} = (\eta\nu/\beta' \cdot (3/\epsilon)^{d/m})^m + e^{-cm} \le (\eta\nu/\beta' \cdot (3/\epsilon)^{1/\gamma})^m + e^{-cm},
\end{eqnarray}
if $m/d \ge \gamma$.
Thus, for sufficient large $\gamma$ and sufficiently small $\eta$, one has 
$\mathbb P(\lambda_{min}^{\|\cdot\|}(W_{rand}) \le \eta^2 m/4) \le e^{-c'm}$,
for some absolute constant $c'$.
We deduce that w.h.p, it holds that
\begin{eqnarray}
\lambda_{min}^{\|\cdot\|}(W_{rand}) \ge \eta^2 m/4.
\label{eq:rmtlow}
\end{eqnarray}
Combining \eqref{eq:rmthigh} and \eqref{eq:rmtlow}, we deduce that
\begin{eqnarray}
\kappa^{\|\cdot\|}(W_{rand}) := \lambda_{max}^{\|\cdot\|}(W_{rand}) / \lambda_{min}^{\|\cdot\|}(W_{rand}) \le 4C_1^2/\eta^2=:C,
\end{eqnarray}
as claimed.
\end{proof}


==> early-stopped adversarial training/sections/scaling_laws.tex <==



==> early-stopped adversarial training/sections/sec1.tex <==
\section{Introduction}
Machine learning models are highly sensitive to small perturbations known as \emph{adversarial examples}~\citep{szegedy2013intriguing}, which are often imperceptible by humans.
While various strategies such as adversarial training~\citep{madry2017towards} can mitigate this vulnerability empirically, % lack of robustness
the situation remains highly problematic for many safety-critical applications like autonomous vehicles or health, and motivates a better theoretical understanding of what mechanisms may be causing this.

From a theoretical perspective, the case of classification is rather well-understood. Indeed, the hardness of classification under test-time adversarial attacks has been crisply characterized \citep{bhagoji2019,bubeck2018}. In the special case of linear classification, explicit lower-bounds have been obtained \citep{schmidt2018,bhattacharjee2020sample}. However, the case of regression is relatively understudied. Recently, \cite{Xing2021} have initiated a theoretical study of linear regression under Euclidean attacks, where an adversary is allowed to attack the input data point at test time. The authors proposed a two-stage estimator and proved its consistency. The optimal estimator obtained in \citep{Xing2021} corresponds to a ridge shrinkage (i.e $\ell_2$ penalization).

In this paper, we consider linear regression under adversarial test-time attacks w.r.t arbitrary norms (not just Euclidean / $\ell_2$-norms as in \citep{Xing2021}), and analyze the robustness of gradient-descent (GD) along the entire optimization path. By doing so we observe that GD might fail to capture a robust predictor along its path especially in the case of non-Euclidean attacks. We propose a variant of the GD scheme where an adapted transformation on the data is performed before applying a GD scheme. This allows us to understand the effect on robustness of early-stopping strategies (not training till the end) for general attacks. Finally we design a generic algorithm able to produce a robust predictor against any norm-attacks.



\subsection{Summary of main contributions}
Our main contributions are summarized as follows.

-- \textbf{Case of gradient-descent (GD).}
In Proposition~\ref{prop:GDisOpt}, we show that early-stopped GD achieves near-optimal adversarial risk in case of Euclidean attacks. Early-stopping is crucial because the predictor obtained by running GD till the end can be arbitrarily sub-optimal in terms of adversarial risk (Proposition~\ref{prop:generative}). Contrasting with Proposition~\ref{prop:GDisOpt}, we show in Proposition~\ref{thm:GDisBadforMan} that early-stopped GD can be arbitrarily sub-optimal in the non-Euclidean case, e.g when the attacker's norm is a Mahalanobis norm. Thus, GD, along its entire optimization path, can fail to find robust model in general.

-- \textbf{An Adapted GD scheme (GD+).} We propose a modified version of GD, termed GD+, in which the dynamics
are forced to be non-uniform across different features and
exhibit different regimes where early-stopped GD+ can achieves near-optimal adversarial risk. More precisely, (i) we show that it achieves near-optimal adversarial risk in the case of Mahalanobis norm attacks (Proposition~\ref{prop:GDPlusIsGood}), (ii) we also prove that it is near-optimally robust under $\ell_p$-norm attacks as soon as the features are uncorrelated (Theorem~\ref{thm-lp-optimal}) and (iii) we study the robustness along the entire optimization path of GD+ in the case of general norm-attacks. In particular, we provide a sufficient condition on the model such that early-stopped GD+ achieves near-optimal adversarial risk under general norm-attacks in Theorem~\ref{thm:GDrocksdeterministic} and we show that when this condition is not satisfied, GD+ can be arbitrarily sub-optimal (Proposition~\ref{thm:bangbang}).

% -- \textbf{An Adapted GD scheme (GD+).} We propose a modified version of GD, termed GD+, in which the dynamics are forced to be non-uniform across different features, and show that it achieves optimal adversarial risk in the case of Mahalanobis norm attacks (Proposition~\ref{prop:GDPlusIsGood}).

% -- \textbf{Sufficient conditions for optimality of GD+.}
% Then we study the effect of whitening on robustness under general attacks as a special case of GD+. We  provide a sufficient condition on the generative model $w_0$ such that this specific GD+ achieves optimal adversarial risk in Theorem \ref{thm:GDrocksdeterministic}. We also show that when this condition fails, the whitening strategy can be arbitrarily sub-optimal (Proposition~\ref{thm:bangbang}).

% -- \textbf{Optimality under $\ell_{p}$-norm-attacks.}
% When we restrict the attacks to be $\ell_p$-attacks with $p\in[1,+\infty]$, we show in Theorem~\ref{thm-lp-optimal} that early stopped GD+ is able to reach near-optimal robustness as soon as the features are uncorrelated.

-- \textbf{A two-stage estimator for the general case.}
Finally, we propose a simple two-stage algorithm (Algorithm \ref{alg:twostage}) which works for arbitrary norm-attacks, and achieves optimal adversarial risk up to within a multiplicative constant factor in the population regime. Consistency and statistical guarantees for the proposed estimator are also provided.

==> early-stopped adversarial training/sections/sec2.tex <==
\subsection{Related Work}
The theoretical understanding of adversarial examples is now an active area of research. Below is a list of works which are most relevant to our current letter.

%-- \emph{Robustness and Accuracy Could Be Reconcilable by (Proper) Definition} \citep{Pang2022RobustnessAA}. Here, adversarial risk is defined it has the same minimizer as standard risk, namely the generative model $f_\star(x) := \mathbb E[y \mid x]$.

\cite{tsipras18} considers a specific data distribution where good accuracy implies poor robustness.
% For example, 
\citep{goldstein,saeed2018, gilmerspheres18,dohmatob19} show that for high-dimensional data distributions which have concentration property (e.g., multivariate Gaussians, distributions satisfying log-Sobolev inequalities, etc.), an imperfect classifier will admit adversarial examples. \cite{dobriban2020provable} studies tradeoffs in Gaussian mixture classification problems, highlighting the impact of class imbalance. On the other hand, \cite{closerlook2020} observed empirically that natural images are well-separated, and so locally-lipschitz classifies shouldn't suffer any kind of test error vs robustness tradeoff.

In the context of linear classification\citep{schmidt2018,bubeck2018,khim2018adversarial,yin2019rademacher,bhattacharjee2020sample,min2021curious,Karbasi2021}, established results show a clear gap between learning in ordinary and adversarial settings.
\cite{li2020} studies the dynamics of linear classification on separable data, with exponential-tail losses. The authors show that GD converges to separator of the dataset, which is minimal w.r.t to a norm which is an interpolation between the the $\ell_2$ norm (reminiscent of normal learning), and $\ell_q$-norm, where $q$ is the harmonic conjugate of the attacker's norm. \cite{Vardi2022GradientMP} showed that on two-layer neural networks, gradient-descent with exponential-tail loss function converges to weights which are vulnerable to adversarial examples.

\cite{Javanmard2020PreciseTI} study tradeoffs between ordinary and adversarial risk in linear regression, and computed exact Pareto optimal curves. \cite{javanmard2021adversarial} also revisit this tradeoff for latent models and show that this tradeoff is mitigated when the data enjoys a low-dimensional structure. \cite{dohmatob2021fundamental,hassani2022curse} study the tradeoffs between interpolation, normal risk, and adversarial risk, for finite-width over-parameterized networks with linear target functions. \cite{javanmard2022precise} investigate the effect of adversarial training on the standard and adversarial risks and derive a precise characterization of them for a class of minimax adversarially trained models.  

The work most related to ours is \citep{Xing2021} which studied minimax estimation of linear models under adversarial attacks in Euclidean norm. They showed that the optimal robust linear model is a ridge estimator whose regularization parameter is a function of the population covariance matrix $\Sigma$ and the generative linear model $w_0$. Since neither $w_0$ nor $\Sigma$ is known in practice, the authors proposed a two-stage estimator in which the first stage is consistent estimators for $w_0$ and $\Sigma$ and the second stage is solving the ridge problem. In \citep{Xing2021}, the authors cover only the case of Euclidean attacks while here, we extend the study of the adversarial risk in linear regression under general norm-attacks. More precisely, here we are interested in understanding the robustness of GD, for general attacks and along the entire optimization path. As a separate contribution, we also propose a new consistent two-stage estimator based on a "dualization" of the adversarial problem that can be applied for general attacks.


% Their work has several notable limitations
% \begin{itemize}
% \item The computation of their proposed estimator is not tractable. It relies on solving a complicated equation to find an optimal ridge penalty parameter used in constructed the estimator. The only exception is when the population covariance matrix $\Sigma$ is known to be the identity matrix.
% \item In terms of scope, the \citep{Xing2021} covers the case of Euclidean attacks.
% \end{itemize}

==> early-stopped adversarial training/sections/sec3.tex <==
 
\section{Gradient-Descent for Linear Regression}
\label{sec:gd}
% In the classical regression setting, one aims at obtaining the generative model, namely $w_0$ by simply minimizing the standard risk over the parametric family of linear functions that is:
% \begin{align*}
%     \min_{w\in\mathbb{R}^d} E(w,w_0)
% \end{align*}
While the optimization of adversarial risk can be complex, the minimization of ordinary risk can be obtained by a simple gradient-descent. When applying a vanilla gradient-descent (GD) scheme with a step-size $\eta>0$, starting at $w_\eta(0):= 0_d$ to the ordinary risk defined in~\eqref{eq-ordinary-risk}, one obtains at each iteration $t\geq 1$  the following updates:
\begin{eqnarray}
\begin{split}
    w_{\eta}(t,w_0)&:=w_{\eta}(t-1) - \eta \nabla_w E(w_{\eta}(t-1),w_0)\\
    &= (I_d - (I_d - \eta \Sigma)^{t})w_0
    \end{split}
\end{eqnarray}
This scheme can be seen as a discrete approximation of the gradient flow induced by the following ODE:
$$
\left\{
    \begin{array}{ll}
       \dot w(t) =-\Sigma(w(t) - w_0) \\
        w(0)=0_d
    \end{array}
\right.
$$
which has a closed-form solution given by 
\begin{eqnarray}
\label{eq:gdynamics}
    w(t,w_0):=(I_d - \exp(-t\Sigma))w_0.
\end{eqnarray}
Our goal is to evaluate the robustness of the predictors obtained along the gradient descent path. We consider the continuous-time GD, as the analysis of discrete-time GD is analogous due to the absence of noise: the former is an infinitely small step-size $\eta$ limit of the latter ~\citep{continuousGDAnul2019,continuousGDAnul2020}. In the following we mean by early-stopped GD, any predictor (indexed by training time, $t$) obtained along the path of the gradient flow. Observe that for such predictors one has always that
\begin{align*}
 E^{\Vert\cdot\Vert_2}(w(t,w_0),w_0,r)\geq E^{\|\cdot\|}_{opt}(w_0,r) 
\end{align*}
and so for any $t\geq 0$. In particular we will focus on the one that minimizes the adversarial risk at test time, that is $ \inf_{t \geq 0} E^{\Vert\cdot\Vert_2}(w(t,w_0),w_0,r)$. 

% In order to do so, we define for all $r\geq 0$, the adversarial risk with respect to a given norm $\Vert\cdot\Vert$ (the attacker's norm) as follows:
% \begin{align*}
%     E^{\Vert\cdot\Vert}(w,w_0,r):=\mathbb{E}_{x~\sim P_x}\left(\sup_{\Vert\delta\Vert \leq r} (w^T(x+\delta) - w_0^T x)^2\right)
% \end{align*}

\subsection{Euclidean Attacks: Almost-optimal Robustness}
\label{subsec:euclidean}
Here we consider Euclidean attacks, meaning that the attacker's norm is $\Vert\cdot\Vert=\Vert\cdot\Vert_{*}=\Vert\cdot\Vert_2$.
% Let us denote $\{v_1,\dots,v_d\}$ an orthonormal basis where $\Sigma$ can be diagonalized, $\lambda_1\geq \dots\geq \lambda_d$ the eigenvalues of $\Sigma$ and set $c_j:= w_0^\top v_j$ for all $j\in [\![1,d]\!]$. The adversarial risk associated to $w(t)$ in population can be written as
% \begin{align*}
%     E^{\Vert\cdot \Vert_2}(w(t),r)&= E_1(t) + r^2 E_2(t) + 2 r \sqrt{2/\pi} \sqrt{E_1(t)E_2(t)}\\
%     E_1(t)&:= \sum_{j=1}^d (1 - \alpha \lambda_j)^{2t} \lambda_j  c_j^2 ~~\text{and}~~\\
%     E_2(t)&:= \sum_{j=1}^d[1 - (1-\alpha\lambda_j)^{t}]^2c_j^2\; .
% \end{align*}
In the following proposition, we first characterize the non-robustness of the generative model $w_0$.
\begin{restatable}{prop}{generative}
\label{prop:generative}
If $r\leq \sqrt{2/\pi}\frac{\Vert w_0\Vert_2}{\Vert w_0\Vert_{\Sigma^{-1}}}$, then we have that
\begin{align*}
    E^{\Vert\cdot\Vert_2}(w_0,w_0,r)=  E^{\Vert\cdot\Vert_2}_{opt}(w_0,r).
\end{align*}
and as soon as $r>\sqrt{2/\pi}\frac{\Vert w_0\Vert_2}{\Vert w_0\Vert_{\Sigma^{-1}}}$, we have
\begin{align*}
     E^{\Vert\cdot\Vert_2}(w_0,w_0,r) / E^{\Vert\cdot\Vert_2}_{opt}(w_0,r)\geq \frac{r^2\Vert w_0\Vert_2^2}{\Vert w_0\Vert_{\Sigma}^2}.
\end{align*}
\end{restatable}
It is important to notice that the generative model $w_0$ can be optimal w.r.t both the standard risk $E(\cdot,w_0)$ and the adversarial risk $E^{\Vert\cdot\Vert_2}(\cdot,w_0,r)$ for Euclidean attacks as soon as $r$ is sufficiently small. However, as $r$ increases, its adversarial risk becomes arbitrarily large. Therefore, applying a GD scheme until convergence may lead to predictors which are not robust to adversarial attacks even in the Euclidean setting. In the next proposition we investigate the robustness of the predictors obtained along the path of the GD scheme $(w(t,w_0))_{t\geq 0}$ and we show that for any attack $r\geq 0$, this path contains an optimally robust predictor (up to an absolute constant $\beta:=1.6862$).
\begin{restatable}{prop}{GDisOpt}
\label{prop:GDisOpt}
The following hold:

-- If $r\leq \sqrt{2/\pi}\frac{\Vert w_0\Vert_2}{\Vert w_0\Vert_{\Sigma^{-1}}}$ or
$r\geq \sqrt{\pi/2}\frac{\Vert w_0\Vert_{\Sigma^2}}{\Vert w_0\Vert_{\Sigma}}$, then
\begin{align}
     \inf_{t \geq 0}E^{\Vert\cdot\Vert_2}(w(t,w_0),w_0,r)= E^{\Vert\cdot\Vert_2}_{opt}(w_0,r).
\end{align}

-- If $\sqrt{2/\pi}\frac{\Vert w_0\Vert_2}{\Vert w_0\Vert_{\Sigma^{-1}}} < r <\sqrt{\pi/2}\frac{\Vert w_0\Vert_{\Sigma^2}}{\Vert w_0\Vert_{\Sigma}}$, we have that
\begin{align}
     \inf_{t \geq 0}E^{\Vert\cdot\Vert_2}(w(t,w_0),w_0,r)\leq \beta E^{\Vert\cdot\Vert_2}_{opt}(w_0,r)
\end{align}
\end{restatable}
Therefore the early-stopped vanilla GD scheme is able to capture an almost-optimally robust predictor for any Euclidean attack of radius $r$ (see Figure~\ref{fig:l2-case} for an illustration).

In our proof of Proposition \ref{prop:GDisOpt}, we show that GD early-stopped at time $t$ has the same adversarial risk (up to multiplicative constant) as a ridge estimator with regularization parameter $\lambda \propto 1/t$. The result then follows from \citep{Xing2021}, where it was shown the minimizer of the adversarial risk under Euclidean attacks is a ridge estimator.
% In terms of ordinary risk, such reduction from early-stopped GD to ridge regression is now well-established \citep{continuousGDAnul2019,continuousGDAnul2020}.

\begin{figure}[h]
\vspace{-0.1cm}
\centering
\includegraphics[width=0.99\linewidth]{figures/error_l2.png}
\caption{We consider a $d=2$ dimensional case where $w_0$ and $\Sigma$ are sampled according to a Gaussian and an Exponential distributions respectively. We plot the adversarial risk under Euclidean attacks of the optimal predictor along the GD path (\textbf{GD: adv. risk}) as well as its standard risk (\textbf{GD: standard risk}) and we compare them to the risks of the optimal predictor (\textbf{Opt}) solving adversarial problem when varying the attack strength $r$.}
\label{fig:l2-case}
\vspace{-0.1cm}
\end{figure}

In the isotropic case, i.e. when $\Sigma=I_d$, early-stopped GD even achieves the exact optimal adversarial risk.
\begin{restatable}{prop}{isoexact}
\label{prop:iso-exact}
Assume that $\Sigma=I_d$, then for all $r\geq 0$, we have $\inf_{t\geq 0} E^{\Vert\cdot\Vert_2}(w(t,w_0),r) =  E^{\Vert\cdot\Vert_2}_{opt}(w_0,r)$.
\end{restatable}

However, such results are only possible when the attacks are Euclidean. In the following section, we show that vanilla GD, along its whole optimization path, can be arbitrarily sub-optimal in terms of adversarial risk for Mahalanobis Attacks.


\subsection{Mahalanobis Attacks: Sub-optimality of Gradient-Descent}
Let us consider attacks w.r.t the Mahalanobis norm induced by a symmetric positive definite matrix $B$, i.e. we consider the case where 
\begin{align*}
    \Vert \cdot \Vert = \Vert \cdot \Vert_{B}:=\Vert B^{1/2} \cdot \Vert_{2}\; .
\end{align*}
In the next proposition, we present a simple case where GD fails to be adversarially robust under such attacks.
\begin{restatable}{prop}{GDisBadforMan}
\label{thm:GDisBadforMan}
Let $d=2$, $\Sigma=I_d$ and for any integer $m \ge 1$, let us consider the following positive-definite matrix
\begin{align}
\label{eq-B-counter-example}
B=B(m)=
\begin{pmatrix}
1/m & 0\\
0 & m
\end{pmatrix}.
\end{align}
Also, consider the following choice of generative model $w_0 = w_0(m) =(1/\sqrt{m},1)$. Then, for any fixed $r>0$,
\begin{align*}
   \underset{m\xrightarrow[]{}+\infty}{\lim}\dfrac{\inf_{t\geq 0}E^{\Vert\cdot\Vert_{B}}(w(t,w_{0}),w_{0},r)}{E^{\Vert\cdot\Vert_{B}}_{opt}(w_{0},r)}=+\infty.
\end{align*}
\end{restatable}
Therefore under Mahalanobis attacks, any predictor obtained along the path of GD can be arbitrarily sub-optimal. To alleviate this issue, we propose in the next section a modified version of the vanilla GD scheme which can handle such attacks and even more general ones.

\section{An Adapted Gradient-Descent: GD+}
\label{sec:gdplus}
In fact, it is possible to obtain an almost optimally robust predictor for Mahalanobis attacks using a modified version of the GD scheme, termed GD+. Let $M\in\mathcal{M}_d(\mathbb{R})$ be an arbitrary invertible matrix. In order to build an almost-optimally robust predictor for such attacks, we propose to apply a GD scheme on a transformed version of the data. More precisely, we propose to apply a GD scheme to the following objective function:
\begin{align*}
    E_{M}(w,w_0):=\mathbb{E}_{(x,y)\sim P_{xy}}(w^\top Mx -y)^2
\end{align*}
which leads to the following optimization dynamics:
\begin{align}
\label{eq:GD+}
    w^{M}(t,w_0):= (I_d - e^{-t M \Sigma M^T})(M^{-1})^{\top}w_0.
\end{align}
% In the following, we first  the robustness of GD+ under Mahalanobis norm-attacks induced by an arbitrary symmetric positive definite matrix $B$.
% \subsection{Optimality to Mahalanobis norm-attacks}
% Here we focus on the robustness of our modified GD (GD+) under Mahalanobis norm-attacks. 
This transformation amounts to apply feature-dependent gradient steps determined by $M$ to the classical GD scheme. In the following proposition, we show that when $M$ is adapted to the attack, early-stopped GD+ is optimally robust (up to an absolute constant).
\begin{restatable}{prop}{GDPlusIsGood}
\label{prop:GDPlusIsGood}
For any $B \in \mathcal{S}_{d}^{++}(\mathbb{R})$ and $r\geq 0$,
$$\inf_{t \geq 0}E^{\Vert\cdot\Vert_{B}}(B^{1/2} w^{B^{1/2}}(t,w_0),r)\leq \beta E^{\Vert\cdot\Vert_{B}}_{opt}(r,w_0).$$
\end{restatable}
% \begin{proof}
% In fact we know that a GD on data of covariance $\Sigma$ and model $w_0$ is optimal for $\ell_2$ attacks up to $\beta$. Now remarks that by our changement of variable, we consider a GD on data of covariance $M\Sigma M^{\top}$ and model $(M^{\top})^{-1}w_0$. Then we obtain that our modified GD minimize 
% \begin{align*}
%     &\Vert w - (M^{T})^{-1}w_0\Vert_{M\Sigma M{\top}}^2 + r^2\Vert w\Vert_2^2 \\
%     &+ 2rc_0\Vert w - (M^{T})^{-1}w_0\Vert_{M\Sigma M{\top}}\Vert w\Vert_2
% \end{align*}
% however we have that:
% \begin{align*}
%   \Vert w - (M^{T})^{-1}w_0\Vert_{M\Sigma M{\top}}^2 =   \Vert M^{\top}w - w_0\Vert_{\Sigma}^2 
% \end{align*}
% and therefore, by applying again a changement of variables, we obtain that $M^{\top}w^{M}$ minimize  
% \begin{align*}
%     &\Vert w -w_0\Vert_{\Sigma}^2 + r^2\Vert (M^{T})^{-1}w\Vert_2^2 \\
%     &+ 2rc_0\Vert w - w_0\Vert_{\Sigma}\Vert  (M^{T})^{-1}\Vert_2
% \end{align*}
% Taking finally $M=B^{1/2}$ shows the result as the dual norm of $\Vert\cdot\Vert_B$ is in fact $\Vert\cdot\Vert_{B^{-1}}$.
% \end{proof}
Therefore by choosing $M=B^{1/2}$, GD+ is able to obtain near-optimality under $\Vert\cdot\Vert_{B}$-norm attack. See Figure~\ref{fig:counter-example-1} for an illustration. Note that when $B=B^{1/2}=I_d$, then $w^{I_d}(t,w_0)=w(t,w_0)$, $\Vert\cdot \Vert_{I_d} = \Vert \cdot \Vert_{2}$, and we recover as a special case our result obtained in Proposition~\ref{prop:GDisOpt}. 

% \subsection{Robustness to Mahalanobis-norm-attacks}
% Another case of interest in when $M=B^{-1/2} \Sigma B^{-1/2}$ where $B\in\mathcal{S}_{d}^{++}(\mathbb{R})$. In that case we obtain that 
% $A_{M}=B^{-1/2}$ and therefore our proposed method is optimally robust (up to an absolute constant) w.r.t to attacks in $\Vert \cdot \Vert_{B}$ for any matrix $B\in \mathcal{S}_{d}^{++}(\mathbb{R})$.

% \begin{corollary}
% For any $B \in \mathcal{S}_{d}^{++}(\mathbb{R}^d)$ and $r\geq 0$, we have
% \begin{align*}
%      \inf_{t \geq 0}E^{\Vert\cdot\Vert_{B}}(B^{-1/2} w^{B^{-1/2} \Sigma B^{-1/2}}_c(t),r)\leq 1.6862 E^{\Vert\cdot\Vert_{B}}_{opt}(r).
% \end{align*}
% \end{corollary}

% Another case of interest is when $M$ is an element of the commutant of $\Sigma$, meaning that $\SigmaM=M\Sigma$, then $A_{\Sigma M} = M^{1/2}$, and therefore our proposed GD scheme becomes almost optimally-robust w.r.t to attacks in $\Vert \cdot \Vert_{M}:=\Vert M^{1/2} \cdot \Vert_{2}$. Note also that a direct consequence of what precedes is when $\Sigma=I_d$, then our method is able to find an optimally-robust predictor w.r.t to attacks in $\Vert \cdot \Vert_{M}$ for any matrix $M$ definite positive, that is any Mahalanobis distance.
\begin{figure}[h!]
\vspace{-0.1cm}
\centering
\includegraphics[width=0.99\linewidth]{figures/counter_example_mala_m.png}
\caption{Here we plot the example studied in Proposition~\ref{thm:GDisBadforMan} for a fixed radius $r=1$ when varying $m$. \textbf{GD+} represents the modified GD scheme with $M=B^{1/2}$ where $B$ is defined in Eq.~(\ref{eq-B-counter-example}),  \textbf{GD} represent the vanilla GD and \textbf{Opt} is the optimal predictor. Observe that the optimal adversarial risk goes to $0$ as $m$ goes to $+\infty$ while the adversarial risk of the vanilla GD converges towards a constant.}
\label{fig:counter-example-1}
\vspace{-0.1cm}
\end{figure}

In the following section, we investigate the robustness of GD+ scheme on more general attacks. 

\subsection{Robustness Under General Attacks}
\label{subsec:general_attacks}
Our goal here is to provide a simple control of the adversarial risk of GD+ under general norm-attack $\Vert\cdot\Vert$. For that purpose, define the \emph{condition number} $\kappa^{\|\cdot\|}(M)$ of any matrix $M$, w.r.t to the attacker's norm $\|\cdot\|$ as
\begin{align*}
    \kappa^{\Vert\cdot\Vert}(M)&:=\lambda_{max}^{\Vert\cdot\Vert}(M)/\lambda_{min}^{\Vert\cdot\Vert}(M),\,\text{where }\\
    \lambda_{max}^{\Vert\cdot\Vert}(M)&:=\sup_{w\neq 0}\frac{\Vert M w\Vert_2}{\Vert w\Vert_*},\text{ and}\\
    \lambda_{min}^{\Vert\cdot\Vert}(M)&:=\inf_{w\neq 0}\frac{\Vert M w\Vert_2}{\Vert w\Vert_*}
\end{align*}
% then we show the following Proposition.
where dual norm $\Vert \cdot \Vert_*$ is defined with respect to the attacker-norm $\|\cdot\|$. We are now ready to show a general upper-bound of our modified GD scheme.
\begin{restatable}{prop}{geneupper}
\label{prop:gene-upper}
For any $r\geq 0$, and invertible matrix $M\in\mathcal{M}_d(\mathbb{R})$, it holds that
%\begin{align*}
$$\dfrac{\inf_{t \geq 0}E^{\Vert\cdot\Vert}(M^{\top}w^{M}(t,w_0),w_0,r)}{E^{\Vert\cdot\Vert}_{opt}(r,w_0)}\leq \beta \kappa^{\Vert\cdot\Vert}\left((M^{\top})^{-1}\right)^2.
     $$
%\end{align*}
\end{restatable}
% \begin{proof}
% Indeed recall that our modified GD scheme minimize $V_{\Vert (M^{T})^{-1}\cdot\Vert,r,w_0,\Sigma}(w)$ defined as:
% \begin{align*}
%     &\Vert w -w_0\Vert_{\Sigma}^2 + r^2\Vert (M^{T})^{-1}w\Vert_2^2 \\
%     &+ 2rc_0\Vert w - w_0\Vert_{\Sigma}\Vert  (M^{T})^{-1}\Vert_2
% \end{align*}
% Now observe that for all $w$
% \begin{align*}
%   \lambda_{min}^{\Vert\cdot\Vert}((M^{T})^{-1}) \Vert w\Vert_{*}\leq \Vert (M^{T})^{-1}w\Vert_2 \leq  \lambda_{max}^{\Vert\cdot\Vert}((M^{T})^{-1}) \Vert w\Vert_{*}
% \end{align*}
% Therefore we obtain that
% \begin{align*}
%     \inf_t  V_{\Vert \cdot\Vert_{*},r,w_0,\Sigma}(w(t))
%     &\leq  \inf_t V_{\Vert (M^{T})^{-1}\cdot\Vert,r/\lambda_{min}^{\Vert\cdot\Vert}((M^{T})^{-1}),w_0,\Sigma}(w)\\
%     &\leq \beta  \inf_w V_{\Vert (M^{T})^{-1}\cdot\Vert,r/\lambda_{min}^{\Vert\cdot\Vert}((M^{T})^{-1}),w_0,\Sigma}(w)\\
%     &\leq \beta \inf_w  V_{\Vert \cdot\Vert_{*},r\kappa^{\Vert\cdot\Vert}(((M^{T})^{-1})),w_0,\Sigma}(w)\\
%     &\leq \beta\kappa^{\Vert\cdot\Vert}(((M^{T})^{-1}))^2 \inf_w  V_{\Vert \cdot\Vert_{*},r,w_0,\Sigma}(w)
% \end{align*}
% \end{proof}
Therefore along the path of GD+ induced by $M$, one can find a $\beta \kappa^{\Vert\cdot\Vert}((M^{\top})^{-1})^2$-optimally robust predictor against $\Vert\cdot\Vert$-attack. In particular, observe that when $M=B^{1/2}$, and $\Vert\cdot\Vert=\Vert\cdot\Vert_{B}$, we obtain that $\kappa^{\Vert\cdot\Vert}((M^{\top})^{-1})=1$ and we recover as a special case the result of Proposition~\ref{prop:GDPlusIsGood}.

\begin{restatable}{rmk}{}
It is important to notice that $M$ can be chosen arbitrarily, and therefore adapted to the norm of the attacks such that $M\to \kappa^{\Vert\cdot\Vert}((M^{\top})^{-1})$ is minimized. However, minimizing this quantity in general is hard due to the arbitrary choice of the norm $\Vert\cdot\Vert$. 
\end{restatable}

In the next section, we study a specific case of GD+ and provide a sufficient condition on the model $w_0$ such that this scheme is near-optimal under general norm-attacks. 


\subsection{A Sufficient Condition for Optimality}
\label{subsec:sufficientGD}
We consider the general case of an arbitrary norm-attack $\|\cdot\|$ with dual $\|\cdot\|_\star$ and we focus on a very specific path induced GD+, which is  when $M=\Sigma^{-1/2}$. In that case, data are normalized and the path drawn by $(M w^{M}(t,w_0))_{t\geq 0}$ is in fact a uniform shrinkage of the generative model. More precisely, the predictors obtained along such a path are exactly the one in the chord $[0,w_0]:=\left\{\gamma w_0 \mid \gamma\in[0,1]\right\}$. In particular, the optimal adversarial risk achieved by this modified GD scheme is given by
\begin{eqnarray}
\begin{split}
    &\inf_{t\geq 0}E^{\Vert\cdot\Vert}(\Sigma^{-1/2} w^{\Sigma^{-1/2}}(t,w_0),w_0,r)\\&\quad\quad=\inf_{\gamma\in[0,1]} E^{\Vert\cdot\Vert}(\gamma w_0,w_0,r)
    % =:E_{shrink}^{\Vert\cdot\Vert}(w_0,r).
    \end{split}
 \end{eqnarray}

Let $g(w_0) \in \mathbb R^d$ be a subgradient of $\Vert\cdot\Vert_\star$ at $w_0$. For example, in the case of $\ell_\infty$-norm-attacks, one may take $g(w_0) = (\mbox{\sign}(w_{0,1}),\ldots,\mbox{sign}(w_{0,d}))$, with $\mbox{sign}(0) := 0$.
In the case of of a Mahalanobis attack where $\|\cdot\| = \|\cdot\|_B$ for some positive-definite matrix $B$, one can take $g(w_0) =B^{1/2}w_0/\|w_0\|_B$ with $g(0) = 0$. 
% For example, in the case of $\ell_\infty$-norm-attacks, we have $\lambda \geq 1/ \sqrt{\text{Trace}(\Sigma^{-1})}$; In the case of euclidean attacks, we have $\lambda\geq\sqrt{\lambda_{min}^{\Vert\cdot\Vert_2}(\Sigma)}$ and more gerenarlly, for Mahalanobis attacks where $\|\cdot\| = \|\cdot\|_B$ with $B$ a positive-definite matrix, we have that $\lambda\geq \sqrt{\lambda_{min}^{\Vert\cdot\Vert_2}(B^{1/2}\Sigma^{1/2}B^{1/2})}$ can be taken.
We can now state our sufficient condition for near-optimality of GD+.
\begin{restatable}{cond}{}
The subgradient $g(w_0) \in \mathbb R^d $ can be chosen such that  
\begin{align*}
    \dfrac{\|g(w_0)\| \|w_0\|_*}{\|g(w_0)\|_{\Sigma^{-1}} \|w_0\|_{\Sigma}}\geq c,
\end{align*}
 where   $c$ is a positive absolute constant. 
\label{cond:dense}
\end{restatable}

The above condition is sufficient in order to obtain near-optimality of GD+ as we show in the next proposition~(see Figure~\ref{fig:sufficient} for an illustration).
\begin{restatable}{thm}{GDrocksdeterministic}
Suppose Condition \ref{cond:dense} is in order. Then, for any positive $r$, it holds for $M=\Sigma^{-1}$ that
\begin{eqnarray*}
\begin{split}
\dfrac{\inf_{t \geq 0}E^{\Vert\cdot\Vert}(M^{\top}w^{M}(t,w_0),w_0,r)}{E^{\Vert\cdot\Vert}_{opt}(r,w_0)}\le (1 \lor 1/c^2)\alpha.
\end{split}
\end{eqnarray*}
\label{thm:GDrocksdeterministic}
\end{restatable}
In particular, for the case of $\ell_\infty$-norm-attacks, we have the following corollary.
\begin{restatable}{cor}{}
Consider the case where $\ell_\infty$-norm-attacks. If there exists an absolute constant $c>0$ such that $\|w_0\|_1 \ge c \sqrt{d}\|w_0\|_2$, then with $M=\Sigma^{-1}$ it holds that 
\begin{eqnarray*}
\begin{split}
\dfrac{\inf_{t \geq 0}E^{\Vert\cdot\Vert_\infty}(M^{\top}w^{M}(t,w_0),w_0,r)}{E^{\Vert\cdot\Vert_\infty}_{opt}(r,w_0)}  \le \left(1 \lor \frac{\kappa^{\Vert\cdot\Vert_2}(\Sigma)}{c^2}\right)\alpha.
\end{split}
\end{eqnarray*}
\label{coro-sufficient}
\end{restatable}
For example, when $w_0=(1,\ldots,1)$ --or equivalently, random $w_0 \sim N(0,I_d)$, one can take $c=1$, and observe that $\|w_0\|_1 \gtrsim d$, $\|w_0\|_2 \asymp \sqrt{d}$, and so the bound in Corollary \ref{coro-sufficient} holds.

\begin{figure}[t!]
\centering
\includegraphics[width=0.99\linewidth]{figures/sufficient_cond.png}
\caption{We consider the case exhibited in the Corollary~\ref{coro-sufficient} when $d=2$, $\Sigma=I_d$ and $w_0=(1,1)$ under $\ell_{\infty}$-attacks. We plot the adversarial as well as the standard risks for both the optimal shrinkage predictor as well as the optimal predictor of the adversarial risk when varying $r$.}
\label{fig:sufficient}
\vspace{-0.1cm}
\end{figure}
The  Condition~\ref{cond:dense} that ensures optimality of GD+ in Theorem \ref{coro-sufficient} cannot be removed. Indeed, we exhibit a simple case where the uniform shrinkage strategy fails miserably to find robust models even when they exist. 
\begin{restatable}{prop}{bangbang}
Let $\Sigma = I_d$, then it is possible to construct $w_0 \in \mathbb R^d$ and $r > 0$ such that in the limit $d \to \infty$, it holds that $r \to 0,\,r\sqrt d \to +\infty$, and
\begin{align*}
 \dfrac{\inf_{t \geq 0}E^{\Vert\cdot\Vert_\infty}( w (t,w_0),w_0,r)}{E^{\Vert\cdot\Vert_\infty}_{opt}(r,w_0)} \to +\infty.
\end{align*}
\label{thm:bangbang}
\end{restatable}
% \begin{proof}
% Let $a,\lambda>0$, $w_0:=(a+\lambda,\dots,a+\lambda,\lambda,\dots,\lambda)$ and let $\alpha\geq 1$ be the number of coordinate such that $w_{0,i}=a+\lambda$. Concrete values for $a$, $\lambda$, and $\alpha$ will be prescribed later. For such model we obtain that
% \begin{align*}
%     \Vert w_0\Vert_1 &= d\lambda + \alpha a~~\text{and}\\
%      \Vert w_0\Vert_2 &=\sqrt{\alpha(a+\lambda)^2 + (d-\alpha) \lambda^2}\\
%      &= \sqrt{\alpha a^2 + d \lambda^2 + 2\alpha a \lambda}.
% \end{align*}
% Therefore the shrinkage model obtains an error equals to:
% \begin{align*}
%     E_{rescale}(w_0,r)=\min(\alpha a^2 + d \lambda^2 + 2\alpha a \lambda, r^2( d\lambda + \alpha a)^2).
% \end{align*}
% Now let $w:=(\underbrace{a,\dots,a}_{\alpha\text{ times}},0,\dots,0)$, we obtain that
% \begin{align*}
%     \sqrt{E_{opt}(w_0,r)}\leq \Vert w - w_0\Vert_2 + r\Vert w\Vert_1=\sqrt{d}\lambda + r\alpha a
% \end{align*}
% Let us now consider the case where \begin{eqnarray}
% r=\lambda=\frac{1}{d^{1/4}\log d},\, 
% \alpha = d^{1/2},\, a=1.
% \end{eqnarray}
% Then, for large $d$ we obtain that
% \begin{align}
% &\Vert w - w_0\Vert_2 + r\Vert w\Vert_1\asymp \frac{d^{1/4}}{\log d}\\
%   &r\Vert w_0\Vert_1 \asymp  \frac{d^{1/2}}{(\log d)^2},\,\Vert w_0\Vert_2 \asymp d^{1/4}
% \end{align}
% from which follows that
% \begin{align*}
%     \frac{E_{rescale}(w_0,r)}{E_{opt}(w_0,r)}\geq \frac{\min(d^{1/2},\frac{d}{(\log d)^4})}{\frac{d^{1/2}}{(\log d)^2}}\asymp (\log d)^2\rightarrow +\infty,
% \end{align*}
% as claimed.
% \end{proof}
% \begin{mdframed}
% Here are the real assumptions of my proof: indeed if we have that
% \begin{align*}
%   \alpha\rightarrow+\infty,~~r\sqrt{d}\rightarrow+\infty,~~r\sqrt{\alpha}&\rightarrow 0, ~~\frac{ a}{\lambda}\asymp\frac{\sqrt{d}}{r\alpha}
% \end{align*}
% Then the result holds. 

% \textcolor{red}{Elvis: In fact one can show that the condition $r \to 0$ is not removable. Indeed, for any $w_0$ and \emph{fixed} $r$, one has
% $E_{rescale}(w_0,r)/E_{opt}(w_0,r) \le \max(1,r)/\min(1,r)$ which cannot turn to $\infty$ in the limit $d \to \infty$.
% }
% \end{mdframed}
Therefore the uniform shrinkage strategy induced by GD+ (which here reduces to vanilla GD since $\Sigma=I_d$) is not adapted for all scenarios; it may fail to find a robust model even when one exists. 

In the next section, we restrict ourselves to the case of $\ell_{p}$-norm-attacks for $p\in[1,+\infty]$ and show that GD+ is able to reach optimal robustness as soon as the data has uncorrelated features.

\subsection{Optimality Under $\ell_{p}$-norm Attacks}
Now, let $p\in[1,+\infty]$ and consider attacks w.r.t the  
 $\ell_p$-norm, i.e the attack strength is measured w.r.t the norm $\Vert\cdot\Vert=\Vert\cdot\Vert_{p}$, with dual norm $\Vert\cdot\Vert_\star=\Vert\cdot\Vert_{q}$, where $q \in [1,+\infty]$ is the harmonic conjugate of $p$. Popular examples in the literature are $p=2$ (corresponding to Euclidean attacks, considered in Section \ref{subsec:euclidean}) and $p=\infty$. In this section we assume that $\Sigma$ is a diagonal positive-definite matrix. This assumption translates the fact that, both norm $\Vert\cdot\Vert_{\Sigma}$ and $\Vert\cdot\Vert_q$ act on the same coordinates system. When these two norms are aligned, we show in the next theorem that the the minimiser of the proxy introduced in Eq.~(\ref{eq:Etilde}) is in fact a non-uniform shrinkage of $w_0$ which can be recovered by GD+. An illustration of the result is provided in Figure~\ref{fig:l1-attack-gene}.
% under this assumption we show in the next Theorem that in fact our modified GD scheme is able to recover this non-uniform shrinkage, and therefore be near-optimal.
\begin{restatable}{thm}{lpoptimal}
\label{thm-lp-optimal}
Let $\Sigma$ be any definite positive diagonal matrix and $p\in [1,+\infty]$, then we have
\begin{align*}
    \inf_{M\in\mathcal{M}_d(\mathbb{R}),t\geq 0} \frac{E^{\Vert\cdot\Vert_p}(M^{\top}w^{M}(t,w_0),w_0,r)}{E^{\Vert\cdot\Vert_p}_{opt}(r,w_0)}\leq \alpha.
\end{align*}
\end{restatable}
Therefore GD+ is able to reach near-optimality in term of adversarial risk, and so for any $\ell_p$-attacks with $p\in[1,+\infty]$ as soon as $\Vert\cdot\Vert_p$ and $\Vert\cdot\Vert_{\Sigma}$ are aligned. 

\begin{figure}[h!]
\vspace{-0.1cm}
\centering
\includegraphics[width=0.99\linewidth]{figures/l1_attack_gene.png}
\caption{We consider the case where $d=2$, $\Sigma$ is diagonal and  $w_0$ and the diagonal coefficients of $\Sigma$ are sampled according to a Gaussian and an exponential distribution respectively. The choice of $M$ is obtained by fine-tuning the GD+. We compare the adversarial and standard risks under $\ell_{\infty}$ of the optimal predictor in the GD+ path with those of the optimally robust predictor when varying the radius $r$.}
\label{fig:l1-attack-gene}
\vspace{-0.1cm}
\end{figure}

Applying a GD+ scheme in practice might be difficult for general attacks, as the choice of the transformation $M$ must be adapted accordingly. To alleviate this issue, we propose in the next section a simple and tractable two-stage estimator able to reach near-optimality and so for general attack.

% \section{Optimal Estimators in Case of General Attacks}
% \textcolor{red}{Elvis: This section is becoming more and more orphaned. Parts of it should be absorbed elsewhere, and the rest should be dumped.}
% Let $\Sigma$ be a diagonal definite positive matrix. We begin with the following useful lemma.
% \begin{restatable}{lm}{}
% Given an extended-value convex function (EVCF) $g:\mathbb R^d \to (-\infty,\infty]$, every minimizer of the EVCF $g_a:\mathbb R^d \to (-\infty,\infty]$ defined by $g_a(x) := \|x-a\|_\Sigma + g(x)$ can be written as $x=\Sigma^{-1/2}\mbox{prox}_{tg(\Sigma^{-1/2}\cdot)}(\Sigma^{1/2}a)$, for some $t \in [0,\infty]$.
% \label{lm:subdifferential}
% \end{restatable}
% % In the above, we use the notation
% % $$
% % \mbox{prox}_{\Lambda,h}(a) := (1/2)\arg\min_x \|x-a\|_\Lambda^2 + h(x),
% % $$
% % i.e the proximal operator of $h$ w.r.t to the Bregman divergence $D(z,z') := (1/2)\|z-z'\|_\Lambda^2$.
% \begin{proof}
% For every $x \in \mathbb R^d$, set $t = t(x):=\|x - a\|_{\Sigma}$. Note that  by first-order optimality conditions, $x$ is a minimizer of $g_a$ iff $0 \in \partial g_a(x)$ iff $0 \in \Lambda(x-a)/t + \partial g(x)$ iff $0 \in (x-a) +  t\Lambda^{-1}\partial g(x)$ iff $x = (I+t\Lambda^{-1} \partial g)^{-1} (a) = \mbox{prox}_{\Lambda,t g}(a)$, by definition of the proximal operator.
% \end{proof}
% In the above proof, we have used the fact that $\partial g$ is a maximal monotone operator (a result of Rockafellar from the 70's \citep{rtmaxmon}), so that $(I+t \Sigma^{-1} \partial g)^{-1}(a)$ is well-defined and single-value.

% \subsection{Bounds for General Attacks}
% \lorem

% Let us denote the commutant of $\Sigma$
% \begin{align*}
%     \mathcal{C}(\Sigma):=\{M\in\mathcal{S}_{d}^{++}(\mathbb{R})~~\text{s.t.}~~\Sigma M = M\Sigma\}\; ,
% \end{align*}
% For any $M\in \mathcal{C}(\Sigma)$, let us consider attacks w.r.t to the norm induced by $M$, i.e. we consider the case where
% \begin{align*}
%     \Vert \cdot \Vert = \Vert \cdot \Vert_{M}:=\Vert M^{1/2} \cdot \Vert_{2}\; .
% \end{align*}
% In order to build an almost-optimally robust predictor to $\Vert \cdot \Vert_{M}$- attacks, we propose to apply a GD scheme on a transformed version of the data. More precisely, we propose to apply to a GD scheme to the following objective function:
% \begin{align*}
%     E_{M}(w):=\mathbb{E}_{(x,y)\sim P_{xy}}(w^T(M^{1/2}x)-y)^2
% \end{align*}
% which leads to the following GD path:
% \begin{align*}
%     w^{M}(t):= (I_d - (I_d - \alpha M\Sigma)^t)M^{-1/2}w_0\; , 
% \end{align*}
% and its continuous version:
% \begin{align*}
%     w^{M}_c(t):= (I_d - e^{-t M\Sigma}) M^{-1/2}w_0\;.
% \end{align*}
% %\textcolor{red}{Elvis: I think you should replace $M\Sigma$ by the symmetric positive-definite matrix $M^{1/2}\Sigma M^{1/2}$ in the above formulae an everywhere hereafter. This should remove the need to consider commutators of $\Sigma$, etc.}
% Note that $w(t)= w^{I_d}_c(t)$ and $w(t)= w^{I_d}(t)$. We are now ready to show our generalization of the $\ell_2$-case on the robustness of the GD scheme.
% \begin{prop}
% For any $M \in \mathcal C(\Sigma)$ and $r\geq 0$, we have
% \begin{align*}
%      \inf_{t \geq 0}E^{\Vert\cdot\Vert_M}(M^{1/2} w^{M}_c(t),r)\leq 1.6862 E^{\Vert\cdot\Vert_M}_{opt}(r).
% \end{align*}
% \end{prop}
% Therefore for any $r\geq 0$, there exists an optimally robust predictor against $\Vert\cdot\Vert_M$-attacks along the path drawn by the GD scheme on the transformed data, namely $((M^{1/2} w^{M}_c(t))_{t\geq 0}$. In the following section, we investigate the robustness of the GD scheme on general attacks.

% \subsection{Case of Euclidean Attacks}
% Applying Lemma \ref{lm:subdifferential} with $a=w_0$ and $g:=r\|\cdot\|_2$, we obtain that the minimize of $w \mapsto \|w-w_0\|_\Sigma + r\|\cdot\|_2$ is of the form $w(t)$, for some $t \in [0,\infty]$, where
% \begin{eqnarray*}
% \begin{split}
% w(t) &= (I+t\Lambda^{-1}\partial \|\cdot\|_2)^{-1}(w_0),\text{ i.e}\\
% w_0 &=
% w(t) + t\Lambda^{-1} w(t)/\|w(t)\|_2,\,w(\infty)=w_0.
% \end{split}
% \end{eqnarray*}
% Fixing $t/\|w(t)\|_2 = \lambda = 1/\eta$, we obtain
% \begin{eqnarray}
% w(\eta) = (\Lambda + \lambda I_d)^{-1}\Lambda w_0 = (\eta\Lambda + I_d)^{-1}\eta\Lambda w_0,
% \end{eqnarray}
% which is a ridge, and we recover the result from \citep{Xing2021}. However, unlike the case of $\ell_\infty$-norm-attacks obtaining the optimal value for $\eta$ is an issue.

% \subsection{Case of Mahalanobis Attacks}
% Applying Lemma \ref{lm:subdifferential} with $a=w_0$ and $g:=r\|\cdot\|_B$, we obtain that the minimize of $w \mapsto \|w-w_0\|_\Sigma + r\|\cdot\|_B$ is of the form $w(t)$, for some $t\in [0,\infty]$, where
% \begin{eqnarray*}
% \begin{split}
% w(t) &= (I+t\Lambda^{-1}\partial \|\cdot\|_B)^{-1}(w_0),\text{ i.e}\\
% w_0 &=
% w(t) + t\Lambda^{-1} Bw(t)/\|w(t)\|_B,\,w(\infty)=w_0.
% \end{split}
% \end{eqnarray*}
% Fixing $t/\|w(t)\|_B = \lambda = 1/\eta$, we obtain
% \begin{eqnarray}
% w(\eta) = (\Lambda + \lambda B)^{-1}\Lambda w_0=(\eta \Lambda + B)^{-1}\eta \Lambda w_0. 
% \end{eqnarray}



% \section{Robustness to General Attacks?}
% In this section we investigate the robustness of our proposed modification of the GD scheme. More precisely, we first provide a general upper-bound of the adversarial-risk for any norm-attack, then we show a sufficient condition under which early-stopping on $(\Sigma^{-1/2}w^{\Sigma^{-1/2}}(t,w_0))_{t\geq 0}$ is near-optimal. Finally we show that when this condition is not respected, such scheme can be arbitrarily sub-optimal.
% \subsection{A general upper-bound}
% Let us consider attacks w.r.t to an arbitrary norm $\Vert\cdot\Vert$. For that purpose, Let us introduce the general condition number associated to $B\in\mathcal{S}_{d}^{++}(\mathbb{R})$ defined as
% \begin{align*}
%     \kappa^{\Vert\cdot\Vert}(B)&:=\lambda_{max}^{\Vert\cdot\Vert}(B)/\lambda_{min}^{\Vert\cdot\Vert}(B),\,\text{where }\\
%     \lambda_{max}^{\Vert\cdot\Vert}(B)&:=\sup_{w\neq 0}\frac{\Vert B^{1/2} w\Vert_2^2}{\Vert w\Vert_*^2},\text{ and}\\
%     \lambda_{min}^{\Vert\cdot\Vert}(M)&:=\inf_{w\neq 0}\frac{\Vert B^{1/2} w\Vert^2}{\Vert w\Vert_*^2}.
% \end{align*}
% % then we show the following Proposition.
% \begin{restatable}{thm}{}
% For any $r\geq 0$ and $M\in\mathcal{S}_{d}^{++}(\mathbb{R})$, we have 
% %\begin{align*}
% $    \dfrac{\inf_{t \geq 0}E^{\Vert\cdot\Vert}(B^{1/2}w^{B}_c(t,w_0),w_0,r)}{E^{\Vert\cdot\Vert}_{opt}(r,w_0)}\leq \beta \kappa^{\Vert\cdot\Vert}(B^{-1}).
%      $
% %\end{align*}
% \end{restatable}
% Therefore along the modified GD scheme induced by $B$, one can find a $\beta \kappa^{\Vert\cdot\Vert}(B^{-1})$-optimally robust predictor against $\Vert\cdot\Vert$-attack. One main issue in the above upper-bound is that we do not have a simple control of $\kappa^{\Vert\cdot\Vert}(\cdot)$ in general, due to the arbitrary choice of the norm $\Vert\cdot\Vert$. In the following section, we provide a sufficient condition for near-optimality of such scheme by controlling the norms of the generative model only.

% However, obtaining in general $\inf_{t \geq 0}E^{\Vert\cdot\Vert}(A_M w^{M}_c(t),r)$, even when $M=\Sigma$ and $\Vert\cdot\Vert = \Vert\cdot\Vert_2$, is hard in general as the function $t\mapsto E^{\Vert\cdot\Vert}(A_M w^{M}_c(t),r)$ may admit several local minima. Therefore obtaining its infimum might require to compute the GD scheme until convergence in order to select the time where the global minimizer is reached. In the following we propose to consider an instance of the proposed method where the infimum can be effectively computed using a simple early-stopping strategy.




==> other_files/beyond.tex <==
\subsection{Going beyond linear models}
\textcolor{red}{Don't activate. This is broken!}

Let $P$ be the marginal distribution of the features and let the ground-truth $f_0$ be any function in $L^2(P)$, linear or not. We will now show that shrinkage always improves the robustness of $f_0$. Given any $\alpha \in [0,1]$, consider the shrunk version $f_\alpha := (1-\alpha) f_0$ of $f_0$. WLOG, suppose $E(f_0,r) > 0$ and define $\beta = \beta(P) := \|f_0\|_{L^1(P)} / \|f_0\|_{L^2(P)}$ and $\theta(r) = \theta(P,r) := \sqrt{E(f_0,r)}/\|f_0\|_{L^2(P)}$, where
\begin{eqnarray}
\|f_0\|_{L^m(P)} := (\mathbb E_P |f(x)|^m)^{1/m},\,\text{ for all }m \in [1,\infty).
\end{eqnarray}
By definition, it is clear that $\beta \le 1$ and $\theta(r) \le r \|f_0\|_{Lip}/\|f_0\|_{L^2(P)}$, where
\begin{eqnarray}
\|f_0\|_{Lip} := \sup_{x,x' \in \mathbb R^d,\,x' \ne x}\frac{|f_0(x')-f_0(x)|}{\|x'-x\|}
\end{eqnarray}
is the Lipschitz constant of $f_0$ w.r.t the attacker's norm $\|\cdot\|$.
% We will prove the following result which shows that shrinkage always improves the robust accuracy of the ground-truth model by at least $67\%$ at the price of a small decrease in normal accuracy.

\begin{restatable}[Robustness boosting by shrinkage]{thm}{}
It holds that
\begin{eqnarray}
\inf_{\alpha \in [0,1]} E(f_\alpha,r) \le E(f_{\alpha_{opt}(r)},r),
\end{eqnarray}
where
\begin{itemize}
\item[(A)] If $\theta(r) \le \beta$, then $\alpha_{opt}(r) = 0$, i.e no shrinking is necessary. If $\theta(r) \ge 1/\beta$, then $\alpha_{opt}(r) = 1$, i.e $f_0$ is shrunk to zero.
    \item[(B)] If $\beta \le \theta(r) \le 1/\beta$, then
$\alpha_{opt}(r) \in [0,1]$ is as given by
\begin{eqnarray}
\label{eq:alphaboost}
\alpha_{opt}(r) := \frac{E(f_0,r)-\|f_0\|_{L^1(P)}\sqrt{E(f_0,r)}}{E(f_0,r) + \|f_0\|_{L^2(P)}^2 - 2\|f_0\|_{L^1(P)}\sqrt{E(f_0,r)}} = \frac{\theta(r)^2 - \beta\theta(r)}{h_\beta(\theta(r))}.
\end{eqnarray}
Moreover, it holds that
\begin{align}
\inf_{\alpha \in [0, 1]}\frac{E(f_\alpha,r)}{E(f_0,r)} &\le \frac{E(f_{\alpha_{opt}(r)},r)}{E(f_0,r)} = \frac{1-\beta^2}{h_\beta(\theta(r))},\\
\frac{E(f_{\alpha_{opt}(r)})}{\|f_0\|_{L^2(P)}^2} &\le \left(\frac{1-\beta}{h_\beta(\theta(r))}\right)^2,
\end{align}
\end{itemize}
\end{restatable}
Note that as expected $\alpha_{opt}(r) = 0$ for $r$ sufficiently small (more precisely, for $\theta(r) \le \beta$), meaning that, in this regime no shrinkage is required. On the other hand, $\alpha_{opt}(r) = 1$ for $r$ sufficiently large (more precisely, for $\theta(r) \ge 1/\beta$), meaning in this regime, that it is to optimal to shrink all the way to the zero model!

\paragraph{Example; linear models.}
For example, if $f_0(w) \equiv x^\top w_0$ (i.e, $f_0$ is linear) and $P=N(0,\Sigma)$, then $\beta = c_0 := \sqrt{2/\pi}$ and $\theta(r) = r\|w_0\|_\star/\|w_0\|_\Sigma = r/r_0$, where $r_0 = \|w_0\|_\Sigma/\|w_0\|_\star$ is the scalar which was encountered before.
% Consequently, $ (1-\beta^2)(1+\beta)/2\le 0.33$ and $(1+\beta)^2/4 \le .81$. This corresponds to a gain in robustness of at least $(100-33/(1+r_0/r)^2)\% \ge 67\%$ at the price of an at most $81/(1+r_0/r)^{2}$ percent decrease in normal accuracy. Note that in the limit $r/r_0 \to 0^+$, this loss in normal accuracy tends to zero, while the $67\%$ gain in robust accuracy remains!

\begin{proof}[Proof of theorem]
The robust risk of $f_\alpha$ writes $E(f_\alpha, r):=\mathbb E_P\sup_{\|\delta\| \le 1}(f_\alpha(x+\delta)-f_0(x))^2=\mathbb E_P \sup_{\|\delta\| \le r}((1-\alpha) f_0(x+\delta) - f_0(x))^2$.
One computes
\begin{eqnarray*}
\begin{split}
&\sup_{\|\delta\| \le r}((1-\alpha)f_0(x+\delta) - f_0(x))^2\\
&\quad = \sup_{\|\delta\| \le r}((1-\alpha)f_0(x+\delta) - (1-\alpha)f_0(x) - \alpha f_0(x))^2\\ &\quad = \sup_{\|\delta\| \le r}(1-\alpha)^2 (f_0(x+\delta) - f_0(x))^2 \\
&\quad\quad\quad- 2\alpha(1-\alpha)f_0(x)(f_0(x+\delta) - f_0(x)) + \alpha^2 f_0(x)^2\\
&\quad \le (1-\alpha)^2\sup_{\|\delta\| \le r}(f_0(x+\delta) - f_0(x))^2  \\
&\quad\quad\quad + 2\alpha(1-\alpha)|f_0(x)|\sup_{\|\delta\| \le r}|f_0(x+\delta) - f_0(x)| + \alpha^2 f_0(x)^2.
\end{split}
\end{eqnarray*}
Taking expectations over $x \sim P$ and invoking the Cauchy-Schwarz inequality, we deduce that
\begin{eqnarray}
\begin{split}
E(f_\alpha,r)
% &:= \mathbb E_P\sup_{\|\delta\| \le r}(f_\alpha(x) - f_0(x))^2\\
&\le (1-\alpha)^2 E(f_0,r) + \alpha^2\|f_0\|_{L^2(P)}^2\\
&\quad\quad + 2\alpha(1-\alpha)\mathbb E_P |f_0(x)|\sup_{\|\delta\| \le r}|f_0(x+\delta) - f_0(x)|\\
&\le (1-\alpha)^2 E(f_0,r) + \alpha^2\|f_0\|_{L^2(P)}^2 + 2\alpha(1-\alpha)\|f_0\|_{L^2(P)}\sqrt{E(f_0,r)}\\
% &= (\alpha\|f_0\|_{L^2(P)} + (1-\alpha) \sqrt{E(f_0,r)})^2.
&= a \alpha^2 - 2b\alpha + c,
\end{split}
\end{eqnarray}
where $a=a(r):=E(f_0,r) + \|f_0\|_{L^2(P)}^2 - 2\|f_0\|_{L^2(P)}\sqrt{E(f_0,r)} = (\sqrt{E(f_0,r)}-\|f_0\|_{L^2(P)})^2 \ge 0$, $b=b(r) := E(f_0,r)- \|f_0\|_{L^2(P)}\sqrt{E(f_0,r)}$, and $c = c(r):= E(f_0,r)$. Now, the quadratic function $\alpha \mapsto a\alpha^2 - 2b\alpha + c$ is minimized when $\alpha = b/a = \alpha_{opt}(r) = \sqrt{E(f_0,r)}/|\sqrt{E(f_0,r)}-\|f_0\|_{L^2(P)}|$, where $\alpha_{opt} \in [0,1]$ is as given in \eqref{eq:alphaboost}. Moreover, the minimal value on this interval is $c-b^2/a = (\|f\|_{L^2(P)}^2-\|f\|_{L^1(P)}^2)E(f_0,r) / a$. Therefore, if $E(f_0,r) > 0$, then
\begin{eqnarray*}
\begin{split}
\inf_{\alpha \in [0, 1]}\frac{E(f_\alpha,r)}{E(f_0,r)} \le \frac{E(f_{\alpha_{opt}(r)},r)}{E(f_0,r)} &\le \frac{\|f\|_{L^2(P)}^2-\|f\|_{L^1(P)}^2}{E(f_0,r) + \|f_0\|_{L^2(P)}^2 - 2\|f_0\|_{L^1(P)}\sqrt{E(f_0,r)}}\\
&= \frac{1-\beta^2}{h_\beta(\theta(r))},
\end{split}
\end{eqnarray*}
and
\begin{eqnarray}
\begin{split}
\frac{E(f_{\alpha_{opt}(r)})}{\|f_0\|_{L^2(P)}^2} = \alpha_{opt}(r)^2 &= \left(\frac{E(f_0,r)-\|f_0\|_{L^1(P)}\sqrt{E(f_0,r)}}{E(f_0,r) + \|f_0\|_{L^2(P)}^2 - 2\|f_0\|_{L^1(P)}\sqrt{E(f_0,r)}}\right)^2\\
&\le \frac{(\theta(r)^2-\beta  \theta(r))^2}{h_\beta(\theta(r))^2}.
\end{split}
\end{eqnarray}
Diving numerators and denominators by $\|f_0\|_{L^2(P)}$ and recalling the definition of $\beta$ and $\theta(r)$ completes the proof.
\end{proof}

==> other_files/ewdd_rob.tex <==
\subsection{Dynamics of robustness}
At time $t$, one computes
\begin{eqnarray}
\begin{split}
\|w(t)\|^2 &= \|\widetilde w(t) + c(t)\|^2 = \|(I_d-sG)^tw(0)+K_t(G)X^\top(Xw_\star+\eta)/n\|^2\\
&= \|(I_d-sG)^t w(0)+K_t(G)Gw_\star+K_t(G)X^\top \eta/n\|^2.
\end{split}
\end{eqnarray}
Noting once again that $w(0)$, $w_\star$, and $\eta$ are independent, one computes
\begin{eqnarray}
\begin{split}
 \overline{\mathfrak{S}}(f_t)^2 &:= \mathbb E_{\{w_\star,X,z,w(0)\}}\mathfrak{S}(f_t)^2 = \mathbb E_{\{w_\star,X,z,w(0)\}} \|w(t)\|^2
    \\
    &=  \mathbb E_{\{X,w(0)\}}\|(I_d-sG)^tw(0)\|^2 +  \mathbb E_{\{w_\star,X\}}\|K_t(G)Gw_\star\|^2 \\
    &\quad\quad\quad +  \mathbb E_{\{X,z\}}\|K_t(G)X^\top \eta/n\|^2\\
    &= \sigma_0^2 \cdot \mathbb E_X \frac{1}{d}\trace((I_d-sG)^{2t}) + \sigma_\star^2\cdot\mathbb E_X \frac{1}{d}\trace((K_t(G)G)^2)\\
    &\quad\quad\quad + \mathbb E_X\trace(K_t(G)^2\cov(X^\top \eta/n \mid X))\\
    &= \sigma_0^2\cdot \mathbb E_X\frac{1}{d}\sum_{j=1}^r (1-s\lambda_j)^{2t} + \sigma_\star^2\cdot\mathbb E_X\frac{1}{d}\sum_{j=1}^r (1-(1-s\lambda_j)^t)^2\\
    &\quad\quad\quad + \sigma_\eta^2\cdot \mathbb E_X\frac{1}{d}\sum_{j=1}^{r_\eta}\frac{(1-(1-s\lambda_j)^t)^2}{\lambda_j}.
\end{split}
\end{eqnarray}
Taking limits, we get
\begin{restatable}{thm}{}
In the limit \eqref{eq:proportionate}, it holds that
\begin{eqnarray}
\begin{split}
\frac{\overline{\mathfrak S}(f_t)^2}{\sigma_\star^2} &\overset{p}{\to} \int_0^\infty (1-(1-s\lambda)^t)^2\mu_{\mathrm{MP}(\gamma)}(\lambda)\,\dv\lambda\\
&\quad\quad\quad+ \mathrm{INR}\int_0^\infty (1-s\lambda)^{2t}\mu_{\mathrm{MP}(\gamma)}(\lambda)\,\dv\lambda\\
&\quad\quad\quad+ \frac{1}{\mathrm{SNR}}\int_1^\infty \frac{(1-(1-s\lambda)^t)^2}{\lambda}\mu_{\mathrm{MP}(\gamma)}(\lambda)\,\dv\lambda
\end{split}
\end{eqnarray}
\end{restatable}

==> other_files/old.tex <==
\begin{abstract}
We consider two-layer neural networks in high dimensions trained via gradient-descent and derive a precise formula for their generalization error and robustness along the entire optimization trajectory. Our analytic expressions reveal the fine structural dependence on all problem specific parameters: scaling of sample size vs input dimension vs network width; level of label-noise; magnitude of network parameters at initialization; etc. Our work is based on techniques from random matrix theory (RMT).
\end{abstract}

\tableofcontents

\section{Introduction}
\subsection{Setup}
Let $P_x$ be a probability distribition on $\mathbb R^d$, and let $(x_1,y_1),\ldots,(x_n,y_n)$ be an iid sample of size $n$ from a distribution $P$ on $\mathbb R^d \times \{\pm 1\}$, such that
\begin{equation}
\label{eq:data}
x_i \sim P_x,\, y_i = f_\star(x_i) + \eta_i,    
\end{equation}
where $\eta_i$ is $\sigma_{\eta}^2$-subGaussian noise which is independent of $x_i$ and $f_\star:\Rd \to \mathbb R$ is possibly random function which independent of the $x_i$'s and $\eta_i$'s. For example, if $w \in \mathbb R^d$ (possibly random), then $f_\star(x) := w^\top x$ corresponds to a linear model.
Let $X$ be the random $n \times d$ matrix with $i$th row $x_i$, $y$ (resp. $\eta$) be the $n$-dimensional vector with $i$th component $y_i$ (resp. $\eta_i$). 

We will work in the so-called \emph{proportionate} high-dimensional regime
\begin{eqnarray}
\label{eq:proportionate}
n,d \to \infty,\, d/n \to \gamma_1 \in (0,\infty).
\end{eqnarray}

Given a smoothly parametrized class of functions $\mathcal F = \{f_\theta \mid \theta \in \Theta\}$ from $\Rd$ to $\mathbb R$ (e.g linear models, neural networks, etc.), the ML objective is to find $\theta \in \Theta$ which minimizes the test error, namely
\begin{eqnarray}
\etest(f_\theta) :=\|f_\theta-f_\star\|_{L^2(P_x)}^2 = \mathbb E_{P_x}|f_\theta(x)-f_\star(x)|^2.
\end{eqnarray}
Here, the parameter space $\Theta$ is a nonempty open subset of some $\mathbb R^m$. In the empirical risk minimization paradigm, one instead minimizes the training error
\begin{eqnarray}
\etrain(f_\theta) := \frac{1}{n}\sum_{i=1}^n(f_\theta(x_i)-y_i)^2.
\end{eqnarray}
and then uses "uniform convergence arguments" to relate this to $\etest(f; P)$.

\subsection{Objective}
In this manuscript, we will consider gradient-flow
\begin{eqnarray}
\theta(t) = -\nabla_{\theta(t)} \etrain(f_{\theta(t)})
\end{eqnarray}
and are interested in dynamics of the test error $\etest(f_{\theta(t)})$ and the "robustness" of $\varepsilon_{\mathrm{rob}}(f_{\theta(t)}) := \mathbb E_{P_x}\|\nabla f_{\theta(t)}(x)\|^2$. For the justification for the use of Dirichelet energy (aka square $H^1$-norm), see our older papers...


\section{Linear models}
We begin with a multivariate Gaussian linear where the features have distribution $P_x$ on $\Rd$ which admits density w.r.t to the Lebesgue measure. Suppose the labels in \eqref{eq:data} are generated from a linear function $f_\star(x) \equiv x^\top \trueweights$, where the weights $\trueweights$ have distribution $N(0,\sigma_\star^2 I_d)$, for some $\sigma_\star>0$. The funciton $f_\star$ is called the \emph{teacher} model.

% Given a "radius" parameter $R>0$, consider a linear function class $\Flin := \{x \mapsto x^\top w \mid w \in \Rd,\,\|w\| \le R\}$. By duality, minimizing $\etest(f)$ over $f \in \Flin$ amounts to solving a Ridge regression problem
% \begin{eqnarray}
% \min_{w \in \mathbb R^d}\frac{1}{n}\sum_{i=1}^n(x_i^\top w - y_i)^2 + \lambda \|w\|^2,
% \label{eq:ridge}
% \end{eqnarray}
% for an appropriate value of $\lambda=\lambda(R)>0$.
% % Defining $G_\lambda := XX^\top / d + \lambda I_n$,
% A simple calculation reveals that \eqref{eq:ridge} has unique solution given by
% \begin{eqnarray}
% \widehat{w} =  (\gram + \lambda I_d)^{-1}X^\top y/n,
% % = (1/n)X^\top \widehat c,\text{ with }\widehat{c} = G_\lambda^{-1} y.
% \end{eqnarray}
% where $\gram := X^\top X/n$.
% Consider a multivariate Gaussian linear where the features have distribution $P_x = N(0,\Sigma)$, and the weights $\trueweights$ have distribution $N(0,\sigma_\star^2 I_d)$, for some $\sigma_\star>0$.
% % , where $\Sigma$ is the covariance matrix and has SVD $\Sigma = \sum_{j=1}^d s_j u_ju_j^\top$.
% % Given a appropriate funciton $\phi:\mathbb R_+ \to \mathbb R_+$,
% % consider a source condition $\trueweights = N(\mu, \sigma_\star^2 \phi(\Sigma))$, where
% % \begin{eqnarray}
% % \phi(\Sigma) := \sum_{j=1}^d \phi(s_i)u_ju_j^\top.
% % \end{eqnarray}
% A simple computation reveals that
% \begin{eqnarray}
% \begin{split}
% \etest(\widehat w) &= B_n + V_n,
% \end{split}
% \end{eqnarray}
% where the bias and variance terms are respectively given by
% \begin{eqnarray}
% \begin{split}
% B_n &:= \sigma_\star^2 \cdot \frac{1}{n}\trace(R_n(\lambda)\Sigma R_n(\lambda)),\\
% V_n &:= \sigma_{\eta}^2\cdot \frac{1}{n}\trace(R_n(\lambda)\Sigma R_n(\lambda)\widehat{\Sigma}_n),
% \end{split}
% \label{eq:biasvariance}
% \end{eqnarray}
% where $R_n(z) := (\gram+zI_d)^{-1}$ defines the \emph{resolvent} of $\gram$.

\subsection{Dynamics of model weights}
We now present a computation which is essentially due to Andrew Saxe and co-workers \url{https://arxiv.org/pdf/1710.03667.pdf}.
Let
\begin{eqnarray}
\gram = V\Lambda V^\top
\end{eqnarray}
be the singular-value decomposition (SVD) of $\gram$, where $\Lambda=\diag(\lambda_1,\ldots,\lambda_d)$ with $\lambda_1\ge \lambda_2 \ge \ldots \ge \lambda_d \ge 0$ being the eigenvalues. 
Now, the gradient-flow evolution of the parameters of the linear model $f_t(x) := x^\top a(t)$ is,
\begin{eqnarray}
\dot a(t) = -\nabla \etrain(f_t) = -X^\top(Xa(t)-y)/n = -Ga(t) + c,
\end{eqnarray}
where $c := X^\top y/n$. This ODE can be alternatively written as $(e^{t\gram}a(t))' = e^{t\gram}c$, and direct integration gives the unique solution
\begin{eqnarray}
a(t) = \overline a(t) + c(t),
% = Ve^{-t\Lambda} V^\top a(0) + VE(t)V^\top c,
\label{eq:dynamics}
\end{eqnarray}
with $\overline a(t):=e^{-t\gram}a(0)$ and $c(t):=K_t(\gram)c$, where $(t,A) \mapsto K_t(A)$ is the mapping \emph{exponential integrator} given for any $t \ge 0$ and psd matrix $A$ by
\begin{eqnarray}
\label{eq:Kt}
K_t(A):=e^{-tA}\int_0^t e^{sA}\,\dv s = (1-e^{-tA})A^\dagger-t\Pi_{\ker A},
% =e^{-t\gram}\left(\frac{e^{t\gram}-I_d}{\gram}\right) := e^{-t\gram}t\sum_{N=0}^\infty \frac{(t\gram)^N}{(N+1)!}.
\end{eqnarray}
Here, $A^\dagger$ being the Moore-Penrose pseudo-inverse of $A$ and $\Pi_{\ker A}:=I_d-A^\dagger A$ is the orthogonal projector onto the kernel of $A$.
The following elementary lemma will be useful in the sequel.
\begin{restatable}{lm}{}{}
\label{lm:Kt}
The exponential integrator \eqref{eq:Kt} has the following properties:
\begin{itemize}
\item[(1)] $K_t(A)$ and $A$ commute for any $t \ge 0$ and psd matrix $A$. Moreover, $K_t(A)A=AK_t(A)=(I_d-e^{-tA})\Pi_{\mathrm{Im}\, A}$, where $\Pi_{\mathrm{Im}\, A} := A^\dagger A$ is the orthogonal projector onto the image of $A$.
\item[(2)] Each eigenvalue $\lambda_j(K_t(A))$ of $K_t(A)$ can be written in terms of time $t$ and the corresponding eigenvalue $\lambda_j(A)$ of $A$ like so
\begin{eqnarray}
\lambda_j(K_t(A)) =
% e^{-t\lambda_j(A)}\int_0^t e^{s\lambda_j(A)}\,\dv s =
% e^{-t\lambda_j}t\sum_{N=0}^\infty \frac{(t\lambda_j)^N}{(N+1)!} =
\begin{cases}
\dfrac{1-e^{-t\lambda_j(A)}}{\lambda_j(A)},&\mbox{ if }\lambda_j(A)>0,\\
t,&\mbox{ if }\lambda_j(A)=0.
\end{cases}
\label{eq:specK}
\end{eqnarray}
% \\
% because $a(0)$, $\trueweights$, and $\eta$ are mutually independent.
\end{itemize}
\end{restatable}
\begin{proof}
Part (1) follows from the fact that $A$ and $e^{\tau A}$ commute for any $\tau \in \mathbb R$. Part (2) follows from the fact that the funciton $g_t:z \mapsto e^{-tz}\int_0^t e^{sz}\,\dv s$ is analytic on $\mathbb C$ and so the eigenvalues of $K_t(A)$ are given by
$$
\lambda_j(K_t(A)) = \lambda_j(g_t(A)) = g_t(\lambda_j(A)) = e^{-\lambda_j(A)}\int_0^t e^{s\lambda_j(A)}\,\dv s,
$$
which evalues to the RHS of \eqref{eq:specK}.
\end{proof}
% Let $\Pi_V := VV^\top$ be the orthogonal projector for the onto the row-space of $V$, and given any $u \in \Rd$, let $u_\parallel := \Pi_V u$ (resp. $u_\perp := u-u_\parallel$) be the component parallel (resp. perpendicular) to this subspace.  We can then rewrite the dynamics \eqref{eq:dynamics} in the eigenbasis $V$ like so
% \begin{eqnarray}
% \begin{split}
% a_\parallel(t) &= e ^{-t\Lambda} a_\parallel(0) + VE(t)V^\top c\\
% a_\perp(t) &= e^{-t\Lambda}a_\perp(0).
% \end{split}
% \end{eqnarray}

\subsection{Dynamics of generalization error (isotropic features)}
For a random test input $x \sim P_x$, one computes the prediction at time $t$ is $f_t(x) = x^\top a(t) = x^\top \overline{a}(t) +x^\top c(t)$.
Thus, letting $\widetilde a(t):= \overline{a}(t)-\trueweights+c(t)$, we deduce that the generalization error at time $t$ is given by
\begin{eqnarray}
\etest(t) :=\mathbb E_x (f_t(x) - x^\top \trueweights)^2 = \mathbb E_x x^\top \widetilde a(t)\widetilde a(t)^\top x = \|\widetilde a(t)\|^2_\Sigma,
\label{eq:errordecomp}
\end{eqnarray}
where $\Sigma := \mathbb E_x \trace(xx^\top)$. Suppose that independently of the training data, the initial weights $a(0) \in \Rd$ of the student are sampled from a Gaussian distribution $N(0,\sigma_0^2 I_d)$ with variance parameter $\sigma_0 \ge 0$.

For simplicity of analysis, we will assume the following
\begin{restatable}{assume}{}{}
$P_x = N(0,I_d)$.
In particularly, this assumption implies that the covariance matrix of the features is $\Sigma=I_d$.
\end{restatable}
Thanks to a simple density argument, it is clear that, almost-surely, the Gram matrix $\gram$ has full rank $r=\min(n,d)$. One then computes
\begin{eqnarray*}
\begin{split}
&\mathbb E_{X,\eta,\trueweights,a(0)}\etest(t) = \mathbb E_{X,\eta,\trueweights,a(0)}\|K_t(\gram)c+e^{-t\Lambda} a(0)- \trueweights\|_{\Sigma}^2\\
&\quad = \mathbb E_{X,\eta}\|K_t(\gram)X^\top (X\trueweights+z)/n + e^{-t\Lambda}a(0)-\trueweights\|^2\\
&\quad = \mathbb E_{X,\eta,\trueweights,a(0)}\|K_t(\gram)X^\top z/n+e^{-t\Lambda}a(0) - (I_d-K_t(\gram)X^\top X/n)\trueweights\|^2\\
&\quad = \mathbb E_{X,\eta,\trueweights,a(0)}\|K_t(\gram)X^\top z/n - e^{-t\Lambda}a(0)-(I_d - K_t(\gram)\gram)\trueweights\|^2\\
&\quad = \sigma_{\eta}^2\cdot\mathbb E_X\frac{1}{n}\trace(K_t(\gram)^2\gram) +  \sigma_0^2\cdot\mathbb E_X\frac{1}{d}\trace(e^{-2t\gram}) + \sigma_\star^2\cdot\mathbb E_{X}\frac{1}{d}\trace((I_d-K_t(\gram)\gram)^2)\\
&\quad = \sigma_{\eta}^2\cdot\mathbb E_X\frac{1}{n}\trace(K_t(\gram)^2\gram) + \sigma_0^2\cdot\mathbb E_X\frac{1}{d}\trace(e^{-2t\gram}) + \sigma_\star^2\cdot \mathbb E_{X}\frac{1}{d}\trace((I_d-K_t(\gram)\gram)^2)\\
&\quad = \underbrace{\sigma_{\eta}^2\cdot \mathbb E_{X}\frac{1}{n}\sum_{j=1}^{r}\frac{(1-e^{-t\lambda_j})^2}{\lambda_j}}_{\text{Variance}} + \underbrace{(\sigma_0^2+\sigma_\star^2)\mathbb E_{X}\frac{1}{d}\left(d-r+\sum_{j=1}^d e^{-2t\lambda_j}\right)}_{\text{Bias}}
\end{split}
\end{eqnarray*}
Let $\mathrm{INR} := 1/\mathrm{SNR}= \sigma_\eta^2/\sigma_\star^2$, the "label-noise ratio", which captures the relative amount of label-noise, and also define $\mathrm{INR} := \sigma_0^2/\sigma_\star^2$, the "initialization-noise ratio" which captures the relative amount of noise in the initialization. We can write things more informatively like so
\begin{eqnarray}
\begin{split}
\mathbb E_{X,\eta,\trueweights,a(0)}\frac{\etest(t)}{\sigma_\star^2} &= \mathrm{INR}\cdot \mathbb E_\Lambda\frac{1}{n}\sum_{j=1}^{r}\frac{(1-e^{-t\lambda_j})^2}{\lambda_j}\\
&\quad\quad + (1+\mathrm{INR})\cdot\left(1-\frac{r}{d}+\mathbb E_\Lambda \frac{1}{d}\sum_{j=1}^r e^{-2t\lambda_j}\right).
\end{split}
\end{eqnarray}
In the limit $t \to \infty$, $n,d \to \infty$, $d/n \to \gamma_1$,
\begin{itemize}
\item The ($\sigma_\star^2$-normalized) variance term converges to $ \dfrac{\mathrm{INR}}{1-\max(1,1/\gamma_1)}$, with a singularity / pole at the interpolation threshold $\gamma_1=1$.
\item The ($\sigma_\star^2$-normalized) bias term converges to zero
$$
(1+\mathrm{INR})\cdot(1-1/\gamma_1)_+ = \begin{cases}
(1+\mathrm{INR})\cdot (1-1/\gamma_1),&\mbox{ if }\gamma_1 \ge 1,\\
0,&\mbox{ if }\gamma_1 \le 1,\\
\end{cases}
$$
\end{itemize}

\section{Dynamics of robustness}
Since the intialization $a(0)$ is centered independent of the training data, the terms $\overline a(t)$ and $c(t)$ in \eqref{eq:dynamics} have zero cross-correlation, i.e
\begin{eqnarray}
\begin{split}
\mathbb E\, \overline a(t)^\top c(t) &= \mathbb E\, a(0)^\top e^{-t\gram}K_t(\gram)X^\top y/n = 0.
\end{split}
\end{eqnarray}
One then computes the average squared $L_2$-norm of the model weights $a(t)$ at time $t$ like so,
\begin{eqnarray*}
\begin{split}
&\mathbb E_{X,\eta,\trueweights,a(0)}\|a(t)\|^2 = \mathbb E_{X,\eta,\trueweights,a(0)} \|\overline a(t)+c(t)\|^2\\
&\quad = \mathbb E_{X,\eta,\trueweights,a(0)} \|\overline a(t)\|^2+\mathbb E_{X,\eta,\trueweights}\|c(t)\|^2\\
&\quad = \mathbb E_{X,a(0)}a(0)^\top e^{-2t\gram} a(0)+ \mathbb E_{X,\eta}\| c(t)\|^2 \\
&\quad = \sigma_0^2\cdot\mathbb E_X \frac{1}{d}\trace(e^{-2t\gram}) + \mathbb E_{X,\eta,\trueweights}\|K_t(\gram)X^\top (X\trueweights+\eta)/n\|^2\\
&\quad = \sigma_0^2\cdot\mathbb E_\Lambda \frac{1}{d}\trace(e^{-2t\Lambda}) + \mathbb E_{X,\trueweights}\,\trueweights^\top \frac{X^\top X}{n} K_t(\gram)^2\frac{X^\top X}{n}\trueweights + \mathbb E_{X,\eta}\,\eta^\top \frac{X K_t(\gram)^2 X^\top}{n^2}\eta\\
&\quad = \sigma_0^2\cdot\mathbb E_\Lambda \frac{1}{d}\trace(e^{-2t\Lambda}) + \sigma_\star^2\cdot \mathbb E_X \frac{1}{d}\trace(\gram K_t(\gram)^2\gram) + \sigma_\eta^2\cdot \mathbb E_X \frac{1}{n}\trace(\gram K_t(\gram)^2)\\
&\quad = \sigma_0^2\cdot\mathbb E_\Lambda \frac{1}{d}\sum_{j=1}^de^{-2t\lambda_j} + \sigma_\star^2\cdot\mathbb E_\Lambda\frac{1}{d}\sum_{j=1}^r(1-e^{-t\lambda_j})^2 + \underbrace{\sigma_\eta^2\cdot \mathbb E_\Lambda \frac{1}{n}\sum_{j=1}^{r} \frac{(1-e^{-t\lambda_j})^2}{\lambda_j}}_{\text{Variance}}.
\end{split}
\end{eqnarray*}
This can be rewritten as 
\begin{eqnarray}
\begin{split}
\mathbb E_{X,\eta,\trueweights,a(0)}\frac{\|a(t)\|^2}{\sigma_\star^2} &= \mathrm{INR}\cdot\mathbb E_\Lambda \frac{1}{d}\sum_{j=1}^de^{-2t\lambda_j} + \mathbb E_\Lambda\frac{1}{d}\sum_{j=1}^d(1-e^{-t\lambda_j})^2\\
&\quad\quad + \mathrm{INR}\cdot \mathbb E_\Lambda \frac{1}{n}\sum_{j=1}^{r} \frac{(1-e^{-t\lambda_j})^2}{\lambda_j}.
\label{eq:linearwnorm}
\end{split}
\end{eqnarray}

\subsection{Linear models with isotropic data}
In particular, suppose an isotropic distribution of data $P_x = N(0,I_d)$. In the limit $t \to \infty$, $n,d \to \infty$, $d/n \to \gamma_1$,
\begin{itemize}
    \item The sum of the first and second terms converges to
    $$
    \mathrm{INR}\cdot (1-1/\gamma_1)_+ + \min(1,1/\gamma_1) =  \begin{cases}
        1,&\mbox{ if }\gamma_1 < 1,\\
    \mathrm{INR}\cdot(1-1/\gamma_1) + 1/\gamma_1,&\mbox{ if }\gamma_1 \ge 1,\\
    \end{cases}
    $$
\end{itemize}

\section{Random features neural network model}
Suppose the distribution of the covariates is $P_z = \phi_{\#} P_x \in \mathcal P(\mathbb R^m)$, the pushforward of $P_x$ under the random feature mapping $\phi$ from $\mathbb R^d$ to $\mathbb R^m$ given by
 \begin{eqnarray}
 \phi(x):=\sigma(Wx) = (\sigma(x^\top w_1),\ldots,\sigma(x^\top w_m))\text{ with }W=(w_1,\ldots,w_m) \in \mathbb R^{m \times d},
 \end{eqnarray}
 where $w_1,\ldots,w_d \overset{iid}{\sim} N(0,(1/m)I_m)$ are the hidden weights of two-layer neural network with activation function $\sigma:\mathbb R \to \mathbb R$. 
 
 \paragraph{Hermite coefficients.}
 We will assume the activation function $\sigma$ is square-integrable w.r.t to $N(0,1)$. For any integer $k \ge 0$, let $c_k(\sigma) := \mathbb E_{g \sim N(0,1)}[\mathrm{He}_k(g)\sigma(g)]$ be the order $k$ Hermite coefficient of $\sigma$ and let $\theta(\sigma):=c_0(\sigma^2)-c_1(\sigma)^2$. By \emph{Stein's Lemma}, it is clear that $\theta(\sigma) \ge 0$.
 
 At time $t$, the prediction of the model on a random test point $x \sim P_x$ is $f_t(x) = a(t)^\top \phi(x)$, where $a(t)$ is the $m$-dimensional vector of output weighs at time $t$, where the output weights $a(t) \in \mathbb R^m$ are given by the gradient-flow
 \begin{eqnarray}
\dot a(t) = -\nabla \etrain(f_t) = -Z^\top(Za(t)-y)/n = -Ga(t) + c,
\end{eqnarray}
where $c:=Z^\top y/n \in \mathbb R^m$ and
% \paragraph{Nonlinear Gram matrix and linear equivalent.}
% Consider the $m\times m$ random matrix $\gram$ defined by
\begin{eqnarray}
\nonlingram:=Z^\top Z/n \in \mathbb R^{m \times m},\text{ with }
Z = \phi(X) = \sigma(XW^\top) \in \mathbb R^{n \times m}.
\label{eq:Z}
\end{eqnarray}

% \begin{restatable}[Centered activation function]{cond}{}{}
% $c_0(\sigma)=0$.
% \label{cond:centered}
% \end{restatable}
It was established in \url{https://arxiv.org/abs/1904.03090} that
\begin{restatable}[Gaussian Equivalence Theorem]{prop}{}{}
The random matrix $\nonlingram$ defined in \eqref{eq:Z} has the same limiting spectral density (LSD) as the random matrix
\begin{eqnarray}
\frac{1}{n}Z_{\mathrm{lin}}^\top Z_{\mathrm{lin}},
\end{eqnarray}
where $Z_{\mathrm{lin}} := \sqrt{\theta(\sigma)}Z_0+c_1(\sigma)XW^\top \in \mathbb R^{n \times m}$, with $Z_0 \in \mathbb R^{n \times m}$ random matrix having iid entries from $N(0,1)$, and independent of $Z$ and $W$.
\end{restatable}

 \subsection{The norm of the output weights $a(t)$}
 Proceeding as in Section xyz, we obtain a representation \eqref{eq:linearwnorm}, but with $d$ replaced with $m$, i.e.,
\begin{eqnarray}
\begin{split}
\mathbb E_{X,\eta,\trueweights,a(0)}\frac{\|a(t)\|^2}{\sigma_\star^2} &= \mathrm{INR}\cdot\mathbb E_\Lambda \frac{1}{m}\sum_{j=1}^me^{-2t\lambda_j} + \mathbb E_\Lambda\frac{1}{m}\sum_{j=1}^m(1-e^{-t\lambda_j})^2\\
&\quad\quad + \mathrm{INR}\cdot \mathbb E_\Lambda \frac{1}{n}\sum_{j=1}^m \frac{(1-e^{-t\lambda_j})^2}{\lambda_j}1_{\lambda_j > 0},%\\
% &\ge \mathrm{INR}\cdot \min(1,\rho)e^{-2t\lambda_1}+(1-\rho)_+\\
% &\quad\quad + \min(1,\rho)\cdot(1-e^{-t\lambda_1})^2 \\
% &\quad\quad +\frac{1}{\mathrm{SNR}}\cdot \min(1,1/\rho)\frac{(1-e^{-t\lambda_1})^2}{\lambda_1}.
\end{split}
\end{eqnarray}
where the $\lambda_j$'s are now the eigenvalues of $\nonlingram$.

\subsection{Dynamics of robustness}
 For a test data point $x \sim \Rd$, let $f_t(x) = a(t)^\top \phi(x)$ be the prediction of the neural network at time $t$. One computes the robustness / stability of $f_t$ as
 \begin{eqnarray}
  \mathfrak{S}(f_t)^2 = \mathbb E_{P_x}\,\|\nabla f_t(x)\|^2 = a(t)^\top Ca(t),
 \end{eqnarray}
 where $C=C(W)$ is the $m \times m$ random psd matrix with entries given by
 \begin{eqnarray}
 C_{jk} = (w_j^\top w_k)\mathbb E_{P_x}[ \sigma'(x^\top w_j)\sigma'(x^\top w_k)].
 \end{eqnarray}
 Note that $\mathfrak{S}(f_t)^2$ is a random variable due to randomness in $X$, $W$, $\eta$, $a(0)$, and $a_\star$.
 Define the $m \times m$ random psd matrix $S(X)$ by
 \begin{eqnarray}
 S(X) := \frac{1}{n}\mathbb E_{f_\star}[f_\star(X)^\top f_\star(X)].
 \end{eqnarray}
 Thanks to \eqref{eq:dynamics} with $\overline{a}(t) = e^{-t\nonlingram}a(0) \in \mathbb R^m$, $c(t) = K_t(\nonlingram)c \in \mathbb R^m$, and $c=Z^\top y/n=Z^\top (f_\star(X)+\eta)/n=Z^\top f_\star(X)/n+Z^\top \eta / n \in \mathbb R^m$, one deduces
 \begin{eqnarray}
 \begin{split}
 \overline{\mathfrak{S}}(f_t)^2 &:=\mathbb E_{\{X,W\}}\, \mathfrak{S}(f_t)^2 = \mathbb E_{\{X,W,\eta,a(0)\}}\,a(0)^\top e^{-t\nonlingram}Ce^{-t\nonlingram} a(0)\\
 &\quad\quad+ \mathbb E_{\{X,W,\eta,f_\star\}}\,\frac{1}{n^2}f_\star(X)Z K_t(\nonlingram)CK_t(\nonlingram) Z^\top f_\star(X)^\top \\
 &\quad\quad + \mathbb E_{\{X,W\}}\,\frac{1}{n^2}\eta^\top ZK_t(\nonlingram)CK_t(\nonlingram)Z^\top \eta \\
 &= \sigma_0^2\cdot \mathbb E_{\{X,W\}}\,\frac{1}{m}\trace(e^{-2t\nonlingram}C)\\
 &\quad\quad + \mathbb E_{\{X,W\}}\,S(X)\frac{1}{n}Z K_t(\nonlingram)CK_t(\nonlingram) Z^\top\\
 &\quad\quad + \sigma_\eta^2\cdot \mathbb E_{\{X,W\}}\,\frac{1}{n}\trace(\nonlingram K_t(\nonlingram)^2C)\\
 &\ge \mathbb E_W \lambda_{\min}(C)\cdot\left(E_1(t)+E_2(t) + E_3(t)\right)-o_m(1),
 \end{split}
 \end{eqnarray}
 where $E_{1,2,3}(t)$ are defined by
 \begin{align}
 E_1(t) &:= \sigma_0^2\cdot \mathbb E_{X,W}\frac{1}{m}\trace(e^{-2t\nonlingram}) = \sigma_0^2\cdot\left(1-\frac{r}{m}+\mathbb E_{W,X}\frac{1}{d}\sum_{j=1}^r e^{-2t\lambda_j}\right)\\
    E_2(t) &:= \mathbb E_{X,W} \trace(S(X)\frac{1}{n}ZK_t(\nonlingram)^2Z^\top),% = \mathbb E_{X,W}\frac{1}{m}\sum_{j=1}^r(1-e^{-t\lambda_j})^2,
    \\
     E_3(t) &:= \sigma_\eta^2\cdot\mathbb E_{X,W}\frac{1}{n}\trace(\nonlingram K_t(\nonlingram)^2) = \sigma_\eta^2\cdot\mathbb E_{X,W}\frac{1}{n}\sum_{j=1}^r\dfrac{(1-e^{-t\lambda_j})^2}{\lambda_j}.
 \end{align}
 
%  In particular, if $\gamma_2 < 1$ and $\sigma_\star>0$, then there exists a sufficiently large (but finite) time $t_0=t_0(\sigma_0,\sigma_\star,\ldots)>0$ such that the first term $E_1(t)$ in the above display is negligible compared to the second and third, and so
%  \begin{eqnarray}
%  \overline{\mathfrak{S}}(f_t)^2 \le \overline{\mathfrak{S}}(f_\star)^2,\,\forall t \ge t_0.
%  \end{eqnarray}
%  That is, the student is eventually more robust / stable than the teacher, on average. For example, in the case where the output weights are initialized at zero, i.e., $\sigma_0=0$, the above inequality holds with $t_0=0$.

\subsection{Special cases}
\paragraph{Linear ground-truth} Suppose the ground-truth function is $f_\star(x) := a_\star(x)^\top \phi(x)$. The we have $S(X) = G$, and so $E_2(t) = \mathbb R$

\subsection{Emergence of double-descent in robustness curve}
Note that if $\sigma_\eta>0$ and
\begin{eqnarray}
\lim_{\substack{n,d,m \to \infty\\d/n \to \gamma_1,\,d/m \to \gamma_2}} \mathbb E_{X,W}\frac{1}{n}\trace(\nonlingram^\dagger) = \infty,
\end{eqnarray}
then $\lim\overline{\mathfrak{S}}(f_t) \ge \lim E_3(t) = \infty$ for any fixed $t \in (0,\infty]$. In particular, this would explain the results empirically observed in Dohmatob (2021).
\lorem
\lorem

\lorem 

\section{EWMD in the "correlated noise" data model}
\label{sec:known}
As in (Stephenson et al.) \url{https://arxiv.org/pdf/2108.12006.pdf}, fix $\sigma_\star^2$ and $\sigma_\epsilon^2$ and consider the following model
\begin{mdframed}
\textbf{Data model with correlated noise.}
\begin{align}
    w_\star &\sim N(0,(\sigma_\star^2/d) I_d),\\
    x_1,\ldots,x_n &\overset{iid}{\sim} P_X = N(0,I_d),\text{ independent of }w_\star,\\
    X &=  (x_1,\ldots,x_n) \in \mathbb R^{n \times d},\\
    \mathrm{SVD}\, X/\sqrt{n} &= U\Lambda^{1/2} V^\top,\text{ with }\Lambda = \diag(\lambda_1,\ldots,\lambda_r),\\
    \epsilon &= U\eta,\text{ with }\eta \sim N(0,\alpha(\Lambda))\text{ independent of }(X,w_\star),\\
    y_i &= x_i^\top w_\star + \epsilon_i,\text{ for all }i \in [n],
\end{align}
where $\alpha(\Lambda)$ is the $r \times r$ diagonal matrix defined by
$$
\alpha(\Lambda)_{j,j} := \begin{cases}0,&\mbox{ if }\lambda_j \le 1,\\
(n/d)\sigma_\epsilon^2,&\mbox{else.}
\end{cases}
$$
\end{mdframed}
Here $r=\min(n,d)$ is the rank of $X$\footnote{Note that indeed, $X$ has full rank, i.e $r=\min(n,d)$ w.p $1$.}.
Thus,
\begin{itemize}
\item The noise is correlated across different samples.
\item Noise enters eigen-directions of design matrix $X$ at different rates; the most informative directions are the most noisy.
\end{itemize}
The signal-to-noise ratio of the problem is given by $\mathrm{SNR} = \sigma_\star^2/\sigma_\epsilon^2$.

We shall work in the following high-dimensional limit
\begin{eqnarray}
\label{eq:proportionate}
n \to \infty,\, d/n \to \gamma \in (0,\infty).
\end{eqnarray}
The edge case $\gamma \to 0^+$ subsumes the setting where the input-dimension $d$ is fixed, while the sample size $n$ is cranked up.

\subsection{Gradient-descent}
Define $Q:=X^\top X/n = \sum_i x_ix_i^\top/n \in \mathbb R^{d \times d}$, $c:=X^\top y/n = X^\top (Xw_\star+\epsilon)/n \in \mathbb R^d$, where $y := (y_1,\ldots,y_n)$ is the response vector and $\epsilon := (\epsilon_1,\ldots,\epsilon_n)$ is the noise vector, so that $y=Xw_\star + \epsilon$.
% Note that, modulo rescaling, $Q$ has the same nonzero eigenvalues as the Gram matrix $G:=XX^\top/d$.
Gradient-descent on mean-squared error $\etrain(w) := \|Xw-y\|^2/n$ with stepsize $s$ gives
\begin{eqnarray}
\begin{split}
w(t) = w(t-1)-\alpha X^\top (Xw-y)/n &= (I_d-\alpha Q)w(t-1)+\alpha c\\
&= \ldots = \widetilde{w}(t)+c(t),
\end{split}
\end{eqnarray}
where $\widetilde{w}(t) := (I_d-\alpha Q)^t w(0) \in \mathbb R^d$, $c(t) := K_t(Q) c \in \mathbb R^d$, with
\begin{eqnarray}
K_t(Q) := \alpha\sum_{s=0}^{t-1}(I_d-\alpha Q)^s.
\end{eqnarray}
It is clear that $Q$ has eigenvalues $(\lambda_j)_{j \in [n]}$, whilst $K_t(Q)$ has eigenvalues given by
\begin{eqnarray}
\lambda_j(K_t(Q)) = K_t(\lambda_j)= \alpha\sum_{s=0}^{t-1}(1-\alpha\lambda_j)^s=\begin{cases}\dfrac{1-(1-\alpha\lambda_j)^t}{\lambda_j},&\mbox{ if }\lambda_j > 0,\\ t,&\mbox{ if }\lambda_j=0,
\end{cases}
\label{eq:specK}
\end{eqnarray}

The initial point $w(0)$ is assumed to be drawn from $N(0,(\sigma_0^2/d)I_d)$, independently of the data the training data. Define the initialization-noise ratio $\mathrm{INR} := \sigma_0^2/\sigma_\star^2$.

\subsection{Dynamics of test error}
At time $t$, the prediction of a random test datapoint $x \sim P_x=N(0,I_d)$ is $x^\top w(t)$, and so one computes the test error as
\begin{eqnarray}
\begin{split}
\etest(w(t)) &= \mathbb E_x(x^\top w(t)-x^\top w_\star)^2 = \|w(t)-w_\star\|^2\\
&= \|(I_d-\alpha Q)^t w(0)+K_t(Q)(X^\top w_\star+\epsilon)/n-w_\star\|^2.
\end{split}
\end{eqnarray}
Assuming that $w(0)$ is independent of $w_\star$ and $\epsilon$, we compute the test error average over all sources of randomness, denoted $\overline\varepsilon(t)$, as follows
\begin{eqnarray}
\label{eq:calc}
\begin{split}
    \overline{\mathrm{err}}_{\mathrm{test}}(t) &:= \mathbb E_{\{w_\star,X,z,w(0)\}} \etest(w(t))\\
    & =  \mathbb E_{\{w_\star,X,\epsilon,w(0)\}}\|(I_d-\alpha Q)^t w(0)+K_t(Q)X^\top(X w_\star+\epsilon)/n-w_\star\|^2\\
    &= \mathbb E_{\{X,w(0)\}}\|(I_d-\alpha Q)^tw(0)\|^2+\mathbb E_{\{X,\epsilon\}}\|K_t(Q)X^\top \epsilon/n\|^2\\
    &\quad\quad\quad+ \mathbb E_{\{w_\star,X\}}\|(I_d-K_t(Q)Q)w_\star\|^2\\
    &= \sigma_0^2\cdot \mathbb E_X \frac{1}{d}\trace((I_d-\alpha Q)^{2t})) + \mathbb E_X\frac{1}{n}\trace(K_t(Q)^2\cov((X/\sqrt{n})^\top \epsilon \mid X))\\
    &\quad\quad\quad + \sigma_\star^2\cdot \mathbb E_X \frac{1}{d}\trace((I_d-K_t(Q)Q)^2)\\
    &= \sigma_0^2\cdot \mathbb E_X \frac{1}{d}\sum_{j}(1-\alpha\lambda_j)^{2t} + \sigma_\epsilon^2\cdot \mathbb E_X\frac{1}{d}\sum_{j \mid \lambda j > 1}\frac{(1-(1-\alpha\lambda_j)^t)^2}{\lambda_j}\\
    &\quad\quad\quad + \sigma_\star^2\cdot \mathbb E_X \frac{1}{d}\sum_{j}(1-\alpha\lambda_j)^{2t}.
\end{split}
\end{eqnarray}
Note that we have used the facts that 
\begin{eqnarray*}
\begin{split}
\cov((X/\sqrt{n})^\top \epsilon \mid X) &= \cov(V\Lambda^{1/2}U^\top \epsilon \mid X)\\
&= \cov(V\Lambda^{1/2} z \mid X) = (n/d)\sigma_\epsilon^2 V\alpha(\Lambda)\Lambda V^\top,
\end{split}
\end{eqnarray*}
and $K_t(Q)^2 = VK_t(\Lambda)^2 V^\top$, which combine with \eqref{eq:specK} to give
\begin{eqnarray}
\begin{split}
\frac{1}{n}\trace(VK_t(Q)^2\cov((X/\sqrt{n})^\top\epsilon \mid X)) &= \frac{(n/d)\sigma_\epsilon^2}{n}\trace(VK_t(\Lambda)^2\alpha(\Lambda)\Lambda V^\top)\\
&= \frac{\sigma_\epsilon^2}{d}\trace(K_t(\Lambda)^2\alpha(\Lambda)\Lambda)\\
&=\frac{\sigma_\epsilon^2}{d}\sum_{j \mid \lambda j > 1}K_t(\lambda_j)^2\lambda_j\\
&= \frac{\sigma_\epsilon^2}{d}\sum_{j \mid \lambda j > 1}\frac{(1-(1-\alpha\lambda_j)^t)^2}{\lambda_j}.
\end{split}
\end{eqnarray}
Taking limits in \eqref{eq:calc}, we recover the following result
\begin{restatable}[Stephenson et al. (2021)]{prop}{}{}
It holds in the limit \eqref{eq:proportionate} that
\begin{eqnarray}
\label{eq:ewdd}
\begin{split}
\frac{\overline{\mathrm{err}}_{\mathrm{test}}(t)}{\sigma_\star^2} &\to
(1+\mathrm{INR})\left(\int_{a(\lambda)}^{b(\lambda)} (1-\alpha\lambda)^{2t}\mu_{\mathrm{MP}(\gamma)}(\lambda)\,\dv\lambda + \left(1-\frac{1}{\gamma}\right)_+\right)\\
&\quad\quad\quad+ \frac{1}{\mathrm{SNR}}\int_1^{b(\lambda)} \frac{(1-(1-\alpha\lambda)^t)^2}{\lambda}\mu_{\mathrm{MP}(\gamma)}(\lambda)\,\dv\lambda
    \end{split}
\end{eqnarray}
where $a(\gamma) := (1-\sqrt{\gamma})^2$ and $b(\gamma):=(1+\sqrt{\gamma})^2$ are the endpoints of bulk of the Marchenko-Pastur density $\mu_{\mathrm{MP}(\gamma)}$ with shape parameter $\gamma$, defined by
\begin{eqnarray}
\mu_{\mathrm{MP}(\gamma)}(\lambda) = \dfrac{\sqrt{(\lambda-a(\gamma))(b(\gamma)-\lambda)}}{2\pi\gamma \lambda}
1_{a(\gamma) \le \lambda \le b(\gamma)} + \left(1-\frac{1}{\gamma}\right)_+\delta_0(\lambda).
\end{eqnarray}
\end{restatable}


\section{Open directions}
\textcolor{red}{\textit{Out dated section contents!}}

\subsection{Other models of data}
We could consider different data models. For example
\begin{itemize}
\item[(2)] Data model with "source condition", i.e the ground-truth weights are given by $w_\star \sim N(0,\phi(\Sigma))$ where $\Sigma$ is the population covariance matrix of the covariates, and $\phi(\Sigma)$ has the same eigenvectors as $\Sigma$ by eigenvalues transformed by $\lambda \mapsto \phi(\lambda)$. For example $\phi(\lambda) \propto 1/\lambda$. Such models have been recently studied by Rozasco and co-workers.
\item[(3)] The signal + noise model suggested by Nourredine.
\item[(4)] ...
\end{itemize}


\subsection{Neural networks and kernel methods} We could consider the case of learning with wide neural networks , in the following regimes:
\begin{itemize}
\item infinite-width RF
\item infintie-width NTK
\item width but finite-width RF
\item width but finite-width NTK
\end{itemize}
The first two regimes as instances of regression in RKHS, and thanks to representer theorems + RMT, should be reducible to the case of ordinary regression (i.e the case studied in Stephenson et al.).

Presumably, the last 2 regimes will be the most difficult (because the Gram matrix $(G)_{ik} = m^{-1}\sum_{j=1}^m \sigma(x_i^\top w_j)\sigma(x_k^\top w_j)$ has nasty structure which is difficult to analyze, unlike the kernel regimes). However, all we need is the limiting spectral distribution of the Gram matrix (even in implicit form, via fixed-point equations, etc.). Maybe we can use Noureddine's "uniform CLT" to reduce the situation to the kernel regime ? 


==> other_files/source_condition.tex <==
\section{Source condition}
Let $\Sigma = V\Lambda V^\top = \sum_{j=1}^d \lambda_j v_j v_j^\top$ and $\phi(\Sigma) := \sum_j \phi(\lambda_j)v_jv_j^\top$. Consider the data model
\begin{eqnarray}
\begin{split}
x_1,\ldots,x_n &\sim N(0,\Sigma),\\
w_\star &\sim N(0, (r_\star^2/d)\phi(\Sigma)),\\
\epsilon &\sim N(0,\sigma_\eta^2 I_n),\\
y_i &= x_i^\top w_\star + \epsilon_i,\text{ for all }i \in [n]
\end{split}
\end{eqnarray}

\begin{eqnarray}
\begin{split}
e(t) &= \mathbb E_{\{X,w_\star,\epsilon,w(0)\}}\|w(t)-w_\star\|^2_\Sigma\\
&= \mathbb E_{\{X,w_\star,\epsilon,w(0)\}}\|(I_d-sQ)^t w(0) + K_t(Q)X^\top (Xw_\star+\epsilon)/n-w_\star\|_\Sigma^2\\
&= \mathbb E_{\{X,w(0)\}}\|(I_d-sQ)^tw(0)\|^2_\Sigma + \mathbb E_{\{X,w_\star\}}\|(I_d-K_t(Q)Q)w_\star\|_\Sigma^2\\
&\quad\quad\quad+ \mathbb E_{\{X,\epsilon\}}\frac{1}{n}\|K_t(Q)(X/\sqrt{n})^\top \epsilon\|_\Sigma^2\\
&= \sigma_0^2 \mathbb E_X\frac{1}{d}\trace((I_d-sQ)^t \Sigma (I_d-sQ)^t)\\
&\quad\quad\quad+ \sigma_\star^2\mathbb E_X\frac{1}{d}\trace(Q(I_d-K_t(Q))\Sigma(I_d-K_t(Q))Q\phi(\Sigma))\\
&\quad\quad\quad+ \sigma_\epsilon^2\mathbb E_X\frac{1}{n}\trace(X K_t(Q)\Sigma K_t(Q) X^\top / n)\\
&= \sigma_0^2 \mathbb E_X\frac{1}{d}\trace((I_d-sQ)^{2t} \Sigma)+ \sigma_\star^2\mathbb E_X\frac{1}{d}\trace((I_d-sQ)^t\Sigma(I_d-sQ)^t\phi(\Sigma))\\
&\quad\quad\quad + \sigma_\epsilon^2\mathbb E_X\frac{1}{n}\trace(K_t(Q)^2 Q\Sigma)\\
\end{split}
\end{eqnarray}

==> sections/GDfailure_l1.tex <==
In high-dimensions (i.e large $d$), consider the ground-truth model $w_0 = (1,1/d^\alpha,\ldots,1/d^\alpha)$, for some positive constant $\alpha \in (0,1)$ to be prescribed later. Note that
\begin{align}
\|w_0\|_2 &= \sqrt{1 + (d-1)/d^{2\alpha}} \asymp 1,\text{ if }\alpha > 1/2,\\
\|w_0\|_1 &= 1 + (d-1)/d^\alpha = 1+d^{1-\alpha} \gg 1.
\end{align}
Thus, the optimal rescaling $a w_0$ achieves an adversarial risk of
\begin{eqnarray}
\|w_0\|_2^2 \land r^2\|w_0\|_1^2 = 1+o_d(1)\text{ for fixed }r\text{ and large }d.
\end{eqnarray}
Now, let $w=(c,0,\ldots,0)$ for some positive scalar $c$ to be prescribed later. It is clear that
\textcolor{red}{Meyer: $\|w-w_0\|_2^2 &= (c-1)^2+\frac{d-1}{d^{2\alpha}}$ ca pose pb du coup...} Ah, oui. Bon, tant pis! Oui... c'est chiant ce truc 
\begin{align}
    \|w-w_0\|_2^2 &= c^2+\frac{d-1}{d^{2\alpha}} \asymp c^2,\text{ if }c \gtrsim d^{1/2-\alpha}\\
    \|w\|_1 &= c.
\end{align}
\begin{mdframed}
The important thing here is that $w$ is a sparse vector (arbitrarily small $L_1$-norm) which approximates $w_0$ in $L_2$-norm, arbitrarily well.
\end{mdframed}

Thus, the adversarial risk of this choice for $w$ is $E(w,r) \asymp (\|w-w_0\|_2 + r\|w\|_1)^2 = (1+r)^2c^2$, and gives an upper bound for the optimal adversarial risk $E_{opt}(r)$. Therefore,
\begin{restatable}{thm}{}
For large $d$ and fixed $r,c>0$, and $\alpha \in (1/2,1)$, one has
\begin{eqnarray}
\frac{\inf_{\widehat w} E(\widehat w,r)}{E_{opt}(r)} \gtrsim \frac{1}{(1+r)^2 c^2},
\label{eq:bang}
\end{eqnarray}
where the infimum is over all rescalings, i.e models of the form $a w_0$ for some $a \in [0,1]$.
\end{restatable}
It is clear that the RHS of \eqref{eq:bang} can be made arbitrarily large by choosing $c$ sufficiently smaller than $1/(1+r)$. For example, taking $c=d^{1/2-\alpha}$, we obtain:
\begin{restatable}{cor}{}
For any $r>0$ and $\alpha \in (1/2,1)$,
\begin{eqnarray}
\frac{\inf_{\widehat w} E(\widehat w,r)}{E_{opt}(r)} \gtrsim \frac{d^{2\alpha-1}}{(1+r)^2} \overset{d \to \infty}{\longrightarrow} \infty,
\label{eq:bangbang}
\end{eqnarray}
\end{restatable}

==> sections/experiments.tex <==



==> sections/junk.tex <==

\section{Without the second condition}
\subsection{Gaussian widths}
Let $g$ be an $N$-dimensional standard Gaussian random vector. Given a subset $T$ of $\mathbb R^N$,  its \emph{Gaussian width} $\omega(T)$, is defined by
\begin{eqnarray}
\mathbb E\,\sup_{x \in T}x^\top g.
\end{eqnarray}
For example, it is well-known that $\omega(B_2^N) \asymp \sqrt{N}$ while $\omega(B_1^N) \asymp \sqrt{\log N}$

\subsection{Gordon's generalization of Slepian's Lemma}
\begin{restatable}{prop}{}
Let $(X_{u,v})$ and $(Y_{u,v})$ be Gaussian processes such that $\|X_{u,v}-X_{u',v'}\| := \sqrt{\mathbb E\,(X_{u,v}-X_{u',v'})^2} \le \|Y_{u,v}-Y_{u',v'}\|$ for all $u,v,u',v'$, with equality if $u=u'$. Then,
\begin{eqnarray}
\mathbb E\,\inf_u \sup_v X_{u,v} \ge  \mathbb E\,\inf_u\sup_v Y_{u,v}.
\end{eqnarray}
\end{restatable}

\subsection{Results}
\begin{restatable}{thm}{}
Let $G$ be a an $m \times d$ random matrix with iid entries from $N(0,1)$. Then,
\begin{eqnarray}
\mathbb E\,\inf_{x \ne 0}\frac{\|(G^\top G)^{1/2}x\|_2}{\|x\|_\star} \ge (\sqrt{m}-\omega(B_{\|\cdot\|_\star}))_+^2,
\end{eqnarray}
\end{restatable}

\begin{restatable}{cor}{}
Let $G$ be as in previous theorem. Then,
\begin{align}
\mathbb E\,\inf_{x \ne 0}\frac{\|(G^\top G)^{1/2}x\|_2}{\|x\|_1} &\ge (\sqrt{m}-\sqrt{d})_+^2,\\
\mathbb E\,\inf_{x \ne 0}\frac{\|(G^\top G)^{1/2}x\|_2}{\|x\|_1} &\ge (\sqrt{m}-c\sqrt{\log d})_+^2,
\end{align}
for some absolute constant $c$.
\end{restatable}

==> sections/minimax.tex <==
\section{Minimax Optimality for $\ell_p$-norm Attacks}
In this section, we will establish a minimax lower-bound for the proxy adversarial risk functional $\widetilde E$ defined in \eqref{eq:Etilde}, in the case of general feature covariance matrix $\Sigma$ and attacker norm is $\|\cdot\|_p$ with $p \in [2,\infty]$. Then, we will show that this lower-bound is attained by our proposed two-stage estimator proposed in the previous section. Thanks to Lemma \ref{lm:sandwich}, these considerations will also give a minimax theory upto a multiplicative constant, for the true adversarial risk functional $E$ defined in \eqref{eq:Ewrdef}.

\subsection{The Statistical Setup}
Consider the case where the ground-truth model $w_0$ is $s$-sparse, i.e $w_0 \in B_0^d(s)$, for some $s \in [d]$.
Consider an $\ell_p$-norm attack of magnitude $r \ge 0$. We are interested in the following minimax problem
\begin{eqnarray}
\label{eq:minimax}
\inf_{\widehat w_n}\sup_{w_0 \in B_0^d(s)}\widetilde E(\widehat w_n,w_0,r),
\end{eqnarray}
where $\widetilde E(w,w_0,r)$ is the (proxy) adversarial risk of the model $w$, as defined in \eqref{eq:Etilde}, and the infimum is taken over all estimators $\widehat w_n$ of $w_0$, based on the iid dataset $\mathcal D_n=\{(x_1,y_1),\ldots,(x_n,y_n)\}$ given in \eqref{eq:generative}. Let $X=(x_1,\ldots,x_n) \in \mathbb R^{n \times d}$ be the design matrix, and
define the following scalars
\begin{align}
\underline\theta(X,s) &:= \inf_{\delta \in B_0^d(s),\,\delta\ne 0} \dfrac{\|X\delta\|_2}{\sqrt{n}\|\delta\|_2}\label{eq:thetalow},\\
\overline\theta(X,s) &:= \sup_{\delta \in B_0^d(s),\,\delta\ne 0} \dfrac{\|X\delta\|_2}{\sqrt{n}\|\delta\|_2}\label{eq:thetahigh}.
\end{align}
In particular, $\overline\theta(X,1) = \max_{j \in [d]}\|Xe_j\|_2/\sqrt{n}$, where $e_j$ is the $j$th standard basis unit-vector in $\mathbb R^d$ so that $Xe_j \in \mathbb R^n$ is the $j$th column of $X$. Also, it should be clear that one always has the following estimates\footnote{As, a side note, these estimates can be arbitrarily loose.}
\begin{eqnarray}
\lambda_{min}(\widehat \Sigma) \le \underline\theta(X,s)^2 \le \overline\theta(X,s)^2 \le \lambda_{max}(\widehat \Sigma),
\end{eqnarray}
 where $\widehat \Sigma := X^\top X/n$ is the empirical covariance matrix as usual.
% \begin{restatable}{rmk}{}
Note that a condition of the form
\begin{eqnarray}
1-\delta_s \le \underline\theta(X,s) \le \overline\theta(X,s) \le  1+\delta_s
\end{eqnarray}
for some $\delta_s \in (0,1)$ is equivalent to a Restricted Isometry Property (RIP) for the rescaled design matrix $X/\sqrt{n}$. 
% \end{restatable}

Let $\lambda_{min} = \lambda_{min}(\Sigma)$ (resp. $\lambda_{max}=\lambda_{\max}(\Sigma)$) be the smallest (resp. largest) eigenvalue of the covariance matrix $\Sigma$. In what follows, we assume the attacker's norm is an $\ell_p$-norm for some $p \in [1,\infty]$. Let $q=q(p) \in [1,\infty]$ be the harmonic conjugate of $p$, i.e., $1/p + 1/q = 1$.

\subsection{Minimax Lower-Bounds}
\begin{restatable}{thm}{minimaxlb}
For any $p \in [2,\infty]$ and $s \in [1,d/2]$, the following minimax lower-bound on robustness error for $\ell_p$-norm attacks holds w.h.p over the noise vector $\epsilon \in \mathbb R^n$
\begin{eqnarray*}
\begin{split}
% &
\inf_{\widehat w_n}\sup_{w_0 \in B_0^d(s)}\frac{\widetilde E(\widehat w_n,w_0,r)}{\sigma_\epsilon^2}
% \\ &\quad\quad\quad
\gtrsim \frac{\log(ed/s)}{n \overline\theta(X,1)^2} (s\lambda_{min} \lor r^2 s^{2/q}).
% \begin{cases}
% r^2s^{2/q},&\mbox{ if }r\gtrsim \sqrt{\lambda_{min}/s^{2/q-1}},\\
% \lambda_{min}s,&\mbox{ else.}
% \end{cases}
\end{split}
\end{eqnarray*}
In particular, consistent $\ell_p$-norm adversarial regression in $B_0^d(s)$ can only happen if
$rs^{1/q}\sqrt{\log(ed/s)} = o(\sqrt n)$.
\label{thm:minimaxlb}
\end{restatable}

The result in proved in Appendix xyz. In the special case of $\ell_\infty$-norm attacks, we have the following corollary.
\begin{restatable}{cor}{}
If $1 \le s \le d/2$, then the following minimax lower-bound on robustness error for $\ell_\infty$-norm attacks holds w.h.p over the noise vector $\epsilon \in \mathbb R^n$
\begin{eqnarray}
\begin{split}
% &
\inf_{\widehat w_n}\sup_{w_0 \in B_0^d(s)} \frac{\widetilde E(\widehat w_n,w_0,r)}{\sigma_\epsilon^2}
% \\
% &\quad\quad\quad
\gtrsim  \frac{s\log(ed/s)}{n \overline\theta(X,1)^2} (\lambda_{min} \lor r^2 s) .
% \begin{cases}
% r^2s^2,&\mbox{ if }r \gtrsim \sqrt{\lambda_{min}/s},\\
% \lambda_{min}s,&\mbox{ else.}
% \end{cases}
\end{split}
\label{eq:minimaxlowerbound}
\end{eqnarray}
In particular, consistent $\ell_\infty$-norm adversarial regression in $B_0^d(s)$ can only happen if
$r s\sqrt{\log(ed/s)} = o(\sqrt n)$.
\end{restatable}

\subsection{Minimax Optimality of Proposed Estimator}
We will now show that our proposed two-stage estimator attains the minimax lower-bound in \eqref{eq:minimaxlowerbound}.

For any $c \ge 0$, define the nonnegative scalar
\begin{eqnarray}
\label{eq:theta}
\theta(X,s,c) := \inf_{\delta \in B^d_1(s,c)}\frac{\|X\delta\|_2}{\sqrt{n}\|\delta\|_2},
\end{eqnarray}
where $B^d_1(s,c) := \{\delta \in \mathbb R^d \mid 0 < \|\delta\|_1 \le (1+c)\sqrt{s}\|\delta\|_2\}$. Note that $B_0^d(s) \subseteq B_0^d(s,c)$ for all $c \ge 0$. The following technical condition was introduced in \cite{BickelSimultaneous2009} (see also \cite{BellecSlopeMeets2018}).
\begin{restatable}[Sparse Restricted Eigenvalue (SRE) condition]{cond}{sre}
\label{cond:sre}
$\overline\theta(X,1) = O(1)$ and $\theta(X,s,c) > 0$.
\end{restatable}
The following result is one of our main contributions.
\begin{restatable}[Minimax optimality of the square-root Lasso for robust learning]{thm}{minimax}
\label{thm:minimax}
Suppose Condition SRE$(s,7)$ is in order with $1 \le s \le d/2$.
Suppose the first stage of our two-stage estimator is the square-root Lasso (SQL) estimator $\widehat w_n^L(\lambda)$ with tuning parameter \begin{eqnarray}
\label{eq:lambdaoptlasso}
\lambda \asymp \sqrt{\dfrac{\log(2d/s)}{n}}.
\end{eqnarray}
Then our final estimator is minimax optimal in \eqref{eq:minimax}, uniformly for all $\ell_p$-norm attacks with $p \in [2,\infty]$.

In particular, in the noiseless case where $\sigma_\epsilon=0$, the OLS estimator (if it exists!), is minimax optimal uniformly on $p$.
\end{restatable}
% \textcolor{red}{Elvis: We probably need an estimator which doesn't require knowledge of the sparsity level $s$. This can be done via a so-called \emph{Lepski-type procedure} \url{https://arxiv.org/pdf/1703.02907.pdf}.}


==> sections/minimax_proofs.tex <==
\section{Minimax Theory}
\subsection{Proof of Theorem \ref{thm:minimaxlb}: Minimax Lower-Bound}
\minimaxlb*
\begin{proof}[Proof of Theorem \ref{thm:minimaxlb}]
It was shown in [Theorem 7.1, Bellec et al. 2018] \url{https://arxiv.org/pdf/1605.08651.pdf} that if $1 \le s \le d/2$, then 
\begin{eqnarray}
\Delta(s,q) := \inf_{\widehat w_n}\sup_{w_0 \in B_0^d(s)}\|\widehat w_n - w_0\|_q \gtrsim \frac{\sigma_\epsilon}{\overline\theta(X,1)}\cdot \psi(q),
\end{eqnarray}
holds w.h.p over the noise vector $\epsilon \in \mathbb R^n$, where
$\psi(s,q) :=  s^{1/q}\sqrt{\dfrac{\log(ed/s)}{n}}$.
Since $\|\widehat w_n - w_0\|_{\Sigma}^2 \ge \lambda_{\min}\|\widehat w_n - w_0\|_2^2$, we deduce from \eqref{eq:reconciled} that w.h.p and in expectation over the noise vector $\epsilon \in \mathbb R^n$,
\begin{eqnarray*}
\begin{split}
\inf_{\widehat w_n}\sup_{w_0 \in B_0^d(s)} \widetilde E_p(\widehat w_n,r)  &\gtrsim \sigma_\epsilon^2\cdot \max(\lambda_{\min}(\Sigma)\Delta(s,2)^2, r^2 \Delta(q,s)^2)\\
&\gtrsim \frac{\sigma_\epsilon^2\cdot}{\overline\theta(X,1)^2} \cdot \max(\lambda_{\min}(\Sigma)\psi(s,2)^2,r^2\psi(s,q)^2)\\
&= \frac{\sigma_\epsilon^2}{\overline\theta(X,1)^2}\cdot \frac{\log(ed/s)}{n}\cdot \max(\lambda_{\min}(\Sigma)s, r^2 s^{2/q}),
\end{split}
\end{eqnarray*}
which completes the proof.
% The first part of the result then follows upon noting that $r^2s^{2/q} \ge \lambda_{\min}\cdot s$ iff $r \ge \sqrt{\lambda_{\min}/s^{2/q-1}}$.
\end{proof}

\subsection{Minimax Optimality of Our Proposed Two-Stage Estimator}
Note the definition of $\theta(X,s,c)$ from \eqref{eq:theta} and recall the following condition
\sre*

We restate the theorem to be proved for convenience.
\minimax*
The following oracle bound which established in \cite{BellecSlopeMeets2018}, will be crucial to the proof.
\begin{restatable}[Corollary 4.3 of \cite{BellecSlopeMeets2018}]{prop}{}
Suppose Condition SRE$(X,s,7)$ is in order and the ground-truth model $w_0$ is $s$-sparse. Consider a Lasso estimator $\widehat w_n^L(\lambda)$ tuned with $\lambda \ge \lambda_{n,d,r,1/2}^\star$ where
\begin{eqnarray}
\lambda_{n,d,s,\gamma}^\star := \sigma_\epsilon\cdot \frac{4+\sqrt{2}}{\gamma}\sqrt{\frac{\log(2e d/s)}{n}},\text{ for all }\gamma \in (0,1).
\end{eqnarray}
Then, for any $1 \le q \le 2$, it holds w.h.p over  the noise vector $\epsilon \in \mathbb R^n$, the following holds for the Lasso estimator 
\begin{align}
    \|\widehat w_n^L(\lambda)-w_0\|_q &\lesssim \frac{ \lambda s^{1/q}}{\theta(X,s,7)^2}.
\end{align}
\label{prop:belleclasso}
\end{restatable}

The following result which is a corollary to Proposition \ref{prop:belleclasso} above, will be one of our main workhorses. 
\begin{restatable}{prop}{}
Suppose Condition SRE$(X,s,7)$ is in order and the ground-truth model $w_0$ is $s$-sparse. Let $p \in [2,\infty]$ and let $q=q(p) \in [1,2]$ be the harmonic conjugate of $p$. Consider an $\ell_p$-norm attack of magnitude $r \ge 0$.
Then, for any $\lambda \ge \lambda_{n,d,s,1/2}^\star$ (defined in Prop. \ref{prop:belleclasso}), it holds w.h.p over the noise vector $\epsilon \in \mathbb R^n$ that
\begin{eqnarray}
\widetilde E(\widehat w_n^L(\lambda),w_0,r) \lesssim  \frac{(s\lambda_{max} \lor r^2s^{2/q})\lambda^2}{\theta(X,s,7)^4}.
\label{eq:lassoEtilde}
\end{eqnarray}
\end{restatable}
\begin{proof}
Thanks to Proposition \ref{prop:belleclasso} above, the following hold w.h.p over the noise vector $\epsilon$
\begin{eqnarray*}
\begin{split}
&\widetilde E(\widehat w_n^L(\lambda),w_0,r) \asymp (\|\widehat w_n^L(\lambda)-w_0\|_{\Sigma} + r\|\widehat w_n^L(\lambda)-w_0\|_q)^2\\
&\quad\quad\le (\sqrt{\lambda_{max}}\|\widehat w_n^L(\lambda)-w_0\|_2+r\|\widehat w_n^L(\lambda)-w_0\|_q)^2\\
&\quad\quad\lesssim \left(\frac{\sqrt{\lambda_{max}}\cdot\lambda s^{1/2}}{\theta(X,s,7)^2} +  \frac{r\lambda s^{1/q}}{\theta(X,s,7)^2}\right)^2\\
&\quad\quad= \frac{\lambda^2(s\lambda_{max} \lor r^2 s^{2/q})}{\theta(X,s,7)^4},
\end{split}
\end{eqnarray*}
as claimed.
\end{proof}
We are now read to proof Theorem \ref{thm:minimax}.

\begin{proof}[Proof of Theorem \ref{thm:minimax}]
Indeed, with the choice of $\lambda$ given in \eqref{eq:lambdaoptlasso}, the upper-bound \eqref{eq:lassoEtilde} matches the minimax lower-bound \eqref{eq:minimaxlowerbound}, upto multiplicative absolute constants which only depend on the design matrix $X$, the covariance matrix $\Sigma$, and the noise level $\sigma_\epsilon$.
\end{proof}


==> sections/not_include/everything_else.tex <==
\section{Isotropic Case}
In that case, we propose to generalize the above strategy to any positive-definite matrix $M\in\mathcal{S}_d^{++}(\mathbb{R})$. More precisely, we consider the GD descent scheme applied to the following objective function:
\begin{align*}
    E_{M,\Sigma_x}(w):=\mathbb{E}_{(x,y)\sim P_{xy}}(w^T(M^{1/2}\Sigma_x^{-1/2}x)-y)^2
\end{align*}
which leads to the following GD path:
\begin{align*}
    w^{M,\Sigma_x}(t):= (I_d - (I_d - \alpha M)^t)M^{-1/2}\Sigma_x^{1/2}w_0\; , 
\end{align*}
and its continuous version:
\begin{align*}
    w^{M,\Sigma_x}_c(t):= (I_d - e^{-t M}) M^{-1/2}\Sigma_x^{1/2}w_0\;.
\end{align*}
Let us also also introduce the general condition number associated to $M\in\mathcal{S}_{d}^{++}(\mathbb{R})$ defined as
\begin{align*}
    \kappa^{\Vert\cdot\Vert}(M)&:=\lambda_{max}^{\Vert\cdot\Vert}(M)/\lambda_{min}^{\Vert\cdot\Vert}(M),\,\text{where }\\
    \lambda_{max}^{\Vert\cdot\Vert}(M)&:=\sup_{w\neq 0}\frac{\Vert M^{1/2}w\Vert_2^2}{\Vert \Sigma_x^{-1/2} w\Vert_*^2},\text{ and}\\
    \lambda_{min}^{\Vert\cdot\Vert}(M)&:=\inf_{w\neq 0}\frac{\Vert M^{1/2}w\Vert_2^2}{\Vert \Sigma_x^{-1/2} w\Vert_*^2}\; ,
\end{align*}


then we show the following Proposition.
\begin{prop}
For any $r\geq 0$ and $M\in\mathcal{S}_{d}^{++}(\mathbb{R})$, we have 
\begin{align*}
     \inf_{t \geq 0}E^{\Vert\cdot\Vert}(\Sigma_x^{-1/2}M^{1/2}w^{M,\Sigma_x}_c(t),r)\leq 1.68 \kappa^{\Vert\cdot\Vert}(M^{-1}) E^{\Vert\cdot\Vert}_{opt}(r)
\end{align*}
\end{prop}
Therefore along the GD schemes on the transformed data, one can find a $1.6862 \kappa^{\Vert\cdot\Vert}(M^{-1})$-optimally robust predictor. 

\begin{restatable}{assume}{}
There exists an absolute constants $\beta,\beta'$ such that $\beta' \le \|w\|_2 / \|\Sigma_x^{-1/2}w\|_\star \le \beta$  for all nonzero $w \in \mathbb R^d$.
\label{assume:coveringnumber}
\end{restatable}
% For example, in the isotropic case, i.e. $\Sigma_x=I_d$, the above assumption is satisfied with $\beta=1$, whenever the attacker's norm $\|\cdot\|$ is an $\ell_p$-norm with $p \in [2,\infty]$. On the other hand, if the attacker's norm $\|\cdot\|$ is induced by a positive-definite matrix $A$, then the condition is satisfied with $\beta=\|A\|_{op}$, the operator norm of $A$.
% This is because in this case, $\|\cdot\|_\star = \|\cdot\|_q$, where $q=q(p) \in [1,2]$ is the harmonic conjugate of $q$, and $\ell_q$ unit-ball is smaller than euclidean unit-ball (since $q \in [1,2]$), combined with the fact that the euclidean unit-ball has covering number of order $O(3/\epsilon)^d$.

Now, let $m$ be a positive integer and $G$ be an $m \times d$ random matrix with with iid entries from $N(0,1)$. Consider the Wishart random matrix $W_{rand}:=G^\top G$.
The following important lemma is proved in Appendix xyz.
\begin{restatable}{lm}{rmt}
Suppose  Assumption \ref{assume:coveringnumber} is in order. There exist absolute constant $C,\gamma \ge 1$ only depending on $\beta$ such that if $m/d \ge \gamma$, then $\kappa^{\|\cdot\|}(W_{rand}) \le C$ w.h.p.

In particular, it holds w.h.p that $W_{rand}$ is non-singular, and therefore positive-definite.
\label{lm:rmt}
\end{restatable}
Thus, normalizing with the inverse-Wishart random matrix $M_{rand} := W_{rand}^{-1}$ makes early-stopping optimal up to within an \emph{absolute} multiplicative constant!

\begin{thm}
Suppose  Assumption \ref{assume:coveringnumber} is in order. There exist absolute constant $C,\gamma \ge 1$ only depending on $\beta$ such that if $m/d \ge \gamma$, then w.h.p.
\begin{align*}
  \inf_{t \geq 0}E^{\Vert\cdot\Vert}(\Sigma_x^{-1/2}M_{rand}^{1/2}w^{M_{rand},\Sigma_x}_c(t),r)\leq 1.68 C E^{\Vert\cdot\Vert}_{opt}(r)
  \end{align*}
\end{thm}


\subsection{General / non-euclidean attacks}
Consider now the case where $\Sigma_x = \sigma^2 I_d$ but the attacker's norm $\|\cdot\|$ is not necessary euclidean. Note that $\mathcal C(\Sigma_x)$ is now the set of all positive-definite matrices of order $d$.
\begin{restatable}{assume}{}
There exists an absolute constant $\beta$ such that $\|w\|_2 \le \beta\|w\|_\star$ for all $w \in \mathbb R^d$.
\label{assume:coveringnumber}
\end{restatable}
For example, the above assumption is satisfied with $\beta=1$, whenever the attacker's norm $\|\cdot\|$ is an $\ell_p$-norm with $p \in [2,\infty]$. On the other hand, if the attacker's norm $\|\cdot\|$ is induced by a positive-definite matrix $A$, then the condition is satisfied with $\beta=\|A\|_{op}$, the operator norm of $A$.
% This is because in this case, $\|\cdot\|_\star = \|\cdot\|_q$, where $q=q(p) \in [1,2]$ is the harmonic conjugate of $q$, and $\ell_q$ unit-ball is smaller than euclidean unit-ball (since $q \in [1,2]$), combined with the fact that the euclidean unit-ball has covering number of order $O(3/\epsilon)^d$.

Now, let $m$ be a positive integer and $G$ be an $m \times d$ random matrix with with iid entries from $N(0,1)$. Consider the Wishart random matrix $W_{rand}:=G^\top G$.
The following important lemma is proved in Appendix xyz.
\begin{restatable}{lm}{rmt}
Suppose  Assumption \ref{assume:coveringnumber} is in order. There exist absolute constant $C,\gamma \ge 1$ only depending on $\beta$ such that if $m/d \ge \gamma$, then $\kappa^{\|\cdot\|}(W_{rand}) \le C$ w.h.p.

In particular, it holds w.h.p that $W_{rand}$ is non-singular, and therefore positive-definite.
\label{lm:rmt}
\end{restatable}
Thus, normalizing with the inverse-Wishart random matrix $M_{rand} := W_{rand}^{-1}$ makes early-stopping optimal up to within an \emph{absolute} multiplicative constant!
\section{A Simple Procedure: Normalization of the Data}


\subsection{Euclidean Attacks on Normalized Data}

\subsection{General Attacks on Normalized Data}


\section{Statistical Study}

\subsubsection{The case where $d=1$}
In the one dimensional setting we obtain the following result.
\begin{prop}
By denoting $\sigma^2$ the covariance of $x$, we obtain that
\begin{itemize}
    \item if $r\leq \sigma \sqrt{2/\pi}$, then $E(t,r)$ is a decreasing function with respect to $t$, in particular we have:
    \begin{align*}
         E(\infty,r)\leq  E(t,r)~~\forall t\geq 0~~\text{and}~~t_{\text{opt}}:=+\infty
    \end{align*}
    \item if $ \sigma \sqrt{2/\pi} < r < \sigma \sqrt{\pi/2}$, then $t\in\mathbb{R}_{+}\xrightarrow{} E(t,r)$ admits a unique mizimizer attained for 
    \begin{align*}
        t_{\text{opt}} := \frac{\log\left(\frac{r(r-\sigma\sqrt{2/\pi})}{\sigma^2 + r^2 - 2\sigma r\sqrt{2/\pi}}\right)}{\log(1-\alpha \sigma^2)}>0
    \end{align*}
    \item if $r\geq \sigma \sqrt{\pi/2}$, then $E(t,r)$ is an increasing function with respect to $t$, in particular we have:
    \begin{align*}
         E(0,r)\leq  E(t,r)~~\forall t\geq 0~~\text{and}~~t_{\text{opt}}:=0\;.
    \end{align*}
\end{itemize}
\label{prop:lowr}
\end{prop}
\begin{proof}\mytodo{Move proof to appendix and only sketch main idea here, mostly in words ?}
In that case we have that 
\begin{align*}
    E(t,r)&= (1 - \alpha \sigma^2)^{2t} \sigma^2  \Vert w_0\Vert^2 + r^2 [1 - (1-\alpha\sigma^2)^{t}]^2 \Vert w_0\Vert^2 \\
    &+ 2 r \sqrt{2/\pi} (1 - \alpha \sigma^2)^{t} \sigma [1 - (1-\alpha\sigma^2)^{t}]\Vert w_0\Vert^2
\end{align*}
which can be written as
\begin{align*}
     E(t,r)&= \Vert w_0\Vert^2[\beta_1 (1 - \alpha \sigma^2)^{2t} +\beta_2 (1 - \alpha \sigma^2)^{t} +\beta_3]
\end{align*}
where
$\beta_1:= [\sigma^2 + r^2 -  2 r \sqrt{2/\pi} \sigma]$, $\beta_2:=-2r^2 +2 r \sqrt{2/\pi}\sigma$ and $\beta_3:=r^2$. Therefore we obtain that
\begin{align*}
    \frac{\partial E}{\partial t}(t,r) = \Vert w_0\Vert^2 \log(1-\alpha \sigma^2)(1 - \alpha \sigma^2)^{t}[2\beta_1 (1 - \alpha \sigma^2)^{t} + \beta_2]
\end{align*}
which gives us that 
\begin{align*}
     \frac{\partial E}{\partial t}(t,r)\leq 0,~~\forall t\geq 0 &\iff \beta_2\geq 0\\
     &\iff r\leq \sqrt{2/\pi}\sigma\; ,
\end{align*}
\begin{align*}
     \frac{\partial E}{\partial t}(t,r)\geq 0,~~\forall t\geq 0 &\iff -\beta_2\geq 2\beta_1\\
     &\iff r\geq \sqrt{\pi/2}\sigma
\end{align*}
otherwise (meaning that $0 < -\beta_2 < 2\beta_1)$ $E$ admits a unique minimizer in $t_{\text{opt}} =\frac{\log(-\beta_2/2\beta_1)}{\log(1-\alpha\sigma^2)}$ from which follows the result.
\end{proof}
In the following proposition, we show that in fact the early-stopping strategy is robust optimal. In the following we denote  $$E^*_r:=\inf_{w \in \mathbb R^d}E(w,r) = \inf_{w\in\mathbb{R}^d}\mathbb{E}\sup_{\Vert \delta\Vert \leq r}(w^\top (x+\delta) - w_0^\top x)^2)$$
\begin{cor}
For all $r\geq 0$, we obtain that the early-stopping strategy is optimal
$E(t_{\text{opt}},r) = E^*_r$.

In particular, we obtain that
\begin{itemize}
    \item If $r\leq \sigma \sqrt{2/\pi}$, then $E(t_{\text{opt}},r) = r^2\Vert w_0\Vert^2$.
    \item If $ \sigma \sqrt{2/\pi} < r < \sigma \sqrt{\pi/2}$, then
    \begin{align*}
    E(t_{\text{opt}},r) =  r^2\Vert w_0\Vert^2  \frac{(1-2/\pi)\sigma^2}{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}.
\end{align*}
\item If $ r \geq \sigma \sqrt{\pi/2}$, then
%\begin{align*}
 $   E(t_{\text{opt}},r) = \Vert w_0\Vert_{\Sigma_x}^2$.
%\end{align*}
\end{itemize}
\end{cor}

\begin{remark}
Observe that the asymptotic regime (true solution of the OLS problem) is not optimal as soon as $r>\sigma \sqrt{2/\pi}$ and therefore early stopping becomes beneficial in this setting. More specifically, we have that if $ \sigma \sqrt{2/\pi} < r < \sigma \sqrt{\pi/2}$
\begin{align*}
   E(t_{\text{opt}},r)/ E(t_{\infty},r)= \frac{(1-2/\pi)\sigma^2}{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}\in]2/\pi,1[
\end{align*}
and if  $ r \geq \sigma \sqrt{\pi/2}$, we obtain that 
\begin{align*}
  E(t_{\text{opt}},r)/ E(t_{\infty},r)= \sigma^2/r^2\leq \frac{2}{\pi}
\end{align*}
Therefore the robust error of the true OLS solution can be arbitrarily large when the radius of the attack $r$ goes to infinity while early stopping is always optimal.   
\end{remark}

Let us now focus on the empirical regime where we have only access to $n\geq 1$ samples from the data distribution. Let us denote $(x_i,y_i)_{i=1}^n$ $n$ i.i.d samples where $x_1\sim\mathcal{N}(0,\Sigma_x)$, $y_1 = w_0^{T}x_1 +\epsilon_1$, $\epsilon_1\sim\mathcal{N}(0,\Sigma_\epsilon)$ and  $\epsilon_1\indep x_1$. In the following we denote $\widehat{\text{Cov}}(x,\epsilon) := \frac{1}{n}\sum_{i=1}^n \epsilon_i x_i$, $\widehat{\Sigma}_x: =\frac{1}{n}\sum_{i=1}^n x_ix_i^\top $, $\widehat{w}(t)=K_t(\widehat{\Sigma}_x)(\widehat{\Sigma}_x w_0+\widehat{\text{Cov}}(x,\epsilon))$ and $\gamma_n:= \widehat{\Sigma}_x^{-1}\widehat{\text{Cov}}(x,\epsilon)$. Let us now present our main result. As we deal with the one dimensional case, we will also denote $\widehat{\sigma}^2:=\widehat{\Sigma}_x$. We have exhibited three regimes which covers all the possible behaviors in the next three following Proposition.


We have an upper-bound control of the tails of $\gamma_n$ as follows.
\begin{prop}
Let $\delta>0$, then as soon as $n>4\log(1/\delta)$ there exists a universal constant $K>0$ such that for all
\begin{align*}
   t\leq \frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})}
\end{align*}

we have that
\begin{align*}
    \mathbb{P}(\gamma_n\geq t)\leq \exp\left(-Knt^2\frac{(1-2\sqrt{log(1/\delta)})^2}{\sigma_\epsilon^4}\right) + \delta
\end{align*}
In particular, as soon as $n>\log(1/\delta)\max(4,1/K)$, then with a probability $\geq 1-2\delta$, we have
\begin{align*}
\gamma_n \leq \sqrt{\frac{\log(1/\delta)}{Kn}}\frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})}
\end{align*}
\end{prop}
\begin{proof}

\end{proof}

% \begin{restatable}{lm}{}
% $|\gamma_n| = o_n(1)$ w.p $1-o_n(1)$.
% \end{restatable}
% \begin{proof}
% Indeed, it is well-known result in classical statistics that, because the dimension is fixed, $\widehat\sigma^2 = \sigma^2+o_{n,\mathbb P}(1)$\footnote{Alternative, a self-contained proof of this fact can be given by direct concentration arguments}. Now, let $z_n:= \frac{1}{n}\sum_{i=1}^n \epsilon_i x_i$. Note that the variance of $z_n$ is $\sigma^2\cdot\sigma_\epsilon^2/n$. A direct application of Chebychev's inequality gives
% $$
% \left|z_n\right| \le t \text{ w.p }1-\frac{\sigma^2\sigma_\epsilon^2}{nt^2}.
% $$
% Taking $t=\sigma\sigma_\epsilon\sqrt{(\log n)/n}$, we deduce that $|z_n| \le \sqrt{(\log n)/n}=o_n(1)$ w.p $1-1/\log n=o_n(1)$.
% \end{proof}
% Note that the confidence in the above lemma can be increased to $1-1/n^c$ (with $c=\Omega(1)$), but $1-1/\log n = o_n(1)$ will suffice for our purposes.

\begin{prop}
Assume that  $\gamma_n\geq 0$, then we obtain that
\begin{itemize}
    \item if $r\in[0,\sigma\sqrt{2/\pi}]$, then $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in
    \begin{align*}
        \hat{t}_{opt} := \frac{\log(\gamma_n/(\gamma_n+\Vert w_0\Vert_2))}{\log(1-\alpha \widehat{\sigma}^2)}>0~~\text{and}~~
        E(\widehat{w}(\hat{t}_{opt}),r) = r^2\Vert w_0\Vert^2
    \end{align*}
    \textcolor{red}{Elvis: Note that $\hat t_{opt} = \omega_{n,\mathbb P}(1)$ since $\gamma_n = o_{n,\mathbb P}(1)$.}
    \item if $r\in]\sigma\sqrt{2/\pi},\sigma\sqrt{\pi/2}[$, then $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in
      \begin{align*}
       & \hat{t}_{opt} := \frac{\log\left(\frac{r^2(\Vert w_0\Vert+\gamma_n)+\sigma^2\gamma_n - r\sqrt{2/\pi}\sigma (\Vert w_0\Vert +2\gamma_n)}{(c+\gamma_n)(\sigma^2 + r^2 - 2r\sqrt{2/\pi}\sigma)}\right)}{\log(1-\alpha \widehat{\sigma}^2)}>0~~\text{and}\\
        &E(\widehat{w}(\hat{t}_{opt}),r) = r^2\Vert w_0\Vert^2  \frac{(1-2/\pi)\sigma^2}{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}
    \end{align*}
    \item if $r\geq\sigma\sqrt{\pi/2} $, then $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in 
     \begin{align*}
        \hat{t}_{opt} := 0~~\text{and}~~
        E(\widehat{w}(\hat{t}_{opt}),r) = \Vert w_0\Vert_{\Sigma_x}^2\;.
    \end{align*}
\end{itemize}
\end{prop}

\begin{prop}
Assume that $\gamma_n\in[-\Vert w_0\Vert,0[$, and let us denote $$\sigma \sqrt{\pi/2}\geq \tilde{r}(\gamma_n):=\frac{2\sqrt{2/\pi}\sigma\left[(\Vert w_0\Vert+2\gamma_n)+\sqrt{\Vert w_0\Vert^2 - (2\pi-4)\gamma_n(\Vert w_0\Vert +\gamma_n)}\right]}{4(\Vert w_0\Vert +\gamma_n)}\geq \sigma\sqrt{2/\pi}.$$ \textcolor{red}{Elvis: Note that $\tilde{r}(\gamma_n) = \sigma\sqrt{2/\pi}+o_{n,\mathbb P}(1)$.} Then we obtain that
\begin{itemize}
    \item  if  $r\in[0,\tilde{r}(\gamma_n)]$ then $t\xrightarrow{} E(\widehat{w}(t),r)$ is a decreasing function, in particular we have that $\hat{t}_{opt} := +\infty$ and 
   \begin{align*}
        E(\widehat{w}(\hat{t}_{opt}),r) = \sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n \textcolor{red}{= r^2\Vert w_0\Vert^2 + o_{n,\mathbb P}(1)}.
    \end{align*}
\item if $r\in]\tilde{r}(\gamma_n), \sigma \sqrt{\pi/2}[$ then $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in 
 \begin{align*}
       & \hat{t}_{opt} := \frac{\log\left(\frac{r^2(\Vert w_0\Vert+\gamma_n)+\sigma^2\gamma_n - r\sqrt{2/\pi}\sigma (\Vert w_0\Vert +2\gamma_n)}{(c+\gamma_n)(\sigma^2 + r^2 - 2r\sqrt{2/\pi}\sigma)}\right)}{\log(1-\alpha \widehat{\sigma}^2)}>0~~\text{and}\\
        &E(\widehat{w}(\hat{t}_{opt}),r) = r^2\Vert w_0\Vert^2  \frac{(1-2/\pi)\sigma^2}{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}
    \end{align*}
\item if $r\geq  \sigma \sqrt{\pi/2}$, then $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in 
     \begin{align*}
        \hat{t}_{opt} := 0~~\text{and}~~
        E(\widehat{w}(\hat{t}_{opt}),r) = \Vert w_0\Vert_{\Sigma_x}^2\;.
    \end{align*}
\end{itemize}
\end{prop}

\begin{prop}
Assume that $\gamma_n<-\Vert w_0\Vert$, then for all $r\geq 0$, $t\xrightarrow{} E(\widehat{w}(t),r)$ admits a unique minimizer in 
     \begin{align*}
        \hat{t}_{opt} := 0~~\text{and}~~
        E(\widehat{w}(\hat{t}_{opt}),r) = \Vert w_0\Vert_{\Sigma_x}^2\;.
    \end{align*}
\end{prop}

Let us now study the optimality of this estimator.
\begin{prop}
We have the following results:
\begin{itemize}
\item If $\gamma_n\geq 0$, then for all $r\geq 0$, we have that 
$$E(\widehat{w}(\hat{t}_{opt}),r) = E^{*}_r\; , $$
\item If $\gamma_n\in[-\Vert w_0\Vert,0[$ and $r>\tilde{r}(\gamma_n)$ we have that 
$$E(\widehat{w}(\hat{t}_{opt}),r) = E^{*}_r\; , $$
\item If $\gamma_n< -\Vert w_0\Vert$ and $r\geq \sigma\sqrt{\pi/2}$ we have that  $$E(\widehat{w}(\hat{t}_{opt}),r) = E^{*}_r\; .$$
\end{itemize}
meaning that under these conditions the empirical estimator obtained using an early-stopping strategy on the test robust error is optimally robust.
\end{prop}
\begin{remark}
It is worth noting that
\begin{align*}
    \tilde{r}(\gamma_n)\xrightarrow[\gamma_n\xrightarrow{}_{-} 0]{} \sigma\sqrt{2/\pi}~~\text{and}~~\tilde{r}(\gamma_n)\xrightarrow[\gamma_n\xrightarrow{}_{+} -\Vert w_0\Vert]{} \sigma \sqrt{\pi/2}
\end{align*}
\end{remark}

We can also quantify in the left regimes, how far is the error of the empirical estimator using early-stopping from the optimally robust error $E^{*}_r$.  

\begin{prop}
If $\gamma_n\in[-\Vert w_0\Vert,0[$, then
     \begin{itemize}
        \item if $r\in[0,\sigma\sqrt{2/\pi}]$, then 
        \begin{align*}
            E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r &= \frac{\sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n}{r^2\Vert w_0\Vert^2} \\
            &\geq 1+(\pi/2 -1)\frac{\gamma_n^2}{\Vert w_0\Vert^2}
        \end{align*}
        \item if $r\in]\sigma\sqrt{2/\pi},\tilde{r}(\gamma_n)]$, then 
                \begin{align*}
                1 \leq E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r\leq  1+(\pi/2 -1)\frac{\gamma_n^2}{\Vert w_0\Vert^2}\textcolor{red}{=1+o_{n,\mathbb P}(1)}.
        \end{align*}
     where $$E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r = (\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}) \frac{ \sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n}{ r^2\Vert w_0\Vert^2 (1-2/\pi)\sigma^2}$$
    \end{itemize}


% \begin{itemize}
%     \item if $\sigma^2\geq 1/2$ then:
%     \begin{itemize}
%         \item if $r\in[0,\tilde{r}(\gamma_n)]$, then 
%         \begin{align*}
%             E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r = \frac{\sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n}{r^2\Vert w_0\Vert^2}\textcolor{red}{=1+o_{n,\mathbb P}(1)}. 
%         \end{align*}
%         \item if $r\in]\tilde{r}(\gamma_n),\sigma\sqrt{2/\pi}]$, then 
%             \begin{align*}
%         1 \leq E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r =\frac{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}{(1-2/\pi)\sigma^2} 
%         \end{align*}
%     \end{itemize}
%     \item if $\sigma^2<1/2$ then:
%      \begin{itemize}
%         \item if $r\in[0,\sigma\sqrt{2/\pi}]$, then 
%         \begin{align*}
%             E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r &= \frac{\sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n}{r^2\Vert w_0\Vert^2} \\
%             &\geq 1+(\pi/2 -1)\frac{\gamma_n^2}{\Vert w_0\Vert^2}
%         \end{align*}
%         \item if $r\in]\sigma\sqrt{2/\pi},\tilde{r}(\gamma_n)]$, then 
%                 \begin{align*}
%                 1 \leq E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r\leq  1+(\pi/2 -1)\frac{\gamma_n^2}{\Vert w_0\Vert^2}\textcolor{red}{=1+o_{n,\mathbb P}(1)}.
%         \end{align*}
%      where $$E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r = (\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}) \frac{ \sigma^2\gamma_n^2+r^2(\Vert w_0\Vert+\gamma_n)^2 - 2r\sqrt{2/\pi}\sigma(\Vert w_0\Vert+\gamma_n)\gamma_n}{ r^2\Vert w_0\Vert^2 (1-2/\pi)\sigma^2}$$
%     \end{itemize}
% \end{itemize}
\end{prop}


We have also that:
\begin{prop}
If $\gamma_n < -\Vert w_0\Vert$, then
\begin{itemize}
    \item if $r\in[0,\sigma\sqrt{2/\pi}]$, then we have
    \begin{align*}
        E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r = \frac{\sigma^2}{r^2}\geq \pi/2
    \end{align*}
    \item if $r\in]\sigma\sqrt{2/\pi},\sigma\sqrt{\pi/2}[$, then 
        \begin{align*}
        1 \leq  E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r = \frac{\sigma^2}{r^2} 
        \frac{\sigma^2 + r^2-2r\sigma\sqrt{2/\pi}}{(1-2/\pi)\sigma^2}\leq \frac{\pi}{2}
    \end{align*}
\end{itemize}
\end{prop}

In the next Proposition we quantify the optimality of the early-stopping estimator in probability.
\begin{prop}
Let $\delta>0$, then we obtain that
\begin{itemize}
    \item if $r \geq \sigma \sqrt{\pi/2}$, then for all $n\geq 1$, $\widehat{w}(\hat{t}_{opt})$ is optimally robust a.s. meaning that
    $$ E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r  = 1 ~~\text{a.s.}$$
   \item  if $ \sigma \sqrt{2/\pi} < r < \sigma \sqrt{\pi/2}$, then for $n\geq N_1(\delta,K,\sigma_\epsilon,\Vert w_0\Vert)$, we have that with probability $\geq 1-2\delta$
 
   \begin{align*}
        E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r \leq 1 + \sqrt{\frac{\pi-2}{2}}  \sqrt{\frac{\log(1/\delta)}{Kn}}\frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})}
   \end{align*}
%   \begin{itemize}
%       \item if $\sigma \sqrt{2/\pi} < r < \sigma \sqrt{2/\pi}+\epsilon$,
%       then with proba s.t. $\tilde{r}(\gamma_n)\leq \sigma \sqrt{2/\pi}+\epsilon$, $-\Vert w_0\Vert_2<\gamma_n<0$ and 
%   $$1+(\pi/2 -1)\frac{\gamma_n^2}{\Vert w_0\Vert^2}\leq E_1$$
%     \item (compute $\tilde{r}(\gamma_n)\leq \sigma \sqrt{2/\pi}+\epsilon$) then with proba  if $r>\sigma \sqrt{2/\pi}+\epsilon$, it is optimal.
%   \end{itemize}
    \item if $r \leq\sigma \sqrt{2/\pi} $, then for $n\geq N_2(\delta,K,\sigma_\epsilon,\Vert w_0\Vert)$  we have that with probability $\geq 1-2\delta$
   \begin{align*}
        E(\widehat{w}(\hat{t}_{opt}),r)/E^{*}_r &\leq 1 +  \frac{2(\sqrt{2/\pi}\sigma-r)}{r\Vert w_0\Vert} \sqrt{\frac{\log(1/\delta)}{Kn}}\frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})}  \\ + &\left(\sqrt{\frac{\log(1/\delta)}{Kn}}\frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})}\right)^2 \frac{r^2+\sigma^2-2r\sqrt{2/\pi}\sigma}{r^2\Vert w_0\Vert^2} 
   \end{align*}
\end{itemize}
\end{prop}
\begin{proof}
Denotes $C(\delta,n,\sigma_\epsilon):=\sqrt{\frac{\log(1/\delta)}{Kn}}\frac{\sigma_\epsilon^2}{(1-2\sqrt{\log(1/\delta)/n})} $, then 
 $N_1(\delta,K,\sigma_\epsilon,\Vert w_0\Vert)$ has to be chosen as the smallest integer $n\geq 1$ such that $n\geq \log(1/\delta)\max(4,1/K)$, $C(\delta,n,\sigma_\epsilon)\leq \Vert w_0\Vert$ and such that $\frac{\sqrt{\Vert w_0\Vert^2 + 2\Vert w_0\Vert(\pi-2)(\Vert w_0\Vert -C(\delta,n,\sigma_\epsilon))C(\delta,n,\sigma_\epsilon)} - \Vert w_0\Vert}{2(\Vert w_0\Vert - C(\delta,n,\sigma_\epsilon))}\leq \frac{\pi-2}{2}$.
 In order to choose  $N_2(\delta,K,\sigma_\epsilon,\Vert w_0\Vert)$, we just require that $n\geq\log(1/\delta) \max(4,1/K)$ and $C(\delta,n,\sigma_\epsilon)\leq \Vert w_0\Vert$.
\end{proof}


\subsection{The case when $d>1$}
In this setting, a simple extension from the 1D case would be to consider $\Sigma_x=\sigma^2\text{Id}_d$ with $\sigma>0$. In that case, we recover the same results as the one obtained in the one dimensional case, meaning that the the early-stopping strategy is optimally robust in population. However in the general case, it may happens that $t\mapsto E_r(w(t),r)$ admits multiple local minima in the population regime, and therefore early-stopping would not be able to recover the global minimizer. In order to alleviate this issue, we propose to normalize the data using the covariance matrix. Assume for now that we are given the covariance matrix $\Sigma_x$ and let us denote $z:=\Sigma_x^{-1/2}x\sim\mathcal{N}(0,\text{Id})$, and $\widetilde{w}_0: = \Sigma_x^{1/2}w_0$, then observe that the model becomes $y=z^\top(\widetilde{w}_0)+\epsilon$. We will also denote in the following the normalized standard risk as
\begin{align*}
    E_{\text{norm}}(w):= \mathbb{E}[(z^\top w - y)^2]
\end{align*}
and $(w_{\text{norm}}(t))_{t\geq 0}$, the sequence produced by the GD scheme on $E_{\text{norm}}$. Let us also denote the adversarial risk on the normalized data as
\begin{align*}
    E_{\text{norm}}(w,r) = \mathbb{E}(\sup_{\Vert \delta\Vert \leq r}(w^\top (z+\delta) - \widetilde{w}_0^\top z)^2).
\end{align*}
First observe that the early stopping strategy on $(w_{\text{norm}}(t))_{t\geq 0}$ is optimally robust w.r.t to $E_{\text{norm}}(w,r)$, meaning that $E_{\text{norm}}(w_{\text{norm}}(t),r)$ admits at most one global minimizer and 
 $$\inf_{t\geq 0} E_{\text{norm}}(w_{\text{norm}}(t),r) = \inf_{w\in\mathbb{R}^d}  E_{\text{norm}}(w,r)\; .$$
Let us now study the robustness of such predictor on the adversarial risk of the true data. 
% Indeed let us first introduce the following result.
% \begin{lm}
% For all $w\in\mathbb{R}^d$, we have that
% \begin{align*}
%     E(w,r) =  E_{\text{norm},\Vert\cdot\Vert_{\Sigma_x}}(\Sigma_x^{1/2}w)
% \end{align*}
% In particular we have that
% \begin{align*}
%     E_r^{*}= \inf_{w\in\mathbb{R}^d}E_{\text{norm},\Vert\cdot\Vert_{\Sigma_x}}(w)
% \end{align*}
% \end{lm}
More precisely, we want to study the optimality of $(\Sigma_x^{-1/2}w_{\text{norm}}(t))_{t\geq 0}$ w.r.t $E(w,r)$. In fact we have the following proposition.
\begin{prop}
We have that
\begin{itemize}
    \item if $r\leq\frac{\sqrt{2/\pi}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert}$, then $t\mapsto  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)$ is a non-increasing function. In particular we have 
    \begin{align*}
        \inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r) = r^2\Vert w_0\Vert^2 ~~\text{and}~~t_{opt}=+\infty
    \end{align*}
     \item if $\frac{\sqrt{2/\pi}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert}\leq r\leq \frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert}$, then $t\mapsto  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)$ admits a unique minimizer. In particular we have 
    \begin{align*}
        \inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r) = \frac{r^2\Vert w_0\Vert^2  \Vert w_0\Vert_{\Sigma_x}^2(1-2/\pi)}{r^2\Vert w_0\Vert^2 +\Vert w_0\Vert_{\Sigma_x}^2 - 2r\sqrt{2/\pi}\Vert w_0\Vert\Vert w_0\Vert_{\Sigma_x}}
    \end{align*}
    and
        \begin{align*}
        t_{\text{opt}}= \frac{\log\left(\frac{r\Vert w_0\Vert(r\Vert w_0\Vert -\sqrt{2/\pi} \Vert w_0\Vert_{\Sigma_x})}{\Vert w_0\Vert_{\Sigma_x}^2 + r^2\Vert w_0\Vert^2 -2r\sqrt{2/\pi}\Vert w_0\Vert \Vert w_0\Vert_{\Sigma_x}}\right)}{\log(1-\alpha)}
    \end{align*}
     \item if $r\geq \frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert}$, then $t\mapsto  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)$ is a non-decreasing function. In particular we have 
    \begin{align*}
        \inf_{t\geq 0} E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r) = \Vert w_0\Vert^2_{\Sigma_x} ~~\text{and}~~t_{opt}=0
    \end{align*}
\end{itemize}
\end{prop}
In the following proposition we study the optimality of our proposed procedure.
\begin{prop}
We have that for all $r\geq 0$, 
\begin{align*}
    E_r^{*} \leq \inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r) \leq E_{r\sqrt{\Vert \Sigma_x\Vert_{\text{op}}\Vert \Sigma_x^{-1}\Vert_{\text{op}}}}^{*}
\end{align*}
In particular we obtain that
\begin{itemize}
    \item if $r\leq\frac{\sqrt{2/\pi}\Vert w_0\Vert}{\Vert w_0\Vert_{\Sigma_x^{-1}}}$, then we have that
    \begin{align*}
          E_r^{*} = \inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)
    \end{align*}
   
   \item if $\frac{\sqrt{2/\pi}\Vert w_0\Vert}{\Vert w_0\Vert_{\Sigma_x^{-1}}} \leq r\leq  \frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x^2}}{\Vert w_0\Vert_{\Sigma_x}}$, then we have that
       \begin{align*}
      1 \leq \frac{\inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)}{E_r^{*}}\leq \Vert \Sigma_x\Vert_{\text{op}}\Vert \Sigma_x^{-1}\Vert_{\text{op}}
    \end{align*}
   
    % \item if  $\frac{\sqrt{2/\pi}\Vert w_0\Vert}{\Vert w_0\Vert_{\Sigma_x^{-1}}}<r<\frac{\sqrt{2/\pi}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert_{\Sigma_x}}$, then we have that
    % \begin{align*}
    %     1 \leq \frac{\inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)}{E_r^{*}} \leq \Vert \Sigma_x\Vert_{\text{op}}\Vert \Sigma_x^{-1}\Vert_{\text{op}}
    % \end{align*}
    
    % \item if $ \frac{\sqrt{2/\pi}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert_{\Sigma_x}} \leq r \leq  \frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert_{\Sigma_x}}$, then we obtain that
    
    % \item  if $\frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x}}{\Vert w_0\Vert_{\Sigma_x}} \leq r < \frac{\sqrt{2/\pi}\Vert w_0\Vert_{\Sigma_x^2}}{\Vert w_0\Vert_{\Sigma_x}}$, then we obtain that
    
    
    \item if $r\geq \frac{\sqrt{\pi/2}\Vert w_0\Vert_{\Sigma_x^2}}{\Vert w_0\Vert_{\Sigma_x}}$, then we have that
       \begin{align*}
          E_r^{*} = \inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)
    \end{align*}
\end{itemize}
\end{prop}
\begin{proof}
Observe that for all $w\in\mathbb{R}^d$, we have that
\begin{align*}
    E_{\text{norm}}(w,r) &= \Vert \Sigma_x^{-1/2}w - w_0\Vert_{\Sigma_x}^2 + r^2\Vert \Sigma_x^{-1/2}w\Vert_{\Sigma_x}^2 \\
    &+2r\sqrt{2/\pi} \Vert \Sigma_x^{-1/2}w - w_0\Vert_{\Sigma_x}\Vert \Sigma_x^{-1/2}w\Vert_{\Sigma_x}
\end{align*}
and recall that we have $$\sqrt{\lambda_{\text{min}}}\Vert w\Vert \leq \Vert w \Vert_{\Sigma_x}\leq \sqrt{\lambda_{\text{max}}}\Vert w\Vert $$
where we have denoted $\lambda_{\text{min}}:=1/\Vert \Sigma_x^{-1}\Vert_{\text{op}}$ and $\lambda_{\text{max}}:=\Vert \Sigma_x\Vert_{\text{op}}$.
Therefore we obtain that for all $w\in\mathbb{R}^d$
\begin{align*}
 E(\Sigma_x^{-1/2}w,\sqrt{\lambda_{\text{min}}}r)  \leq  E_{\text{norm}}(w,r)\leq E(\Sigma_x^{-1/2}w,\sqrt{\lambda_{\text{max}}}r).
\end{align*}
In addition recall that for all $r'\geq 0$ we have 
\begin{align*}
    \inf_{w\in\mathbb{R}^d}E_{\text{norm}}(w,r') = \inf_{t\geq 0}E_{\text{norm}}(w_{\text{norm}}(t),r') 
\end{align*}
from which follows that
\begin{align*}
 E_r^{*}\leq \inf_{t\geq 0}E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r) &\leq \inf_{t\geq 0}E_{\text{norm}}(w_{\text{norm}}(t),r/\sqrt{\lambda_{\text{min}}}) \\
 &\leq  \inf_{w\in\mathbb{R}^d}E_{\text{norm}}(w,r/\sqrt{\lambda_{\text{min}}})\\
 &\leq E_{\sqrt{\lambda_{\text{max}}/\lambda_{\text{min}}}r}^*
\end{align*}
% Then we have that
% \begin{align*}
%   \frac{\inf_{w\in\mathbb{R}^d}E_{\text{norm}}(w,r)}{\max(1,\Vert \Sigma_x\Vert_{\text{op}})}  \leq E_r^{*}:=\inf_{w\in\mathbb{R}^d}E(w,r)\leq \frac{\inf_{w\in\mathbb{R}^d}E_{\text{norm}}(w,r)}{\min(1,1/\Vert \Sigma_x^{-1}\Vert_{\text{op}})}
% \end{align*}
% Therefore we obtain that
% \begin{align*}
%     \inf_{t\geq 0}E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r)&\leq \frac{\inf_{t\geq 0}E_{\text{norm}}(w_{\text{norm}}(t),r)}{\min(1,1/\Vert \Sigma_x^{-1}\Vert_{\text{op}})}\\
%     &\leq \frac{\inf_{w\in\mathbb{R}^d}E_{\text{norm}}(w,r)}{\min(1,1/\Vert \Sigma_x^{-1}\Vert_{\text{op}})}\\
%     &\leq  \frac{\max(1,\Vert \Sigma_x\Vert_{\text{op}})}{\min(1,1/\Vert \Sigma_x^{-1}\Vert_{\text{op}})} E_r^{*}
% \end{align*}
\end{proof}
The above Proposition shows that for all $r\geq 0$, there exists $r'$ such that
\begin{align*}
     \sqrt{\frac{\lambda_{\text{min}}}{\lambda_{\text{max}}}} r\leq r'\leq r~~~\text{and}~~\inf_{t\geq 0}  E(\Sigma_x^{-1/2}w_{\text{norm}}(t),r') = E_r^{*}
\end{align*}
Therefore the early-stopping strategy with normalized data is able to recover exactly the optimally robust predictor which requires to solve the above equation. In order to alleviate this issue, we propose instead a simple predictor where we choose the radius of the attack on the normalized data to be exactly the same as the one on the true data, meaning that we consider here $r'=r$. By doing so, that we show that early-stopping is both optimally robust  with respect to $\ell_2$ attacks on the normalized data (i.e.  $E_{\text{norm}}$) uniformly on $r$ and almost optimally robust on $\ell_2$ attacks on the unormalized data (i.e. $E$) uniformly on $r$ as soon as the problem is well conditioned. 


In order to obtain an estimator of such predictors we simply propose to use an empirical estimator of the covariance matrix using half of the dataset $\widehat{\Sigma}_x:= \frac{2}{n}\sum_{i=1}^{\lfloor n/2 \rfloor} x_ix_i^T$. Then, we can perform a GD descent scheme with an early stopping strategy on the left points, namely $(\widehat{\Sigma}_x^{-1/2} x_i,y_i)_{i=1}^{\lceil n/2 \rceil}$, and show that this strategy is with high probability almost optimally robust. 



\section{Robustness via shrinkage to zero}
\mytodo{Link the ideas presented hereunder to the so-called "Stein shrinkage" \url{http://proceedings.mlr.press/v32/muandet14.pdf}}

In the particular case where $M=I_d$, we obtain that $A_M=\Sigma_x^{-1/2}$ and we can write the updates of GD scheme as follows:
\begin{align*}
    w^{I_d}(t):= (1 - (1 - \alpha)^t)\Sigma^{1/2}w_0\; .
\end{align*}
This scheme corresponds to apply a GD scheme on the normalized data, i.e. on the following objective 
\begin{align*}
    E_{I_d}(w)=\mathbb{E}_{(x,y)\sim P_{xy}}(w^T(\Sigma_x^{-1/2} x)-y)^2\; .
\end{align*}
Therefore by considering the following path $(A_{I_d} w^{I_d}(t))_{t\geq 0}$, the proposed GD scheme is drawing all the predictors on the chord $[0,w_0] := \{\beta w_0 \mid \beta \in [0, 1]\}$ that joins $w_0$ to the origin. In the following, we focus on the robustness of such predictors.

\subsection{Optimizing over a chord}
We set $c_0:=\sqrt{2/\pi}$. Consider the problem of minimizing the robust risk $w \mapsto E^{\Vert\cdot\Vert }(w,r)$ over $[0,w_0]$. Now, for any $\beta \in [0, 1]$, one has
\begin{align*}
E^{\Vert\cdot\Vert}(\beta w_0,r) &= (1-\beta)^2\|w_0\|_{\Sigma_x}^2  + \beta^2r^2\|w_0\|_\star^2 \\
&+ 2c_0\beta(1-\beta)r\|w_0\|_{\Sigma_x}\|w_0\|_\star \\
&= a\beta^2 - 2b\beta + c,
\end{align*}
a quadratic polynomial in $\alpha$ with coefficients $a=a(w_0,r) := \|w_0\|_{\Sigma_x}^2 + r^2\|w_0\|_\star^2 - 2c_0r\|w_0\|_{\Sigma_x}\|w_0\|_\star$, $b=b(w_0,r) := \|w_0\|_{\Sigma_x}^2-c_0r\|w_0\|_{\Sigma_x}\|w_0\|_\star$, and $c=c(w_0,r) = \|w_0\|_{\Sigma_x}^2$. On the other hand, it is clear that the leading coefficient $a(w_0,r)$ is itself a quadratic in $r$ with discriminant $\|w_0\|_\Sigma^2\|w_0\|_\star^2(c_0^2-1)$ which is strictly negative because $c_0^2 = 2/\pi < 1$. Thus, $\beta \mapsto E^{\Vert\cdot\Vert}(\beta w_0, r)$ is a convex one-dimensional quadratic function. Therefore a simple early-stopping strategy is able to capture its minimum. 


Let us now focus on the robustness of such the minimizer of this specific path. First, we observe that this function is minimized at $\beta_{opt}(w_0,r)$ the unique point of $[0,1]$ which is closest to the real number $\widetilde\beta_{opt}(w_0,r) \in \mathbb R$ defined by
\begin{align*}
\widetilde\beta_{opt}(w_0,r) := \frac{\|w_0\|_{\Sigma_x}^2-c_0r\|w_0\|_{\Sigma_x}\|w_0\|_\star}{\|w_0\|_{\Sigma_x}^2 + r^2\|w_0\|_\star^2 - 2c_0r\|w_0\|_{\Sigma_x}\|w_0\|_\star}.
\end{align*}

% \begin{restatable}{lm}{}
% For any fixed $z \in \mathbb R^d$, it holds that
% \begin{eqnarray}
% \lim_{r \to 0^+}\widetilde\alpha_{opt}(z,r) = 1,\,\lim_{r \to \infty}\widetilde\alpha_{opt}(z,r) = 0.
% \end{eqnarray}
% Moreover, if $\|\cdot\|_\star = \|\cdot\|_\Sigma$ (i.e if the attacker's norm is $\|\cdot\|_{\Sigma{-1}}$), then
% \begin{eqnarray}
% \widetilde\alpha_{opt}(z,r) = (1-c_0 r) / (1+r^2-2c_0r).
% \end{eqnarray}
% \end{restatable}

% \begin{restatable}{rmk}{}
% In isotropic case, we know from Prop \ref{prop:normalized} that the minimizer of the normalized energy $w \mapsto E(w,r)$ is $w_{opt}(r) = (1+\lambda_{opt}(r))^{-1} w_0$,
% where $\lambda_{opt}(r)$ is given in \eqref{eq:lambdaopt}. This is consistent with the above lemma as one easily verifies that for $c_0 < r < 1/c_0$, 
% $$
% (1+\lambda_{opt}(r))^{-1} = ((r^2+1-2c_0 r)/(1-c_0r))^{-1} = (1-c_0r)/(1+r^2-2c_0 r) = \alpha_{opt}(r).
% $$
% \end{restatable}

Now, define $r_0(w_0)$, $r_1(w_0)$, and $r_2(w_0)$ by 
\begin{align*}
r_0(w_0)&:=\frac{\|w_0\|_{\Sigma_x}}{\|w_0\|_\star},\, r_1(w_0):=c_0r_0(w_0),\,\\
r_2(w_0)&:= \frac{1}{c_0^2} r_1(w_0) = \frac{1}{c_0}r_0(w_0).
\end{align*}
We will denote them respectively $r_0$, $r_1$ and $r_2$ in the following for simplicity. In the case where the attacker's norm is the $\ell_\infty$-norm so that its dual $\|\cdot\|_\star$ is the $\ell_1$-norm, $r_0$ (in fact, $1/r_0(w_0)$) can be thought of as the sparsity level of $w_0$.
A simple computation reveals that
\begin{eqnarray}
\beta_{opt}(z,r)% \min(\max(\widetilde\alpha_{opt}(z,r),0), 1)
= \begin{cases}
1, &\mbox{ if }0 \le r < r_1,\\
\widetilde\beta_{opt}(w_0,r),&\mbox{ if }r_1\le r \le r_2,\\
0,&\mbox{ if } r > r_2.
\end{cases}
\end{eqnarray}
Finally, note that
\begin{eqnarray*}
E(\beta_{opt}(z,r)z,r) = \begin{cases}
r^2\Vert w_0\Vert_{*}^2, &\mbox{ if }0 \le r < r_1,\\
\dfrac{(1-c_0^2)\|w_0\|_{\Sigma_x}^2}{h(r_0/r)},&\mbox{ if }r_1 \le r \le r_2,\\
\|w_0\|_{\Sigma_x}^2,&\mbox{ if } r > r_2.
\end{cases}
\end{eqnarray*}
where the function $h:\mathbb R \to \mathbb R$ is defined by
\begin{eqnarray}
h(t) := t^2+1-2c_0 t.
\end{eqnarray}
% FWIW, note that
% $(t-1)^2 \le h(t) \le t^2 + 1$ for any $t \in \mathbb R$.

% Putting things together, we obtain the following result.
% \begin{restatable}{prop}{}
% For any nonzero $z \in \mathbb R^d$, the minimum of $w \mapsto E(w,r)$ over the chord $[0,z]$ is attained at the point $\alpha_{opt}(z,r) z$. That is,
% \begin{eqnarray}
% \inf_{w \in [0,z]}E(w, r) = E(\alpha_{opt}(z,r)z,r)
% = \begin{cases}
% E(z,r),&\mbox{ if }0 \le r < r_1(z),\\
% \dfrac{r^2(1-c_0^2)\|z\|_\Sigma^2\|z\|_\star^2}{a(z,r)},&\mbox{ if }r_1(z) \le r \le r_2(z),\\
% E(0,r) = \|w_0\|_\Sigma^2,&\mbox{ if }r > r_2(z).
% \end{cases}
% \end{eqnarray}
% \label{prop:alpha}
% \end{restatable}

The following Proposition quantifies the improvement of the robust error of our proposed predictor compared to the generative model.
\begin{prop}
 For any nonzero model $w_0 \in \mathbb R^d$, it holds that
\begin{itemize}
\item[(A)] If $0 \le r \le r_1(w_0)$, then $E^{\Vert\cdot\Vert}(\beta_{opt}(w_0,r),r) = E^{\Vert\cdot\Vert }(w_0,r)$.
\item[(B)] If $r_1(w_0) \le r \le r_2(w_0)$, then
$\dfrac{E^{\Vert\cdot\Vert}(\beta_{opt}(w,r),r)}{E^{\Vert\cdot\Vert}(w_0,r)} = \dfrac{1-c_0^2}{h(r/r_0(w))} \le 1$.
\item[(C)] If $r \ge r_2(w)$, then $\dfrac{E^{\Vert\cdot\Vert}(\beta_{opt}(w,r),r)}{E^{\Vert\cdot\Vert}(w,r)} =  \dfrac{\|w_0\|_\Sigma^2}{r^2\Vert w_0\Vert_{*}^2} \le 1$.
\end{itemize}
\end{prop}




\subsection{A note on the euclidean case}
In the case of euclidean attacks, we can obtain finer results. 
\begin{restatable}{rmk}{}
Define $R_1 = R_1(w_0) := c_0\|w_0\|_2/\|w_0\|_{\Sigma^{-1}}$ and $R_1 = R_2(w_0):=(1/c_0)\|w_0\|_{\Sigma^2}/\|w_0\|_{\Sigma}$. 
It was shown in Proposition 1 of \url{https://arxiv.org/pdf/2012.10278.pdf} that 
\begin{itemize}
    \item If $ 0 \le r \le R_1$, then $E_{opt}(r) = E(w_0,r) = r^2\|w_0\|_2^2$.
    \item If $r \ge R_2$, then
    $E_{opt}(r) = E(0,r) = \|w_0\|_\Sigma^2$.
\end{itemize}
\label{rmk:extremes}
\end{restatable}
Little was said for $r \in [R_1,R_2]$; the analysis in that interval is untractable, except in the special case where the covariance matrix is the identity matrix. We will remedy the situation by settling for near-optimal solutions: that is points whose robust risk $E(w,r)$ is within a multiplicative factor the global minimum $E_{opt}(r)$. 

The following lemma will be useful in the special case of euclidean attacks.
\begin{restatable}{lm}{}
In the case of euclidean attacks, it holds that
$r_1 \ge R_1$ and $R_2 \ge r_2$.
\end{restatable}
\begin{proof}
Indeed,  we have
\begin{align}
r_1 &\ge R_1 \text{ iff } \|w_0\|_{\Sigma^{-1}}\|w_0\|_{\Sigma} \ge \|w_0\|_2^2 = \langle w_0, w_0\rangle,\\
R_2 &\ge r_2 \text{ iff }\|w_0\|_{\Sigma^2}\|w_0\|_2 \ge \|w_0\|_\Sigma^2 \text{ iff }\|\Sigma w_0\|_2 \|w_0\|_2 \ge \langle \Sigma w_0,w_0\rangle.
\end{align}
Thanks to Cauchy-Schwarz inequality, and the fact that the $\ell_2$-norm is self-dual while $\|\cdot\|_{\Sigma}$ and $\|\cdot\|_{\Sigma^{-1}}$ are duals of one another, the rightmost side (and therefore the leftmost side too) of the each of the above equivalencies is satisfied.
\end{proof}
In particularly, if $\Sigma = \sigma^2 I_d$ (or more generally, if $w_0$ is an eigenvector of $\Sigma$), then $r_1 = R_1$ and $r_2 = R_2$.

\subsection{Main results}
Let $\lambda_{min}$ (resp. $\lambda_{max}$) be the smallest (resp. largest) value of the ratio $r_0(w) := \|w\|_\Sigma/\|w\|_\star$ over non-zero vectors $w \in \mathbb R^d$. That is,
\begin{eqnarray}
\lambda_{max} := \sup_{w \in \mathbb R^d,\,w \ne 0}r_0(w)^2,\, \lambda_{min} := \inf_{w \in \mathbb R^d,\,w \ne 0}r_0(w)^2.
\end{eqnarray}
Also, let $\kappa(\Sigma)=\kappa^{\|\cdot\|}(\Sigma)$ be the \emph{condition number} of $\Sigma$ w.r.t the norm $\|\cdot\|$, i.e
\begin{eqnarray}
\kappa(\Sigma) := \lambda_{max}/\lambda_{min},\,\kappa^0(\Sigma):=\lambda_{max}/r_0(w_0)^2,\,\kappa^1(\Sigma) := r_0(w_0)^2/\lambda_{min}.
\end{eqnarray}
In the particular case of euclidean attacks, $\lambda_{max}$ (resp. $\lambda_{min}$) corresponds to the largest (resp. smallest) eigenvalue of $\Sigma$. In this case $\kappa(\Sigma)$ is the usual condition number of $\Sigma$.
In any case, it always holds that $\kappa(\Sigma) \ge \max(\kappa^0(\Sigma),\kappa^1(\Sigma))$ and $\min(\kappa^0(\Sigma),\kappa^1(\Sigma)) \ge 1$ with $\kappa(\Sigma) = 1$ iff the attacker's norm $\|\cdot\|$ is proportional to $\|\cdot\|_{\Sigma^{-1}}$. For example, this is the case when $\Sigma = \sigma^2 I_d$ and the attacker's norm is euclidean.
On the other hand, note that $\kappa(\Sigma)$ can be arbitrarily large. For example, if $\Sigma=I_d$ and the attacker's norm $\|\cdot\|$ is the $\ell_\infty$-norm, then it is easy to see that $\kappa(\Sigma) = d$.

The following lemma will be useful.
\begin{restatable}{lm}{}
Define $\gamma_r(w_0) := \inf_{w \in \mathbb R^d}\|w-w_0\|_\Sigma + r\|w\|_\star$. Then,
\begin{align}
     \gamma_r(w_0) &\ge \min(1,r/\sqrt \lambda_{max})\|w_0\|_\Sigma,\\
     \gamma_r(w_0) &\ge \min(\sqrt \lambda_{min},r)\|w_0\|_\star.
\end{align}
\label{lm:densesparse}
\end{restatable}
\begin{proof}
Let $w \in \mathbb R^d$.
Indeed, by definition of $\lambda_{max}$, it holds that $\|w\|_\star \ge \|w\|_\Sigma/\sqrt\lambda_{max}$, and so one may write $$
\|w-w_0\|_\Sigma + r\|w\|_\star \ge \|w-w_0\|_\Sigma + (r/\sqrt\lambda_{max})\|w\|_\Sigma \ge \min(1,r/\sqrt\lambda_{max})\|w_0\|_\Sigma,
$$
which proves the first lower-bound.
Similarly, by definition of $\lambda_{min}$, it holds that $\|w-w_0\|_\Sigma \ge \sqrt\lambda_{min}\|w-w_0\|_\star$, and so
$$
\|w-w_0\|_\Sigma + r\|w\|_\star \ge \sqrt\lambda_{min}\|w-w_0\|_\star + r\|w\|_\star \ge \min(\sqrt\lambda_{min},r)\|w_0\|_\star,
$$
which proves the second lower-bound.
\end{proof}

We are now ready to state the main result of this section wherein we show that optimizing on the chord $[0,w_0]$ gives a point which is optimal up to within a multiplicative factor of $1.747\kappa(\Sigma)$. Viz,
\begin{restatable}{thm}{}
We have the following:
\begin{itemize}
\item[(A)] In the case of an attack of magnitude $r$ w.r.t to an arbitrary norm $\|\cdot\|$, for  $r_1 \le r \le r_2$, it holds that
\begin{eqnarray}
\dfrac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)}
% \le \dfrac{2(1-c_0^2)}{1+c_0}\frac{\lambda_{min} \land r^2}{h(r_0/r)}\kappa(\Sigma)
\le \dfrac{2}{(1+c_0)c_0^2}\kappa^0(\Sigma) \approx 1.747\kappa^0(\Sigma).
\end{eqnarray}
\item[(B)] In the case of euclidean attacks, if $0 \le r \le R_1$ or $r \ge R_2$, then it holds that $E(\alpha_{opt}(w_0,r),r) = E_{opt}(r)$. In addition, if $R_1 < r <R_2 $, then $\dfrac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} \leq\kappa^1(\Sigma)$.
\end{itemize}
\end{restatable}
\mytodo{Extend part (B) to general non-euclidean norm attacks.}\\
\begin{proof}
We first prove part A of the result. One computes
\begin{eqnarray}
\begin{split}
\frac{2}{1+c_0} \cdot E_{opt}(r) &\ge \left(\inf_{w \in \mathbb R^d} \|w-w_0\|_\Sigma + r\|w\|_\star\right)^2\\
% &\ge \left(\inf_{w \in \mathbb R^d}\sqrt{\lambda_{min}}\|w-w_0\|_\star + r\|w\|_\star\right)^2\\
&\ge (\lambda_{min} \land r^2)\|w_0\|_\star^2 \lor (1 \land r^2/\lambda_{max})\|w_0\|_\Sigma^2,
\end{split}
\label{eq:toto}
\end{eqnarray}
where the first step is thanks to Lemma \ref{lm:burger} below and the second step is thanks to Lemma \ref{lm:densesparse}.
On the other hand, for $r_1 \le r \le r_2$, we deduce from Proposition \ref{prop:alpha} that
\begin{eqnarray}
\begin{split}
E(\alpha_{opt}(w_0,r),r) &= \frac{(1-c_0^2)\|w_0\|_\Sigma^2}{h(r_0/r)}
% &\le \frac{(1-c_0^2)\|w_0\|_\Sigma^2}{h(r_0/r_2)}
\le \frac{1-c_0^2}{h(r_0/r)}\lambda_{max}\|w_0\|_\star^2 \le \lambda_{max}\|w_0\|_\star^2,
\end{split}
\label{eq:tata}
\end{eqnarray}
where we have used the fact that $h(t) := t^2+1-2tc_0 \ge h(c_0) = 1-c_0^2$ for all $t \in \mathbb R$. On the same interval, \eqref{eq:toto} further gives
\begin{eqnarray}
\begin{split}
\frac{2E_{opt}(r)}{(1+c_0)\|w_0\|_\star^2} &\ge \lambda_{min} \land r^2 \ge \lambda_{min} \land r_1^2 \ge  \lambda_{min} \land c_0^2\lambda_{min}=c_0^2\lambda_{min},\\
\frac{2E_{opt}(r)}{(1+c_0)\|w_0\|_\Sigma^2} &\ge 1 \land r^2/\lambda_{max} \ge 1\land r_1^2/\lambda_{max} \ge  1 \land c_0^2 r_0^2/\lambda_{max} =\frac{c_0^2r_0^2}{\lambda_{max}} = \frac{c_0^2}{\kappa^0(\Sigma)},
\end{split}
\end{eqnarray}
and we deduce that
\begin{eqnarray}
\begin{split}
E_{opt}(r) &\ge \frac{(1+c_0)}{2}(\lambda_{min} \land r^2)\|w_0\|_\star^2 \ge \dfrac{(1+c_0)c_0^2}{2}\lambda_{min}\|w_0\|_\star^2,\\
E_{opt}(r) &\ge \frac{(1+c_0)}{2}(1 \land r^2/\lambda_{max})\|w_0\|_\Sigma^2 \ge \dfrac{(1+c_0)c_0^2}{2}\kappa^0(\Sigma)\|w_0\|_\Sigma^2.
\end{split}
\label{eq:titi}
\end{eqnarray}
Putting \eqref{eq:tata} and \eqref{eq:titi} together gives
\begin{eqnarray*}
\begin{split}
1 \le \frac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} &\le \frac{2}{(1+c_0)c_0^2}\frac{(1-c_0^2)}{h(r_0/r)}\kappa^0(\Sigma) = \frac{2}{(1+c_0)c_0^2}\frac{1-c_0^2}{h(r_0/r)}\kappa^0(\Sigma)\\
&\le \frac{2}{(1+c_0)c_0^2}\kappa^0(\Sigma),
%1 \le \frac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} &\le \frac{2}{(1+c_0)c_0^2}\frac{(1-c_0^2)}{h(r_0/r)}\frac{\lambda_{max}}{\lambda_{min}} = \frac{2}{(1+c_0)c_0^2}\frac{1-c_0^2}{h(r_0/r)}\kappa(\Sigma)\\
%&\le \frac{2}{(1+c_0)c_0^2}\kappa(\Sigma),
\end{split}
\end{eqnarray*}
as desired.

We now prove part B. If $r \le R_1$ or $r \ge R_2$, part B follows directly from Proposition \ref{prop:alpha} and Remark \ref{rmk:extremes}, since $R_1 \ge r_1$ and $R_2 \le r_2$ as already mentioned above.

If $R_1 \le r \le r_1$ (resp. $r_2 \le r \le R_2$), then thanks to Proposition \ref{prop:alpha} we have $E_{opt}(r) \ge E_{opt}(R_1) = R_1^2\|w_0\|_2^2$ and $E(\alpha_{opt}(w_0,r),r)\leq r_1^2\|w_0\|_2^2$ which gives that
\begin{align*}
    E(\alpha_{opt}(w_0,r),r)/E_{opt}(r)\leq r_1^2/R_1^2\leq \kappa^1(\Sigma).
\end{align*}
In addition if $r_2 \le r \le R_2$, we have that $E(\alpha_{opt}(w_0,r),r)=\|w_0\|_{\Sigma}^2$ and $E_{opt}(r) \ge E_{opt}(R_1) = R_1^2\|w_0\|_2^2$, which gives that
\begin{align*}
    E(\alpha_{opt}(w_0,r),r) / E_{opt}(r)\leq
    \frac{1}{c_0^2}\frac{\|w_0\|_{\Sigma^{-1}}^2\|w_0\|_{\Sigma}^2}{\|w_0\|_2^2 \|w_0\|_2^2}\leq \frac{ \kappa^1(\Sigma)}{c_0^2}
\end{align*}
\end{proof}

\begin{restatable}{lm}{}
\label{lm:burger}
If $u,v,\beta \ge 0$ with $\beta \le 1$, then
\begin{eqnarray}
\frac{(1+\beta)}{2}(u+v)^2 \le u^2 + v^2 + 2\beta u v \le (u+v)^2.
\end{eqnarray}
\end{restatable}
\begin{proof}
The second inequality follows directly from the fact that $0 \le \beta \le 1$. For the first inequality, simply observe that
$$
2(u^2 + v^2 + 2\beta u v)  - (1+\beta)(u+v)^2 = (1-\beta)(u-v)^2 \ge 0.
$$
\end{proof}


\subsection{Exact Optimality for Euclidean Attacks}
There is a setting however where we can guarantee that early-stopping captures the infimum. Indeed let us consider the case where  $\Sigma=\sigma^2 I_d$ and $\Vert\cdot\Vert=\Vert\cdot\Vert_2$, then we obtain the following sharper result.
\begin{prop}
For all $r\geq 0$, we have 
\begin{align*}
    \inf_{t\geq 0} E^{\Vert\cdot\Vert_2}(w(t),r) =  E^{\Vert\cdot\Vert_2}_{opt}(r).
\end{align*}
In addition, if $r\leq \sqrt{2/\pi}\frac{\Vert w_0\Vert_2}{\Vert w_0\Vert_{\Sigma_x^{-1}}}$ or 
$r\geq \sqrt{\pi/2}\frac{\Vert w_0\Vert_{\Sigma_x^2}}{\Vert w_0\Vert_{\Sigma_x}}$, then $t\mapsto  E^{\Vert\cdot\Vert_2}(w(t),r) $ is monotone and if $\sqrt{2/\pi}\frac{\Vert w_0\Vert_2}{\Vert w_0\Vert_{\Sigma_x^-1}}<r<\sqrt{\pi/2}\frac{\Vert w_0\Vert_{\Sigma_x^2}}{\Vert w_0\Vert_{\Sigma_x}}$, then $t\mapsto  E^{\Vert\cdot\Vert_2}(w(t),r) $ admits exactly one local minimum which is global.
\end{prop}
Therefore in the isotropic case we obtain exact optimal robustness and we show that early-stopping on the GD scheme is able to capture it. In order to generalize the above idea in the general setting we will focus in the following on the robustness of the GD descent on normalized data.


\section{Some cleanup and refinements}
\textcolor{red}{The objective is to refine / clarify some of the ideas developed in the previous section. Most importantly, we try to see how far we can go without ever uttering the work "gradient descent".}
\subsection{Redefining spectral quantities}
Define scalars $\lambda_{max}$, $\lambda_{\min}$, and $\kappa(\Sigma)$, by
\begin{align}
\lambda_{max} &:= \|\Sigma^{1/2}\|_\star^2 = \sup_{w \ne 0}\frac{\|\Sigma^{1/2} w\|_\star^2}{\|w\|_\star^2},\\
\lambda_{\min} &:= \|\Sigma^{-1/2}\|_\star^{-2} = \inf_{w \ne 0}\frac{\|\Sigma^{1/2} w\|_\star^2}{\|w\|_\star^2},\\
\kappa(\Sigma) &:= \lambda_{max}/\lambda_{min}.
\end{align}
In the particular case where the attacker's norm is euclidean, we have $\lambda_{max} = \|\Sigma\|_{op}$, $\lambda_{\min} = 1/\|\Sigma^{-1}\|_{op}$, and $\kappa(\Sigma) = \|\Sigma\|_{op} \|\Sigma^{-1}\|_{op}$ is the usual condition number of $\Sigma$. Of course, these perfectly match the considerations of the previous subsection. In the case of $\ell_\infty$-norm attacks, it might be handy to note that for any matrix $A=(a_{ij})_{i,j} \in \mathbb R^{m \times d}$, one has
\begin{eqnarray}
\|A\|_1 = \max_{1 \le j \le d} \sum_{i=1}^m|a_{ij}| = \text{ max }\ell_1\text{ norm of a column of }A.
\end{eqnarray}

\begin{restatable}{lm}{}
For any $w \in \mathbb R^d$ and $r \ge 0$, we have
\begin{align}
 E(\Sigma^{-1/2}w,r\sqrt{\lambda_{min}})  \leq  E_{norm}(w,r)\leq E(\Sigma^{-1/2}w,r\sqrt{\lambda_{max}}).
\end{align}
\end{restatable}
\begin{proof}
Indeed, by definition of $E_{norm}$, $\tilde w_0$, $\lambda_{max}$, and $\lambda_{min}$, one computes
\begin{eqnarray*}
\begin{split}
E_{norm}(w,r) &= \|w-\tilde w_0\|_2^2 + r^2\|w\|_\star^2 + 2c_0\|w-\tilde w_0\|_\star\|w\|_\star\\
&= \|\Sigma^{-1/2}w-w_0\|_{\Sigma}^2 + r^2\|w\|_\star^2 + 2c_0\|\Sigma^{-1/2}w-w_0\|_\Sigma \|w\|_\star\\
&= \|\Sigma^{-1/2}w-w_0\|_{\Sigma}^2 + r^2\|\Sigma^{1/2}\Sigma^{-1/2}w\|_\star^2\\
&\quad\quad\quad + 2c_0\|\Sigma^{-1/2}w-w_0\|_\Sigma \|\Sigma^{1/2}\Sigma^{-1/2}w\|_\star\\
&\le \|\Sigma^{-1/2}w-w_0\|_{\Sigma}^2 + r^2\lambda_{max}\|\Sigma^{-1/2}w\|_\star^2\\
&\quad\quad\quad + 2c_0r\sqrt\lambda_{max}\|\Sigma^{-1/2}w-w_0\|_\Sigma \|\Sigma^{-1/2} w\|_\star\\
&= E(\Sigma^{-1/2} w,r\sqrt\lambda_{max}).
\end{split}
\end{eqnarray*}
Analogously, one shows that $E_{\mathrm{norm}}(w,r) \ge E(\Sigma^{-1/2}w,r\sqrt\lambda_{min})$.
\end{proof}

\subsection{Reduction to "one-dimensional" case: normalization}
The following is a refinement of the first statement of Prop 4.11. The aim is to make it clear that the aforementioned proposition has nothing to do with gradient-descent, etc.
\begin{restatable}{thm}{}
For any $r \ge 0$, let $w_{norm}(r)$ be a minimizer of $E_{norm}(w,r)$ over $w \in \mathbb R^d$. Then, it holds that
\begin{align}
E(w_{norm}(r),r) &\le E_{opt}(r\sqrt{\kappa(\Sigma)})\\
&\le \kappa(\Sigma) E_{opt}(r).
\end{align}
\end{restatable}
\mytodo{Tightness: construct an example where $r > 0$, $\kappa(\Sigma) > 1$, and $E(w_{norm}(r),r) = \kappa(\Sigma)E_{opt}(r)$.}
\begin{proof}
Indeed, using the previous lemma, one computes
\begin{eqnarray*}
\begin{split}
E_{opt}(r) &:= \inf_w E(w,r) \le E(w_{norm}(r),r) \\
&\le E_{norm}(w_{norm}(r),r/\sqrt\lambda_{min}) = \inf_w E_{norm}(w,r/\sqrt\lambda_{min})\\
&\le \inf_w E(\Sigma^{-1/2} w,r\sqrt{\lambda_{max}/\lambda_{min}}) = \inf_w E(\Sigma^{-1/2} w,r\sqrt{\kappa(\Sigma)}) \\
&= \inf_w E(w,r\sqrt{\kappa(\Sigma)}) = E_{opt}(r\sqrt{\kappa(\Sigma)}).
\end{split}
\end{eqnarray*}
The second part of the claimed inequalities follows from the lemma below applied with $a = \sqrt{\kappa(\Sigma)}$.
\end{proof}
\begin{restatable}{lm}{}
For any $w \in \mathbb R^d$, $r \ge 0$, and $a \ge 1$, it holds that
\begin{eqnarray}
E(w,ar) \le a^2 E(w,r),
\end{eqnarray}
with equality if $w=w_0$.
\end{restatable}
\begin{restatable}{rmk}{}
Note that if $w$ is close to zero, then $E(w,ar)$ ought to be close to $E(w,r)$ which is $\|w_0\|_\Sigma^2$, and can be much less than upper-bound than $a^2\|w_0\|_\Sigma^2$ proposed by the lemma. thus, the upper-bound in the lemma can be arbitrarily off / bad.
\end{restatable}

\begin{proof}[Proof of lemma]
Indeed, one computes
\begin{eqnarray*}
\begin{split}
E(w,ar) &= \|w-w_0\|_\Sigma^2 + a^2r^2\|w\|_\star^2 + 2ac_0r\|w-w_0\|_\Sigma\|w\|_\star\\
&\le a^2\|w-w_0\|_\Sigma^2 + a^2r^2\|w\|_\star^2 + 2ac_0r\|w-w_0\|_\Sigma\|w\|_\star\\
&\le a^2 (\|w-w_0\|_\Sigma^2 + r^2\|w\|_\star^2 + 2(1/a) c_0r\|w-w_0\|_\Sigma\|w\|_\star)\\
&\le a^2 E(w,r),
\end{split}
\end{eqnarray*}
where we have used the fact that $1 \le a^2$ and $1/a \le 1$, on the second and last lines respectively.
\end{proof}

We can now generalize this procedure to all attacks. Indeed the main difference is that in the general we do not have acccess to $R_1$ and $R_2$, however we can still obtain an approximation of $R_1$ and $R_2$ using our approximation $\gamma_r(w_0)$. Note also that in the general case, we still have a bias which has a U form and therefore we can still apply early-stopping on the normalized data and obtain for free our best estimator. 


\subsection{Explicit solution for isotropic case}
Proposition 1  of \url{https://arxiv.org/pdf/2012.10278.pdf} can be used to salvage an explicit formula for minimizer of $w \mapsto E_{\text{norm}}(w,r)$ in the case of euclidean attacks.
Indeed,
\begin{restatable}{prop}{}
For any $r \ge 0$, a minimizer of $w \mapsto E_{norm}(w,r)$ is given by $w_{norm}(r) = (1+\lambda_{opt}(r))^{-1}w_0$, where
\begin{eqnarray}
\lambda_{opt}(r) = \begin{cases}
0,&\mbox{ if }r \le c_0,\\
(r^2 - c_0 r)/(1 - c_0 r), &\mbox{ if }c_0 < r < 1/c_0,\\
\infty,&\mbox{ if }r \ge 1/c_0.
\end{cases}
\label{eq:lambdaopt}
\end{eqnarray}
\label{prop:normalized}
\end{restatable}
Importantly, $w_{norm}(r)$ corresponds to \textit{shrinking} $w_0$ towards zero!












% \section{Robustness via shrinkage to zero}
% \mytodo{Link the ideas presented hereunder to the so-called "Stein shrinkage" \url{http://proceedings.mlr.press/v32/muandet14.pdf}}
% \subsection{Optimizing over a chord}
% For any model nonzero $z \in \mathbb R^d$, consider the chord $[0,z] := \{\alpha z \mid \alpha \in [0, 1]\}$ that joins $z$ to the origin. This chord corresponds to shrinking $z$ to zero. As before, set $c_0:=\sqrt{2/\pi}$. Consider the problem of minimizing the robust risk $w \mapsto E(w,r)$ over $[0,z]$. Now, for any $\alpha \in [0, 1]$, one has
% \begin{eqnarray}
% E(\alpha z,r) = (1-\alpha)^2\|z\|_\Sigma^2  + \alpha^2r^2\|z\|_\star^2  + 2c_0\alpha(1-\alpha)r\|z\|_\Sigma\|z\|_\star = a\alpha^2 - 2b\alpha + c,
% \end{eqnarray}
% a quadratic polynomial in $\alpha$ with coefficients $a=a(z,r) := \|z\|_\Sigma^2 + r^2\|z\|_\star^2 - 2c_0r\|z\|_\Sigma\|z\|_\star$, $b=b(z,r) := \|z\|_\Sigma^2-c_0r\|z\|_\Sigma\|z\|_\star$, and $c=c(z,r) = \|z\|_\Sigma^2$. On the other hand, it is clear that the leading coefficient $a(z,r)$ is itself a quadratic in $r$ with discriminant $\|z\|_\Sigma^2\|z\|_\star^2(c_0^2-1)$ which is strictly negative because $c_0^2 = 2/\pi < 1$. Thus, $\alpha \mapsto E(\alpha z, r)$ is a convex one-dimensional quadratic function. We conclude that this function is minimized at $\alpha_{opt}(z,r) = $ the unique point of $[0,1]$ which is closest to the real number $\widetilde\alpha_{opt}(z,r) \in \mathbb R$ defined by
% \begin{eqnarray}
% \widetilde\alpha_{opt}(z,r) := \frac{b(z,r)}{a(z,r)} = \frac{\|z\|_\Sigma^2-c_0r\|z\|_\Sigma\|z\|_\star}{\|z\|_\Sigma^2 + r^2\|z\|_\star^2 - 2c_0r\|z\|_\Sigma\|z\|_\star}.
% \end{eqnarray}

% \begin{restatable}{lm}{}
% For any fixed $z \in \mathbb R^d$, it holds that
% \begin{eqnarray}
% \lim_{r \to 0^+}\widetilde\alpha_{opt}(z,r) = 1,\,\lim_{r \to \infty}\widetilde\alpha_{opt}(z,r) = 0.
% \end{eqnarray}
% Moreover, if $\|\cdot\|_\star = \|\cdot\|_\Sigma$ (i.e if the attacker's norm is $\|\cdot\|_{\Sigma{-1}}$), then
% \begin{eqnarray}
% \widetilde\alpha_{opt}(z,r) = (1-c_0 r) / (1+r^2-2c_0r).
% \end{eqnarray}
% \end{restatable}

% \begin{restatable}{rmk}{}
% In isotropic case, we know from Prop \ref{prop:normalized} that the minimizer of the normalized energy $w \mapsto E(w,r)$ is $w_{opt}(r) = (1+\lambda_{opt}(r))^{-1} w_0$,
% where $\lambda_{opt}(r)$ is given in \eqref{eq:lambdaopt}. This is consistent with the above lemma as one easily verifies that for $c_0 < r < 1/c_0$, 
% $$
% (1+\lambda_{opt}(r))^{-1} = ((r^2+1-2c_0 r)/(1-c_0r))^{-1} = (1-c_0r)/(1+r^2-2c_0 r) = \alpha_{opt}(r).
% $$
% \end{restatable}

% Now, in the general case, define $r_0(z)$, $r_1(z)$, and $r_2(z)$ by \begin{eqnarray}
% r_0(z):= \frac{\|z\|_\Sigma}{\|z\|_\star},\, r_1(z):=c_0r_0(z),\,
% r_2(z) := \frac{1}{c_0^2} r_1(z) = \frac{1}{c_0}r_0(z).
% \end{eqnarray}
% In the case where the attacker's norm is the $\ell_\infty$-norm so that its dual $\|\cdot\|_\star$ is the $\ell_1$-norm, $r_0$ (in fact, $1/r_0(z)$) can be thought of as the sparsity level in $z$.
% A simple computation reveals that
% \begin{eqnarray}
% \alpha_{opt}(z,r) = % \min(\max(\widetilde\alpha_{opt}(z,r),0), 1)
% = \begin{cases}
% 1, &\mbox{ if }0 \le r < r_1(z),\\
% \widetilde\alpha_{opt}(z,r),&\mbox{ if }r_1(z) \le r \le r_2(z),\\
% 0,&\mbox{ if } r > r_2(z).
% \end{cases}
% \end{eqnarray}
% Finally, note that
% \begin{eqnarray}
% E(\alpha_{opt}(z,r)z,r) = \begin{cases}
% E(z,r), &\mbox{ if }0 \le r < r_1(z),\\
% c(z,r)-\dfrac{b(z,r)^2}{a(z,r)} =\dfrac{(1-c_0^2)\|z\|_\Sigma^2}{h(r_0(z)/r)},&\mbox{ if }r_1(z) \le r \le r_2(z),\\
% E(0,r) = \|z\|_\Sigma^2,&\mbox{ if } r > r_2(z).
% \end{cases}
% \end{eqnarray}
% where the function $h:\mathbb R \to \mathbb R$ is defined by
% \begin{eqnarray}
% h(t) := t^2+1-2c_0 t.
% \end{eqnarray}
% FWIW, note that
% $(t-1)^2 \le h(t) \le t^2 + 1$ for any $t \in \mathbb R$.

% Putting things together, we obtain the following result.
% \begin{restatable}{prop}{}
% For any nonzero $z \in \mathbb R^d$, the minimum of $w \mapsto E(w,r)$ over the chord $[0,z]$ is attained at the point $\alpha_{opt}(z,r) z$. That is,
% \begin{eqnarray}
% \inf_{w \in [0,z]}E(w, r) = E(\alpha_{opt}(z,r)z,r)
% = \begin{cases}
% E(z,r),&\mbox{ if }0 \le r < r_1(z),\\
% \dfrac{r^2(1-c_0^2)\|z\|_\Sigma^2\|z\|_\star^2}{a(z,r)},&\mbox{ if }r_1(z) \le r \le r_2(z),\\
% E(0,r) = \|w_0\|_\Sigma^2,&\mbox{ if }r > r_2(z).
% \end{cases}
% \end{eqnarray}
% \label{prop:alpha}
% \end{restatable}

% The following theorem quantifies the improvement of the robust error of any model.
% \begin{restatable}{thm}{}
%  For any nonzero model $w \in \mathbb R^d$, it holds that
% \begin{itemize}
% \item[(A)] If $0 \le r \le r_1(w)$, then $E(\alpha_{opt}(w,r),r) = E(w,r)$.
% \item[(B)] If $r_1(w) \le r \le r_2(w)$, then
% $\dfrac{E(\alpha_{opt}(w,r),r)}{E(w,r)} = \dfrac{1-c_0^2}{h(r/r_0(w))} \le 1$.
% \item[(C)] If $r \ge r_2(w)$, then $\dfrac{E(\alpha_{opt}(w,r),r)}{E(w,r)} =  \dfrac{\|w_0\|_\Sigma^2}{E(w,r)} \le 1$.
% \end{itemize}
% \end{restatable}

% For simplicity of notation, write $r_1  := c_0 r_0$, and $r_2 := r_0/c_0$, where $r_0:=\|w_0\|_\Sigma/\|w_0\|_\star$.

% \subsection{A note on the euclidean case}
% In the case of euclidean attacks, we can obtain finer results. 
% \begin{restatable}{rmk}{}
% Define $R_1 = R_1(w_0) := c_0\|w_0\|_2/\|w_0\|_{\Sigma^{-1}}$ and $R_1 = R_2(w_0):=(1/c_0)\|w_0\|_{\Sigma^2}/\|w_0\|_{\Sigma}$. 
% It was shown in Proposition 1 of \url{https://arxiv.org/pdf/2012.10278.pdf} that 
% \begin{itemize}
%     \item If $ 0 \le r \le R_1$, then $E_{opt}(r) = E(w_0,r) = r^2\|w_0\|_2^2$.
%     \item If $r \ge R_2$, then
%     $E_{opt}(r) = E(0,r) = \|w_0\|_\Sigma^2$.
% \end{itemize}
% \label{rmk:extremes}
% \end{restatable}
% Little was said for $r \in [R_1,R_2]$; the analysis in that interval is untractable, except in the special case where the covariance matrix is the identity matrix. We will remedy the situation by settling for near-optimal solutions: that is points whose robust risk $E(w,r)$ is within a multiplicative factor the global minimum $E_{opt}(r)$. 

% The following lemma will be useful in the special case of euclidean attacks.
% \begin{restatable}{lm}{}
% In the case of euclidean attacks, it holds that
% $r_1 \ge R_1$ and $R_2 \ge r_2$.
% \end{restatable}
% \begin{proof}
% Indeed,  we have
% \begin{align}
% r_1 &\ge R_1 \text{ iff } \|w_0\|_{\Sigma^{-1}}\|w_0\|_{\Sigma} \ge \|w_0\|_2^2 = \langle w_0, w_0\rangle,\\
% R_2 &\ge r_2 \text{ iff }\|w_0\|_{\Sigma^2}\|w_0\|_2 \ge \|w_0\|_\Sigma^2 \text{ iff }\|\Sigma w_0\|_2 \|w_0\|_2 \ge \langle \Sigma w_0,w_0\rangle.
% \end{align}
% Thanks to Cauchy-Schwarz inequality, and the fact that the $\ell_2$-norm is self-dual while $\|\cdot\|_{\Sigma}$ and $\|\cdot\|_{\Sigma^{-1}}$ are duals of one another, the rightmost side (and therefore the leftmost side too) of the each of the above equivalencies is satisfied.
% \end{proof}
% In particularly, if $\Sigma = \sigma^2 I_d$ (or more generally, if $w_0$ is an eigenvector of $\Sigma$), then $r_1 = R_1$ and $r_2 = R_2$.

% \subsection{Main results}
% Let $\lambda_{min}$ (resp. $\lambda_{max}$) be the smallest (resp. largest) value of the ratio $r_0(w) := \|w\|_\Sigma/\|w\|_\star$ over non-zero vectors $w \in \mathbb R^d$. That is,
% \begin{eqnarray}
% \lambda_{max} := \sup_{w \in \mathbb R^d,\,w \ne 0}r_0(w)^2,\, \lambda_{min} := \inf_{w \in \mathbb R^d,\,w \ne 0}r_0(w)^2.
% \end{eqnarray}
% Also, let $\kappa(\Sigma)=\kappa^{\|\cdot\|}(\Sigma)$ be the \emph{condition number} of $\Sigma$ w.r.t the norm $\|\cdot\|$, i.e
% \begin{eqnarray}
% \kappa(\Sigma) := \lambda_{max}/\lambda_{min},\,\kappa^0(\Sigma):=\lambda_{max}/r_0(w_0)^2,\,\kappa^1(\Sigma) := r_0(w_0)^2/\lambda_{min}.
% \end{eqnarray}
% In the particular case of euclidean attacks, $\lambda_{max}$ (resp. $\lambda_{min}$) corresponds to the largest (resp. smallest) eigenvalue of $\Sigma$. In this case $\kappa(\Sigma)$ is the usual condition number of $\Sigma$.
% In any case, it always holds that $\kappa(\Sigma) \ge \max(\kappa^0(\Sigma),\kappa^1(\Sigma))$ and $\min(\kappa^0(\Sigma),\kappa^1(\Sigma)) \ge 1$ with $\kappa(\Sigma) = 1$ iff the attacker's norm $\|\cdot\|$ is proportional to $\|\cdot\|_{\Sigma^{-1}}$. For example, this is the case when $\Sigma = \sigma^2 I_d$ and the attacker's norm is euclidean.
% On the other hand, note that $\kappa(\Sigma)$ can be arbitrarily large. For example, if $\Sigma=I_d$ and the attacker's norm $\|\cdot\|$ is the $\ell_\infty$-norm, then it is easy to see that $\kappa(\Sigma) = d$.

% The following lemma will be useful.
% \begin{restatable}{lm}{}
% Define $\gamma_r(w_0) := \inf_{w \in \mathbb R^d}\|w-w_0\|_\Sigma + r\|w\|_\star$. Then,
% \begin{align}
%      \gamma_r(w_0) &\ge \min(1,r/\sqrt \lambda_{max})\|w_0\|_\Sigma,\\
%      \gamma_r(w_0) &\ge \min(\sqrt \lambda_{min},r)\|w_0\|_\star.
% \end{align}
% \label{lm:densesparse}
% \end{restatable}
% \begin{proof}
% Let $w \in \mathbb R^d$.
% Indeed, by definition of $\lambda_{max}$, it holds that $\|w\|_\star \ge \|w\|_\Sigma/\sqrt\lambda_{max}$, and so one may write $$
% \|w-w_0\|_\Sigma + r\|w\|_\star \ge \|w-w_0\|_\Sigma + (r/\sqrt\lambda_{max})\|w\|_\Sigma \ge \min(1,r/\sqrt\lambda_{max})\|w_0\|_\Sigma,
% $$
% which proves the first lower-bound.
% Similarly, by definition of $\lambda_{min}$, it holds that $\|w-w_0\|_\Sigma \ge \sqrt\lambda_{min}\|w-w_0\|_\star$, and so
% $$
% \|w-w_0\|_\Sigma + r\|w\|_\star \ge \sqrt\lambda_{min}\|w-w_0\|_\star + r\|w\|_\star \ge \min(\sqrt\lambda_{min},r)\|w_0\|_\star,
% $$
% which proves the second lower-bound.
% \end{proof}

% We are now ready to state the main result of this section wherein we show that optimizing on the chord $[0,w_0]$ gives a point which is optimal up to within a multiplicative factor of $1.747\kappa(\Sigma)$. Viz,
% \begin{restatable}{thm}{}
% We have the following:
% \begin{itemize}
% \item[(A)] In the case of an attack of magnitude $r$ w.r.t to an arbitrary norm $\|\cdot\|$, for  $r_1 \le r \le r_2$, it holds that
% \begin{eqnarray}
% \dfrac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)}
% % \le \dfrac{2(1-c_0^2)}{1+c_0}\frac{\lambda_{min} \land r^2}{h(r_0/r)}\kappa(\Sigma)
% \le \dfrac{2}{(1+c_0)c_0^2}\kappa^0(\Sigma) \approx 1.747\kappa^0(\Sigma).
% \end{eqnarray}
% \item[(B)] In the case of euclidean attacks, if $0 \le r \le R_1$ or $r \ge R_2$, then it holds that $E(\alpha_{opt}(w_0,r),r) = E_{opt}(r)$. In addition, if $R_1 < r <R_2 $, then $\dfrac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} \leq\kappa^1(\Sigma)$.
% \end{itemize}
% \end{restatable}
% \mytodo{Extend part (B) to general non-euclidean norm attacks.}\\
% \begin{proof}
% We first prove part A of the result. One computes
% \begin{eqnarray}
% \begin{split}
% \frac{2}{1+c_0} \cdot E_{opt}(r) &\ge \left(\inf_{w \in \mathbb R^d} \|w-w_0\|_\Sigma + r\|w\|_\star\right)^2\\
% % &\ge \left(\inf_{w \in \mathbb R^d}\sqrt{\lambda_{min}}\|w-w_0\|_\star + r\|w\|_\star\right)^2\\
% &\ge (\lambda_{min} \land r^2)\|w_0\|_\star^2 \lor (1 \land r^2/\lambda_{max})\|w_0\|_\Sigma^2,
% \end{split}
% \label{eq:toto}
% \end{eqnarray}
% where the first step is thanks to Lemma \ref{lm:burger} below and the second step is thanks to Lemma \ref{lm:densesparse}.
% On the other hand, for $r_1 \le r \le r_2$, we deduce from Proposition \ref{prop:alpha} that
% \begin{eqnarray}
% \begin{split}
% E(\alpha_{opt}(w_0,r),r) &= \frac{(1-c_0^2)\|w_0\|_\Sigma^2}{h(r_0/r)}
% % &\le \frac{(1-c_0^2)\|w_0\|_\Sigma^2}{h(r_0/r_2)}
% \le \frac{1-c_0^2}{h(r_0/r)}\lambda_{max}\|w_0\|_\star^2 \le \lambda_{max}\|w_0\|_\star^2,
% \end{split}
% \label{eq:tata}
% \end{eqnarray}
% where we have used the fact that $h(t) := t^2+1-2tc_0 \ge h(c_0) = 1-c_0^2$ for all $t \in \mathbb R$. On the same interval, \eqref{eq:toto} further gives
% \begin{eqnarray}
% \begin{split}
% \frac{2E_{opt}(r)}{(1+c_0)\|w_0\|_\star^2} &\ge \lambda_{min} \land r^2 \ge \lambda_{min} \land r_1^2 \ge  \lambda_{min} \land c_0^2\lambda_{min}=c_0^2\lambda_{min},\\
% \frac{2E_{opt}(r)}{(1+c_0)\|w_0\|_\Sigma^2} &\ge 1 \land r^2/\lambda_{max} \ge 1\land r_1^2/\lambda_{max} \ge  1 \land c_0^2 r_0^2/\lambda_{max} =\frac{c_0^2r_0^2}{\lambda_{max}} = \frac{c_0^2}{\kappa^0(\Sigma)},
% \end{split}
% \end{eqnarray}
% and we deduce that
% \begin{eqnarray}
% \begin{split}
% E_{opt}(r) &\ge \frac{(1+c_0)}{2}(\lambda_{min} \land r^2)\|w_0\|_\star^2 \ge \dfrac{(1+c_0)c_0^2}{2}\lambda_{min}\|w_0\|_\star^2,\\
% E_{opt}(r) &\ge \frac{(1+c_0)}{2}(1 \land r^2/\lambda_{max})\|w_0\|_\Sigma^2 \ge \dfrac{(1+c_0)c_0^2}{2}\kappa^0(\Sigma)\|w_0\|_\Sigma^2.
% \end{split}
% \label{eq:titi}
% \end{eqnarray}
% Putting \eqref{eq:tata} and \eqref{eq:titi} together gives
% \begin{eqnarray*}
% \begin{split}
% 1 \le \frac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} &\le \frac{2}{(1+c_0)c_0^2}\frac{(1-c_0^2)}{h(r_0/r)}\kappa^0(\Sigma) = \frac{2}{(1+c_0)c_0^2}\frac{1-c_0^2}{h(r_0/r)}\kappa^0(\Sigma)\\
% &\le \frac{2}{(1+c_0)c_0^2}\kappa^0(\Sigma),
% %1 \le \frac{E(\alpha_{opt}(w_0,r),r)}{E_{opt}(r)} &\le \frac{2}{(1+c_0)c_0^2}\frac{(1-c_0^2)}{h(r_0/r)}\frac{\lambda_{max}}{\lambda_{min}} = \frac{2}{(1+c_0)c_0^2}\frac{1-c_0^2}{h(r_0/r)}\kappa(\Sigma)\\
% %&\le \frac{2}{(1+c_0)c_0^2}\kappa(\Sigma),
% \end{split}
% \end{eqnarray*}
% as desired.

% We now prove part B. If $r \le R_1$ or $r \ge R_2$, part B follows directly from Proposition \ref{prop:alpha} and Remark \ref{rmk:extremes}, since $R_1 \ge r_1$ and $R_2 \le r_2$ as already mentioned above.

% If $R_1 \le r \le r_1$ (resp. $r_2 \le r \le R_2$), then thanks to Proposition \ref{prop:alpha} we have $E_{opt}(r) \ge E_{opt}(R_1) = R_1^2\|w_0\|_2^2$ and $E(\alpha_{opt}(w_0,r),r)\leq r_1^2\|w_0\|_2^2$ which gives that
% \begin{align*}
%     E(\alpha_{opt}(w_0,r),r)/E_{opt}(r)\leq r_1^2/R_1^2\leq \kappa^1(\Sigma).
% \end{align*}
% In addition if $r_2 \le r \le R_2$, we have that $E(\alpha_{opt}(w_0,r),r)=\|w_0\|_{\Sigma}^2$ and $E_{opt}(r) \ge E_{opt}(R_1) = R_1^2\|w_0\|_2^2$, which gives that
% \begin{align*}
%     E(\alpha_{opt}(w_0,r),r) / E_{opt}(r)\leq
%     \frac{1}{c_0^2}\frac{\|w_0\|_{\Sigma^{-1}}^2\|w_0\|_{\Sigma}^2}{\|w_0\|_2^2 \|w_0\|_2^2}\leq \frac{ \kappa^1(\Sigma)}{c_0^2}
% \end{align*}
% \end{proof}

% \begin{restatable}{lm}{}
% \label{lm:burger}
% If $u,v,\beta \ge 0$ with $\beta \le 1$, then
% \begin{eqnarray}
% \frac{(1+\beta)}{2}(u+v)^2 \le u^2 + v^2 + 2\beta u v \le (u+v)^2.
% \end{eqnarray}
% \end{restatable}
% \begin{proof}
% The second inequality follows directly from the fact that $0 \le \beta \le 1$. For the first inequality, simply observe that
% $$
% 2(u^2 + v^2 + 2\beta u v)  - (1+\beta)(u+v)^2 = (1-\beta)(u-v)^2 \ge 0.
% $$
% \end{proof}

% \section{Estimation}
% In order to estimate our new predictor we propose the following estimator
% \begin{align*}
%     \widehat{w}_{0,\text{rob}}:= \max(\min(1,b(\widehat{w_0},r)/a(\widehat{w_0},r)),0)\widehat{w_0}
% \end{align*}
% where $\widehat{w}_0$ is an estimator of the generative model $w_0$ given samples. We just need to control the error in the different norm of our estimator $\widehat{w}_0$ compared to the true $w_0$ in order to control the robust error of our estimator.

% \input{beyond.tex}

% \section{Spectral decomposition in case of euclidean attack}
% Assume the attacker's norm is euclidean.
% Also, suppose the "ridge-ing matrix" $\Sigma$ diagonalizes in the same orthonormal basis $\{v_1,v_2,\ldots\}$ as population covariance matrix of the features, namely $L_K=\Sigma_x$.
% As we already saw, in the case of gradient-descent with / without robustness training, we should have the dynamics $w_M(t) = K_t(L_K)L_K w_0 = \sum_j \sum_{ 0\leq s\leq t-1} (1-\alpha \lambda_j)^{s} \lambda_j c_j v_j$, where $c_j := \langle v_j, w_0\rangle$. Thus, at time $t$, the hard robust risk writes
% \begin{eqnarray}
% \begin{split}
%     E_M(t;r) := E(w_M(t);r) = B(t) + r^2 V(t) + r\sqrt{8/\pi} \sqrt{A(t)}\sqrt{V(t)},
% \end{split}
% \end{eqnarray}
% where $B(t):=\sum_j (1-\beta_j(t)\lambda_j)^2\lambda_j c_j^2$ and
% $V(t) := \sum_j (1-\alpha\widetilde\lambda_j)^{2t}\lambda_jc_j^2$,
% and $c_j := \langle v_j,w_0\rangle$.
% Note that for any $t$, $V(t)$ is an non-increasing function of $\Sigma$, whilst $B(t)$ is a non-decreasing function of $\Sigma$.

% \section{Interlude: some interesting computations}
% Noting that $1/2 \le \sqrt{2/\pi} \le 1$, it is clear from \eqref{eq:E} that for any $w \in \mathbb R^d$, we have
% \begin{eqnarray}
% \label{eq:sandwich}
% \sqrt{2/\pi}\overline E(w; r) \le E(w; r) \le \overline E(w; r),
% \end{eqnarray}
% where $\overline E(w; r) := (\|w-w_0\|_\Sigma + r\|w\|_\star)^2$, where, $\|\cdot\|_\star$ is the dual of the attacker's norm $\|\cdot\|$. Thus, the functions $E$ and $\overline E$ are within a constant factor of one another, i.e they are comparable. The gain here is that, compared to $E(w; r)$, it is easier to analyze $\overline E(w; r)$ w.r.t $w$.
% Though the $1/2$ factor is clearly not optimal, it will suffice for our purposes\footnote{In fact positive constant factor $\alpha = \Omega(1)$ will do.}

\subsection{Optimizing over sub-level curves of ordinary test error}
Note that the robustness test error of the ground-truth model $w_0$ (which minimizes the ordinary test error) is $E(w_0;r) = r^2\|w_0\|_\star^2$.
We shall now compute lower-bounds for the robustness test error $E(w; r)$, on sub-level sets of the ordinary test error $E(w)= E(w,0) = \|w-w_0\|_{\Sigma_x}^2$, i.e over all $w$'s which have a given value of ordinary test error $E(w)\le E_0$, where $E_0 \ge 0$ is a fixed threshold / level.
We will do analogous computations over sub-level sets of ordinary training error later.

\begin{restatable}{thm}{}
For any threshold $E_0 \ge 0$, it holds that
\begin{eqnarray}
    \inf_{E(w) \le E_0} E(w; r) \ge \frac{r^2}{2}\left(\inf_{\|v\|_2 \le E_0}\|w_0-\Sigma_x^{-1/2}v\|_\star^2\right).
\end{eqnarray}
In particular, if the attacker's norm is an $\ell_p$-norm for some $p \in [1,\infty]$, then
\begin{eqnarray}
\inf_{E(w) \le E_0} \frac{E(w; r)}{E(w_0;r)} \ge \frac{C_p}{2}\cdot  \left(1-\sqrt{\frac{E_0}{\|\Sigma_x\|_{\mathrm{op}}\|w_0\|_{p^\star}^2}}\right)_+^2,
\end{eqnarray}
where $p^\star \in [1,\infty]$ is the harmonic conjugate of $p$, i.e $1/p+1/p^\star = 1$, and
\begin{eqnarray}
C_p := \begin{cases}
d^{1-2/p},&\mbox{ if }1 \le p < 2,\\
1,&\mbox{ else.}
\end{cases}.
\end{eqnarray}
\end{restatable}
Thus, for $\ell_p$-norm attacks with $p \in [2,\infty]$, if $E_0 \lesssim \|\Sigma_x\|_{\mathrm{op}}\|w_0\|_{p^\star}^2$, any linear model $w$ with ordinary test error at least $E_0$ must suffer robustness test error $E(w; r) \gtrsim E(w_0; r)=r^2\|w_0\|_\star^2$.
\begin{proof}
To simplify notations, let $\Sigma_x=\Sigma$. One computes
\begin{eqnarray}
\begin{split}
\inf_{\|w-w_0\|_{\Sigma}^2 \le E_0} \sqrt{\overline E(w; r)}&= \inf_{\|w-w_0\|_{\Sigma}^2 \le E_0} \|w-w_0\|_\Sigma + r\|w\|_\star\\
&= \inf_{\|w\|_{\Sigma} \le E_0} \|w\|_\Sigma+r\|w+w_0\|_\star\\
&= \inf_{\|w\|_2 \le E_0} \|w\|_2+r\|\Sigma^{-1/2}w+w_0\|_\star\\
&= \inf_{\|w\|_2 \le E_0} \|w\|_2+\sup_{\|z\| \le r}z^\top(\Sigma^{-1/2}w+w_0)\\
&=\sup_{\|z\| \le r}z^\top w_0 + \inf_{\|w\|_2\le E_0}\|w\|_2+\overline z^\top w,\text{ with }\overline z := \Sigma^{-1/2}z\\
&= \sup_{\|z\| \le r}z^\top w_0 + \inf_{\|w\|_2 \le E_0} \sup_{\|u\|_2 \le 1}u^\top w + \overline z^\top w\\
&=\sup_{\|z\| \le r}z^\top w_0 + \sup_{\|u\|_2 \le 1}\inf_{\|w\|_2 \le E_0} u^\top w + \overline z^\top w\\
&= \sup_{\|z\| \le r}z^\top w_0 + \sup_{\|u\|_2 \le 1}-E_0\cdot\|u+\overline z\|_2\\
&= \sup_{\|z\| \le r}z^\top w_0 - E_0\cdot \inf_{\|u\|_2 \le 1}\|u+\overline z\|_2\\
&= \sup_{\|z\| \le r}z^\top w_0 -  E_0\cdot(\|\overline z\|_2-1)_+ \\
 &\ge \sup_{\|z\| \le r}z^\top w_0 -  E_0\cdot \|\overline z\|_2\\
 &=\inf_{\|v\|_2 \le E_0}\sup_{\|z\| \le r}z^\top w_0 -  z^\top\Sigma^{-1/2}v\\
 &= r\inf_{\|v\|_2 \le E_0}\|w_0-\Sigma^{-1/2}v\|_\star,
\end{split}
\end{eqnarray}
which proves the first part upon combining with \eqref{eq:E}.

Finally, if the attacker's norm is an $\ell_p$-norm, then thanks to Lemma \ref{lm:noneuclideanlstsq} below applied with $q=p^\star=p/(p-1)$, the last expression can be further lower-bounded by $$
r\cdot\min(1,d^{1/2-1/p})\cdot \left(\|w_0\|_\star-\sqrt{\dfrac{E_0}{\|\Sigma_x\|_{\mathrm{op}}}}\right)_+.
$$
\end{proof}
\begin{restatable}{lm}{}
\label{lm:noneuclideanlstsq}
Let $A$ be an $m \times d$ matrix and $b \in \mathbb R^m$. Then, for any $q \in [1,\infty]$, it holds that
\begin{eqnarray}
\inf_{\|v\|_2 \le r} \|Av-b\|_q \ge \min(1,d^{1/q-1/2})(\|b\|-r\|A\|_{\mathrm{op}})_+.
\end{eqnarray}
\end{restatable}
\begin{proof}
Define $\alpha_q :=\inf_{\|v\|_2 \le r}\|Av-b\|_q$. Since $\|v\|_q \ge \min(1,d^{1/q-1/2})\|v\|_2$ for any $v \in \mathbb R^d$, we know that
$\alpha_q \ge \min(1,d^{1/q-1/2})\alpha_2$.
We now lower-bound $\alpha_2$ to complete the proof. By "dualizing", one has
\begin{eqnarray}
\begin{split}
\alpha_2 &= \inf_{\|z\|_2 \le r}\|Az-b\|_2 = \inf_{\|z\|_2 \le r}\sup_{\|v\|_2 \le 1}v^\top(b-Az)\\
&= \sup_{\|v\|_2 \le 1}v^\top b+\inf_{\|z\|_2 \le r}-v^\top Az
= \sup_{\|v\|_2 \le 1} v^\top b - r\|Av\|_2\\
&\ge \sup_{\|v\|_2 \le 1} v^\top b - r\|A\|_{\mathrm{op}}\|v\|_2 = (\|b\|-r\|A\|_{\mathrm{op}})_+.
\end{split}
\end{eqnarray}
Putting things together gives the claimed lower-bound.
\end{proof}

==> sections/powerlaw.tex <==
\section{Power-Law Phenomena in the Finite-Sample Regime}
Let  $\Sigma = \sum_{j=1}^d \lambda_j v_jv_j^\top$ be the SVD of the feature covariance matrix $\Sigma$. As usual, let $w_0 \in \mathbb R^d$ be the ground-truth linear model, and set $c_j := w_0^\top v_j$ for all $j \in [d]$.
We make the following structural assumption motivated by \url{https://arxiv.org/pdf/2203.06176.pdf}.
\begin{mdframed}
\begin{restatable}[Power law regime]{assume}{}
    Suppose there exist constants $\gamma \in (0,\infty)$ and $\delta \in [0,\infty)$ such that 
    \begin{eqnarray}
    \lambda_j \asymp j^{-1-\gamma}\text{ and }c_j^2 \asymp j^{-\delta}\text{ for all }j \in [d].
    \label{eq:powerlaws}
    \end{eqnarray}
    \label{ass:powerlaws}
\end{restatable}
\end{mdframed}
Such a spectral decay has been observed in real world datasets like MNIST, FashionMNIST, etc. See \url{https://arxiv.org/pdf/2203.06176.pdf} and references therein.

In the regime covered by Assumption \ref{ass:powerlaws}, we shall provide a complete analysis of GD, and prescribe a closed-form expression for the optimal stopping time w.r.t adversarial risk.

\subsection{Local Random Matrix Theory}
Recently, the scope of applicability of RMT-based arguments has significantly been extended by \cite{Knowles2014AnisotropicLL}. For our own purposes, we shall only need a very rudimentary version of these developments, which we now present below. 

\begin{restatable}{df}{}
Let $S$ be a $d \times d$ positive-definite matrix with eigenvalues $\lambda_1(S),\ldots,\lambda_d(S)$.
For any positive $\lambda$, let $\kappa_S(\lambda,n)$ be the unique positive solution to the algebraic equation
\begin{equation}
    1 = \frac{\lambda}{\kappa} + \frac{1}{n}\sum_{j=1}^d \frac{\lambda_j(S)}{\lambda_j(S) + \kappa}.
\end{equation}
In particular, when $S$ is the covariance matrix $\Sigma$ of the features, we will simply write $\kappa = \kappa(\lambda,n) = \kappa_\Sigma(\lambda,n)$.
\label{df:kappa}
\end{restatable}
 The parameter $\lambda$ should be thought of as \emph{explicit} ridge regularization, while $\kappa$ should be thought of as \emph{implicit} ridge regularization.  Note that in the fixed-$d$ large-$n$ regime, one has $\kappa(\lambda,n) \approx \lambda$ with equality if $n=\infty$.

Let $\widehat\lambda_1,\widehat \lambda_2,\ldots,\widehat\lambda_d \ge 0$ be the eigenvalues of the empirical covariance matrix $\widehat\Sigma := X^\top X/n$. The following hypothesis allows us to swap in the population covariance matrix $\Sigma$ for empirical covariance matrix $\widehat\Sigma$ in setting computations, even though we do not have the convergence $\widehat\Sigma \to \Sigma$.
\begin{restatable}[A Local Marchenko-Pastur Hypothesis]{assume}{}
Let $I \subseteq (0,\infty)$. Assume that: for all $u,v \in \mathbb R^d$ such that $\|u\|_\Sigma^2,\|v\|_\Sigma^2 \le 1$, the following holds
\begin{align}
\frac{1}{n}\sum_{i=1}^n \frac{1}{\widehat\lambda_i + \lambda} &= \frac{1}{\kappa} + o_{\mathbb P}(1)\label{eq:hype1},\\
u^\top \lambda(\widehat\Sigma + \lambda I_d)^{-1} v &= u^\top \kappa(\Sigma+\kappa I_d)^{-1} v + o_{\mathbb P}(1)\label{eq:hype2},
\end{align}
uniformly over $\lambda \in I$.
\end{restatable}
Under setting mild regularity conditions on covariance matrix $\Sigma$, the above assumption is in order, thanks to \cite[Theorem 3.6]{Knowles2014AnisotropicLL}.

 \subsection{Main Results}
For any positive $\lambda$, let $\widehat w(\lambda,n)$ correspond to the ridge estimator obtained from the dataset $\mathcal D_n$, i.e
\begin{equation}
\label{eq:ridge}
    \widehat w(\lambda,n) = (\widehat\Sigma + \lambda I_d)^{-1} X^\top y/n \in \mathbb R^{d}.
\end{equation}
One can show that $\widehat w(\lambda,n)$ has the same Euclidean adversarial risk as vanilla GD stopped at $t \propto 1/\lambda$. Thus, analyzing the latter is equivalent to analyzing the former.

 Define scale parameters $\alpha$ and $\beta$ by
 \begin{eqnarray}
 \alpha := (\delta + \gamma) / (1+\gamma),\,\beta := (1 + \delta)/(1+\gamma).
 \end{eqnarray}
 The following computes the adversarial risk attained by the ridge estimator, as a function of $\alpha$, $\beta$, $\kappa$, and the attack strength $r$.
\begin{restatable}{thm}{Epower}
\label{thm:Epower}
Grant Assumption \ref{ass:powerlaws}. For any $r \ge 0$, the Euclidean adversarial risk of the ridge estimator $\widehat w(\lambda,n)$ is given by
\begin{equation}
\label{eq:Escaling}
\begin{split}
    &E^{\|\cdot\|_2}(\widehat w(\lambda,n),w_0,r) \\
   % &\quad\quad\asymp \left(\sqrt{\kappa(\lambda,n)^\alpha + \sigma^2} + \frac{r} {\kappa(\lambda,n)^{\beta/2}}\right)^2 + o_{\mathbb P}(1)\\
    &\quad\quad \asymp \left(\kappa(\lambda,n)^{\alpha/2}  + \frac{r} {\kappa(\lambda,n)^{\beta/2}} + \sigma\right)^2 + o_{\mathbb P}(1).
    \end{split}
\end{equation}
\end{restatable}

The following corollary gives a  closed-form expression for the (inverse) time when GD should be stopped to achieve optimal (up to within a multiplicative absolute constant) adversarial risk under Assumption \ref{ass:powerlaws}.
\begin{restatable}{cor}{Epowercor}
\label{cor:Epowercor}
Grant Assumption \ref{ass:powerlaws}. If $\lambda^\star(r,n)$ is the unique $\lambda \in [0,\infty)$ which solves $\kappa(\lambda,n) = (r\beta/\alpha)^{(\alpha+\beta)/2}$, then 
\begin{equation}
    1 \le \sup_{r \ge 0}\frac{E^{\|\cdot\|_2}(\widehat w(\lambda^\star(r,n)),w_0,r)}{ E^{\|\cdot\|_2}_{opt}(w_0,r)} = O_{\mathbb P}(1).
\end{equation}
\end{restatable}
\begin{restatable}{rmk}{}
Even in the infinite-sample case (i.e $n=\infty$) where $\kappa(\lambda,n) = \lambda$, the above corollary already tells us something highly nontrivial: the optimal ridge (i.e inverse-time) parameter is given by $\lambda^\star(r) = (r\beta/\alpha)^{(\alpha+\beta)/2}$,  a nontrivial polynomial in the attack strength $r$.
\end{restatable}
\begin{proof}[Proof of Corollary \ref{cor:Epowercor}]
Differentiating $\kappa^{\alpha/2} + r\kappa^{-\beta/2}$ w.r.t $\kappa$ and setting to zero, gives $\kappa = (r\beta/\alpha)^{(\alpha+\beta)/2}$. Combining with the preceding theorem shows the optimality of the prescribed value of ridge regularization $\lambda$. The proof is completed by recalling the following result established in \cite{Xing2021}: the linear model which achieves optimal adversarial risk is a ridge.
\end{proof}

==> sections/powerlaws_proofs.tex <==
\section{Power-Law Phenomena in Finite-Sample Regimes: Proof Theorem \ref{thm:Epower}}
\Epower*

For the proof of the theorem, we will need some auxiliary results.

 \subsection{Some Preliminary computations}
\paragraph{Change of variables.}
As observed in \url{https://arxiv.org/pdf/2203.06176.pdf}, the dataset $\mathcal D_n$ can be equivalently realized as follows. Fix a smoothing parameter $\theta > 0$  and let $\widetilde x_i(\theta) := (x_i, \theta^{1/2}\epsilon_i) \in \mathbb R^{d + 1}$ and $w_0(\theta) := (w_0, \theta^{-1/2}) \in \mathbb R^{d + 1}$ for all $i \in [n]$, and note that $y_i = \widetilde x_i^\top \widetilde w_0$. That is, we have effectively absorbed the label noises $\epsilon_i$ into the features $x_i$.

Observe that $\theta \mapsto x_i(\theta)$ is a continuous function from $(0,\infty)$ to $\mathbb R^{d+1}$ with
$ \lim_{\theta \to 0^+} x_i(\theta) = (x_i,0)$. Moreover, it is clear that the covariance matrix $\Sigma(\theta) \in \mathcal S_{++}^{d+1}$ of of each $\widetilde x_i$ is given by
\begin{eqnarray}
\Sigma(\theta) = \begin{bmatrix}
\Sigma & 0\\
0 & \theta\sigma^2
 \end{bmatrix}.
 \end{eqnarray}
 Clearly, $\theta \mapsto \Sigma(\theta)$ defines a continuous function from $(0,\infty)$ to $\mathcal S_{++}^{d+1}$, with 
 \begin{eqnarray}
\lim_{\theta \to 0^+}\Sigma(\theta) = \begin{bmatrix}
\Sigma & 0\\
0 & 0
 \end{bmatrix}.
 \end{eqnarray}
  Note that the eigenvectors of $\Sigma(\theta)$ are of the form $v_j(\theta) = (v_j,0) \in \mathbb R^{d + 1}$ for all $j \in [d]$, and $v_{d+1}(\theta) = (0_d,1) \in \mathbb R^{d+1}$, with corresponding eigenvalues $\lambda_j(\theta)$ being $\lambda_j$ and $\theta\sigma^2$ respectively. One computes the alignment between $w_0(\theta)$ and each of these eigenvectors as
 $$
 c_j(\theta) := w_0(\theta)^\top v_j(\theta) =
 \begin{cases}
 w_0^\top v_j =: c_j,&\mbox{ if }1 \le j \le d,\\
 \theta^{-1/2},&\mbox{ if }j=d+1.
 \end{cases}
 $$
 
 Finally, let $X(\theta) := (x_1(\theta),\ldots,x_n(\theta)) \in \mathbb R^{n \times (d+1)}$ be the smoothed design matrix and let $\widehat\Sigma(\theta) := X(\theta)^\top X(\theta)/n \in \mathcal S_+^{d+1}$ be the associated empirical covariance matrix.

 
 \paragraph{Power-law computations.}
 Consider the power laws \eqref{eq:powerlaws}. Let $j^\star := \inf\{j \in [d] \mid \kappa \ge \lambda_j\}$ with the convention that $\inf\emptyset = \infty$. Then, it is easy to see that if $j^\star \ne \infty$, then
 \begin{eqnarray}
j^\star \asymp \kappa^{-\frac{1}{1+\gamma}}.
\end{eqnarray}
Now, $\sum_{j=1}^d \dfrac{\lambda_j}{\lambda_j + \kappa} \asymp j^\star + \dfrac{1}{\kappa}\sum_{j=j^\star}^d \lambda_j \asymp j^\star + \dfrac{1}{\kappa}\int_{j^\star}^d t^{-1-\gamma}\dv t \asymp j^\star + \dfrac{(j^\star)^{-\gamma}}{\kappa} \asymp j^\star \asymp \kappa^{-\frac{1}{1+\gamma}}$. We conclude that $\kappa=\kappa(\lambda,n)$ must satisfy
$1 \asymp \lambda\kappa^{-1} + \dfrac{1}{n}\kappa^{-\frac{1}{1+\gamma}}$.
In particular, we have
\begin{align}
    \kappa &\asymp \lambda+1/n\text{ in the limit }\gamma\to 0^+\\
    \kappa &\asymp \lambda + 1/n^2 + \sqrt \lambda/n \asymp (\sqrt\lambda + 1/n)^2 \text{ in the limit }\gamma \to 1.
\end{align}
Also, for $\lambda$ sufficiently small, we have
\begin{equation}
\label{eq:ridgelesskappa}
    \kappa \asymp 1/n^{1+\gamma}.
\end{equation}
 
\subsection{Dynamics of Ordinary Risk}
Let $\widehat w(\lambda,n,\theta)$ be the ridge estimator obtained from $X(\theta)$ and $y$, i.e
\begin{eqnarray}
\widehat w(\lambda,n,\theta) = (X(\theta)^\top X(\theta)/n+\lambda I_{d+1})^{-1}X(\theta)^\top y/n = (\widehat\Sigma(\theta) + \lambda I_{d+1})^{-1}\widehat\Sigma(\theta) w_0(\theta)  \in \mathbb R^{d+1}.
\end{eqnarray}
Note that the first $d$ coordinates of $\lim_{\theta \to 0^+}\widehat w(\lambda,n,\theta)$ correspond tot eh ridge estimator obtained from $X$ and $y$, i.e
\begin{equation}
    \widehat w(\lambda,n) = (\widehat\Sigma + \lambda I_d)^{-1} X^\top y/n \in \mathbb R^{d}.
\end{equation}
Let $\kappa(\theta) := \kappa_{\Sigma(\theta)}(\lambda,n)$. One computes the risk of $\widehat w(\lambda,n,\theta)$ as follows
\begin{equation}
\begin{split}
    E(\widehat w(\lambda,n,\theta)) &= \|(\widehat\Sigma(\theta) + \lambda I_d)^{-1}\widehat\Sigma(\theta) w_0(\theta)-w_0(\theta)\|_\Sigma^2 = \|\lambda(\widehat \Sigma(\theta) + \lambda I_{d+1})^{-1}w_0(\theta)\|_{\Sigma(\theta)}^2 \\
    &= w_0^\top \lambda(\widehat\Sigma(\theta) + \lambda I_{d+1})^{-1}\Sigma(\theta)\lambda (\widehat\Sigma(\theta) + \lambda I_{d+1})^{-1}w_0(\theta)
    \\
    &= w_0(\theta)^\top \kappa(\theta) (\Sigma(\theta) + \kappa(\theta) I_{d+1})^{-1}\Sigma(\theta)\kappa(\theta) (\Sigma(\theta) + \kappa(\theta) I_{d+1})^{-1}w_0(\theta) + o_{\mathbb P}(1),\text{ thanks to \eqref{eq:hype2}}\\
    &= \kappa(\theta)^2w_0(\theta)^\top \Sigma(\theta)(\Sigma(\theta)+\kappa(\theta) I_{d+1})^{-2}w_0(\theta) + o_{\mathbb P}(1) = \kappa(\theta)^2\sum_{j=1}^{d+1}\dfrac{\lambda_j(\theta)c_j^2}{(\lambda_j(\theta)+\kappa(\theta))^2} + o_{\mathbb P}(1)\\
    &= \kappa(\theta)^2\sum_{j=1}^d \dfrac{\lambda_j c_j^2}{(\lambda_j+\kappa(\theta))^2} + \kappa^2\frac{\theta\sigma^2(\theta^{-1/2})^2}{(\theta\sigma^2 + \kappa(\theta))^2} + o_{\mathbb P}(1)\\
    &= \kappa(\theta)^2\sum_{j=1}^d \dfrac{\lambda_j c_j^2}{(\lambda_j+\kappa(\theta))^2} + \frac{\sigma^2}{(\theta\sigma^2/\kappa(\theta) + 1)^2} + o_{\mathbb P}(1),
    \end{split}
    \label{eq:wizard}
\end{equation}
In the limit $\theta\to 0^+$, the second term in the rightmost side of \eqref{eq:wizard} tends to $\sigma^2$. As, for the second term, let $\kappa(0^+) := \lim_{\theta\to 0^+}\kappa(\theta)$. By definition, one has
$$
1 = \frac{\lambda}{\kappa(\theta)} + \frac{1}{n}\sum_{j=1}^d\frac{\lambda_j}{\lambda_j + \kappa(\theta)} + \frac{1}{n}\frac{\theta\sigma^2}{\theta\sigma^2 + \kappa(\theta)} \overset{\theta\to 0^+}{\longrightarrow} \frac{\lambda}{\kappa(0^+)} + \frac{1}{n}\sum_{j=1}^d\frac{\lambda_j}{\lambda_j + \kappa(0^+)},
$$
and we deduce that $\kappa(0^+) = \kappa$, by Definition \ref{df:kappa}. Thus, in the limit $\theta \to 0^+$, the second term in \eqref{eq:wizard} simplifies to
\begin{equation}
    \begin{split}
    \kappa^2\sum_{j=1}^d \dfrac{\lambda_j c_j^2}{(\lambda_j+\kappa)^2} &\asymp \kappa^2\sum_{j=1}^{j^\star}\frac{c_j^2}{\lambda_j} + \sum_{j=j^\star}^d \lambda_jc_j^2 = \kappa^2\sum_{j=1}^{j^\star}j^{1+\gamma-\delta} + \sum_{j=j^\star}^d j^{-1-\gamma-\delta}\\
    &\asymp \kappa^2\int_1^{j^\star} t^{1+\gamma-\delta}\dv t + \int_{j^\star}^d t^{-1-\gamma-\delta}\dv t \asymp \kappa^2 (j^\star)^{2+\gamma-\delta} + (j^\star)^{-\gamma-\delta}\\
    &\asymp \kappa^{2-1-(1-\delta)/(1+\gamma)} + \kappa^{(\gamma+\delta)/(1+\gamma)} \asymp  \kappa^\alpha,
    \end{split}
\end{equation}
where $\alpha := (\delta + \gamma)/(1+\gamma) \in (0,1)$.
We have thus proved the following result.
\begin{restatable}{prop}{}
For any $\lambda \ge 0$, it holds under Assumption \ref{ass:powerlaws} that \begin{eqnarray} 
E(\widehat w(\lambda,n)) \asymp \kappa(\lambda,n)^\alpha + \sigma^2 + o_{\mathbb P}(1).
\end{eqnarray}
where $\alpha := (\delta+\gamma)/(1+\gamma) \in (0,1)$. In particular, $\lim_{\lambda \to 0^+}E(\widehat w(\lambda,n)) = 1/n^{(\delta+\gamma)} + \sigma^2 + o_{\mathbb P}(1)$.
\end{restatable}


% \paragraph{Variance term: ridgeless case.}
% The variance of the generalization error of the ridge estimator $\widehat w(\lambda,n)$ is given for $\lambda \to 0^+$ and $n \ge d + 2$ by
% \begin{equation*}
%     \begin{split}
%     \lim_{\lambda\to 0^+}Var (\widehat w(\lambda,n)) &= \epsilon^\top X\widehat\Sigma^{-1}\Sigma\widehat\Sigma^{-1}X^\top \epsilon/n^2 = \frac{\sigma^2}{n}\trace (\Sigma \widehat \Sigma^{-1})  + o_{\mathbb P}(1) \\
%      &=  \sigma^2 \frac{d}{n-d-1}\trace(\Sigma\Sigma^{-1}) + o_{\mathbb P}(1) \asymp  \sigma^2d \cdot \frac{d/n }{1-d/n} + o_{\mathbb P}(1). 
%     \end{split}
% \end{equation*}
 
% \paragraph{Variance term: ridgeful case.}
% Let $X/n = USW^\top$ be the SVD of $X/n$.
% \begin{restatable}[Correlated noise]{assume}{}
% Suppose the noise vector $\epsilon \in \mathbb R^n$ is such that $X^\top \epsilon/$, with $z \sim N(0,D)$.
% \end{restatable}
% Under the above assumption, one computes
% \begin{equation}
%     \begin{split}
%     Var(\widehat w(\lambda,n)) = \epsilon^\top X(\widehat\Sigma + \lambda I_d)^{-1}\Sigma(\widehat\Sigma + \lambda I_d)^{-1} X^\top \epsilon/n^2 
%     \end{split}
% \end{equation}
\subsection{Dynamics of Adversarial Risk}
The squared Euclidean norm of the ridge estimator $\widehat w(\lambda,n)$ is given by
\begin{equation}
    \begin{split}
    \|\widehat w(\lambda,n)\|^2_2 &= w_0^\top\widehat\Sigma^2(\widehat\Sigma + \lambda I_d)^{-2}w_0 = w_0^\top \Sigma^2(\Sigma + \kappa I_d)^{-2}w_0 + o_{\mathbb P}(1),\text{ thanks to \eqref{eq:hype2}}\\
    &= \sum_{j=1}^d \frac{\lambda_j^2 c_j^2}{(\lambda_j+\kappa)^2} + o_{\mathbb P}(1) \asymp \sum_{j=1}^{j^\star} c_j^2 + \frac{1}{\kappa^2}\sum_{j=j^\star}^d \lambda_j^2 c_j^2 + o_{\mathbb P}(1)\\
    &\asymp \int_1^{j^\star}t^{-\delta}\dv t + \frac{1}{\kappa^2}\int_{j^\star}^d t^{-2-2\gamma-\delta}\dv t + o_{\mathbb P}(1)\\
    &\asymp (j^\star)^{1-\delta} + \frac{1}{\kappa^2}(j^\star)^{-1-2\gamma-\delta} + o_{\mathbb P}(1) \asymp (j^\star)^{1-\delta} + o_{\mathbb P}(1)\\
    &\asymp \kappa^{-(1-\delta)/(1+\gamma)} + \kappa^{-2+(1+2\gamma+\delta)/(1+\gamma)} + o_{\mathbb P}(1)\\
    &\asymp \kappa^{-(1+\delta)/(1+\gamma)} + o_{\mathbb P}(1).
    \end{split}
\end{equation}
We have thus proved the following result.
\begin{restatable}{prop}{}
For any $\lambda \ge 0$, it holds under Assumption \ref{ass:powerlaws} that
\begin{equation}
    \|\widehat w(\lambda,n)\|^2_2 \asymp \kappa(\lambda,n)^{-\beta} + o_{\mathbb P}(1),
\end{equation}
where $\beta := (1+\delta) / (1+\gamma) \in (1,2)$.
\end{restatable}
\begin{restatable}{rmk}{}
Interestingly, note that if $\kappa(\lambda,n) \to 0$ (which is what happens in the ridgeless case, because we can show via \eqref{eq:hype1} that the derivative of $\kappa(\lambda,n)$ w.r.t $\lambda$ is at least $1$ for any $\lambda > 0$), one has
\begin{eqnarray}
E(\widehat w(\lambda,n) ) \to \sigma^2,\text{ while } \|\widehat w(\lambda,n)\|_2^2 \to \infty,\text{ even  though }\|w_0\|_2^2 = \sum_{1 \le j \le d}j^{-1-\gamma} \le \zeta(1+\gamma)  < \infty.
\end{eqnarray}
\end{restatable}

\subsection{The Proof}
We are no in shape to proof Theorem \ref{thm:Epower}.
\begin{proof}[Proof of Theorem \ref{thm:Epower}]
Indeed, thanks to the preceding two propositions, and the fact that
$$
E^{\|\cdot\|_2}(\widehat w(\lambda,n),w_0,r) \asymp (\sqrt{E(\widehat w(\lambda,n))}+r\|\widehat w(\lambda,n)\|_2)^2,
$$
the claimed identity \eqref{eq:Escaling} holds.
\end{proof}

==> sections/rmt.tex <==

\section{Proof of Lemma \ref{lm:rmt}}
Recall that $G$ is and $m \times d$ random matrix with iid entries from $N(0,1)$ (where $m/d \ge \gamma > 1$), and $W_{rand} := G^\top G$.

% \rmt*
Recall that "w.h.p" (with high-probability) is used to characterize a statement which holds except for an event with probability exponentially small in $d$.

For proving the lemma, We will need the following well-known auxiliary lemmas.
\begin{restatable}{lm}{}
There exists an absolute constant $c$ such that if $z \sim N(0,I_m)$, then $\mathbb P(\|z\|_2 \le u\sqrt{m}) \le (cu)^m$, for all $u \ge 0$.
\end{restatable}
\begin{proof}
Let $\mathcal S_\epsilon$ a maximal $(\|\cdot\|_\star,\epsilon)$-net for the unit-sphere $\mathcal S_{\|\cdot\|_\star}(\mathbb R^d) := \{w \in \mathbb R^d \mid \|w\|_\star = 1\}$. By a simple volume-packing argument it is easy to see that $|\mathcal S_\epsilon| = O(3/\epsilon)^d$ for any $\epsilon \in (0,1]$. By a clear abuse of language, we will identity each element of $\mathcal S_\epsilon$ by it center $w$. We will use a classical "epsilon-net" argument to control $\lambda_{max}^{\|\cdot\|}(W_{rand})$ and $\lambda_{min}^{\|\cdot\|}(W_{rand})$ separately.

\paragraph{Step 1: Controlling $\lambda_{max}^{\|\cdot\|}(W_{rand})$.}
By compactness of the unit-sphere $\mathcal S_{\|\cdot\|_\star}(\mathbb R^d)$ and continuity of $w \mapsto \|Gw\|_2$, the exists $z \in S_{\|\cdot\|_\star}(\mathbb R^d)$ such that $\|Gz\|_2 = \sup_{\|w\|_\star=1}\|Gw\|_2$. Let $w \in \mathcal S_\epsilon$ such that $\|z-w\|_\star \le \epsilon$.
A simple computation reveals that, if $\epsilon \le 1/2$, then
\begin{eqnarray}
\sqrt{\lambda_{max}^{\|\cdot\|}(W_{rand})} = \sup_{\|w\|_\star=1}\|Gw\|_2 = \|Gz\|_2 \le \|Gw(z)\|_2 + \|G(z-w(z))\|_2 \le \sup_{w \in S_\epsilon}\|Gw\|_2 + \sqrt{\lambda_{max}^{\|\cdot\|}(W_{rand})}/2,
\end{eqnarray}
that is $\lambda_{max}^{\|\cdot\|}(W_{rand}) \le 4\sup_{w \in \mathcal S_\epsilon}\|Gw\|_2^2$.
Thus, for any $\epsilon \le 1/2$ and $s \ge 0$, we have
\begin{eqnarray}
\begin{split}
\mathbb P(\lambda_{max}^{\|\cdot\|}(W_{rand}) \ge s^2m)
% = \mathbb P(\sup_{\|w\|_\star=1}\|Gw\|_2 \ge s)
&\le \mathbb P(\sup_{w \in \mathcal S_\epsilon}\|Gw\|_2 \ge s\sqrt{m}/2)\\
&\le |\mathcal S_\epsilon|\cdot\sup_{w \in \mathcal S_\epsilon}\mathbb P(\|Gw\|_2 \ge s/2)\\
&= O(3/\epsilon)^d\cdot\sup_{w \in \mathcal S_\epsilon}\mathbb P(\|Gw\|_2 \ge s/2).
\end{split}
\end{eqnarray}
Taking $\epsilon=1/2$ gives
$$
\mathbb P(\lambda_{max}^{\|\cdot\|}(W_{rand}) \ge s^2 m) \lesssim 6^d \cdot\sup_{\|w\|_\star=1}\mathbb P(\|Gw\|_2^2 \ge s^2m/4) \lesssim 6^d\cdot \sup_{\|w\|_\star=1}e^{-csm/\|w\|_2} \le 6^d e^{-csm/\beta},
$$
where the last but one inequality is because $Gw$ is random vector in $\mathbb R^m$ with iid coordinates from $N(0,\|w\|_2^2)$. Taking $s = 8\beta/c$ ensures that the rightmost side is of order $e^{-\Omega(d)}$. We deduce that for $C_1 := s =8\beta/c$, it holds w.h.p that
\begin{eqnarray}
\lambda_{max}^{\|\cdot\|}(W_{rand}) \le C_1^2 m.
\label{eq:rmthigh}
\end{eqnarray}

\paragraph{Step 2: Controlling
$\lambda_{min}^{\|\cdot\|}(W_{rand})$.}
By compactness, there exists $z \in \mathbb R^d$ with $\|z\|_\star=1$ such that $\|Gz\|_2 = \inf_{\|w\|_\star=1}\|Gw\|_2$. Let $w \in \mathcal S_\epsilon$ such that $\|w-z\|_\star \le \epsilon$. We deduce that
\begin{eqnarray}
\begin{split}
\sqrt{\lambda_{min}^{\|\cdot\|}(W_{rand})} = \inf_{\|w\|_\star=1}\|Gw\|_2 = \|Gz\|_2 &\ge \inf_{w \in \mathcal S_\epsilon}\|Gw\|_2 - \|G(z-w)\|_2\\
&\ge \|Gw\|_2 - \|G(z-w)\|_2\\
&\ge \inf_{w \in \mathcal S_\epsilon}\|Gw\|_2-\epsilon \sqrt{\lambda_{max}^{\|\cdot\|}(W_{rand})}\\
&\ge \inf_{w \in \mathcal S_\epsilon}\|Gw\|_2 - \epsilon C_1 \sqrt{m},\text{ w.h.p.}
\end{split}
\label{eq:smintrick}
\end{eqnarray}
On the other hand, for any $\eta > 0$, we have
\begin{eqnarray}
\begin{split}
% \mathbb P(\lambda_{min}^{\|\cdot\|}(W_{rand}) \le s^2m) = \mathbb P(\inf_{\|w\|_\star=1}\|Gw\|_2 \le s\sqrt{m}) &\le
\mathbb P(\inf_{w \in \mathcal S_\epsilon}\|Gw\|_2 \le \eta \sqrt{m})
&\le (3/\epsilon)^d \cdot \sup_{w \in \mathcal S_\epsilon} \mathbb P(\|Gw\|_2 \le \eta \sqrt{m})\\
&= (3/\epsilon)^d \cdot \sup_{w \in \mathcal S_\epsilon} \mathbb P(\|Gw/\|w\|_2\|_2 \le \eta \sqrt{m}/\|w\|_2)\\
&\le (3/\epsilon)^d \cdot \sup_{\|w\|_2 = 1} \mathbb P(\|Gw\|_2 \le \eta \sqrt{m}/\beta'),\text{ Thanks to Assumption \ref{assume:coveringnumber}}\\
&\le (3/\epsilon)^d\cdot (\eta \nu / \beta')^m,
\end{split}
\label{eq:smintrick2}
\end{eqnarray}
for an absolute constant $\nu > 0$. Thus, if $\epsilon \le \eta/(2C_1)$ with $\eta < 2C_1$, we deduce from \eqref{eq:smintrick} and \eqref{eq:smintrick2} that
\begin{eqnarray}
\mathbb P(\lambda_{min}^{\|\cdot\|}(W_{rand}) \le \eta^2 m/4) \le (3/\epsilon)^d\cdot(\eta\nu/\beta')^m + e^{-cm} = (\eta\nu/\beta' \cdot (3/\epsilon)^{d/m})^m + e^{-cm} \le (\eta\nu/\beta' \cdot (3/\epsilon)^{1/\gamma})^m + e^{-cm},
\end{eqnarray}
if $m/d \ge \gamma$.
Thus, for sufficient large $\gamma$ and sufficiently small $\eta$, one has 
$\mathbb P(\lambda_{min}^{\|\cdot\|}(W_{rand}) \le \eta^2 m/4) \le e^{-c'm}$,
for some absolute constant $c'$.
We deduce that w.h.p, it holds that
\begin{eqnarray}
\lambda_{min}^{\|\cdot\|}(W_{rand}) \ge \eta^2 m/4.
\label{eq:rmtlow}
\end{eqnarray}
Combining \eqref{eq:rmthigh} and \eqref{eq:rmtlow}, we deduce that
\begin{eqnarray}
\kappa^{\|\cdot\|}(W_{rand}) := \lambda_{max}^{\|\cdot\|}(W_{rand}) / \lambda_{min}^{\|\cdot\|}(W_{rand}) \le 4C_1^2/\eta^2=:C,
\end{eqnarray}
as claimed.
\end{proof}

